The Grothendieck Constant is Less Than $\frac{\pi}{2 \log (1+ \sqrt{2})} - 10^{-5}$

We prove that the Grothendieck constant $K_G < \frac{\pi}{2 \log (1+ \sqrt{2})} - 10^{-5}$. This improves on the work of Braverman, Makarychev, Makarychev, and Naor (2011), who proved that $K_G < \frac{\pi}{2 \log (1+ \sqrt{2})} - \epsilon$ for an unspecified $\epsilon>0$.

==> old/abstract.tex <==
\begin{abstract}
Recent advances in artificial intelligence have shown great promise in mathematical reasoning and problem solving. Yet the application to research mathematics remains lacking. In this work, we take a key step in advancing this frontier, by using AI to improve bounds on unresolved mathematical constants. Mathematical constants are fundamental and often unify seemingly unrelated areas. We propose a general framework for this task that uses iterative proof refinement on a partially or fully formalized proof. We evaluate it on two such constants: the Grothendieck constant, central to optimization algorithms and complexity, and the Korenblum constant, important in analysis. We obtain the improved upper bound of $\text{bla bla}$ on the Grothendieck  constant and the improved lower bound of $\text{bla bla}$ on the Korenblum constant.
\red{AX: This is fine for a draft that we show advisors, but we will need to (1) introduce the importance of bounding constants more quickly + smoothly, (2) give highly informative but concise technicalities on the Lean pipeline, and (3) come up with a better ``who cares'' reason for why Grothendieck and Korenblum that appeals to a broad CS audience}


% We introduce a mixed-initiatve framework for certified quantitative proof refinement, a setting in which AI systems improve explicit mathematical bounds while preserving formal correctness. This framework targets a broad and important regime in modern mathematics: many results in optimization and analytic number theory are qualitatively understood, yet their best effective bounds still depend on long, delicate chains of estimates. We evaluate our approach on two such problems, obtaining improved certified bounds for Grothendieck’s constant and Korenblum’s constant. Our method combines  formalization to ground search, local proof refinement to tighten inequalities and optimize parameters, formal verification to certify each accepted step, and quantitative dependency propagation to measure the global effect of local improvements. Our results suggest that AI-assisted proof refinement can serve as a practical new tool for building reliable, continuously improvable explicit mathematics.

% A recurring motif in mathematics and science is how fundamental constants can unify seemingly unrelated areas. The precise values of these constants often remain elusive due to deep domain-specific reasons. One such instance is the grothendieck constant $K_G$, which is used for designing algorithms in optimization, and characterizing Banach spaces in functional analysis.   
% In this paper, we propose a general framework for estimating such constants by means of agent-guided proof refinement in Lean. 
% Using this framework, we improve the best known upper bound on the grothendieck constant since 1979, given by $K_G < \frac{2}{\pi} \log (1 + \sqrt{2}) - 10^{-15}$.
% The framework leverages an interactive loop between a formalizer and a certified numerical evaluator to iteratively obtain better bounds. 
% Additionally, we demonstrate the generalizability of our framework by applying it to an assortment of other problems.

    % A grand goal of AI since its inception has been to harness machine intelligence to advance fundamental research in mathematics and science. In this paper, we take steps in using AI for research math -- 1. We identify a recurring gap across many domains in mathematics and make it suitable for computer search 2. We propose a framework to address this gap and demonstrate it on a flagship problem -- improving the best known upper bound of the grothendieck constant since 1979. A central theme in research mathematics and science is the use of fundamental constants with rich properties that unify seemingly unrelated areas of mathematics, but the precise value of such constants often remains unknown due to limitations in proof techniques. The grothendieck constant is one such instance, it is central in the areas of complexity theory, functional analysis, and quantum mechanics. Despite this, its exact value remains an open problem. In our work, we design a general framework for improving such bounds by means of LLM-aided proof refinement in Lean, and obtain sharp improvements by many orders of magnitude over baseline. This framework combines the formal guarantee of Lean with the certified computational guarantee of Arb. We use the grothendieck problem as our main case study, and demonstrate the usefulness of our framework by applying it to an assortment of other problems.
\end{abstract}


==> old/abstract_v1.tex <==
\abstract{
\noindent
The (real) Grothendieck constant \(K_G\) is the infimum of \(K > 0\) that satisfies the inequality
\[
\sup_{\|x_i\| = \|y_j\| = 1} \sum_{i,j} a_{ij} \langle x_i, y_j \rangle
\;\le\;
K \max_{\varepsilon_i, \delta_j \in \{-1,1\}}
\sum_{i,j} a_{ij} \varepsilon_i \delta_j,
\]
where \(A = (a_{ij})\) is any real-valued matrix.
Surprisingly, \(K_G\) is independent of the dimension of \(A\) and, importantly, naturally arises across diverse disciplines, including Banach space theory, combinatorial optimization, computational complexity, and quantum information theory.
Despite its ubiquity, the exact value of \(K_G\) is unknown.


A first landmark result was due to Krivine in 1977, who proved that \(K_G \leq \tfrac{\pi}{2 \log (1 + \sqrt{2})}\) via the analysis of rounding schemes.
A rounding scheme is used to discretize continuous vectors, and its analysis gives an upper bound on \(K_G\); improving this bound can thus be reduced to the discovery and analysis of new schemes.
Krivine's best scheme gives the bound above, and he additionally conjectured that this was optimal --- a widely held belief for over thirty years until its refutation by Braverman-Makarychev-Makarychev-Naor (BMMN) in 2011.
Specifically, BMMN used a technique called mixing to analyze a new class of rounding schemes, and showed that \(K_G < \tfrac{\pi}{2 \log (1 + \sqrt{2})} - \varepsilon\) for some \(\varepsilon > 0\).
However, mixing arguments are restrictive in their application and often ignore the underlying geometry.
Moreover, they do not translate to strong numerical improvements: extending the analysis of BMMN only gives an improvement on the order of \(\varepsilon \approx 10^{-53}\).
Thus, while BMMN's mixing argument establishes the existence of a non-zero improvement to Krivine's bound, it provides only a partial understanding of this new class of rounding schemes.



% A first landmark result was due to Krivine, who proved in 1977 that \(K_G \leq \tfrac{\pi}{2 \log (1 + \sqrt{2})}\) and conjectured that this bound was optimal.
% This conjecture stood for nearly thirty years, and was refuted by Braverman-Makarychev-Makarychev-Naor (BMMN) in 2011, who showed that \(K_G < \tfrac{\pi}{2 \log (1 + \sqrt{2})} - \varepsilon\) for some \(\varepsilon > 0\) that is not explicitly given.
% This strategy relied on the construction and analysis of \textit{rounding schemes}, which are used to discretize continuous vectors.
% However, the argument in BMMN is restricted to the special case of \textit{suboptimal mixed rounding schemes}, which lead to only tiny numerical improvements (\(\varepsilon \approx 10^{-53}\)) when the argument is fleshed out and {\color{red}XXXXX}.
% While this would establish an explicit bound, it is not significant enough to make an impact in applied contexts.


% The specific technique employed was to construct and analyze ``rounding schemes'' that would evidence this gap.
% However, the particular analysis used in BMMN relied on the use of suboptimal mixed rounding schemes, which they used to show the existence of such an \(\varepsilon\), for which a numerical value was not given.
% Importantly, even when such an argument was fleshed out, the analysis yields only tiny numerical improvements on the order of \(\varepsilon \approx 10^{-53}\) that would not make a significant impact in applied contexts.


In this work, we overcome the limitations of BMMN's mixing arguments, allowing us to more tightly analyze a broader class of rounding schemes and thus achieve tighter bounds on \(K_G\).
Notably, our discovery and analysis of schemes is automatable within an AI-agentic discovery loop, using which we prove that
\[
K_G < \frac{\pi}{2 \log (1 + \sqrt{2})} - 10^{-5}.
\]
As part of this effort, we additionally refute BMMN's conjecture on the optimality of ``tiger partition'' rounding schemes.
Furthermore, we establish asymptotic results on the K\"onig bilinear form, which is related to the Grothendieck constant.
In summary, this work establishes the best known numerical upper bound on the Grothendieck constant, and also improves our understanding on the analysis of rounding schemes.

% In this work, we remove this main obstruction from their argument, which allows us to access a broader class of both pure and mixed rounding schemes that obtain improved upper bounds on $K_G$.  
% Towards computing the Grothendieck constant, we computationally refute a conjecture of BMNN that a certain class of rounding schemes they call tiger partitions are optimal for the Grothendieck constant. 
% This overturns the prevailing search paradigm for rounding schemes and reveals that the space of potentially optimal partitions is far larger and mostly unexplored. To effectively explore this search space, we do an AI-assisted search, which yields new schemes that give us our best improvement,
% \[
% K_G < \frac{\pi}{2 \log (1 + \sqrt{2})} - 10^{-5}.
% \]
% Additionally, we prove an asymptotic result about the K\"onig bilinear form, which is closely related to the Grothendieck constant. 





% The smallest such constant is called the (real) \textit{Grothendieck constant}, and is notably independent of the dimensions of \(A\).
% This constant naturally arises across diverse disciplines, including Banach space theory, combinatorial optimization, computational complexity, and quantum information theory.
% Despite its ubiquity, the exact value of \(K_G\) is unknown.

% {\color{red} PREVIOUS TEXT BELOW}


% The Grothendieck inequality is very important in many areas of mathematics, including the theory of Banach spaces, combinatorial optimization, complexity theory, $C^*$ algebras, and quantum information theory. 
% Despite its ubiquity in many seemingly unrelated disciplines, the value of $K_G$ remains unknown. Krivine proved that $K_G \le \frac{\pi}{2 \log(1 + \sqrt{2})}$, and he further conjectured that this bound is optimal. This conjecture stood for nearly thirty years, and was refuted by Barverman-Makarychev-Markarychev-Naor in a seminal paper where they showed that $K_G < \frac{\pi}{2 \log(1 + \sqrt{2})} - \epsilon$ for some $\epsilon$ that they do not explicitly compute. 
% Their method, despite being effective, faces an analytic obstruction that makes them use \textit{suboptimal mixed rounding schemes}, which then lead to poor bounds on $K_G$.
% In this work, we remove this main obstruction from their argument, which allows us to access a broader class of both pure and mixed rounding schemes that obtain improved upper bounds on $K_G$.  
% Towards computing the Grothendieck constant, we computationally refute a conjecture of Braverman et. al that a certain class of rounding schemes they call tiger partitions are optimal for the grothendieck constant. 
% This overturns the prevailing search paradigm for rounding schemes, and reveals that the space of potentially optimal partitions is far larger and mostly unexplored. To effectively explore this search space, we do an AI assisted search, which yields new schemes that give us our best improvement,
% \[
% K_G < \frac{\pi}{2 \log (1 + \sqrt{2})} - 10^{-5}.
% \]
% Additionally, we prove an asymptotic result about the K\"onig bilinear form, which is closely related to the Grothendieck constant. 



%%%%%%

%%% Start of May 25 version

% \color{blue}
% The Grothendieck inequality asserts the existence of a universal constant $K_G < \infty$ such that for every real matrix $A = (a_{ij})$,
% \[
% \sup_{\|x_i\| = \|y_j\| = 1} \sum_{i,j} a_{ij} \langle x_i, y_j \rangle
% \;\le\;
% K_G \sup_{\varepsilon_i, \delta_j \in \{-1,1\}}
% \sum_{i,j} a_{ij} \varepsilon_i \delta_j .
% \]
% The smallest such constant is called the (real) \textit{Grothendieck constant}, and is notably independent of the dimensions of the matrix. 
% The Grothendieck inequality is very important in many areas of mathematics, including the theory of Banach spaces, combinatorial optimization, complexity theory, $C^*$ algebras, and quantum information theory. 
% Despite its ubiquity in many seemingly unrelated disciplines, the value of $K_G$ remains unknown. Krivine proved that $K_G \le \frac{\pi}{2 \log(1 + \sqrt{2})}$, and he further conjectured that this bound is optimal. This conjecture stood for nearly thirty years, and was refuted by Barverman-Makarychev-Markarychev-Naor in a seminal paper where they showed that $K_G < \frac{\pi}{2 \log(1 + \sqrt{2})} - \epsilon$ for some $\epsilon$ that they do not explicitly compute. 
% Their method, despite being effective, faces an analytic obstruction that makes them use \textit{suboptimal mixed rounding schemes}, which then lead to poor bounds on $K_G$.
% In this work, we remove this main obstruction from their argument, which allows us to access a broader class of both pure and mixed rounding schemes that obtain improved upper bounds on $K_G$.  
% Towards computing the Grothendieck constant, we computationally refute a conjecture of Braverman et. al that a certain class of rounding schemes they call tiger partitions are optimal for the grothendieck constant.
% % In particular, they do a weighted combination of rounding schemes (which are partitions of $\R^n$ to show that one can beat the hyperplane. However, their weighting dilutes the gains from the rounding schemes themselves. They conjecture that this weighting may not be necessary. 
% % In this work, we remove this obstruction and are thus able to use a broader class of mixed rounding schemes  
% % Our argument unlocks certain types of weightings that were not allowed in the Braverman paper. We observe a phenomenon that weighting can sometimes do better than the component schemes. This is due to the mixing allowing the rounding to implicitly choose different geometries for different vectors. 
% This overturns the prevailing search paradigm for rounding schemes, and reveals that the space of potentially optimal partitions is far larger and mostly unexplored. To effectively explore this search space, we do an AI assisted search, which yields new schemes that give us our best improvement,
% \[
% K_G < \frac{\pi}{2 \log (1 + \sqrt{2})} - 10^{-5}.
% \]
% Additionally, we prove an asymptotic result about the K\"onig bilinear form, which is closely related to the Grothendieck constant. 

%%% end-of May version




% \noindent The Grothendieck inequality asserts the existence of a universal constant
% $K_G < \infty$ such that for every real matrix $A = (a_{ij})$,
% \[
% \sup_{\|x_i\| = \|y_j\| = 1} \sum_{i,j} a_{ij} \langle x_i, y_j \rangle
% \;\le\;
% K_G \sup_{\varepsilon_i, \delta_j \in \{-1,1\}}
% \sum_{i,j} a_{ij} \varepsilon_i \delta_j .
% \]
% The smallest such constant is called the (real) Grothendieck constant, and is notably independent of the dimensions of the matrix. The Grothendieck inequality is very important in many major areas of mathematics, including computational complexity, combinatorial optimization, theory of $C^*$ algebras, and quantum information theory. Krivine proved that $K_G \le \frac{\pi}{2 \log(1 + \sqrt{2})}$, and conjectured that this bound is optimal. This was refuted by BMMN in a seminal paper, where they show that $K_G < \frac{\pi}{2 \log(1 + \sqrt{2})} - \epsilon$ for some non-explicit $\epsilon$. 

% In their paper, they take the following approach for a proof: they consider a perturbation of the hyperplane, and use this analytic object called K\"onig's bilinear form to obtain an improvement over the baseline hyperplane. Then they do a mixing argument, where they mix the perturbation with the hyperplane rounding. This gives a rounding scheme which they show beats the hyperplane, thus obtaining a better bound. 

% The main obstruction to getting a good explicit bound is the mixing argument in its current form. Their approach requires the mixing parameter to be extremely small, which makes gains in $K_G$ very small. They talk about this obstruction by conjecturing that the mixing might not be needed, but do not resolve this. 

% In this paper, we remove this obstruction through an analytic argument that bypasses the mixing argument. This readily improves the bound significantly. 

% In particular, our argument still allows for mixing, but unlike BMMN's argument, it no longer requires the mixing parameters to be miniscule. 

% Indeed, we observe a phenomenon, that mixing rounding schemes can sometimes improve the upper bound on $K_G$ compared to both component schemes. This is due to the mixing allowing the rounding to implicitly choose different geometries for different vectors.   

% BMMN conjecture, in particular, that a certain class of rounding schemes given by tiger partitions are optimal for the grothendieck constant. In this paper, we computationally refute this. In addition, we give an example where improving the K\"onig form is not sufficient to improve $K_G$.  This overturns the prevailing search paradigm for rounding schemes, and reveals that the space of potentially optimal partitions is far larger and mostly unexplored. 

% We do an AI assisted search, and it yields new mixed schemes that give us our best improvement. 
% \[
% K_G < \frac{\pi}{2 \log (1 + \sqrt{2})} - 10^{-5}
% \]
% }

    
\medskip

% \tableofcontents

==> old/acknowledgements.tex <==
Thank people and also grants that fund us. 

==> old/approach.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{harness.png}
    \caption{Workflow}
    \label{fig:placeholder}
\end{figure}

\begin{itemize}
    \item \textbf{Input}: A proof graph is provided by a human. Nodes in this proof graph can contain trusted axioms. The proof needs to compile. Also numerical oracles are provided. 
    \item \textbf{Approach}: Use an agent harness to refine the proof graph. It consists of three parts -  
    \begin{itemize}
        \item \textbf{Planner} - creates a comprehensive plan of how to modify the proof graph. 
        \item \textbf{Generator} - writes lean code, executes the modification to the proof graph. 
        \item \textbf{Evaluator} - checks the numerical bounds, checks that everything has been generated honestly, no axioms have been added. This is semi automatic. 
    \end{itemize}
    \item \textbf{Output}: Refined proof graph. 
\end{itemize}


\hrulewidth

Approach involves partial formalization and AI-guided proof refinement.

Humans provide:
\begin{itemize}
\item Partial formalization of an existing proof of the bound on the constant $C$. What this means is parts of the proof is formalized, with the rest fixed as axioms. In our problems this involves breaking up the proof into subproblems, and each is resolved with axiom. This will be seeded as the initial proof candidate for the AI-guided iterative loop, so human bias on what parts of the proof can be encoded here. In particular, the partial formalization/proof skeleton defines the scaffolding the AI agent is able to use in its iterative proof refinement, so the more fine grained the easier it is for the AI to perform edits. We want to provide more of this scaffolding in areas where we want it to improve on, and for areas where we don't forsee needing to change we can just axiomize it in the simplest way possible. 

\item Trusted numerical library of functions that can be useful in the proof. There are still many gaps in the capabilities of mathlib, and particularly for heavy numerical computation it can be much more feasible to perform them externally in python. As such, we provided a curated set of numerical functions such as [...] The proof candidate would be able to call any of these functions and declare its output to be an axiom. (should we enforce just Arb?)

\item Evaluator/Verifier. This checks every proof candidate, ensuring that the axioms that are declared are either a) from the paper as in the original partial formaization, or b) a result of calling a numerical function and using the output correctly and honestly. Note that effective bound for the constant $C$ is alreadly included in the proof candidate, so the evaluator does not need to check for this.

\end{itemize}


The AI-guided iterative loop:
\begin{itemize}

% file structure?
% abstract out the tool use and the experience.md as part of the AI system?

\item Humans provide the initial prompt to the AI system, giving it instructions and suggestions on what to try improving, and potential ideas.

\item The AI system takes the current database of proof candidates (and past experience), and thinks about what approach it wants to take for the next proof candidate.

\item As the AI system writes the proof candidate, it is able to run numerical experiments to guide its writing.

\item Once it is done, the proof candidate is passed to the evaluator, and if it is certified to be correct, then it is stored in the database.

\item Throughout this process, the AI system updates a .md file with its findings that it want to pass along to future iterations.

\item At any point the human can converse with the AI system, and steer it based on what it is outputting.
\end{itemize}

We want to design the AI system used here to be such that it both encourages novelty and efficiency. We use the following agentic framework:

\begin{itemize}
    \item The orchestration agent controls everything. This uses the strongest LLM model and continually comes up with new mathematical ideas and spawns/directs subagents to work on it.

    \item The subagents create proof candidates, runs experiments and reports back to the orchestration agent.

    \item The orchestration agent can decide when to kill a subagent.
\end{itemize}

While other frameworks can be easily plugged in here, we show experimentally that our framework performs better than other popular approaches (ShinkaEvolve).

Justification of our approach:
\begin{itemize}
    \item Full formalization is hard and computationally expensive. Moreover, mathlib is still lacking in many areas.

    \item On the other hand, if we had no formalization at all and the AI worked with natural language or code, then there is no grounding and the AI becomes very prone to hallucinations.

    \item Partial formalization provides the best of both worlds. The key insight is that what can be improved on are only specific parts of the proof, and there is no need to formalize all the other parts.

    \item Our framework allows for humans to provide domain knowledge/bias by choosing what to focus on in the partial formalization, what to include in the numerical library, and how to prompt the AI.

    \item (Talk about why our agentic framework is better than shinkaevolve?)
\end{itemize}

==> old/background.tex <==


% define the task formally using notation
Let $C$ be a constant that is being optimized. Let $L$ be a fully or partially formalized lean proof of some bound $C \ge c_0$ (for upper bound simply negate $C$). The goal is to have an algorithm $\mathcal{A}$ that takes $L$ as an input, and spits out $L'$ proving $C \ge c$ for $c > c_0$. 

{\color{red}
I am not a big fan of formalizing what a constant is so early because (1) I think introducing formalization too fast can make you lose readers, and (2) I think it will be very hard to formalize what a constant even is, rigorously. However, relevant notation to this discussion is hard to avoid, so we need to vague-post in a semi-formalized manner. One idea sketch is below.

We broadly define bounding constants as the following problem.
Let \(\varphi\) be a proof (whether in English prose, Lean, etc) of some constant for which there are corresponding values \(c_- < c_+\) that bound it.
The idea is to use an AI agent \(\mathcal{A}\) to find a sequence of refined proofs
\[
    \varphi^{(0)} \xrightarrow{\mathcal{A}} \varphi^{(1)} \xrightarrow{\mathcal{A}} \varphi^{(2)} \xrightarrow{\mathcal{A}} \cdots,
\]
such that the lower and upper-bounds monotonically improve as \(c_- ^{(0)} \leq c_- ^{(1)} \leq \cdots\) and \(c_+ ^{(0)} \geq c_+ ^{(1)} \geq \cdots\).
}

\red{Wasn't one of the OG constant-bounders Archimedes drawing $n$-gons in the sand so that he could better approximate $\pi$, and thus do better astronomy? IMO, historical anecdotes are often a little out of place for modern ML papers, but I think it's well-warranted here if you guys want to try it out.}




% define grothendieck's constant and importance 
\paragraph{The Grothendieck constant}
Groethendieck's inequality states that there exists a constant \(K_G > 0\), such that for all \(A \in \R^{m \times n}\):
\begin{equation}
    \max_{x_i, y_j \in \{\pm 1\}} \bigg|
    \sum_{i, j} a_{ij} x_i y_j \bigg|
    \leq \sup_{d \geq 1} \max_{\substack{u_i, v_i \in \mbb{R}^{d} \\ \norm{u_i} = \norm{v_j} = 1}} \bigg| \sum_{i, j} a_{ij} \angles{u_i, v_j} \bigg|
    \leq \max_{x_i, y_j \in \{\pm 1\}}
    K_G \bigg| \sum_{i, j} a_{ij} x_i y_j \bigg|,
\end{equation}
This constant is independent of \(m\) and \(n\), with the current best lower \cite{Ree91} and upper bound \cite{braverman2011grothendieckconstantstrictlysmaller} being:
\begin{equation}
    1.676\ldots < K_G < 1.782\ldots
\end{equation}
Groethendieck's inequality is of interest in combinatorial optimization because it establishes a fundamental limitation of how well continuous programs can approximate discrete ones.
One connection is in the optimality gap between an integer quadratic program and its semidefinite relaxation. Consider the following integer quadratic program:
\begin{equation}
\mrm{IQP}(A)
    \quad \defeq \quad
    \max_{x \in \{\pm 1\}^m, y \in \{\pm 1\}^n}
    \enskip \sum_{i,j} a_{ij} x_i y_j,
\end{equation}
and its continuous relaxation, which is a semidefinite program of the form:
\[
\mathrm{SDP}(A)\;\defeq\;
\max_{\substack{x_1,\ldots,x_m\in S^{d-1}\\ y_1,\ldots,y_n\in S^{d-1}}}
\;\sum_{i=1}^{m}\sum_{j=1}^{n} a_{ij}\,\langle x_i, y_j\rangle ,
\]
Groethendieck's inequality then states that:
\begin{equation}
    \abs{\mrm{IQP}(A)}
    \leq \abs{\mrm{SDP}(A)}
    \leq K_G \cdot \abs{\mrm{IQP}(A)}.
\end{equation}
One way to upper-bound \(K_G\) is via the design and analysis of
\emph{rounding schemes}.
A rounding scheme is a (possibly randomized) procedure that maps a solution
\(\{x_i\}_{i=1}^m,\{y_j\}_{j=1}^n \subset S^{d-1}\) of the semidefinite relaxation
to signs \(x_i,y_j \in \{\pm1\}\).
We say that a rounding scheme has approximation ratio
$\alpha \in (0,1]$ if for every real matrix $A$,
\[
\mathbb{E} \left[\sum_{i=1}^{m}\sum_{j=1}^{n}
a_{ij}\,\hat{x}_i \hat{y}_j \right]
\;\ge\;
\alpha \cdot \mathrm{SDP}(A),
\]
where $\hat{x}_i,\hat{y}_j \in \{\pm1\}$ denote the rounded variables.

Since $\mathrm{IQP}(A)$ is defined as the maximum of
$\sum_{i,j} a_{ij} x_i y_j$ over all sign assignments
$x_i,y_j \in \{\pm1\}$, it follows that for any rounding scheme,
\[
\mathbb{E} \left[\sum_{i,j} a_{ij}\,\hat{x}_i \hat{y}_j \right]
\;\le\;
\mathrm{IQP}(A).
\]
Combining these inequalities, we obtain
\[
\mathrm{SDP}(A)
\;\le\;
\alpha^{-1}\,\mathrm{IQP}(A),
\]
and hence any rounding scheme with approximation ratio $\alpha$
yields the bound $K_G \le \alpha^{-1}$ on the Grothendieck constant.

\red{Given the nature of this work, we also need to describe the proof strategy of Grothendieck and identify the specific points at which it is AI-blastable.
If we want to fit this in NeurIPS-constraints, we can afford at about one page of background + proof technique for each Grothendieck and Korenblum (some may feel that this is even too generous!).
Writing that concisely is very hard, so I encourage you guys to word barf as much as you want, and then we can polish after.
}


% define koremblum's constant and importance
\paragraph{The Korenblum constant.}
The Korenblum constant arises in complex analysis, specifically in the theory of Bergman spaces. At a high level, it measures how much of an analytic function on the unit disk is controlled by its behavior near the boundary. This is a genuinely Bergman-space phenomenon: for the supremum norm, domination on any outer annulus immediately controls the full disk by the maximum modulus principle, and for Hardy spaces the analogous statement follows from radial monotonicity of integral means. In the Bergman space, however, the norm is an area norm over the disk, so a function can in principle concentrate mass near the origin while remaining small near the boundary. Korenblum's problem asks whether analyticity prevents this from happening once the annulus of domination is sufficiently thick. The sharp threshold at which this becomes true is Korenblum's constant.

Let \(\mathbb{D}=\{z\in \mathbb{C}: |z|<1\}\), and let \(A^2(\mathbb{D})\) denote the Bergman space of analytic functions \(f:\mathbb{D}\to \mathbb{C}\) with finite norm
\[
    \|f\|_{A^2(\mathbb{D})}^2
    =
    \frac{1}{\pi}\int_{\mathbb{D}} |f(z)|^2\,dA(z).
\]
Equivalently, if \(f(z)=\sum_{k=0}^{\infty} a_k z^k\), then
\[
    \|f\|_{A^2(\mathbb{D})}^2
    =
    \sum_{k=0}^{\infty}\frac{|a_k|^2}{k+1}.
\]
For \(0<c<1\), write
\[
    A(c,1)=\{z\in \mathbb{C}: c<|z|<1\}
\]
for the outer annulus. Korenblum conjectured that there exists a universal \(c\in(0,1)\) such that for all \(f,g\in A^2(\mathbb{D})\),
\[
    |f(z)|\le |g(z)| \quad \text{for all } z\in A(c,1)
    \qquad\Longrightarrow\qquad
    \|f\|_{A^2(\mathbb{D})}\le \|g\|_{A^2(\mathbb{D})}.
\]
The sharp transition radius is called the Korenblum constant:
\[
    \kappa
    :=
    \sup\left\{c\in(0,1):
    \begin{array}{l}
    \text{for all } f,g\in A^2(\mathbb{D}),\ 
    |f|\le |g| \text{ on } A(c,1)\\
    \text{implies } \|f\|_{A^2(\mathbb{D})}\le \|g\|_{A^2(\mathbb{D})}
    \end{array}
    \right\}.
\]
Thus the Korenblum maximum principle holds for annuli \(A(c,1)\) with \(c<\kappa\), and fails for \(c>\kappa\). Hayman first proved the existence of such a positive constant, obtaining an explicit lower bound; later work of Hinkkanen and Wang improved the lower bound, while counterexamples based on singular inner functions and Blaschke products give upper bounds. The proofs are highly quantitative: they compare the positive mass of \(|g|^2-|f|^2\) on an outer annulus against the possible excess of \(|f|^2-|g|^2\) near the origin. This makes Korenblum's constant a natural target for our framework: the argument has a rigid analytic structure, but the final certified bound depends on many explicit inequalities and numerical choices that can be locally refined and globally propagated through a proof graph.

\red{Ditto for Korenblum}


==> old/checklist.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1--2 sentence) justification right after your answer (even for \answerNA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will also be asked to include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While \answerYes{} is generally preferable to \answerNo{}, it is perfectly acceptable to answer \answerNo{} provided a proper justification is given (e.g., error bars are not reported because it would be too computationally expensive'' or ``we were unable to find the license for the dataset we used''). In general, answering \answerNo{} or \answerNA{} is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> old/coefficient_computation_formulas_v1.tex <==

First, we describe how to do the necessary computation of the coefficients of the Taylor series. 

\section{Coefficient Computation Formulas}
\label{sec:coefficient-computation-formulas}

In this section, we describe the analytic facts needed to compute the coefficients of Taylor series of $H_{f,g}$ and $H_{f,g}^{-1}$ used in the proof.
\vspace{1em}
Let \(h_n\) denote the physicist's Hermite polynomial and set
\[
    \HermBasis_n(x):=\frac{h_n(x)}{\sqrt{2^n n!}},
    \qquad
    d\mu(x):=\pi^{-1/2}e^{-x^2}\,dx.
\]
Then \(\{\HermBasis_n\}_{n\ge0}\) is an orthonormal basis for \(L^2(\mu)\).

\begin{lemma}[Hermite--Mehler reduction]\label[lemma]{lemma:hermite-mehler-reduction}
For the \(\Hermite\) scheme, define the Hermite coefficients
\[
    \HermCoeff_{a,b}
    :=
    \int_{\mathbb R^2}
        f(x,y)\HermBasis_a(x)\HermBasis_b(y)
    \,d\mu(x)d\mu(y).
\]
Then
\[
    H(z)
    =
    \frac{\pi}{2}
    \sum_{a,b\ge0}
        (-1)^a \HermCoeff_{a,b}^2 z^{a+b}.
\]
Equivalently,
\[
    [z^n]H(z)
    =
    \frac{\pi}{2}
    \sum_{a=0}^{n}
        (-1)^a \HermCoeff_{a,n-a}^2.
\]
Moreover, the two-dimensional coefficients reduce to the one-dimensional
integrals
\[
    \HermCoeff_{a,b}
    =
    \int_{\mathbb R}
        \HermBasis_a(x)
        \ThresholdCoeff_b\!\left(\tau\HermBasis_3(x)\right)
    \,d\mu(x),
\]
where
\[
    \ThresholdCoeff_0(u)=-\operatorname{erf}(u),
\]
and, for \(b\ge1\),
\[
    \ThresholdCoeff_b(u)
    =
    \frac{2}{\sqrt\pi}
    e^{-u^2}
    \frac{\HermBasis_{b-1}(u)}{\sqrt{2b}}.
\]
\end{lemma}

\begin{proof}
Expanding \(f\) in the orthonormal tensor-product basis gives
\[
    f(x,y)=\sum_{a,b\ge0}
        \HermCoeff_{a,b}\HermBasis_a(x)\HermBasis_b(y).
\]
For the \(\Hermite\) scheme we have \(g(x,y)=f(-x,y)\).  Since
\(\HermBasis_a(-x)=(-1)^a\HermBasis_a(x)\), the corresponding coefficient of
\(g\) is \((-1)^a\HermCoeff_{a,b}\).

The Mehler kernel diagonalizes in this basis: the basis vector
\(\HermBasis_a(x)\HermBasis_b(y)\) has eigenvalue \(z^{a+b}\).  Therefore
\[
    H(z)
    =
    \frac{\pi}{2}
    \sum_{a,b\ge0}
        (-1)^a \HermCoeff_{a,b}^2 z^{a+b},
\]
which gives the displayed coefficient formula.

It remains to reduce \(\HermCoeff_{a,b}\) to one dimension.  For fixed \(x\),
the partition is
\[
    f(x,y)=\operatorname{sgn}\!\left(y-\tau\HermBasis_3(x)\right).
\]
Thus the \(y\)-coefficient is
\[
    \ThresholdCoeff_b(u)
    :=
    \int_{\mathbb R}
        \operatorname{sgn}(y-u)\HermBasis_b(y)\,d\mu(y).
\]
For \(b=0\), this equals \(-\operatorname{erf}(u)\).  For \(b\ge1\), using
\[
    \frac{d}{dy}\left(e^{-y^2}h_{b-1}(y)\right)
    =
    -e^{-y^2}h_b(y)
\]
gives
\[
    \ThresholdCoeff_b(u)
    =
    \frac{2}{\sqrt\pi}
    e^{-u^2}
    \frac{\HermBasis_{b-1}(u)}{\sqrt{2b}}.
\]
Substituting \(u=\tau\HermBasis_3(x)\) gives the claimed one-dimensional
formula for \(\HermCoeff_{a,b}\).
\end{proof}

Next we convert the Taylor coefficients of \(H\) into the Taylor coefficients
of its inverse.

\begin{lemma}[Inverse coefficients by Lagrange inversion]
\label[lemma]{lemma:lagrange-inverse-coefficients}
Since \(H\) is odd, write
\[
    H(z)=z\OddFactor(z^2).
\]
Then \(H^{-1}\) has only odd coefficients, and
\[
    a_{2k+1}
    =
    \frac{1}{2k+1}
    [t^k]\OddFactor(t)^{-(2k+1)},
    \qquad
    a_{2k}=0.
\]
\end{lemma}

\begin{proof}
This is the standard Lagrange inversion formula applied to the odd map
\(H(z)=z\OddFactor(z^2)\).  Oddness of \(H\) implies oddness of the local
inverse branch, so the even inverse coefficients vanish.
\end{proof}

==> old/discussion.tex <==
{\bf \color{red} For each constant, have the following. 

Agent search:
\begin{itemize}
    \item What did the agent try?
    \item What local quantities did it optimize?
    \item What numerical feedback was available?
    \item What failed?
\end{itemize}

Improved certificate:
\begin{itemize}
    \item Which local lemma improved?
\end{itemize}
}

\subsection{The Grothendieck Constant}



\subsection{The Korenblum Constant}


==> old/explicit.tex <==
\section{The Explicit $10^{-5}$ Improvement}
\label{sec:ai}


\todo{Add figures of partitions}

The pure $h_3/\!-\!h_3$ scheme of Section~2.2 already gives a Krivine
parameter $\gamma$ satisfying $\gamma - \rhostar \in
(4.8 \cdot 10^{-6},\, 5.2 \cdot 10^{-6})$. To push the bound by a
further order of magnitude we search over a much broader family of
partitions and over their convex combinations. This section describes
the search and reports its result.

The entire search pipeline below was orchestrated by an AI coding
agent (Anthropic's Opus~4.7), which generated candidate partitions,
trained them, assembled dictionaries, and ran the mixture
optimisations. Every numerical statement in this section is a
heuristic produced by that pipeline; the certified versions, with
strict Arb interval arithmetic, are obtained by the same machinery as
in Section~3.2 and are reported in Theorem~4.1 below.

% ---------------------------------------------------------------------
\subsection{Mixtures of correlation functions}
\label{sec:ai-mixtures}

Let $(f^{(1)}, g^{(1)}), \ldots, (f^{(k)}, g^{(k)})$ be pairs of odd
measurable maps $\R^d \to \{-1, 1\}$, and let
$H^{(i)} = H_{f^{(i)}, g^{(i)}}$ be the arcsine-normalised correlation
function attached to the $i$-th pair. For a probability vector
$p \in \simplex^{k-1}$, define the \emph{mixture}
\begin{equation}
  H_p(t) := \sum_{i=1}^{k} p_i\, H^{(i)}(t).
  \label{eq:mixture-def}
\end{equation}
The function $H_p$ is itself the arcsine-normalised correlation of an
honest rounding scheme: before rounding, sample an index
$i \in \{1, \ldots, k\}$ with probability $p_i$, then apply
$(f^{(i)}, g^{(i)})$. Linearity in $p$ is preserved coefficient by
coefficient,
\begin{equation}
  [z^{n}]\, H_p(z) \;=\; \sum_{i=1}^{k} p_i \, [z^{n}]\, H^{(i)}(z).
  \label{eq:bseries-linear}
\end{equation}
Consequently, if $H_p^{-1}(\zeta) = \sum_{n \geq 1} a_n(p)\, \zeta^n$
denotes the local inverse branch at the origin, the inverse Taylor
coefficients $a_n(p)$ are computable from the $H^{(i)}$'s by Lagrange
inversion applied to~\eqref{eq:bseries-linear}.

For each $p \in \simplex^{k-1}$ the inverse-majorant
\[
  M_p(\gamma) \;:=\; \sum_{n \geq 1} |a_n(p)|\, \gamma^n
\]
is strictly increasing in $\gamma$ on $[0, \rhostar + \delta)$ for some
$\delta > 0$ (because $a_1(p) > 0$ for every mixture we use). Let
$\gamma(p)$ denote the unique solution of $M_p(\gamma) = 1$. The
Krivine criterion (Section~2.1) gives
\begin{equation}
  K_G \;\leq\; \frac{\pi}{2\, \gamma(p)}
  \quad \text{for every } p \in \simplex^{k-1}.
  \label{eq:KG-from-gamma-p}
\end{equation}
The search problem of this section is therefore
\begin{equation}
  \boxed{\;\;
  \gamma^{\star} \;:=\; \max_{p \in \simplex^{k-1}} \gamma(p).
  \;\;}
  \label{eq:search-problem}
\end{equation}

Two remarks.
First, the pure $h_3$ scheme corresponds to taking $k = 1$ with
$(f^{(1)}, g^{(1)})$ the partition of Section~2.2; the search
in~\eqref{eq:search-problem} therefore tautologically improves on
that scheme provided the dictionary contains it.
Second, mixing is genuinely useful: we will find that the optimum
$\gamma(p)$ over a small dictionary strictly exceeds the maximum of
the individual $\gamma(e_i)$, with the second-best component
contributing a few percent of the mixture mass.

% ---------------------------------------------------------------------
\subsection{The search space: trainable Hermite-threshold partitions}
\label{sec:ai-family}

We allow the partition pair $(f, g)$ to come from one of two families.

\paragraph{Two-dimensional partitions.}
For an odd polynomial $\Phi \colon \R \to \R$, set
\begin{equation}
  f_\Phi(x_1, x_2) \;=\; \sgn\bigl(x_2 - \Phi(x_1)\bigr),
  \qquad
  g_\Phi(x_1, x_2) \;=\; f_\Phi(-x_1,\, x_2).
  \label{eq:2D-family}
\end{equation}
The $h_3$ partition of Section~2.2 is the choice $\Phi = \tau \psi_3$
with $\tau = 0.03175$, so this family strictly contains the baseline.

\paragraph{Three-dimensional partitions.}
For an odd polynomial $\Phi \colon \R^2 \to \R$, set
\begin{equation}
  f_\Phi(x_1, x_2, x_3) \;=\; \sgn\bigl(x_3 - \Phi(x_1, x_2)\bigr),
  \qquad
  g_\Phi(x_1, x_2, x_3) \;=\; f_\Phi(-x_1,\, x_2,\, x_3).
  \label{eq:3D-family}
\end{equation}
Allowing $\Phi$ to depend on two variables enlarges the geometric
freedom of the threshold surface.

\paragraph{Parameterisation.}
In both families we write $\Phi$ in the orthonormal physicist-Hermite
basis, expanded up to total degree $D$:
\[
  \Phi(x) \;=\; \sum_{|\alpha| \leq D,\; \text{odd}} c_\alpha\,
  \psi_{\alpha_1}(x_1)\, \psi_{\alpha_2}(x_2) \cdots,
\]
where $\psi_n(x) = \Hphys_n(x)/\sqrt{2^n n!}$ is the orthonormal
physicist-Hermite basis function and the sum runs over odd multi-indices
$\alpha$ with $|\alpha| \leq D$. In the two-dimensional family the
multi-index has one entry; in the three-dimensional family it has two.
The parameters $\{c_\alpha\}$ form the trainable vector that the search
optimises in Stage~1 below.

% ---------------------------------------------------------------------
\subsection{Methodology}
\label{sec:ai-method}

Maximising $\gamma$ jointly over all partition parameters
$\{c_\alpha\}$ and over the mixture weights $p$ is non-convex and
high-dimensional. We solve it in two stages.

\paragraph{Stage 1 — candidate training.}
For each ambient dimension and each total degree
$D \in \{3, 5, 7, 9\}$, the agent runs the following loop. Starting
from a random initialisation of the parameters $\{c_\alpha\}$, it
performs gradient ascent on
\begin{equation}
  L_{\text{single}}(\Phi) \;:=\; \gamma\bigl(H_{f_\Phi, g_\Phi}\bigr),
  \label{eq:single-loss}
\end{equation}
where $\gamma(H)$ is the inverse-majorant root of the single-partition
correlation function $H$. The gradient is taken with respect to
$\{c_\alpha\}$ and is backpropagated through three components:
(i) a Gauss-Hermite quadrature for the Hermite expansion coefficients
$F_{a,b}$ of $f_\Phi, g_\Phi$;
(ii) the Newton iteration that produces $a_n$ from $[z^n] H$ by series
inversion;
(iii) the bisection that solves $M(\gamma) = 1$.
All three are differentiable in PyTorch, and the entire stack runs in
\texttt{float64} on CPU. Adam is used as the optimiser with a learning
rate of $\eta = 10^{-3}$, decaying on plateaus.

Whenever the trained $\gamma$ improves on a running best for the given
$(\text{dimension}, D)$ pair, the resulting $\Phi$ is added to the
dictionary of candidate partitions. We refer to candidates by the
labels
\texttt{N3\_V1, \ldots, N3\_V9} (two-dimensional, $9$ candidates) and
\texttt{N4\_V1, \ldots, N4\_V4} (three-dimensional, $4$ candidates).
The hyperplane (corresponding to $\Phi \equiv 0$, whose $H$ is exactly
$\arcsin$) is always included as an additional dictionary atom.

\paragraph{Stage 2 — mixture optimisation.}
With the dictionary $\{H^{(i)}\}_{i=1}^{k}$ fixed, the agent solves
\[
  \max_{p \in \simplex^{k-1}} \gamma(p)
\]
using SLSQP from many random Dirichlet initialisations $p^{(0)} \sim
\mathrm{Dir}(\mathbf{1}/2)$. The evaluation of $\gamma(p)$ for each
candidate $p$ involves one application
of~\eqref{eq:bseries-linear} (linear in $p$), one Newton series
inversion, and one bisection — at total cost $O(\Ncap^2)$ per call.
We terminate when independent random-seed runs agree on the first four
significant digits of $\gamma(p^\star)$; in our experiments this
occurred within $200$ restarts.

\paragraph{Numerical precision during search.}
All Stage~1 and Stage~2 evaluations truncate the Taylor expansion at
$\Ncap = 60$ and use a Gauss-Hermite quadrature with $\nq = 32$ nodes
per dimension (two-dimensional candidates) or $\nq = 22$
(three-dimensional candidates, where each Hermite coefficient is a
$\nq^{2}$-node integral). Earlier experiments at $\Ncap = 40$ exhibited
truncation-driven inflation of $\gamma - \rhostar$ of order
$10^{-6}$; the $\Ncap = 60$ runs are stable in the fourth digit across
seeds. The final certified $\gamma$ is computed in the same Arb
interval-arithmetic framework used in Section~3.2, with the same kind
of strict tail bound on the inverse series.

% 
% ---------------------------------------------------------------------
\subsection{Results}
\label{sec:ai-results}

We report certified $K_G$ upper bounds for four two-atom mixtures
$\mathcal{M}_3, \mathcal{M}_5, \mathcal{M}_7, \mathcal{M}_9$, indexed by the
maximum odd Hermite degree $d \in \{3, 5, 7, 9\}$ that appears in the
non-hyperplane component. Each mixture is defined as follows.

\paragraph{Definition of the mixtures.}
Let $h_k(x) := \mathrm{He}_k(x) / \sqrt{k!}$ denote the orthonormal
probabilist Hermite polynomial of degree $k$; the family
$\{h_k\}_{k \geq 0}$ is orthonormal with respect to the standard
Gaussian inner product
$\langle u, v\rangle := \mathbf{E}[u(X)\,v(X)]$ with $X \sim N(0, 1)$.
For each odd $d \in \{3, 5, 7, 9\}$, fix a coefficient vector
$c^{(d)} = (c_1^{(d)}, c_3^{(d)}, \ldots, c_d^{(d)}) \in \R^{(d+1)/2}$
and a hyperplane weight $p_d \in (0, 1)$, and set
\begin{equation}
  \Phi_d(x) \;:=\; \sum_{\substack{k\ \text{odd}\\ 1 \le k \le d}}
                   c_k^{(d)} \, h_k(x).
  \label{eq:phi-d}
\end{equation}
The mixture $\mathcal{M}_d$ is the convex combination of two rounding
schemes on $\R^2$: with probability $p_d$, the hyperplane scheme
$(\sgn(x_2),\, \sgn(x_2))$; with probability $1 - p_d$, the
Hermite-threshold pair from the two-dimensional family of §4.2,
\begin{equation}
  f_{\Phi_d}(x_1, x_2) \;=\; \sgn\bigl(x_2 - \Phi_d(x_1)\bigr),
  \qquad
  g_{\Phi_d}(x_1, x_2) \;=\; \sgn\bigl(x_2 + \Phi_d(x_1)\bigr).
  \label{eq:partition-restated}
\end{equation}
(For odd $\Phi_d$ this is the same as $g_{\Phi_d}(x_1,x_2)
= f_{\Phi_d}(-x_1, x_2)$ used in~\eqref{eq:2D-family}.)
The mixture's arcsine-normalised correlation function is
\begin{equation}
  H_{\mathcal{M}_d}(t) \;=\; p_d \, \arcsin(t)
  \;+\; (1 - p_d)\, H_{f_{\Phi_d},\, g_{\Phi_d}}(t).
  \label{eq:H-mixture-d}
\end{equation}

\paragraph{Coefficient vectors and hyperplane weights.}
The vectors $c^{(d)}$ and weights $p_d$ are produced by the search of
§4.3. Numerically,
\begin{center}
\renewcommand{\arraystretch}{1.2}
\small
\begin{tabular}{c|c|c|c|c|c|c}
$d$ & $p_d$ & $c_1^{(d)}$ & $c_3^{(d)}$ & $c_5^{(d)}$ & $c_7^{(d)}$ & $c_9^{(d)}$ \\
\hline
$3$ & $0.70058$ & $0$         & $-0.07508$ & ---        & ---        & ---        \\
$5$ & $0.70582$ & $-0.00100$  & $-0.07073$ & $-0.00970$ & ---        & ---        \\
$7$ & $0.70582$ & $-0.00100$  & $-0.07073$ & $-0.00970$ & $-0.00202$ & ---        \\
$9$ & $0.70582$ & $-0.00100$  & $-0.07073$ & $-0.00970$ & $-0.00202$ & $+0.00365$ \\
\end{tabular}
\end{center}
(For $d = 3$, $\Phi_3$ was obtained from a separate two-parameter
Adam optimisation over $(c_3, p_3)$; for $d \in \{5, 7, 9\}$, the
non-zero entries of $c^{(d)}$ and the hyperplane weight $p_d$ are taken
from the Stage 2 SLSQP convergence point at ambient degree $9$, with
the higher-degree coefficients set to zero and $p_d$ renormalised so
that the two atom weights sum to one. This explains why $c^{(5)},
c^{(7)}, c^{(9)}$ share their first three entries and a common $p_d$.)

\paragraph{Certified $K_G$ bounds.}
For each mixture $\mathcal{M}_d$, let $\gamma_d^{\text{search}}$ be
the heuristic value at which $M_{p_d}(\gamma) = 1$ holds at the search
precision ($\Ncap = 60$, IEEE \texttt{float64}). Let $\gamma_d^+$ be a
strict lower bound on the true root of $M_{p_d}(\gamma) = 1$, obtained
by the Arb-interval inverse-majorant pipeline of §3.2 at $b$-series
truncation $N = 240$, working precision $256$ bits, and certified
Gauss-Legendre quadrature with the panel parameters shown below.
The Krivine criterion~\eqref{eq:KG-from-gamma-p} then yields the
certified $K_G$ improvement
\[
  \Delta_d^{K_G} \;:=\; \frac{\pi}{2\rhostar}
                       - \frac{\pi}{2\,\gamma_d^+}.
\]

\begin{center}
\renewcommand{\arraystretch}{1.2}
\small
\setlength{\tabcolsep}{6pt}
\begin{tabular}{ccccc}
\hline
$d$ & $\gamma_d^{\text{search}} - \rhostar$ &
$\gamma_d^+ - \rhostar$ & $\Delta_d^{K_G}$ certified & $(L, \text{panels})$ \\
\hline
$3$ & $1.40 \cdot 10^{-5}$ & $1.00 \cdot 10^{-5}$
    & $2.022 \cdot 10^{-5}$ & $(8, 80)$ \\
$5$ & $2.71 \cdot 10^{-5}$ & $2.00 \cdot 10^{-5}$
    & $4.044 \cdot 10^{-5}$ & $(8, 80)$ \\
$7$ & $2.83 \cdot 10^{-5}$ & $2.50 \cdot 10^{-5}$
    & $5.055 \cdot 10^{-5}$ & $(8, 80)$ \\
$9$ & $3.06 \cdot 10^{-5}$ & \todo{$2.25\!\cdot\!10^{-5}$}
    & \todo{$4.55\!\cdot\!10^{-5}$ in progress} & $(6, 240)$ \\
\hline
\end{tabular}
\end{center}

Two effects compete across the rows of the table.
First, increasing $d$ enlarges the search space for the partition pair,
which yields a larger $\gamma_d^{\text{search}}$. Second, increasing $d$
also amplifies the maximum value of $|\varphi(\Phi_d(z))|$ on a complex
disk of radius $r$ centred on a real point of $[-L, L]$, where
$\varphi$ is the standard Gaussian density. This quantity controls the
Cauchy radius in the certified Gauss-Legendre quadrature of §3.2,
which forces narrower integration panels (smaller $r$) at larger $d$;
$d = 9$ requires both a smaller $L$ and a four-fold increase in panel
count compared with $d \in \{3, 5, 7\}$. The amplification of
$|\varphi(\Phi_d(z))|$ comes from the $z^{d}$ leading term of $h_d$,
so it grows like $\exp\bigl((c_d \cdot d \cdot L^{d-1}\cdot r /
\sqrt{d!})^2\bigr)$.
The certification at $d = 9$ also uses a parity identity
$I_g[i, j] = (-1)^i\,I_f[i, j]$, valid because the partition pair
satisfies $g_{\Phi_d}(x_1, x_2) = f_{\Phi_d}(-x_1, x_2)$ for odd
$\Phi_d$ and the variables are Gaussian; this halves the b-series
assembly cost.

\paragraph{Headline.}
Each row of the table delivers a certified $K_G$ upper bound
\[
  K_G \;\leq\; \frac{\pi}{2 \rhostar} - \Delta_d^{K_G}.
\]
The amplification factor between $\gamma_d - \rhostar$ and
$\Delta_d^{K_G}$ is $\pi/(2 \rhostar^2) \approx 2.022$; in particular
every certified $\Delta_d^{K_G}$ in the table comfortably exceeds the
headline threshold of $10^{-5}$. Combining the strongest of these
certified bounds with the Krivine preprocessing of Section~2 yields
our main quantitative result.

\begin{theorem}[Restatement of Theorem~1.2]
\label{thm:main-explicit}
There exists a Krivine rounding scheme, realised as a probability
mixture of two odd Hermite-threshold partitions in $\R^{2}$
(the hyperplane and the degree-$7$ polynomial threshold of the
form~\eqref{eq:partition-restated} with coefficient vector
$c^{(7)}$ above), whose inverse-majorant parameter $\gamma$ is
certified by Arb-interval arithmetic to satisfy
\[
  \gamma \;\geq\; \rhostar + 2.5 \cdot 10^{-5}.
\]
In particular,
\[
  K_G \;\leq\; \frac{\pi}{2\gamma}
  \;\leq\; \frac{\pi}{2 \log(1+\sqrt 2)} \;-\; 5 \cdot 10^{-5}.
\]
\end{theorem}

\todo{Once the $d = 9$ cert completes, restate
Theorem~\ref{thm:main-explicit} with the corresponding (stronger) bound.}

\paragraph{Robustness checks.}
The agent ran two further families of candidates to probe whether the
optimum at $\gamma^{\star}_{\text{2D+3D}}$ could be improved.
First, we added Krivine rotating-hyperplane partitions
\todo{cite Krivine 2023 rotating-hyperplane}
at $\sim\!20$ choices of the rotation parameter $\varepsilon$ and
ambient dimension $d$, and re-ran Stage~2. None of these atoms
received weight above $1.5 \cdot 10^{-3}$ in any seed, and
$\gamma^{\star}$ did not move.
Second, we added several hundred random Hermite-threshold partitions
of total degree up to $9$ and re-ran Stage~2. The optimum was again
unchanged.
These are evidence (not proof) that the value reported in
Theorem~\ref{thm:main-explicit} is at the ceiling of the search,
within the precision of $\Ncap = 60$ truncation.

\paragraph{Reproducibility.}
The dictionary state-dicts, the SLSQP output JSONs containing
$p^\star$ for every seed, and the training-time logs are available in
the project repository. The agent's full session transcripts,
including every prompt and every script invocation, are archived at
\todo{repo path of agent transcripts}, so that the entire search is
reproducible end-to-end.


==> old/filled_in_proof_outline.tex <==

\newcommand{\source}[1]{{\color{blue}\textsc{#1}}}
\newcommand{\gzero}{\gamma_0}
\newcommand{\rhostarval}{\rho_*}
\crefname{definition}{Definition}{Definitions}
\Crefname{definition}{Definition}{Definitions}
\crefname{theorem}{Theorem}{Theorems}
\Crefname{theorem}{Theorem}{Theorems}
\crefname{lemma}{Lemma}{Lemmas}
\Crefname{lemma}{Lemma}{Lemmas}
\crefname{corollary}{Corollary}{Corollaries}
\Crefname{corollary}{Corollary}{Corollaries}
\crefname{remark}{Remark}{Remarks}
\Crefname{remark}{Remark}{Remarks}


\section{The no-mixing theorem}

\begin{definition}[Real Grothendieck constant]\label{def:real-grothendieck-constant}
\source{Grothendieck.}
The real Grothendieck constant $K_G$ is the infimum over all $K>0$ such that, for every $m,n\in\mathbb N$ and every real matrix $A=(a_{ij})\in\R^{m\times n}$,
\[
\max_{x_i,y_j\in S^{m+n-1}}
\sum_{i=1}^m\sum_{j=1}^n a_{ij}\ip{x_i}{y_j}
\le
K\max_{\varepsilon_i,\delta_j\in\{-1,1\}}
\sum_{i=1}^m\sum_{j=1}^n a_{ij}\varepsilon_i\delta_j .
\]
\end{definition}

\begin{definition}[Gaussian correlation]\label{def:gaussian-correlation}
\source{Krivine/BMMN.}
Fix $k \in \mathbb{N}$, and let $f,g:\mathbb{R}^k\to\{-1,1\}$ be odd measurable functions.
Let $G_1,G_2$ be independent standard Gaussian vectors in $\mathbb{R}^k$.

The \emph{arcsine-normalized correlation} associated to $(f,g)$ is
\[
H_{f,g}(t)
:=
\frac{\pi}{2}\,
\mathbb{E}\left[
f\left(\frac{G_1}{\sqrt{2}}\right)
g\left(
\frac{tG_1+\sqrt{1-t^2}G_2}{\sqrt{2}}
\right)
\right],
\qquad -1<t<1.
\]
\end{definition}

\begin{lemma}[Basic analytic properties]\label{lem:correlation-profile-analytic}
Let $f,g:\mathbb{R}^k\to\{-1,1\}$ be odd measurable functions. Then $H_{f,g}$ is odd and
extends holomorphically to the strip
\[
S:=\{z\in\mathbb{C}: |\operatorname{Re}z|<1\}.
\]
In particular, if $H_{f,g}'(0)\neq 0$, then $H_{f,g}$ has a unique local inverse branch at
the origin, and this inverse branch is odd.
\end{lemma}

\begin{proof}
\source{BMMN.}
This is the standard analytic continuation of the Gaussian correlation kernel.  In the planar case used below we prove the stronger quantitative version in Lemma~\ref{lem:strip-bound}.
\end{proof}

\begin{definition}[Inverse majorant]\label{def:inverse-majorant}
Assume $H_{f,g}'(0)\neq 0$, and write the local inverse branch at the origin as
\[
H_{f,g}^{-1}(\zeta)=\sum_{n\ge 1} a_n \zeta^n .
\]
For $s\ge 0$, define the inverse-majorant series
\[
M_{f,g}(s):=\sum_{n\ge 1}|a_n|s^n,
\]
with the convention that $M_{f,g}(s)=+\infty$ if the series diverges.
\end{definition}

\begin{definition}[$\gamma$-admissible Krivine scheme]\label{def:gamma-admissible}
\source{Krivine/BMMN.}
Let $\gamma>0$. We say that $(f,g)$ is a \emph{$\gamma$-admissible Krivine rounding scheme}
if:
\begin{enumerate}[label=(\roman*)]
    \item $f,g:\mathbb{R}^k\to\{-1,1\}$ are odd and measurable;
    \item $H_{f,g}'(0)\neq 0$;
    \item the inverse-majorant inequality
    \[
    M_{f,g}(\gamma)=\sum_{n\ge 1}|a_n|\gamma^n \le 1
    \]
    holds.
\end{enumerate}
We call $(f,g)$ a \emph{Krivine rounding scheme} if it is $\gamma$-admissible for some
$\gamma>0$.
\end{definition}

\begin{theorem}[Krivine preprocessing in arcsine units]\label{thm:krivine-preprocessing}
If $(f,g)$ is a $\gamma$-admissible Krivine rounding scheme, then
\[
K_G \le \frac{\pi}{2\gamma}.
\]
\end{theorem}

\begin{proof}
\source{Krivine/BMMN.}
This is the standard Krivine preprocessing argument.  In the unnormalized convention it gives $K_G\le 1/c$; the present arcsine normalization is $c=2\gamma/\pi$, giving $K_G\le \pi/(2\gamma)$.  The use of $M_{f,g}(\gamma)\le 1$ rather than equality is harmless: the usual tensor-power embeddings have squared norm at most one, and one pads them by orthogonal coordinates to make them unit vectors.
\end{proof}

\begin{definition}[The $H_3$ scheme]\label{def:h3-scheme}
Let
\[
H_3(x)=8x^3-12x,
\qquad
\tau=0.03175,
\qquad
\eta=\frac{\tau}{\sqrt{48}}
=0.004582717761692655\ldots .
\]
Define odd measurable functions $f,g:\R^2\to\{\pm1\}$ by
\[
    f(x,y)=\sgn(y-\eta H_3(x)),
    \qquad
    g(x,y)=\sgn(y+\eta H_3(x)).
\]
We call $(f,g)$ the $H_3/-H_3$ scheme.
\end{definition}

The following is our main theorem.
\begin{tcolorbox}
\begin{theorem}[No Mixing Beats Hyperplane]\label{thm:no-mixing-beats-hyperplane}
Let
\[
\rhostarval:=\log(1+\sqrt2),
\qquad
\gzero:=\rhostarval+4.8\cdot 10^{-6}.
\]
Then the $H_3/-H_3$ scheme is a $\gzero$-admissible Krivine scheme.  In particular,
\[
K_G
\le \frac{\pi}{2\gzero}
<
\frac{\pi}{2\log(1+\sqrt2)}
-
9.7\cdot 10^{-6}.
\]
\end{theorem}
\end{tcolorbox}

\paragraph{Proof architecture.}
The proof has two independent modules after the scheme is fixed.  The analytic module proves a uniform inverse disk; the numerical module computes the inverse-majorant head and uses the analytic disk for the tail:
\[
\begin{array}{ccccc}
Lemma~\ref{lem:strip-bound}
&\Longrightarrow&
Lemma~\ref{lem:sine-coordinate-bound}
&\Longrightarrow&
Corollary~\ref{cor:F-inverse-radius}
\Longrightarrow
Corollary~\ref{cor:H-inverse-radius}
\\[0.5em]
&&&&\Downarrow
\\[-0.1em]
Lemma~\ref{lem:majorant-head-value}
&+&
Lemma~\ref{lemma:tail-bound}
&\Longrightarrow&
Corollary~\ref{cor:gamma0-admissibility}
\Longrightarrow
Theorem~\ref{thm:no-mixing-beats-hyperplane}.
\end{array}
\]
The central device is the change of variables $F(w)=H(\sin w)$: in this coordinate the hyperplane profile becomes the identity map, so the inverse problem becomes a perturbative Rouch\'e estimate around $w\mapsto w$.

\section{The analytic inverse disk}

\begin{lemma}[Strip bound]\label{lem:strip-bound}
Let $f,g:\R^2\to\{-1,1\}$ be measurable and let $H=H_{f,g}$ be the
arcsine-normalized correlation function.
Then $H$ extends holomorphically to
\[
 S=\{z\in\C: |\operatorname{Re}z|<1\}.
\]
Moreover, if $z=a+ib\in S$, then
\[
 |H(z)|\le \frac{\pi}{2}\frac{|1-z^2|}{1-a^2}.
\]
\end{lemma}

\begin{proof}
For real $|t|<1$, the arcsine-normalized correlation admits the integral representation
\[
H(t)=\frac{1}{2\pi(1-t^2)}
\int_{\R^2}\int_{\R^2}
f(x)g(y)
\exp\left(
-\frac{\|x\|^2+\|y\|^2-2t\ip{x}{y}}{1-t^2}
\right)\,dx\,dy .
\]
For $z\in S$, this formula defines the candidate holomorphic extension.  Since $|f|=|g|=1$,
\[
|H(z)|\le
\frac{1}{2\pi |1-z^2|}
\int_{\R^2}\int_{\R^2}
\exp\left(
-\operatorname{Re}\frac{\|x\|^2+\|y\|^2-2z\ip{x}{y}}{1-z^2}
\right)\,dx\,dy .
\]
Use the identity
\[
\frac{\|x\|^2+\|y\|^2-2z\ip{x}{y}}{1-z^2}
=
\frac12\frac{\|x+y\|^2}{1+z}
+
\frac12\frac{\|x-y\|^2}{1-z}.
\]
Writing $z=a+ib$, set
\[
A_+ := \operatorname{Re}\frac{1}{1+z}
=\frac{1+a}{(1+a)^2+b^2},
\qquad
A_- := \operatorname{Re}\frac{1}{1-z}
=\frac{1-a}{(1-a)^2+b^2}.
\]
Both are positive for $|a|<1$.  With $u=x+y$ and $v=x-y$, the Jacobian from $(u,v)$ to $(x,y)$ in $\R^4$ is $1/4$.  Thus the Gaussian integral is
\[
\frac14\cdot\frac{2\pi}{A_+}\cdot\frac{2\pi}{A_-}
=\frac{\pi^2}{A_+A_-}.
\]
Finally,
\[
A_+A_-=
\frac{1-a^2}{|1+z|^2|1-z|^2}
=
\frac{1-a^2}{|1-z^2|^2}.
\]
Substitution gives
\[
|H(z)|\le
\frac{1}{2\pi |1-z^2|}\cdot
\frac{\pi^2 |1-z^2|^2}{1-a^2}
=
\frac{\pi}{2}\frac{|1-z^2|}{1-a^2}.
\]
The same estimate is uniform on compact subsets of $S$, so the integral converges locally uniformly and the extension is holomorphic by dominated convergence.
\end{proof}

\begin{definition}[The key change of variable]\label{def:key-change-of-variable}
For the rest of the proof, put
\[
F(w)\defeq H(\sin w).
\]
For the hyperplane scheme $H_0(t)=\arcsin t$, hence $H_0(\sin w)=w$ on the principal strip.  This is why the comparison below is made against the identity map.
\end{definition}

\begin{lemma}[Sine-coordinate bound]\label{lem:sine-coordinate-bound}
For $F(w)=H(\sin w)$, the function $F$ is holomorphic on $|w|<1.1$ and
\[
 |F(w)-w|<15.3\qquad (|w|\le1.1).
\]
\end{lemma}

\begin{proof}
Write $w=u+iv$. Then
\[
\operatorname{Re}(\sin w)=\sin u\cosh v.
\]
By Lemma~\ref{lem:disk-to-strip-check}, if $u^2+v^2\le 1.1^2$, then
\[
|\sin u|\cosh v<0.946<1.
\]
Therefore $\sin w\in S$ for $|w|\le 1.1$, and Lemma~\ref{lem:strip-bound} implies that $F$ is holomorphic on $|w|<1.1$.  Applying Lemma~\ref{lem:strip-bound} with $z=\sin w$ gives
\[
|F(w)|
\le
\frac{\pi}{2}\frac{|1-\sin^2 w|}{1-(\operatorname{Re}\sin w)^2}
=
\frac{\pi}{2}\frac{|\cos w|^2}{1-(\operatorname{Re}\sin w)^2}.
\]
By Lemma~\ref{lem:cosine-ratio-check}, the last expression is $<14.19$ on $|w|\le 1.1$.  Hence
\[
|F(w)-w|\le |F(w)|+|w|<14.19+1.1<15.3.
\]
\end{proof}

\begin{lemma}[Rouch\'e inverse disk]\label{lem:rouche-inverse-disk}
Let $F$ be holomorphic on $|w|<r$, with $F(0)=0$, and suppose that for some
$R<M<r$,
\[
 \sup_{|w|=M}|F(w)-w|<M-R.
\]
Then:
\begin{enumerate}[label=(\roman*)]
    \item $F^{-1}$ is holomorphic on $R\D$;
    \item for $|\zeta|<R$, the inverse satisfies $|F^{-1}(\zeta)|<M$.
\end{enumerate}
\end{lemma}

\begin{proof}
Fix $|\zeta|<R$.  On $|w|=M$,
\[
|(F(w)-\zeta)-(w-\zeta)|=|F(w)-w|<M-R<M-|\zeta|\le |w-\zeta|.
\]
By Rouch\'e's theorem, $F(w)-\zeta$ and $w-\zeta$ have the same number of zeros in $|w|<M$, counted with multiplicity.  Since $w-\zeta$ has exactly one zero in this disk, $F(w)=\zeta$ has exactly one solution in $|w|<M$, counted with multiplicity.  In particular, the solution is simple.  The holomorphic inverse function theorem gives local inverse branches, and uniqueness makes these branches glue over $R\D$.  The same argument gives $|F^{-1}(\zeta)|<M$.
\end{proof}

\begin{corollary}[Radius and supremum of $|F^{-1}|$]\label{cor:F-inverse-radius}
Taking $r=1.1$, $R=0.975$, and $M=0.98$, the inverse $F^{-1}$ is holomorphic on $0.975\D$ and
\[
|F^{-1}(\zeta)|<0.98\qquad (|\zeta|<0.975).
\]
\end{corollary}

\begin{proof}
Let
\[
\Delta(w):=F(w)-w=\sum_{n\ge1}d_nw^n.
\]
The Arb coefficient computation gives the finite head estimate
\[
\sum_{n\le 220}|d_n|0.98^n<0.00454106848.
\]
By Lemma~\ref{lem:sine-coordinate-bound} and Cauchy's estimate, taking the Cauchy radius to $1.1$ from below gives
\[
\sum_{n>220}|d_n|0.98^n
\le
15.3\frac{(0.98/1.1)^{221}}{1-0.98/1.1}
<1.149\cdot10^{-9}.
\]
Therefore
\[
\sup_{|w|=0.98}|F(w)-w|
\le
\sum_{n\ge1}|d_n|0.98^n
<0.00454106848+1.149\cdot 10^{-9}
<0.005.
\]
Since $M-R=0.98-0.975=0.005$, Lemma~\ref{lem:rouche-inverse-disk} applies with $r=1.1$, $M=0.98$, and $R=0.975$.
\end{proof}

\begin{corollary}[Radius and supremum of $|H^{-1}|$]\label{cor:H-inverse-radius}
Undoing the change of variables, we get
\[
H^{-1}=\sin\circ F^{-1}.
\]
Thus $H^{-1}$ is holomorphic on $0.975\D$ and
\[
|H^{-1}(\zeta)|<\sinh(0.98)<1.145
\qquad (|\zeta|<0.975).
\]
\end{corollary}

\begin{proof}
Since $F=H\circ\sin$, the identity $F^{-1}=\arcsin\circ H^{-1}$ is equivalent to
$H^{-1}=\sin\circ F^{-1}$ on the inverse branch at the origin.  By Corollary~\ref{cor:F-inverse-radius}, $|F^{-1}(\zeta)|<0.98$ for $|\zeta|<0.975$.  The elementary bound
\[
|\sin z|\le \sinh |z|
\]
for complex $z$ gives
\[
|H^{-1}(\zeta)|=|\sin(F^{-1}(\zeta))|<\sinh(0.98)<1.145.
\]
\end{proof}

\section{The inverse-majorant theorem}

\begin{lemma}[Majorant tail bound]\label{lemma:tail-bound}
Let
\[
H^{-1}(\zeta)=\sum_{n\ge1}a_n\zeta^n,
\qquad
\gzero=\log(1+\sqrt2)+4.8\cdot10^{-6}.
\]
Then
\[
\sum_{n>220}|a_n|\gzero^n<2.5\cdot10^{-9}.
\]
\end{lemma}

\begin{proof}
By Corollary~\ref{cor:H-inverse-radius}, $H^{-1}$ is holomorphic on $0.975\D$ and satisfies $|H^{-1}(\zeta)|<1.145$ there.  Hence, for every $s<0.975$, Cauchy's estimate with radius tending to $0.975$ gives
\[
\sum_{n>220}|a_n|s^n
\le
1.145\frac{(s/0.975)^{221}}{1-s/0.975}.
\]
Taking $s=\gzero$ yields
\[
1.145\frac{(\gzero/0.975)^{221}}{1-\gzero/0.975}
<2.44\cdot10^{-9}
<2.5\cdot10^{-9},
\]
as claimed.
\end{proof}

\begin{lemma}[Majorant head value]\label{lem:majorant-head-value}
Let
\[
 M_{f,g}(s)=\sum_{n\ge 1} |a_n|s^n
\]
be the inverse majorant for the $H_3/-H_3$ scheme.  For
\[
\gzero=\log(1+\sqrt2)+4.8\cdot10^{-6},
\]
one has
\[
\sum_{1\le n\le220}|a_n|\gzero^n
<1-2.5\cdot10^{-9}.
\]
\end{lemma}

\begin{proof}
\source{Arb certificate.}
We record the coefficient computation used by the certificate.  Let $\mathsf H_n$ be the physicist's Hermite polynomial and set
\[
\psi_n(x):=\frac{\mathsf H_n(x)}{\sqrt{2^n n!}},
\qquad
 d\mu(x):=\pi^{-1/2}e^{-x^2}\,dx.
\]
Then $\{\psi_n\}_{n\ge0}$ is an orthonormal basis for $L^2(\mu)$.  Expanding
\[
f(x,y)=\sum_{a,b\ge0}F_{a,b}\psi_a(x)\psi_b(y),
\]
and using $g(x,y)=f(-x,y)$, the coefficient of $\psi_a(x)\psi_b(y)$ in $g$ is $(-1)^aF_{a,b}$.  Mehler diagonalization gives
\[
H(z)=\frac{\pi}{2}\sum_{a,b\ge0}(-1)^aF_{a,b}^2z^{a+b},
\]
so
\[
[z^n]H(z)=\frac{\pi}{2}\sum_{a=0}^{n}(-1)^aF_{a,n-a}^2.
\]
The two-dimensional coefficients reduce to one-dimensional integrals:
\[
F_{a,b}=\int_{\R}\psi_a(x)S_b(\tau\psi_3(x))\,d\mu(x),
\]
where
\[
S_0(u)=-\erf(u),
\qquad
S_b(u)=\frac{2}{\sqrt\pi}e^{-u^2}\frac{\psi_{b-1}(u)}{\sqrt{2b}}
\quad (b\ge1).
\]
These formulas determine the Taylor coefficients of $H$ through degree $220$ using one-dimensional Arb integrations and outward-rounded interval arithmetic.

Since $H$ is odd, the inverse has only odd coefficients.  Writing
\[
H(z)=z\Phi(z^2),
\]
Lagrange inversion gives
\[
a_{2k+1}=\frac{1}{2k+1}[t^k]\Phi(t)^{-(2k+1)},
\qquad
 a_{2k}=0.
\]
Applying this formula with Arb ball arithmetic gives the certified enclosure
\[
\sum_{n\le220}|a_n|\gzero^n<0.999999729.
\]
Since $0.999999729<1-2.5\cdot10^{-9}$, the stated bound follows.  Independent floating-point and PyTorch checks are useful diagnostics, but the displayed inequality is certified only by the outward-rounded Arb computation.
\end{proof}

\begin{corollary}[$\gamma_0$-admissibility]\label{cor:gamma0-admissibility}
For the $H_3/-H_3$ scheme,
\[
M_{f,g}(\gzero)<1.
\]
Consequently, the scheme is $\gzero$-admissible.
\end{corollary}

\begin{proof}
By Lemma~\ref{lem:majorant-head-value},
\[
\sum_{1\le n\le220}|a_n|\gzero^n<1-2.5\cdot10^{-9}.
\]
By Lemma~\ref{lemma:tail-bound},
\[
\sum_{n>220}|a_n|\gzero^n<2.5\cdot10^{-9}.
\]
Adding the two inequalities gives $M_{f,g}(\gzero)<1$.  The inverse branch exists on a neighborhood of $\gzero\overline{\D}$ by Corollary~\ref{cor:H-inverse-radius}, since $\gzero<0.975$.  Thus the $H_3/-H_3$ scheme satisfies Definition~\ref{def:gamma-admissible}.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:no-mixing-beats-hyperplane}]
By Corollary~\ref{cor:gamma0-admissibility}, the $H_3/-H_3$ scheme is $\gzero$-admissible.  Applying Theorem~\ref{thm:krivine-preprocessing} gives
\[
K_G\le \frac{\pi}{2\gzero}.
\]
Finally, with $\rhostarval=\log(1+\sqrt2)$ and $\gzero=\rhostarval+4.8\cdot10^{-6}$,
\[
\frac{\pi}{2\rhostarval}-\frac{\pi}{2\gzero}
=
\frac{\pi(4.8\cdot10^{-6})}{2\rhostarval\gzero}
>9.7\cdot10^{-6}.
\]
Therefore
\[
K_G
\le
\frac{\pi}{2\gzero}
<
\frac{\pi}{2\log(1+\sqrt2)}-9.7\cdot10^{-6}.
\]
\end{proof}

\begin{remark}[Equality convention]\label{rem:equality-convention}
The equality convention for Krivine schemes can also be recovered.  The same Arb computation gives
\[
\sum_{n\le220}|a_n|(\rhostarval+5.2\cdot10^{-6})^n>1.000000291.
\]
Since $M_{f,g}$ is continuous on $[0,0.975)$, there exists
\[
\gamma\in(\rhostarval+4.8\cdot10^{-6},\rhostarval+5.2\cdot10^{-6})
\]
with $M_{f,g}(\gamma)=1$.
\end{remark}

\appendix
\section{Sine-coordinate maximization checks}

\begin{lemma}[Disk-to-strip check]\label{lem:disk-to-strip-check}
Let $\rho=1.1$.  For all $u,v\in\R$ with $u^2+v^2\le\rho^2$,
\[
|\sin u|\cosh v<0.946.
\]
\end{lemma}

\begin{proof}
Since $\rho<\pi/2$, by symmetry we may assume $0\le u\le\rho$ and $v\ge0$.  For fixed $u$, $\cosh v$ is increasing in $v\ge0$, so it suffices to maximize
\[
\varphi(u):=\sin u\cosh s(u),
\qquad
s(u):=\sqrt{\rho^2-u^2},
\qquad
0\le u\le\rho.
\]
For $0<u<\rho$,
\[
\varphi'(u)=\sin u\cosh s(u)
\left(\cot u-\frac{u}{s(u)}\tanh s(u)\right).
\]
Let
\[
h(u):=\cot u-\frac{u}{s(u)}\tanh s(u).
\]
The function $u\mapsto\cot u$ is strictly decreasing.  Also
\[
A(s):=\frac{\tanh s}{s}
\]
is strictly decreasing for $s>0$, since
\[
A'(s)=\frac{s\operatorname{sech}^2s-\tanh s}{s^2}<0,
\]
the final inequality being equivalent to $\sinh s\cosh s-s>0$.  Since $s(u)$ is decreasing, $A(s(u))$ is increasing, and hence $uA(s(u))$ is increasing.  Therefore $h$ is strictly decreasing.

Outward-rounded Taylor bounds give
\[
h(0.898)>0.796708-0.793956>0,
\qquad
h(0.900)<0.793553-0.796524<0.
\]
Thus the unique maximizer $u_*$ of $\varphi$ lies in $(0.898,0.900)$.  Take $c=0.899$.  On $[0.898,0.900]$,
\[
\varphi''(u)=
\sin u\cosh s\left(\frac{u^2}{s^2}-1\right)
-2\frac{u}{s}\cos u\sinh s
-\frac{\rho^2}{s^3}\sin u\sinh s,
\]
where $s=s(u)$.  Throughout this interval,
\[
s^2\ge0.4,
\qquad
0.632<s<0.636,
\qquad
\cosh s<1.21,
\qquad
\sinh s<0.68.
\]
These bounds give $|\varphi''(u)|<7$.  Since $|u_*-c|\le10^{-3}$,
\[
\varphi(u_*)\le \varphi(c)+\frac72\cdot10^{-6}.
\]
Now
\[
s(c)^2=1.21-0.899^2=0.401799<0.6339^2,
\]
so $\cosh s(c)<\cosh(0.6339)<1.20774$.  Also,
\[
\sin(0.899)<0.899-\frac{0.899^3}{6}+\frac{0.899^5}{120}<0.7828.
\]
Thus
\[
\varphi(c)<0.7828\cdot1.20774<0.945419,
\]
and consequently
\[
\varphi(u_*)<0.945419+0.0000035<0.946.
\]
\end{proof}

\begin{lemma}[Cosine-ratio check]\label{lem:cosine-ratio-check}
For every $w\in\C$ with $|w|\le1.1$,
\[
\frac{\pi}{2}\frac{|\cos w|^2}{1-(\operatorname{Re}\sin w)^2}<14.19.
\]
\end{lemma}

\begin{proof}
Write $w=u+iv$ and put $\rho=1.1$.  We maximize over $u^2+v^2\le\rho^2$.  We have
\[
\operatorname{Re}(\sin w)=\sin u\cosh v,
\qquad
|\cos w|^2=\cos^2u+\sinh^2v.
\]
It is enough to bound
\[
Q(u,v):=\frac{\cos^2u+\sinh^2v}{1-\sin^2u\cosh^2v}.
\]
The denominator is positive by Lemma~\ref{lem:disk-to-strip-check}.  Set
\[
x:=\sin^2u,
\qquad
y:=\sinh^2v.
\]
Then
\[
Q(u,v)=\frac{1-x+y}{1-x-xy},
\]
and, for fixed $x$,
\[
\frac{\partial}{\partial y}\frac{1-x+y}{1-x-xy}
=
\frac{(1-x)^2}{(1-x-xy)^2}>0.
\]
Thus, for each fixed $u$, the maximum occurs at $|v|=\sqrt{\rho^2-u^2}$.  By evenness in $u$, it remains to maximize
\[
\Phi(u):=
\frac{\cos^2u+\sinh^2s(u)}{1-\sin^2u\cosh^2s(u)},
\qquad
s(u):=\sqrt{\rho^2-u^2},
\qquad
0\le u\le\rho.
\]
For $0<u<\rho$, differentiating gives
\[
\Phi'(u)=
\frac{\sinh(2s)\cos u}{(1-\sin^2u\cosh^2s)^2}
\left[
\sin u\tanh s(1+\cosh^2s)
-\frac{u}{s}\cos u(1+\sin^2u)
\right],
\]
where $s=s(u)$.  The prefactor is positive.  Therefore the sign of $\Phi'(u)$ is the sign of $A(u)-1$, where
\[
A(u):=\frac{s(u)\tan u\tanh s(u)(1+\cosh^2s(u))}{u(1+\sin^2u)}.
\]
We show that $A$ is strictly decreasing.  Let
\[
B(s):=s\tanh s(1+\cosh^2s).
\]
Then
\[
\frac{d}{du}\log A(u)
=
\left(\frac{1}{\sin u\cos u}-\frac{1}{u}\right)
-\frac{\sin(2u)}{1+\sin^2u}
-\frac{u}{s}\frac{B'(s)}{B(s)}.
\]
Moreover,
\[
\frac{B'(s)}{B(s)}
=
\frac{1}{s}
+
\frac{1}{\sinh s\cosh s}
+
\frac{2\sinh s\cosh s}{1+\cosh^2s}.
\]
Since
\[
\frac{2\sinh s\cosh s}{1+\cosh^2s}\ge \tanh s
\qquad\text{and}\qquad
\frac{1}{\sinh s\cosh s}+\tanh s=\coth s>\frac1s,
\]
we have $B'(s)/B(s)>2/s$.  On the other hand, for $0<u<\rho$,
\[
\sin u\cos u=\frac12\sin(2u)>u-\frac23u^3.
\]
Therefore
\[
\frac{1}{\sin u\cos u}-\frac1u
=
\frac{u-\sin u\cos u}{u\sin u\cos u}
<\frac{2u}{3-2u^2}
<\frac{2u}{\rho^2-u^2}
=\frac{2u}{s^2}.
\]
Combining the estimates gives
\[
\frac{d}{du}\log A(u)
<
\frac{2u}{s^2}
-\frac{\sin(2u)}{1+\sin^2u}
-\frac{2u}{s^2}
<0.
\]
Thus $A$ is strictly decreasing.  Since $A(u)>1$ for small $u>0$ and $A(u)\to0$ as $u\uparrow\rho$, the function $\Phi$ increases up to the unique point where $A(u)=1$ and decreases afterward.

A final outward-rounded interval computation gives
\[
A(0.8289364)>1.0000019,
\qquad
A(0.8289372)<0.9999992.
\]
Hence the maximizer lies in
\[
I=[0.8289364,0.8289372].
\]
Evaluating $\Phi$ on this interval, again with outward-rounded interval arithmetic, gives
\[
\Phi(I)\subset[9.0332175,9.03345993].
\]
Consequently
\[
\sup_{|w|\le1.1}
\frac{\pi}{2}\frac{|\cos w|^2}{1-(\operatorname{Re}\sin w)^2}
=
\frac{\pi}{2}\sup_{0\le u\le\rho}\Phi(u)
\le
\frac{\pi}{2}\cdot9.03345993
<14.18973<14.19.
\]
\end{proof}

==> old/introduction.tex <==
\section{Introduction}

Outline:
\begin{enumerate}
    \item Definition of Grothendieck constant: numerical improvement. 
    \item Rounding schemes and analysis. 
    \item Main theorem: For f = blah, g=blah, we have constant < blah.
    \item Proof outline: (0) We do a variable change to simplify analysis. (1) Numerical computation of Taylor series upto 220. (2) Bounding the remainder term. 

    The variable change helps, and changes how the remainder term is bounded. 
    \item Bounding the remainder term without mixing. This is new, and deviates significantly from [BMMN]. Make this as modular as  possible. 
    \item Section on numerical computation: Discuss computation and cross-verification with pytorch, etc. Why this is trustable (why can't this just be a floating point artifact)?
    \item AI-guided search of rounding schemes. 
    \item Koenig bilinear form: Related to Grothendieck. Main result. Best constant, higher dimensions give the constant. Not clear if it is realizable in two-dimensions.  
\end{enumerate}
In 1953, Alexander Grothendieck published a paper on the metric theory of tensor products, \emph{R\'esum\'e de la th\'eorie m\'etrique des produits tensoriels topologiques}, 
which had far-reaching impacts on functional analysis and the theory of Banach spaces.
While this paper was initially ignored, its central result, now referred to as the \textit{Grothendieck inequality}, has since found applications in a large 
number of seemingly unrelated areas, including computational hardness thresholds, quantum 
mechanics, geometry, harmonic analysis, and operator theory. 

The \textit{Grothendieck inequality}, states that there exists a universal constant \(K_G < \infty\) such 
that for every \(m,n \in \N\) and every matrix \(A=(a_{ij}) \in \R^{m \times n}\),
\begin{equation}
    \max_{\varepsilon_i,\delta_j \in \{\pm 1\}}
    \bigg|
    \sum_{i=1}^m \sum_{j=1}^n a_{ij}\varepsilon_i\delta_j
    \bigg|
    \leq 
    \sup_{d \geq 1}
    \max_{\substack{u_i,v_j \in S^{d-1}}}
    \bigg|
    \sum_{i=1}^m \sum_{j=1}^n a_{ij}\angles{u_i,v_j}
    \bigg|
    \leq 
    K_G
    \max_{\varepsilon_i,\delta_j \in \{\pm 1\}}
    \bigg|
    \sum_{i=1}^m \sum_{j=1}^n a_{ij}\varepsilon_i\delta_j
    \bigg|.
\end{equation}
Here \(S^{d-1}\) denotes the unit sphere in \(\R^d\). The smallest constant \(K_G\) for which
this inequality holds is called the real Grothendieck constant.

The Grothendieck constant is fundamental in combinatorial optimization because it controls
how well certain integer optimization problems can be approximated by continuous relaxations.
One important example is the problem of efficiently computing the cut norm of a matrix, which
is used in a variety of algorithms, including constructions of
Szemerédi partitions of graphs ~\cite{AN06}. A particularly nice complexity-theoretic
interpretation of \(K_G\) is that it gives the Unique Games hardness threshold for approximating
the following integer quadratic program:
\begin{equation}
    \mrm{IQP}(A)
    \quad \defeq \quad
    \max_{\varepsilon \in \{\pm 1\}^m,\ \delta \in \{\pm 1\}^n}
    \sum_{i=1}^m \sum_{j=1}^n a_{ij}\varepsilon_i\delta_j .
\end{equation}
The natural continuous relaxation is the semidefinite program
\begin{equation}
    \mrm{SDP}(A)
    \quad \defeq \quad
    \sup_{d \geq 1}
    \max_{\substack{u_1,\ldots,u_m \in S^{d-1}\\
                    v_1,\ldots,v_n \in S^{d-1}}}
    \sum_{i=1}^{m}\sum_{j=1}^{n} a_{ij}\,\angles{u_i,v_j}.
\end{equation}
Equivalently, one may take \(d=m+n\). With this notation, Grothendieck's inequality says that
\begin{equation}
    \mrm{IQP}(A)
    \leq 
    \mrm{SDP}(A)
    \leq 
    K_G \cdot \mrm{IQP}(A).
\end{equation}
The Raghavendra--Steurer theorem shows that this constant has a sharp complexity-theoretic
meaning: if there were a polynomial-time algorithm that approximates \(\mrm{IQP}(A)\) to
within a factor \(c<K_G\), then the Unique Games Conjecture would be false. Due to this, there have been major attempts at obtaining better bounds on $K_G$.   

\textbf{Rounding schemes.} One way to upper bound \(K_G\) is through the design and analysis of \emph{rounding schemes}.
A rounding scheme is a possibly randomized procedure that takes a solution
\[
    \{u_i\}_{i=1}^m,\{v_j\}_{j=1}^n \subset S^{d-1}
\]
of the semidefinite relaxation and produces signs
\[
    \varepsilon_1,\ldots,\varepsilon_m,\delta_1,\ldots,\delta_n \in \{\pm 1\}.
\]
Krivine proved his upper bound \(K_G \le \tfrac{\pi}{2 \log(1 + \sqrt{2})}\) using a very clever randomized hyperplane rounding
scheme. The idea is to preprocess the vectors  $\{u_i\}_{i=1}^m,\{v_j\}_{j=1}^n$ by lifting them to an infinite dimensional space, then projecting them onto a random hyperplane and rounding based on which side of the hyperplane the vectors lie on. Krivine conjectured this to be the optimal rounding scheme, and this conjecture stood for nearly thirty years.  

This conjecture was then refuted by Braverman,
Makarychev, Makarychev, and Naor (BMMN) to improve on Krivine's bound. They generalized Krivine's schemes by using projections that rounded based on non-linear geometries. At a high level, these
rounding schemes can be viewed as pairs of partitions of \(\R^d\). The choice of partition
encodes geometric information about which configurations of vectors make Grothendieck's
inequality hardest to round.

There is, however, an analytic difficulty in turning a promising partition into an actual Grothendieck rounding scheme.
The main obstruction in the work of BMMN was that in order to make certain analytic statements hold, they had to \textit{mix} their new rounding scheme with the classical hyperplane scheme. 

A mixed rounding scheme is a simple randomized procedure. Instead of choosing one rounding
rule once and for all, we first flip a biased coin. With probability \(p\), we use the new
rounding scheme, and with probability \(1-p\), we use the hyperplane rounding scheme. After
this choice is made, we apply the chosen scheme to all the SDP vectors.

This kind of mixing is useful because, when \(p\) is small, the resulting procedure remains
very close to hyperplane rounding, which is much easier to analyze. The drawback is that the
new rounding scheme is only used with probability \(p\). Braverman et al. requires $p$ to be very small, thus most of the potential improvement is washed out before it can meaningfully affect the final Grothendieck bound.

Our first contribution is removing the need for mixing. The theorem gives a pure, unmixed perturbation in the same family as Braverman et al. that already beats the hyperplane.

\begin{theorem}[A pure planar perturbation beats hyperplane rounding]
\label{thm:pure-h3}
Let \(H_3(x)=8x^3-12x\), and set
\[
 \tau=0.03175,
 \qquad
 \eta=\frac{\tau}{\sqrt{48}}
 =0.004582717761692655\ldots .
\]
Define odd planar partitions \(f,g:\R^2\to\{\pm1\}\) by
\[
    f(x,y)=\sgn(y-\eta H_3(x)),
    \qquad
    g(x,y)=\sgn(y+\eta H_3(x)).
\]
The rounding scheme generated by this pair of partitions gives the upper bound,
\[
    K_G
    <
   \frac{\pi}{2\log(1+\sqrt2)} - 
    9.7\cdot 10^{-6}
\]
\end{theorem}

This theorem shows that the obstruction was not geometric: one does not need to mix the
perturbation with the hyperplane merely to obtain a valid Krivine scheme. Once the analytic
step is handled correctly, a much broader class of pure and mixed strategies becomes
available. In fact, the proof of Theorem~\ref{thm:pure-h3} applies even for mixed schemes. 

But why should mixing remain useful after we have spent so much effort removing the need
for it? The answer lies in \emph{why} BMMN used mixing
in the first place. In their argument, the mixing parameter \(p\) had to be very small in
order to control certain analytic properties of the rounding scheme. In that regime, mixing
is primarily a technical device: the new rounding is used only rarely, so its effect on the
final Grothendieck bound is necessarily diluted.

In this paper, we observe a different and more interesting phenomenon. A mixture of two
rounding schemes can sometimes give a \emph{strictly} better Grothendieck bound than either
scheme gives individually. Intuitively, one should think of different schemes as performing
well on different difficult configurations of vectors. A randomized mixture can combine strengths of different schemes. This observation changes the search problem for rounding schemes.  

\textbf{Tiger Partitions}. A natural first place to look for better roundings chemes is the class of ``tiger partitions'' suggested by BMMN. These partitions arise from a variational problem related to their proof. BMMN conjectured that the roundings derived from these partitions may provide the optimal candidates for the best bound on $K_G$. 
However, our computations show that tiger partitions are not competitive
for improving the Grothendieck bound. This is an important negative result: it means that
the most natural geometric candidates do not appear to be the correct ones, and the space of
useful rounding schemes is much larger than the previously studied examples.

\textbf{AI-Guided Search}. In order to effectively explore this larger space of rounding schemes, we therefore use an AI-assisted search. The search is over
explicit partitions of low-dimensional Gaussian space, especially partitions whose boundary
is given by threshold functions. In two dimensions, these have the form
\[
    f_\Phi(x_1,x_2)=\sgn(x_2-\Phi(x_1)),
    \qquad
    g_\Phi(x_1,x_2)=\sgn(x_2+\Phi(x_1)),
\]
where \(\Phi\) is an odd Hermite polynomial. We also allow higher-dimensional analogues in
which the threshold depends on several Gaussian coordinates. The AI agent is asked to
generate candidate threshold functions, optimize their coefficients, store the best
candidates, and then search over mixtures of those candidates. The final candidates are then checked by a separate rigorous certification procedure.

This search produces an explicit mixed planar scheme giving our best quantitative bound.

\begin{theorem}[Explicit improvement over Krivine's bound]
\label{thm:explicit-improvement}
There is an explicit mixed Krivine rounding scheme such that
\[
    K_G
    \leq
    \frac{\pi}{2\log(1+\sqrt2)}
    -
    5.56\cdot 10^{-5}.
\]
The scheme is a probability mixture of the classical hyperplane rounding and an explicit
degree-\(9\) Hermite-threshold rounding of the form
\[
    f_\Phi(x_1,x_2)=\sgn(x_2-\Phi(x_1)),
    \qquad
    g_\Phi(x_1,x_2)=\sgn(x_2-\Phi(x_1)),
\]
where the polynomial \(\Phi\) and the mixture weights are listed in
\cref{sec:explicit-improvement}.
\end{theorem}


\textbf{K\"onig Bilinear Form}. {\color{blue} FOR ALAN: DEFINE KONIG IN BRIEF HERE, THEN LINK TO SECTION WHERE IT IS DEFINED PROPERLY} We prove an asymptotic theorem for a tractable high-dimensional
family of rotated hyperplane partitions. 
Let
\[
    a(\theta)=\operatorname{arsinh}(\cos\theta),
\]
viewed as a \(2\pi\)-periodic analytic function. For \(d\in\N\) and parameters
\(\alpha,\beta\in\R\), define
\[
    Q_d(u)=4\norm{u}_2^2-d,
    \qquad
    \psi_{d,\alpha,\beta}(u)=\beta+\alpha Q_d(u),
\]
and let \(K_d(\alpha,\beta)\) denote the corresponding reduced König value for the affine
radial rotated-hyperplane family defined in Section~\ref{sec:konig-not-sufficient}. The
large-\(d\) limit is governed by the periodic Airy flow.

\begin{theorem}[Airy limit for the affine radial König problem]
\label{thm:airy-limit-intro}
Fix \(0<\rho<\rho_*\) and \(\kappa_0>0\). Then there exist constants
\(C=C(\rho,\kappa_0)\) and \(d_0=d_0(\rho,\kappa_0)\) such that for all \(d\geq d_0\),
all \(|\kappa|\leq \kappa_0\), and all \(\beta\in\R\),
\[
    \left|
    K_d\!\left(\kappa d^{-1/3},\beta\right)
    -
    \frac{2}{\pi}
    \left(e^{-\tau_\kappa \partial_\theta^3}a\right)(2\beta)
    \right|
    \leq
    C d^{-1/3},
\]
where
\[
    \tau_\kappa=\frac{16}{3}\kappa^3.
\]
Equivalently,
\[
    K_d\!\left(\kappa d^{-1/3},\beta\right)
    \longrightarrow
    \frac{2}{\pi}
    \left(e^{-\tau_\kappa \partial_\theta^3}a\right)(2\beta)
\]
uniformly for \((\kappa,\beta)\in[-\kappa_0,\kappa_0]\times\R\).
\end{theorem}

Theorem~\ref{thm:airy-limit-intro} gives an explicit asymptotic model for the König bilinear form in this family. 

The rest of the paper is organized as follows. Section~\ref{sec:krivine-schemes} recalls
Krivine rounding schemes and proves the pure \(h_3/-h_3\) improvement. Section~\ref{sec:analytic-obstruction}
develops the sine-coordinate inverse certificate that removes the analytic obstruction.
Section~\ref{sec:explicit-improvement} describes the AI-assisted search over Hermite-threshold
partitions and proves the explicit \(10^{-5}\) improvement. Finally,
Section~\ref{sec:konig-not-sufficient} analyzes the affine radial family and proves the Airy
limit for the König bilinear form.



% {\color{red}
% In 1953, Alexander Grothendieck published a paper on the metric theory of tensor products with wide reaching impacts on functional analysis and the theory of Banach spaces. While this paper was initially ignored, its results have since found applications in a large number of seemingly unrelated areas, including $C^*$ algebras, Bell's inequality in quantum mechanics, and in polynomial-time approximation algorithms for certain NP-hard problems.

% Groethendieck's inequality states that there exists a constant \(K_G > 0\), such that for all \(A \in \R^{m \times n}\):
% \begin{equation}
%     \max_{x_i, y_j \in \{\pm 1\}} \bigg|
%     \sum_{i, j} a_{ij} x_i y_j \bigg|
%     \leq \sup_{d \geq 1} \max_{\substack{u_i, v_i \in \mbb{R}^{d} \\ \norm{u_i} = \norm{v_j} = 1}} \bigg| \sum_{i, j} a_{ij} \angles{u_i, v_j} \bigg|
%     \leq \max_{x_i, y_j \in \{\pm 1\}}
%     K_G \bigg| \sum_{i, j} a_{ij} x_i y_j \bigg|,
% \end{equation}
% This constant is independent of \(m\) and \(n\), with the current best lower (CITE) and upper bound (CITE) being:
% \begin{equation}
%     1.676\ldots < K_G < 1.782\ldots
% \end{equation}
% Groethendieck's inequality is of interest in combinatorial optimization because it establishes a fundamental limitation of how well continuous programs can approximate discrete ones.
% One connection is in the optimality gap between an integer quadratic program and its semidefinite relaxation. Consider the following integer quadratic program:
% \begin{equation}
% \mrm{IQP}(A)
%     \quad \defeq \quad
%     \max_{x \in \{\pm 1\}^m, y \in \{\pm 1\}^n}
%     \enskip \sum_{i,j} a_{ij} x_i y_j,
% \end{equation}
% and its continuous relaxation, which is a semidefinite program of the form:
% \[
% \mathrm{SDP}(A)\;\defeq\;
% \max_{\substack{x_1,\ldots,x_m\in S^{d-1}\\ y_1,\ldots,y_n\in S^{d-1}}}
% \;\sum_{i=1}^{m}\sum_{j=1}^{n} a_{ij}\,\langle x_i, y_j\rangle ,
% \]
% Groethendieck's inequality then states that:
% \begin{equation}
%     \abs{\mrm{IQP}(A)}
%     \leq \abs{\mrm{SDP}(A)}
%     \leq K_G \cdot \abs{\mrm{IQP}(A)}.
% \end{equation}
 

% \begin{theorem}[Removing mixture obstruction]
% We show that a perturbation on its own is a rounding scheme that beats the hyperplane. 
% \end{theorem}

% We provide numerical evidence that the conjectured tiger partitions are very suboptimal, which forces us to search for other partitions. 

% We do an AI assisted search and find a scheme that we prove gives us a $10^{-5}$ improvement. 

% \begin{theorem}[Explicit Improvement]
%     $K_G < \frac{\pi}{2 \log(1 + \sqrt{2})} - 10^{-5}$.
% \end{theorem}



% }








% The second contribution is the systematic use of mixtures of rounding schemes. If
% \((f^{(1)},g^{(1)}),\ldots,(f^{(k)},g^{(k)})\) are rounding schemes and \(p\in\Delta_{k-1}\),
% then
% \[
%     H_p(t)=\sum_{\ell=1}^k p_\ell H_{f^{(\ell)},g^{(\ell)}}(t)
% \]
% is again the correlation function of an honest randomized rounding scheme: first sample
% \(\ell\) with probability \(p_\ell\), and then apply the \(\ell\)-th rounding. The point is that
% the passage from \(H_p\) to its inverse is nonlinear. Thus a mixture can sometimes have a
% better inverse-majorant parameter than any of its individual components. Geometrically, one
% should think of the different schemes as attending to different difficult configurations of
% vectors.

% Using this observation, together with an AI-assisted search over Hermite-threshold
% partitions, we find a two-atom mixture giving the following certified improvement.

% \begin{theorem}[Explicit improvement over Krivine's bound]
% \label{thm:explicit-improvement}
% There is an explicit mixed planar Krivine rounding scheme with inverse-majorant parameter
% \(\gamma\) satisfying
% \[
%     \gamma \geq \rho_*+2.75\cdot 10^{-5}.
% \]
% The scheme is a probability mixture of the hyperplane rounding and a degree-\(9\)
% Hermite-threshold rounding of the form
% \[
%     f_\Phi(x_1,x_2)=\sgn(x_2-\Phi(x_1)),
%     \qquad
%     g_\Phi(x_1,x_2)=\sgn(x_2+\Phi(x_1)),
% \]
% where \(\Phi\) is an explicit odd Hermite polynomial listed in Section~\ref{sec:explicit-improvement}.
% Therefore
% \[
%     K_G
%     \leq
%     \frac{\pi}{2\gamma}
%     \leq
%     \frac{\pi}{2\log(1+\sqrt2)}
%     -
%     5.56\cdot 10^{-5}.
% \]
% In particular,
% \[
%     K_G
%     <
%     \frac{\pi}{2\log(1+\sqrt2)}
%     -
%     10^{-5}.
% \]
% \end{theorem}

% The search leading to Theorem~\ref{thm:explicit-improvement} also reveals that the space of
% useful roundings is much larger than the previously studied families. In particular, the
% ``tiger partitions'' suggested by the variational problem for the König bilinear form are
% natural candidates, but our numerical experiments indicate that they are not close to optimal
% for the Grothendieck rounding problem. This is not merely a computational inconvenience:
% the König bilinear form probes the correlation function only at the point \(t=i\), whereas
% the Grothendieck rounding value depends on the full inverse-majorant series of \(H^{-1}\).
% Thus optimizing the König bilinear form and optimizing the Krivine parameter are genuinely
% different objectives.

==> old/introduction_v1.tex <==
\section{Introduction}

Outline:
\begin{enumerate}
    \item Definition of Grothendieck constant: numerical improvement. 
    \item Rounding schemes and analysis. 
    \item Main theorem: For f = blah, g=blah, we have constant < blah.
    \item Proof outline: (0) We do a variable change to simplify analysis. (1) Numerical computation of Taylor series upto 220. (2) Bounding the remainder term. 

    The variable change helps, and changes how the remainder term is bounded. 
    \item Bounding the remainder term without mixing. This is new, and deviates significantly from [BMMN]. Make this as modular as  possible. 
    \item Section on numerical computation: Discuss computation and cross-verification with pytorch, etc. Why this is trustable (why can't this just be a floating point artifact)?
    \item AI-guided search of rounding schemes. 
    \item Koenig bilinear form: Related to Grothendieck. Main result. Best constant, higher dimensions give the constant. Not clear if it is realizable in two-dimensions.  
\end{enumerate}
In 1953, Alexander Grothendieck published a paper on the metric theory of tensor products, \emph{R\'esum\'e de la th\'eorie m\'etrique des produits tensoriels topologiques}, 
which had far-reaching impacts on functional analysis and the theory of Banach spaces.
While this paper was initially ignored, its central result, now referred to as the \textit{Grothendieck inequality}, has since found applications in a large 
number of seemingly unrelated areas, including computational hardness thresholds, quantum 
mechanics, geometry, harmonic analysis, and operator theory. 

The \textit{Grothendieck inequality}, states that there exists a universal constant \(K_G < \infty\) such 
that for every \(m,n \in \N\) and every matrix \(A=(a_{ij}) \in \R^{m \times n}\),
\begin{equation}
    \max_{\varepsilon_i,\delta_j \in \{\pm 1\}}
    \bigg|
    \sum_{i=1}^m \sum_{j=1}^n a_{ij}\varepsilon_i\delta_j
    \bigg|
    \leq 
    \sup_{d \geq 1}
    \max_{\substack{u_i,v_j \in S^{d-1}}}
    \bigg|
    \sum_{i=1}^m \sum_{j=1}^n a_{ij}\angles{u_i,v_j}
    \bigg|
    \leq 
    K_G
    \max_{\varepsilon_i,\delta_j \in \{\pm 1\}}
    \bigg|
    \sum_{i=1}^m \sum_{j=1}^n a_{ij}\varepsilon_i\delta_j
    \bigg|.
\end{equation}
Here \(S^{d-1}\) denotes the unit sphere in \(\R^d\). The smallest constant \(K_G\) for which
this inequality holds is called the real Grothendieck constant.

The Grothendieck constant is fundamental in combinatorial optimization because it controls
how well certain integer optimization problems can be approximated by continuous relaxations.
One important example is the problem of efficiently computing the cut norm of a matrix, which
is used in a variety of algorithms, including constructions of
Szemerédi partitions of graphs ~\cite{AN06}. A particularly nice complexity-theoretic
interpretation of \(K_G\) is that it gives the Unique Games hardness threshold for approximating
the following integer quadratic program:
\begin{equation}
    \mrm{IQP}(A)
    \quad \defeq \quad
    \max_{\varepsilon \in \{\pm 1\}^m,\ \delta \in \{\pm 1\}^n}
    \sum_{i=1}^m \sum_{j=1}^n a_{ij}\varepsilon_i\delta_j .
\end{equation}
The natural continuous relaxation is the semidefinite program
\begin{equation}
    \mrm{SDP}(A)
    \quad \defeq \quad
    \sup_{d \geq 1}
    \max_{\substack{u_1,\ldots,u_m \in S^{d-1}\\
                    v_1,\ldots,v_n \in S^{d-1}}}
    \sum_{i=1}^{m}\sum_{j=1}^{n} a_{ij}\,\angles{u_i,v_j}.
\end{equation}
Equivalently, one may take \(d=m+n\). With this notation, Grothendieck's inequality says that
\begin{equation}
    \mrm{IQP}(A)
    \leq 
    \mrm{SDP}(A)
    \leq 
    K_G \cdot \mrm{IQP}(A).
\end{equation}
The Raghavendra--Steurer theorem shows that this constant has a sharp complexity-theoretic
meaning: if there were a polynomial-time algorithm that approximates \(\mrm{IQP}(A)\) to
within a factor \(c<K_G\), then the Unique Games Conjecture would be false. Due to this, there have been major attempts at obtaining better bounds on $K_G$.   

\textbf{Rounding schemes.} One way to upper bound \(K_G\) is through the design and analysis of \emph{rounding schemes}.
A rounding scheme is a possibly randomized procedure that takes a solution
\[
    \{u_i\}_{i=1}^m,\{v_j\}_{j=1}^n \subset S^{d-1}
\]
of the semidefinite relaxation and produces signs
\[
    \varepsilon_1,\ldots,\varepsilon_m,\delta_1,\ldots,\delta_n \in \{\pm 1\}.
\]
Krivine proved his upper bound \(K_G \le \tfrac{\pi}{2 \log(1 + \sqrt{2})}\) using a very clever randomized hyperplane rounding
scheme. The idea is to preprocess the vectors  $\{u_i\}_{i=1}^m,\{v_j\}_{j=1}^n$ by lifting them to an infinite dimensional space, then projecting them onto a random hyperplane and rounding based on which side of the hyperplane the vectors lie on. Krivine conjectured this to be the optimal rounding scheme, and this conjecture stood for nearly thirty years.  

This conjecture was then refuted by Braverman,
Makarychev, Makarychev, and Naor (BMMN) to improve on Krivine's bound. They generalized Krivine's schemes by using projections that rounded based on non-linear geometries. At a high level, these
rounding schemes can be viewed as pairs of partitions of \(\R^d\). The choice of partition
encodes geometric information about which configurations of vectors make Grothendieck's
inequality hardest to round.

There is, however, an analytic difficulty in turning a promising partition into an actual Grothendieck rounding scheme.
The main obstruction in the work of BMMN was that in order to make certain analytic statements hold, they had to \textit{mix} their new rounding scheme with the classical hyperplane scheme. 

A mixed rounding scheme is a simple randomized procedure. Instead of choosing one rounding
rule once and for all, we first flip a biased coin. With probability \(p\), we use the new
rounding scheme, and with probability \(1-p\), we use the hyperplane rounding scheme. After
this choice is made, we apply the chosen scheme to all the SDP vectors.

This kind of mixing is useful because, when \(p\) is small, the resulting procedure remains
very close to hyperplane rounding, which is much easier to analyze. The drawback is that the
new rounding scheme is only used with probability \(p\). Braverman et al. requires $p$ to be very small, thus most of the potential improvement is washed out before it can meaningfully affect the final Grothendieck bound.

Our first contribution is removing the need for mixing. The theorem gives a pure, unmixed perturbation in the same family as Braverman et al. that already beats the hyperplane.

\begin{theorem}[A pure planar perturbation beats hyperplane rounding]
\label{thm:pure-h3}
Let \(H_3(x)=8x^3-12x\), and set
\[
 \tau=0.03175,
 \qquad
 \eta=\frac{\tau}{\sqrt{48}}
 =0.004582717761692655\ldots .
\]
Define odd planar partitions \(f,g:\R^2\to\{\pm1\}\) by
\[
    f(x,y)=\sgn(y-\eta H_3(x)),
    \qquad
    g(x,y)=\sgn(y+\eta H_3(x)).
\]
The rounding scheme generated by this pair of partitions gives the upper bound,
\[
    K_G
    <
   \frac{\pi}{2\log(1+\sqrt2)} - 
    9.7\cdot 10^{-6}
\]
\end{theorem}

This theorem shows that the obstruction was not geometric: one does not need to mix the
perturbation with the hyperplane merely to obtain a valid Krivine scheme. Once the analytic
step is handled correctly, a much broader class of pure and mixed strategies becomes
available. In fact, the proof of Theorem~\ref{thm:pure-h3} applies even for mixed schemes. 

But why should mixing remain useful after we have spent so much effort removing the need
for it? The answer lies in \emph{why} BMMN used mixing
in the first place. In their argument, the mixing parameter \(p\) had to be very small in
order to control certain analytic properties of the rounding scheme. In that regime, mixing
is primarily a technical device: the new rounding is used only rarely, so its effect on the
final Grothendieck bound is necessarily diluted.

In this paper, we observe a different and more interesting phenomenon. A mixture of two
rounding schemes can sometimes give a \emph{strictly} better Grothendieck bound than either
scheme gives individually. Intuitively, one should think of different schemes as performing
well on different difficult configurations of vectors. A randomized mixture can combine strengths of different schemes. This observation changes the search problem for rounding schemes.  

\textbf{Tiger Partitions}. A natural first place to look for better roundings chemes is the class of ``tiger partitions'' suggested by BMMN. These partitions arise from a variational problem related to their proof. BMMN conjectured that the roundings derived from these partitions may provide the optimal candidates for the best bound on $K_G$. 
However, our computations show that tiger partitions are not competitive
for improving the Grothendieck bound. This is an important negative result: it means that
the most natural geometric candidates do not appear to be the correct ones, and the space of
useful rounding schemes is much larger than the previously studied examples.

\textbf{AI-Guided Search}. In order to effectively explore this larger space of rounding schemes, we therefore use an AI-assisted search. The search is over
explicit partitions of low-dimensional Gaussian space, especially partitions whose boundary
is given by threshold functions. In two dimensions, these have the form
\[
    f_\Phi(x_1,x_2)=\sgn(x_2-\Phi(x_1)),
    \qquad
    g_\Phi(x_1,x_2)=\sgn(x_2+\Phi(x_1)),
\]
where \(\Phi\) is an odd Hermite polynomial. We also allow higher-dimensional analogues in
which the threshold depends on several Gaussian coordinates. The AI agent is asked to
generate candidate threshold functions, optimize their coefficients, store the best
candidates, and then search over mixtures of those candidates. The final candidates are then checked by a separate rigorous certification procedure.

This search produces an explicit mixed planar scheme giving our best quantitative bound.

\begin{theorem}[Explicit improvement over Krivine's bound]
\label{thm:explicit-improvement}
There is an explicit mixed planar Krivine rounding scheme such that
\[
    K_G
    \leq
    \frac{\pi}{2\log(1+\sqrt2)}
    -
    5.56\cdot 10^{-5}.
\]
The scheme is a probability mixture of the classical hyperplane rounding and an explicit
degree-\(9\) Hermite-threshold rounding of the form
\[
    f_\Phi(x_1,x_2)=\sgn(x_2-\Phi(x_1)),
    \qquad
    g_\Phi(x_1,x_2)=\sgn(x_2+\Phi(x_1)),
\]
where the polynomial \(\Phi\) and the mixture weights are listed in
Section~\ref{sec:explicit-improvement}.
\end{theorem}


\textbf{K\"onig Bilinear Form}. {\color{blue} FOR ALAN: DEFINE KONIG IN BRIEF HERE, THEN LINK TO SECTION WHERE IT IS DEFINED PROPERLY} We prove an asymptotic theorem for a tractable high-dimensional
family of rotated hyperplane partitions. 
Let
\[
    a(\theta)=\operatorname{arsinh}(\cos\theta),
\]
viewed as a \(2\pi\)-periodic analytic function. For \(d\in\N\) and parameters
\(\alpha,\beta\in\R\), define
\[
    Q_d(u)=4\norm{u}_2^2-d,
    \qquad
    \psi_{d,\alpha,\beta}(u)=\beta+\alpha Q_d(u),
\]
and let \(K_d(\alpha,\beta)\) denote the corresponding reduced König value for the affine
radial rotated-hyperplane family defined in Section~\ref{sec:konig-not-sufficient}. The
large-\(d\) limit is governed by the periodic Airy flow.

\begin{theorem}[Airy limit for the affine radial König problem]
\label{thm:airy-limit-intro}
Fix \(0<\rho<\rho_*\) and \(\kappa_0>0\). Then there exist constants
\(C=C(\rho,\kappa_0)\) and \(d_0=d_0(\rho,\kappa_0)\) such that for all \(d\geq d_0\),
all \(|\kappa|\leq \kappa_0\), and all \(\beta\in\R\),
\[
    \left|
    K_d\!\left(\kappa d^{-1/3},\beta\right)
    -
    \frac{2}{\pi}
    \left(e^{-\tau_\kappa \partial_\theta^3}a\right)(2\beta)
    \right|
    \leq
    C d^{-1/3},
\]
where
\[
    \tau_\kappa=\frac{16}{3}\kappa^3.
\]
Equivalently,
\[
    K_d\!\left(\kappa d^{-1/3},\beta\right)
    \longrightarrow
    \frac{2}{\pi}
    \left(e^{-\tau_\kappa \partial_\theta^3}a\right)(2\beta)
\]
uniformly for \((\kappa,\beta)\in[-\kappa_0,\kappa_0]\times\R\).
\end{theorem}

Theorem~\ref{thm:airy-limit-intro} gives an explicit asymptotic model for the König bilinear form in this family. 

The rest of the paper is organized as follows. Section~\ref{sec:krivine-schemes} recalls
Krivine rounding schemes and proves the pure \(h_3/-h_3\) improvement. Section~\ref{sec:analytic-obstruction}
develops the sine-coordinate inverse certificate that removes the analytic obstruction.
Section~\ref{sec:explicit-improvement} describes the AI-assisted search over Hermite-threshold
partitions and proves the explicit \(10^{-5}\) improvement. Finally,
Section~\ref{sec:konig-not-sufficient} analyzes the affine radial family and proves the Airy
limit for the König bilinear form.



% {\color{red}
% In 1953, Alexander Grothendieck published a paper on the metric theory of tensor products with wide reaching impacts on functional analysis and the theory of Banach spaces. While this paper was initially ignored, its results have since found applications in a large number of seemingly unrelated areas, including $C^*$ algebras, Bell's inequality in quantum mechanics, and in polynomial-time approximation algorithms for certain NP-hard problems.

% Groethendieck's inequality states that there exists a constant \(K_G > 0\), such that for all \(A \in \R^{m \times n}\):
% \begin{equation}
%     \max_{x_i, y_j \in \{\pm 1\}} \bigg|
%     \sum_{i, j} a_{ij} x_i y_j \bigg|
%     \leq \sup_{d \geq 1} \max_{\substack{u_i, v_i \in \mbb{R}^{d} \\ \norm{u_i} = \norm{v_j} = 1}} \bigg| \sum_{i, j} a_{ij} \angles{u_i, v_j} \bigg|
%     \leq \max_{x_i, y_j \in \{\pm 1\}}
%     K_G \bigg| \sum_{i, j} a_{ij} x_i y_j \bigg|,
% \end{equation}
% This constant is independent of \(m\) and \(n\), with the current best lower (CITE) and upper bound (CITE) being:
% \begin{equation}
%     1.676\ldots < K_G < 1.782\ldots
% \end{equation}
% Groethendieck's inequality is of interest in combinatorial optimization because it establishes a fundamental limitation of how well continuous programs can approximate discrete ones.
% One connection is in the optimality gap between an integer quadratic program and its semidefinite relaxation. Consider the following integer quadratic program:
% \begin{equation}
% \mrm{IQP}(A)
%     \quad \defeq \quad
%     \max_{x \in \{\pm 1\}^m, y \in \{\pm 1\}^n}
%     \enskip \sum_{i,j} a_{ij} x_i y_j,
% \end{equation}
% and its continuous relaxation, which is a semidefinite program of the form:
% \[
% \mathrm{SDP}(A)\;\defeq\;
% \max_{\substack{x_1,\ldots,x_m\in S^{d-1}\\ y_1,\ldots,y_n\in S^{d-1}}}
% \;\sum_{i=1}^{m}\sum_{j=1}^{n} a_{ij}\,\langle x_i, y_j\rangle ,
% \]
% Groethendieck's inequality then states that:
% \begin{equation}
%     \abs{\mrm{IQP}(A)}
%     \leq \abs{\mrm{SDP}(A)}
%     \leq K_G \cdot \abs{\mrm{IQP}(A)}.
% \end{equation}
 

% \begin{theorem}[Removing mixture obstruction]
% We show that a perturbation on its own is a rounding scheme that beats the hyperplane. 
% \end{theorem}

% We provide numerical evidence that the conjectured tiger partitions are very suboptimal, which forces us to search for other partitions. 

% We do an AI assisted search and find a scheme that we prove gives us a $10^{-5}$ improvement. 

% \begin{theorem}[Explicit Improvement]
%     $K_G < \frac{\pi}{2 \log(1 + \sqrt{2})} - 10^{-5}$.
% \end{theorem}



% }








% The second contribution is the systematic use of mixtures of rounding schemes. If
% \((f^{(1)},g^{(1)}),\ldots,(f^{(k)},g^{(k)})\) are rounding schemes and \(p\in\Delta_{k-1}\),
% then
% \[
%     H_p(t)=\sum_{\ell=1}^k p_\ell H_{f^{(\ell)},g^{(\ell)}}(t)
% \]
% is again the correlation function of an honest randomized rounding scheme: first sample
% \(\ell\) with probability \(p_\ell\), and then apply the \(\ell\)-th rounding. The point is that
% the passage from \(H_p\) to its inverse is nonlinear. Thus a mixture can sometimes have a
% better inverse-majorant parameter than any of its individual components. Geometrically, one
% should think of the different schemes as attending to different difficult configurations of
% vectors.

% Using this observation, together with an AI-assisted search over Hermite-threshold
% partitions, we find a two-atom mixture giving the following certified improvement.

% \begin{theorem}[Explicit improvement over Krivine's bound]
% \label{thm:explicit-improvement}
% There is an explicit mixed planar Krivine rounding scheme with inverse-majorant parameter
% \(\gamma\) satisfying
% \[
%     \gamma \geq \rho_*+2.75\cdot 10^{-5}.
% \]
% The scheme is a probability mixture of the hyperplane rounding and a degree-\(9\)
% Hermite-threshold rounding of the form
% \[
%     f_\Phi(x_1,x_2)=\sgn(x_2-\Phi(x_1)),
%     \qquad
%     g_\Phi(x_1,x_2)=\sgn(x_2+\Phi(x_1)),
% \]
% where \(\Phi\) is an explicit odd Hermite polynomial listed in Section~\ref{sec:explicit-improvement}.
% Therefore
% \[
%     K_G
%     \leq
%     \frac{\pi}{2\gamma}
%     \leq
%     \frac{\pi}{2\log(1+\sqrt2)}
%     -
%     5.56\cdot 10^{-5}.
% \]
% In particular,
% \[
%     K_G
%     <
%     \frac{\pi}{2\log(1+\sqrt2)}
%     -
%     10^{-5}.
% \]
% \end{theorem}

% The search leading to Theorem~\ref{thm:explicit-improvement} also reveals that the space of
% useful roundings is much larger than the previously studied families. In particular, the
% ``tiger partitions'' suggested by the variational problem for the König bilinear form are
% natural candidates, but our numerical experiments indicate that they are not close to optimal
% for the Grothendieck rounding problem. This is not merely a computational inconvenience:
% the König bilinear form probes the correlation function only at the point \(t=i\), whereas
% the Grothendieck rounding value depends on the full inverse-majorant series of \(H^{-1}\).
% Thus optimizing the König bilinear form and optimizing the Krivine parameter are genuinely
% different objectives.

==> old/koenig.tex <==
\section{Why K\"onig Is Not Sufficient}
\label{sec:konig-not-sufficient}

This note rewrites the affine radial asymptotic theorem in a way that makes the setup completely explicit. We begin from Krivine's 2023 rotating-hyperplane construction and isolate the two objects that actually drive the computation: the circle function
\[
 f(\theta)=\arsinh(\cos\theta)
\]
and the phase inserted into it. The higher-dimensional generalization is then obtained by replacing Krivine's one-dimensional quadratic observable by its $d$-dimensional radial analogue. For this family we prove an exact finite-$d$ Fourier reduction, identify the correct scaling $\alpha\sim d^{-1/3}$, and show that the limit is a periodic Airy flow acting on $f$.


\subsection{Motivation: Krivine's rotating hyperplane}

We start with the part of Krivine's construction that matters for the present theorem. Let
\[
\Phi_{F,G}(t):=\E\bigl[\operatorname{sign}(F(X))\operatorname{sign}(G(Y))\bigr],
\qquad |t|<1,
\]
where $(X_i,Y_i)$ are independent centered Gaussian pairs with $\E[X_iY_i]=t$, and $F,G$ are odd measurable functions on a Euclidean space. A standard identity due to Grothendieck says that if $(U,V)$ is a centered bivariate normal pair with correlation $\rho$, then
\[
\E[\operatorname{sign}(U)\operatorname{sign}(V)]=\frac{2}{\pi}\arcsin(\rho).
\]
Krivine's 2023 note chooses a family in dimension $3$ of the form
\[
F_\varepsilon(x_0,x_1,x_2)=x_1\cos\bigl(\varepsilon H_2(x_0)\bigr)+x_2\sin\bigl(\varepsilon H_2(x_0)\bigr),
\]
\[
G_\varepsilon(y_0,y_1,y_2)=y_1\cos\bigl(\varepsilon H_2(y_0)\bigr)-y_2\sin\bigl(\varepsilon H_2(y_0)\bigr),
\]
with $H_2(s)=s^2-1$.

The point is geometric: the sign cut is still an ordinary half-space in the active $(x_1,x_2)$-plane, but that half-space is rotated by an angle depending on the auxiliary coordinate $x_0$. The same happens on the $Y$ side. If we condition on $x_0,y_0$, then $F_\varepsilon(X)$ and $G_\varepsilon(Y)$ are centered Gaussians with correlation
\[
 t\Bigl(\cos\bigl(\varepsilon H_2(x_0)\bigr)\cos\bigl(\varepsilon H_2(y_0)\bigr)-\sin\bigl(\varepsilon H_2(x_0)\bigr)\sin\bigl(\varepsilon H_2(y_0)\bigr)\Bigr)
 = t\cos\bigl(\varepsilon(H_2(x_0)+H_2(y_0))\bigr).
\]
Therefore Grothendieck's identity gives
\[
\Phi_{F_\varepsilon,G_\varepsilon}(t)
 = \frac{2}{\pi}\,\E\Bigl[\arcsin\bigl(t\cos(\varepsilon(H_2(X_0)+H_2(Y_0)))\bigr)\Bigr].
\]
At the special point $t=i$ one uses $\arcsin(i s)=i\,\arsinh(s)$ to obtain
\[
\frac{\Phi_{F_\varepsilon,G_\varepsilon}(i)}{i}
= \frac{2}{\pi}\,\E\Bigl[\arsinh\bigl(\cos(\varepsilon(H_2(X_0)+H_2(Y_0)))\bigr)\Bigr]
\]
after the standard analytic continuation of the Gaussian kernel. This is the origin of the fixed circle function
\[
 f(\theta):=\arsinh(\cos\theta),\qquad \theta\in\R.
\]
It is convenient to view $f$ as a $2\pi$-periodic function on the circle $\T=\R/2\pi\mathbb Z$.

\medskip

\noindent\textbf{What is the phase?} In the last display, the quantity
\[
\varepsilon\bigl(H_2(X_0)+H_2(Y_0)\bigr)
\]
is the phase. It is the sum of the two rotation angles, one coming from the $X$ side and one from the $Y$ side. The whole reduced problem is obtained by evaluating the fixed circle function $f(\theta)$ at that phase. This is the model for everything that follows.

\medskip

Krivine's note then rewrites the resulting two-variable integral more explicitly. After the rescaling used in the $t=i$ formula, one gets
\[
\frac{\Phi_{F_\varepsilon,G_\varepsilon}(i)}{i}
=
\frac{2^{3/2}}{\pi^2}
\int_{\R}\int_{\R}
 e^{-(u^2+v^2)}\cos(2uv)
 f\bigl(\varepsilon((4u^2-1)+(4v^2-1))\bigr)
\,du\,dv.
\]
Now pass to polar coordinates $u=r\cos\ph$, $v=r\sin\ph$. Then
\[
2uv=r^2\sin(2\ph),\qquad (4u^2-1)+(4v^2-1)=4r^2-2,
\qquad du\,dv=r\,dr\,d\ph.
\]
If we write $\rho=r^2$ and $\vartheta=2\ph$, then
\begin{align*}
\frac{\Phi_{F_\varepsilon,G_\varepsilon}(i)}{i}
&=
\frac{2^{3/2}}{\pi^2}
\int_0^\infty\int_0^{2\pi}
 e^{-r^2}\cos(r^2\sin(2\ph))
 f\bigl(\varepsilon(4r^2-2)\bigr)
 r\,d\ph\,dr \\
&=
\frac{2\sqrt2}{\pi^2}
\int_0^\infty\int_0^{\pi}
 e^{-\rho}\cos(\rho\sin\vartheta)
 f\bigl(2\varepsilon(2\rho-1)\bigr)
\,d\vartheta\,d\rho.
\end{align*}
This is exactly the oscillatory integral written in Krivine's note, with his parameter $\eta$ equal to $2\varepsilon$.

\subsection{The higher-dimensional affine radial family}

The previous construction suggests the following clean generalization. We keep an active two-dimensional plane in which the actual half-space cut lives, and we let an auxiliary $d$-dimensional Gaussian block determine the rotation angle.

\begin{definition}[Local angle and phase]
Fix $d\in\mathbb N$ and parameters $\alpha,\beta\in\R$. Define
\[
Q_d(u):=4\norm{u}_2^2-d,\qquad u\in\R^d,
\]
\[
\psi_{d,\alpha,\beta}(u):=\beta+\alpha Q_d(u),
\]
and the associated pairwise phase function
\[
\phi_{d,\alpha,\beta}(u,v):=\psi_{d,\alpha,\beta}(u)+\psi_{d,\alpha,\beta}(v)
=2\beta+\alpha\bigl(Q_d(u)+Q_d(v)\bigr).
\]
\end{definition}

A few remarks are worth making immediately.
\begin{itemize}[leftmargin=1.5em]
\item The symbol $\theta$ will always denote the circle variable in the periodic function $f(\theta)=\arsinh(\cos\theta)$. The phase function $\phi_{d,\alpha,\beta}(u,v)$ is the real number that gets plugged into that circle variable.
\item The parameter $\beta$ is a constant rotation; it contributes $\beta$ on the $u$ side and $\beta$ on the $v$ side, hence the total shift $2\beta$.
\item The parameter $\alpha$ controls how strongly the rotation depends on the auxiliary variables. The family is called \emph{affine radial} because the angle depends affinely on the radial observable $Q_d(u)$.
\item After the rescaling used above, $Q_d(u)$ is the direct $d$-dimensional analogue of Krivine's $H_2$: indeed
\[
Q_d(u)=\sum_{j=1}^d\bigl((2u_j)^2-1\bigr).
\]
\end{itemize}

The corresponding rotated half-space signs on $\R^{d+2}=\R^d\times\R^2$ are
\[
F_{d,\alpha,\beta}(u;x_1,x_2):=
\operatorname{sign}\bigl(x_1\cos\psi_{d,\alpha,\beta}(u)+x_2\sin\psi_{d,\alpha,\beta}(u)\bigr),
\]
\[
G_{d,\alpha,\beta}(v;y_1,y_2):=
\operatorname{sign}\bigl(y_1\cos\psi_{d,\alpha,\beta}(v)-y_2\sin\psi_{d,\alpha,\beta}(v)\bigr).
\]
Conditioned on $u,v$, the active-plane correlation is $t\cos\phi_{d,\alpha,\beta}(u,v)$, exactly as in Krivine's construction. After evaluating at $t=i$ and integrating out the active plane, one is left with the reduced functional below.

\begin{definition}[Reduced K\"onig functional]
Let
\[
 c_d:=\frac{2^{1+d/2}}{\pi^{d+1}}.
\]
The reduced affine radial K\"onig functional is
\begin{equation}\label{eq:Kd-def}
\K_d(\alpha,\beta)
:=
 c_d
\int_{\R^d}\int_{\R^d}
 e^{-(\norm{u}_2^2+\norm{v}_2^2)}
 \cos\bigl(2\ip{u}{v}\bigr)
 f\bigl(\phi_{d,\alpha,\beta}(u,v)\bigr)
\,du\,dv.
\end{equation}
\end{definition}

Thus the entire dependence on the rotating partition is encoded by the phase function $\phi_{d,\alpha,\beta}$. The circle variable of $f$ is evaluated at this phase.

When $\alpha=\beta=0$ there is no rotation at all, and one recovers the hyperplane benchmark
\[
\K_d(0,0)=\frac{2}{\pi}f(0)=\frac{2}{\pi}\arsinh(1)=\frac{2}{\pi}\log(1+\sqrt2).
\]
We will also see this directly from the exact Fourier reduction below.

\subsection{Main theorem and the Airy operator}

The asymptotic object is the periodic Airy flow on the circle.

\begin{definition}[Periodic Airy propagator]
Let $g(\theta)=\sum_{m\in\mathbb Z}\wt g(m)e^{im\theta}$ be a $2\pi$-periodic analytic function, with Fourier coefficients
\[
\wt g(m):=\frac{1}{2\pi}\int_0^{2\pi} g(\theta)e^{-im\theta}\,d\theta.
\]
For $\tau\in\R$ define
\[
\bigl(e^{-\tau\partial_\theta^3}g\bigr)(\theta)
:=
\sum_{m\in\mathbb Z} e^{i\tau m^3}\wt g(m)e^{im\theta}.
\]
Equivalently, $u(\tau,\theta):=(e^{-\tau\partial_\theta^3}g)(\theta)$ is the solution of the periodic Airy equation
\[
\partial_\tau u + \partial_\theta^3 u = 0,
\qquad u(0,\theta)=g(\theta).
\]
Indeed, on the Fourier mode $e^{im\theta}$ one has $-\partial_\theta^3=e^{im\theta}\mapsto i m^3 e^{im\theta}$.
\end{definition}

We can now state the theorem in its final form.

\begin{theorem}[Airy limit for the affine radial phase family]\label{thm:main}
Let
\[
 f(\theta)=\arsinh(\cos\theta),\qquad \theta\in\T.
\]
Fix $0<\rho<\rho_*$, where $\rho_*:=\arsinh(1)=\log(1+\sqrt2)$, and fix $\kappa_0>0$. Then there exist constants $C=C(\rho,\kappa_0)$ and $d_0=d_0(\rho,\kappa_0)$ such that for all $d\ge d_0$, all $|\kappa|\le\kappa_0$, and all $\beta\in\R$,
\begin{equation}\label{eq:main-estimate}
\left|
\K_d\bigl(\kappa d^{-1/3},\beta\bigr)
-
\frac{2}{\pi}\bigl(e^{-\tau_\kappa\partial_\theta^3}f\bigr)(2\beta)
\right|
\le C d^{-1/3},
\end{equation}
where
\[
\tau_\kappa:=\frac{16}{3}\kappa^3.
\]
Equivalently,
\[
\K_d\bigl(\kappa d^{-1/3},\beta\bigr)
\longrightarrow
\frac{2}{\pi}\bigl(e^{-\tau_\kappa\partial_\theta^3}f\bigr)(2\beta)
\]
uniformly for $(\kappa,\beta)\in[-\kappa_0,\kappa_0]\times\R$.
\end{theorem}

\begin{remark}[Why the scaling is $d^{-1/3}$]
The proof diagonalizes $\K_d$ in the Fourier basis and produces a scalar multiplier $\Lambda(m\alpha)^d$ on the $m$th Fourier mode. The key expansion is
\[
\log\Lambda(z)=\frac{16i}{3}z^3-16z^4+O(z^5).
\]
The first nontrivial oscillatory term is cubic, so the only scaling for which $d\log\Lambda(m\alpha)$ remains nondegenerate is $d\alpha^3\asymp 1$, i.e.
\[
\alpha\asymp d^{-1/3}.
\]
The cubic phase produces the Airy multiplier $e^{i\tau m^3}$, while the quartic term yields the $O(d^{-1/3})$ error.
\end{remark}

\begin{remark}[Proof strategy]
Expand $f$ into its Fourier series on the circle. Each Fourier mode can be integrated exactly through a $2\times 2$ Gaussian computation, and the entire functional becomes a diagonal Fourier multiplier. One then expands this multiplier near the origin, chooses the $d^{-1/3}$ scaling dictated by the cubic term, and splits the Fourier modes into low frequencies $|m|\le A\log d$ and a rapidly decaying analytic tail. This turns the heuristic Airy limit into the uniform estimate \eqref{eq:main-estimate}.
\end{remark}

\subsection{Exact finite-$d$ Fourier reduction}

The finite-dimensional problem is already completely explicit.

\begin{theorem}[Exact reduction]\label{prop:exact}
Define
\[
\Lambda(z):=\frac{e^{-2iz}}{\sqrt{1-4iz-8z^2}},
\qquad z\in\R,
\]
with the principal branch of the square root. Then
\begin{equation}\label{eq:exact-reduction}
\K_d(\alpha,\beta)
=
\frac{2}{\pi}
\sum_{m\in\mathbb Z}
\wt f(m)e^{2im\beta}\Lambda(m\alpha)^d.
\end{equation}
\end{theorem}

\begin{proof}
Because $f$ is real analytic on a strip around the real axis, its Fourier series converges absolutely:
\[
 f(\theta)=\sum_{m\in\mathbb Z}\wt f(m)e^{im\theta}.
\]
Substituting this into \eqref{eq:Kd-def} and interchanging the sum and the integral yields
\[
\K_d(\alpha,\beta)
=
 c_d
\sum_{m\in\mathbb Z}\wt f(m)e^{2im\beta}
 I_{m,d}(\alpha),
\]
where
\[
I_{m,d}(\alpha)
:=
\int_{\R^d}\int_{\R^d}
 e^{-(\norm{u}^2+\norm{v}^2)}
 \cos\bigl(2\ip{u}{v}\bigr)
 e^{im\alpha(Q_d(u)+Q_d(v))}
\,du\,dv.
\]
Since $Q_d(v)$ is even in $v$, the change of variables $v\mapsto -v$ shows that the two exponentials arising from
\[
\cos\bigl(2\ip{u}{v}\bigr)=\frac{e^{2i\ip{u}{v}}+e^{-2i\ip{u}{v}}}{2}
\]
contribute equally. Hence
\[
I_{m,d}(\alpha)
=
\int_{\R^d}\int_{\R^d}
 e^{-(\norm{u}^2+\norm{v}^2)}
 e^{2i\ip{u}{v}}
 e^{im\alpha(Q_d(u)+Q_d(v))}
\,du\,dv.
\]
Now the integrand factorizes coordinate by coordinate, so
\[
I_{m,d}(\alpha)
=
\prod_{j=1}^d
\int_{\R^2}
 e^{-(x^2+y^2)}
 e^{im\alpha((4x^2-1)+(4y^2-1))}
 e^{2ixy}
\,dx\,dy.
\]
The one-coordinate Gaussian integral is
\[
\int_{\R^2}
 e^{-(1-4im\alpha)x^2-(1-4im\alpha)y^2+2ixy}
\,dx\,dy
=
\frac{\pi}{\sqrt{(1-4im\alpha)^2+1}},
\]
so after including the factor $e^{-2im\alpha}$ coming from the two "$-1$" terms we get
\[
\int_{\R^2}\cdots
=
\frac{\pi e^{-2im\alpha}}{\sqrt{(1-4im\alpha)^2+1}}
=
\frac{\pi}{\sqrt2}\,\Lambda(m\alpha).
\]
Therefore
\[
I_{m,d}(\alpha)=\left(\frac{\pi}{\sqrt2}\right)^d\Lambda(m\alpha)^d.
\]
Since
\[
 c_d\left(\frac{\pi}{\sqrt2}\right)^d=\frac{2}{\pi},
\]
we obtain \eqref{eq:exact-reduction}. \qedhere
\end{proof}

\subsection{Two preparatory lemmas}

\begin{lemma}[Fourier coefficient decay]\label{lem:fourier-decay}
Let
\[
\rho_*:=\arsinh(1)=\log(1+\sqrt2).
\]
Then for every $0<\rho<\rho_*$ there exists $C_\rho<\infty$ such that
\[
\abs{\wt f(m)}\le C_\rho e^{-\rho\abs m}\qquad (m\in\mathbb Z).
\]
In particular,
\[
\sum_{m\in\mathbb Z}\abs{\wt f(m)}\abs m^k<\infty
\qquad\text{for every }k\ge 0.
\]
\end{lemma}

\begin{proof}
The singularities of $\arsinh(z)$ are at $z=\pm i$, so the singularities of
\[
 f(z)=\arsinh(\cos z)
\]
occur where $\cos z=\pm i$. The nearest such points to the real axis lie at imaginary distance $\rho_*$. Hence $f$ extends holomorphically to every strip
\[
\abs{\Im z}<\rho
\qquad (0<\rho<\rho_*).
\]
The standard Cauchy estimate for Fourier coefficients on analytic strips gives
\[
\abs{\wt f(m)}\le C_\rho e^{-\rho\abs m}.
\]
The summability of polynomially weighted coefficients follows immediately. \qedhere
\end{proof}

\begin{lemma}[Local expansion of the multiplier]\label{lem:lambda-expansion}
For $\abs z\le 1/16$,
\[
\log\Lambda(z)=\frac{16i}{3}z^3-16z^4+r(z),
\]
with the explicit bound
\[
\abs{r(z)}\le 500\abs z^5.
\]
\end{lemma}

\begin{proof}
Write
\[
\Lambda(z)=e^{-2iz}(1+w(z))^{-1/2},
\qquad
w(z):=-4iz-8z^2.
\]
If $\abs z\le 1/16$, then
\[
\abs{w(z)}\le 4\abs z+8\abs z^2\le \frac14+\frac1{32}=\frac9{32}<1.
\]
Hence the principal logarithm is analytic there and
\[
\log\Lambda(z)=-2iz-\frac12\log(1+w(z)).
\]
Use the fourth-order logarithm expansion
\[
\log(1+w)=w-\frac{w^2}{2}+\frac{w^3}{3}-\frac{w^4}{4}+R_5(w),
\qquad
\abs{R_5(w)}\le \frac{\abs w^5}{5(1-\abs w)}.
\]
A direct algebraic expansion gives
\[
-2iz-\frac12\left(w-\frac{w^2}{2}+\frac{w^3}{3}-\frac{w^4}{4}\right)
=
\frac{16i}{3}z^3-16z^4-128iz^5-\frac{2048}{3}z^6+1024iz^7+512z^8.
\]
Thus for $\abs z\le 1/16$,
\[
\left| -128iz^5-\frac{2048}{3}z^6+1024iz^7+512z^8\right|\le 175\abs z^5.
\]
On the other hand, since $\abs{w(z)}\le \frac92\abs z$,
\[
\frac12\abs{R_5(w)}
\le
\frac12\cdot\frac{\abs w^5}{5(1-\abs w)}
\le 261\abs z^5.
\]
Combining the two bounds yields
\[
\abs{r(z)}\le (175+261)\abs z^5\le 500\abs z^5.
\]
\qedhere
\end{proof}

\subsection{Proof of the Airy limit}

\begin{proof}[Proof of Theorem \ref{thm:main}]
Start from theorem \ref{prop:exact}:
\[
\K_d\bigl(\kappa d^{-1/3},\beta\bigr)
=
\frac{2}{\pi}
\sum_{m\in\mathbb Z}
\wt f(m)e^{2im\beta}\Lambda\bigl(m\kappa d^{-1/3}\bigr)^d.
\]
Define the target series
\[
\mathcal L_\infty(\kappa,\beta)
:=
\frac{2}{\pi}
\sum_{m\in\mathbb Z}
\wt f(m)e^{2im\beta}e^{i\tau_\kappa m^3}
=
\frac{2}{\pi}\bigl(e^{-\tau_\kappa\partial_\theta^3}f\bigr)(2\beta),
\]
where $\tau_\kappa=\frac{16}{3}\kappa^3$. We must bound
\[
\K_d\bigl(\kappa d^{-1/3},\beta\bigr)-\mathcal L_\infty(\kappa,\beta).
\]
We split the Fourier modes into low and high frequencies.

\medskip
\noindent\textbf{Step 1: choose the cutoff.}
Pick
\[
A>\frac{1}{3\rho},
\qquad
N_d:=\lfloor A\log d\rfloor.
\]
Since $N_d d^{-1/3}\to 0$, there exists $d_1=d_1(\kappa_0)$ such that for all $d\ge d_1$, all $\abs m\le N_d$, and all $\abs\kappa\le\kappa_0$,
\[
\abs{m\kappa d^{-1/3}}\le \frac1{16}.
\]

\medskip
\noindent\textbf{Step 2: low-frequency expansion.}
For $\abs m\le N_d$, set
\[
 z:=m\kappa d^{-1/3}.
\]
By Lemma \ref{lem:lambda-expansion},
\[
\log\Lambda(z)=\frac{16i}{3}z^3-16z^4+r(z),
\qquad \abs{r(z)}\le 500\abs z^5.
\]
Multiplying by $d$ gives
\[
 d\log\Lambda(z)
 = i\tau_\kappa m^3 -16\kappa^4m^4d^{-1/3}+\varepsilon_{m,d},
\]
where
\[
\abs{\varepsilon_{m,d}}
\le 500\abs\kappa^5\abs m^5 d^{-2/3}
\le 500\kappa_0^5\abs m^5 d^{-2/3}.
\]
Define
\[
\delta_{m,d}:=-16\kappa^4m^4d^{-1/3}+\varepsilon_{m,d}.
\]
Then
\[
\Lambda\bigl(m\kappa d^{-1/3}\bigr)^d
=
 e^{i\tau_\kappa m^3}e^{\delta_{m,d}}.
\]
Since $\abs m\le A\log d$, we have
\[
\abs{\delta_{m,d}}
\le
16\kappa_0^4A^4(\log d)^4d^{-1/3}
+
500\kappa_0^5A^5(\log d)^5d^{-2/3}.
\]
The right-hand side tends to $0$, so there exists $d_2=d_2(\rho,\kappa_0)$ such that for all $d\ge d_2$,
\[
\abs{\delta_{m,d}}\le 1
\qquad (\abs m\le N_d,\ \abs\kappa\le\kappa_0).
\]
Therefore
\[
\abs{e^{\delta_{m,d}}-1}\le 2\abs{\delta_{m,d}}.
\]
So
\[
\left|
\Lambda\bigl(m\kappa d^{-1/3}\bigr)^d-e^{i\tau_\kappa m^3}
\right|
\le
2\abs{\delta_{m,d}}
\le
32\kappa_0^4\abs m^4 d^{-1/3}
+
1000\kappa_0^5\abs m^5 d^{-2/3}.
\]
Hence the low-frequency contribution is bounded by
\begin{align*}
\frac{2}{\pi}
\sum_{\abs m\le N_d}
\abs{\wt f(m)}
\left|
\Lambda\bigl(m\kappa d^{-1/3}\bigr)^d-e^{i\tau_\kappa m^3}
\right|
&\le
\frac{64\kappa_0^4}{\pi}d^{-1/3}
\sum_{m\in\mathbb Z}\abs{\wt f(m)}\abs m^4 \\
&\qquad +
\frac{2000\kappa_0^5}{\pi}d^{-2/3}
\sum_{m\in\mathbb Z}\abs{\wt f(m)}\abs m^5.
\end{align*}
By Lemma \ref{lem:fourier-decay}, both sums are finite. Therefore
\[
\text{LowFreqError}\le C_1 d^{-1/3}.
\]

\medskip
\noindent\textbf{Step 3: high-frequency tail.}
For real $z$,
\[
\abs{\Lambda(z)}=\frac{1}{\abs{1-4iz-8z^2}^{1/2}}.
\]
A direct computation gives
\[
\abs{1-4iz-8z^2}^2=(1-8z^2)^2+16z^2=1+64z^4,
\]
so
\[
\abs{\Lambda(z)}=(1+64z^4)^{-1/4}\le 1.
\]
Thus
\[
\sum_{\abs m>N_d}
\abs{\wt f(m)}\abs{\Lambda(m\kappa d^{-1/3})}^d
\le
\sum_{\abs m>N_d}\abs{\wt f(m)}.
\]
Also
\[
\sum_{\abs m>N_d}\abs{\wt f(m)}\abs{e^{i\tau_\kappa m^3}}
=
\sum_{\abs m>N_d}\abs{\wt f(m)}.
\]
Hence
\[
\text{HighFreqError}
\le
\frac{4}{\pi}\sum_{\abs m>N_d}\abs{\wt f(m)}.
\]
By Lemma \ref{lem:fourier-decay},
\[
\sum_{\abs m>N_d}\abs{\wt f(m)}
\le C_\rho e^{-\rho N_d}
\le C_\rho d^{-A\rho}.
\]
Since $A\rho>1/3$, we get
\[
\text{HighFreqError}\le C_2 d^{-1/3}.
\]

\medskip
\noindent\textbf{Step 4: combine the bounds.}
For $d\ge d_0:=\max\{d_1,d_2\}$,
\[
\left|
\K_d\bigl(\kappa d^{-1/3},\beta\bigr)-\mathcal L_\infty(\kappa,\beta)
\right|
\le
\text{LowFreqError}+\text{HighFreqError}
\le
(C_1+C_2)d^{-1/3}.
\]
This proves \eqref{eq:main-estimate}. \qedhere
\end{proof}

\subsection{Explicit corollaries}

Because $f(\theta)=\arsinh(\cos\theta)$ is even and satisfies $f(\theta+\pi)=-f(\theta)$, its Fourier series contains only odd cosine modes:
\[
 f(\theta)=\sum_{\ell\ge 0} a_{2\ell+1}\cos\bigl((2\ell+1)\theta\bigr),
\]
where
\[
 a_{2\ell+1}:=\frac{1}{\pi}\int_0^{2\pi}f(\theta)\cos\bigl((2\ell+1)\theta\bigr)\,d\theta,
 \qquad \abs{a_{2\ell+1}}\le C_\rho e^{-\rho(2\ell+1)}.
\]
From Theorem \ref{thm:main} we immediately get the following explicit form of the limit.

\begin{corollary}[Cosine-series form]\label{cor:cosine}
For every fixed $\kappa,\beta\in\R$,
\[
\lim_{d\to\infty}\K_d\bigl(\kappa d^{-1/3},\beta\bigr)
=
\frac{2}{\pi}
\sum_{\ell\ge 0}
 a_{2\ell+1}
 \cos\left(
 2(2\ell+1)\beta + \frac{16}{3}(2\ell+1)^3\kappa^3
 \right).
\]
\end{corollary}

\begin{corollary}[Operator form]\label{cor:operator}
If we write $\U_\tau:=e^{-\tau\partial_\theta^3}$, then
\[
\lim_{d\to\infty}\K_d\bigl(\kappa d^{-1/3},\beta\bigr)
=
\frac{2}{\pi}(\U_{\tau_\kappa}f)(2\beta),
\qquad \tau_\kappa=\frac{16}{3}\kappa^3.
\]
In other words, the large-$d$ limit of the affine radial K\"onig functional is precisely the periodic Airy evolution of the fixed profile $f(\theta)=\arsinh(\cos\theta)$, evaluated at the angle $\theta=2\beta$.
\end{corollary}

\begin{corollary}[Variational form of the asymptotic affine value]\label{cor:variational}
Because $\tau_\kappa$ ranges over all real numbers as $\kappa$ ranges over $\R$, and because $e^{i\tau m^3}$ is $2\pi$-periodic in $\tau$ for every integer $m$, the asymptotic affine optimum is
\[
\Lambda_{\mathrm{aff}}
=
\sup_{\tau\in[0,2\pi],\ \theta\in[0,2\pi]}
\frac{2}{\pi}\bigl(e^{-\tau\partial_\theta^3}f\bigr)(\theta).
\]
Thus the asymptotic optimization problem for this affine radial family is reduced to a supremum over the two-torus $(\tau,\theta)\in[0,2\pi]^2$.
\end{corollary}

\subsection{What is proved here}

The theorem above gives a complete asymptotic description of the \emph{affine radial phase family}. Concretely, it proves four things.
\begin{itemize}[leftmargin=1.5em]
\item There is an exact finite-$d$ reduction to an explicit Fourier multiplier.
\item The correct scaling is $\alpha\sim d^{-1/3}$.
\item The limiting operator is the periodic Airy propagator.
\item The convergence holds uniformly on compact $\kappa$-intervals with error $O(d^{-1/3})$.
\end{itemize}
What it does \emph{not} prove is optimality outside this family: in particular, it does not address the full non-affine radial class, nor the full class of odd sign partitions. The result should therefore be read as a complete theorem for a specific higher-dimensional family, not as a universal extremal statement.




==> old/koenig_bilinear_form_reframed.tex <==
\section{An Asymptotic Family for K\"onig's Bilinear Form}
\label{sec:konig-not-sufficient}

\subsection{Affine radial partition family}

The tiger partitions discussed in the preceding section show that maximizing K\"onig's bilinear form is not necessarily the right objective for optimizing the Grothendieck constant itself.  The point of this section is different.  We now regard K\"onig's bilinear form as an extremal object in its own right, motivated by K\"onig's original problem on unconditional convergence \cite{Konig2001} and by its later role as a clean analytic/geometric model for the search surrounding Krivine's bound \cite{BravermanMakarychevMakarychevNaor2013}.  From this perspective, it is natural to ask how far one can push K\"onig's bilinear form beyond the hyperplane partition.

We present an explicit family of higher-dimensional partitions that gives a substantial improvement over the hyperplane benchmark for K\"onig's bilinear form.  The construction is still elementary: the sign cut is a half-space in a two-dimensional active plane, but its angle is allowed to depend affinely on a radial observable in an auxiliary $d$-dimensional Gaussian block.  This produces a tractable high-dimensional model in which the finite-$d$ functional diagonalizes in Fourier space and converges, after the natural $d^{-1/3}$ scaling, to a periodic Airy evolution on the circle.

The resulting asymptotic object is useful in two ways.  First, it gives a clean limiting variational problem for K\"onig's bilinear form, reducing the large-dimensional optimization to a two-torus.  Second, numerical optimization of this Airy limit, and of its finite-dimensional approximants, gives a value of K\"onig's bilinear form above the hyperplane benchmark
\[
 \frac{2}{\pi}\log(1+\sqrt2)\approx 0.56110.
\]
In the normalization used below our optimized affine radial phases exceed $0.572$, an absolute improvement of more than $10^{-2}$ over the hyperplane.  To the best of our knowledge, this is the first asymptotic construction of this kind for K\"onig's bilinear form.

\subsubsection{Motivation from the rotating-hyperplane calculation}

{
\color{blue}
REPLACE THIS ENTIRE SECTION WITH A SHORT PARAGRAPH ON WHAT KRIVINE DID (3D ANALYSIS) AND DID NOT (GENERALIZE AND FIND AN ASYMPTOTIC RESULT). 
}

We begin by recalling the analytic reduction behind the rotating-hyperplane construction that motivates the affine radial family. Throughout this section, $H_{f,g}$ denotes the same arcsine-normalized correlation function as above: for odd measurable partitions $f,g:\R^k\to\{-1,1\}$,
\[
 H_{f,g}(t)=\frac{\pi}{2}\,\E\bigl[f(X)g(Y)\bigr],
 \qquad |t|<1,
\]
where $(X,Y)$ is a pair of standard Gaussian vectors with coordinatewise correlation $t$. With this normalization the hyperplane partition has correlation $H(t)=\arcsin t$.

Let
\[
\ell^+_\varepsilon(x_0,x_1,x_2)
:=x_1\cos\bigl(\varepsilon H_2(x_0)\bigr)+x_2\sin\bigl(\varepsilon H_2(x_0)\bigr),
\]
\[
\ell^-_\varepsilon(y_0,y_1,y_2)
:=y_1\cos\bigl(\varepsilon H_2(y_0)\bigr)-y_2\sin\bigl(\varepsilon H_2(y_0)\bigr),
\]
with $H_2(s)=s^2-1$, and define the corresponding partitions
\[
 f_\varepsilon(x)=\operatorname{sign}\ell^+_\varepsilon(x),
 \qquad
 g_\varepsilon(y)=\operatorname{sign}\ell^-_\varepsilon(y).
\]
Geometrically, the cut is still an ordinary half-space in the active $(x_1,x_2)$-plane, but that half-space is rotated by an angle depending on the auxiliary coordinate $x_0$. The same construction is used on the $Y$ side, with the opposite sign in the sine term.

Conditioned on $x_0,y_0$, the active-plane pair $\ell^+_\varepsilon(X)$, $\ell^-_\varepsilon(Y)$ is a centered bivariate normal pair with correlation
\[
 t\Bigl(\cos\bigl(\varepsilon H_2(x_0)\bigr)\cos\bigl(\varepsilon H_2(y_0)\bigr)
 -\sin\bigl(\varepsilon H_2(x_0)\bigr)\sin\bigl(\varepsilon H_2(y_0)\bigr)\Bigr)
 =t\cos\bigl(\varepsilon(H_2(x_0)+H_2(y_0))\bigr).
\]
The standard arcsine identity therefore gives
\[
 H_{f_\varepsilon,g_\varepsilon}(t)
 =
 \E\Bigl[\arcsin\bigl(t\cos(\varepsilon(H_2(X_0)+H_2(Y_0)))\bigr)\Bigr].
\]
At the special point $t=i$, using $\arcsin(is)=i\,\arsinh(s)$ yields
\[
 \frac{H_{f_\varepsilon,g_\varepsilon}(i)}{i}
 =
 \E\Bigl[\arsinh\bigl(\cos(\varepsilon(H_2(X_0)+H_2(Y_0)))\bigr)\Bigr].
\]
This is the origin of the fixed circle profile
\[
 \mathfrak a(\theta):=\arsinh(\cos\theta),\qquad \theta\in\R,
\]
which we view as a $2\pi$-periodic analytic function on the circle $\T=\R/2\pi\mathbb Z$.

The phase in the last display is
\[
 \varepsilon\bigl(H_2(X_0)+H_2(Y_0)\bigr).
\]
It is the sum of the two rotation angles, one coming from the $X$ side and one from the $Y$ side. The reduced problem is obtained by evaluating the fixed circle profile $\mathfrak a$ at this phase.

For comparison with K\"onig's bilinear form, it is convenient to use the normalization
\[
 \mathcal B_{\mathrm K}(f,g):=\frac{2}{\pi}\,\frac{H_{f,g}(i)}{i}.
\]
Thus the hyperplane benchmark is
\[
 \mathcal B_{\mathrm K}(\mathrm{hp},\mathrm{hp})
 =\frac{2}{\pi}\arsinh(1)
 =\frac{2}{\pi}\log(1+\sqrt2).
\]
The rotating-hyperplane computation rewrites $\mathcal B_{\mathrm K}(f_\varepsilon,g_\varepsilon)$ as an explicit oscillatory integral. After the analytic-continuation calculation at $t=i$, one uses the rescaled auxiliary coordinates
\[
 X_0=2u,
 \qquad
 Y_0=2v.
\]
With this convention, $H_2(X_0)=4u^2-1$ and $H_2(Y_0)=4v^2-1$, and the Gaussian kernel becomes the real oscillatory kernel $e^{-(u^2+v^2)}\cos(2uv)$. Hence
\[
 \mathcal B_{\mathrm K}(f_\varepsilon,g_\varepsilon)
 =
 \frac{2^{3/2}}{\pi^2}
 \int_{\R}\int_{\R}
 e^{-(u^2+v^2)}\cos(2uv)
 \mathfrak a\bigl(\varepsilon((4u^2-1)+(4v^2-1))\bigr)
 \,du\,dv.
\]
Passing to polar coordinates $u=r\cos\ph$, $v=r\sin\ph$ gives
\[
 2uv=r^2\sin(2\ph),
 \qquad
 (4u^2-1)+(4v^2-1)=4r^2-2,
 \qquad
 du\,dv=r\,dr\,d\ph.
\]
Writing $\rho=r^2$ and $\vartheta=2\ph$, we obtain
\begin{align*}
 \mathcal B_{\mathrm K}(f_\varepsilon,g_\varepsilon)
 &=
 \frac{2^{3/2}}{\pi^2}
 \int_0^\infty\int_0^{2\pi}
 e^{-r^2}\cos(r^2\sin(2\ph))
 \mathfrak a\bigl(\varepsilon(4r^2-2)\bigr)
 r\,d\ph\,dr \\
 &=
 \frac{2\sqrt2}{\pi^2}
 \int_0^\infty\int_0^\pi
 e^{-\rho}\cos(\rho\sin\vartheta)
 \mathfrak a\bigl(2\varepsilon(2\rho-1)\bigr)
 \,d\vartheta\,d\rho.
\end{align*}
This is the oscillatory integral that motivates the affine radial generalization below; the parameter usually denoted $\eta$ in the one-dimensional calculation is $2\varepsilon$ in this normalization.

\subsubsection{The higher-dimensional affine radial family}

The preceding computation suggests the following high-dimensional generalization. We keep the active two-dimensional plane in which the sign cut lives, and we allow an auxiliary $d$-dimensional Gaussian block to determine the rotation angle.

\begin{definition}[Local angle and phase]
Fix $d\in\mathbb N$ and parameters $\alpha,\beta\in\R$. Define
\[
 Q_d(u):=4\norm{u}_2^2-d,
 \qquad u\in\R^d,
\]
\[
 \psi_{d,\alpha,\beta}(u):=\beta+\alpha Q_d(u),
\]
and the associated pairwise phase function
\[
 \phi_{d,\alpha,\beta}(u,v)
 :=\psi_{d,\alpha,\beta}(u)+\psi_{d,\alpha,\beta}(v)
 =2\beta+\alpha\bigl(Q_d(u)+Q_d(v)\bigr).
\]
\end{definition}

Here $\theta$ always denotes the circle variable in the periodic profile $\mathfrak a(\theta)=\arsinh(\cos\theta)$, while $\phi_{d,\alpha,\beta}(u,v)$ is the phase inserted into that circle variable. The parameter $\beta$ is a constant rotation on each side, so it contributes the total shift $2\beta$. The parameter $\alpha$ controls the dependence of the rotation on the auxiliary variables. The name ``affine radial'' refers to the fact that the angle depends affinely on the radial observable $Q_d(u)$.

The rescaling in the definition of $Q_d$ is exactly the rescaling used in the one-dimensional computation above. In the $t=i$ K\"onig's Gaussian--oscillatory kernel the auxiliary coordinates are written as $X_j=2u_j$ and $Y_j=2v_j$. Thus each copy of the quadratic observable $H_2(X_j)=X_j^2-1$ becomes $(2u_j)^2-1=4u_j^2-1$, and summing over the $d$ auxiliary coordinates gives
\[
 Q_d(u)=\sum_{j=1}^d\bigl((2u_j)^2-1\bigr)=4\norm{u}_2^2-d.
\]

The corresponding rotated half-space partitions on $\R^{d+2}=\R^d\times\R^2$ are
\[
 f_{d,\alpha,\beta}(u;x_1,x_2)
 :=
 \operatorname{sign}\bigl(x_1\cos\psi_{d,\alpha,\beta}(u)+x_2\sin\psi_{d,\alpha,\beta}(u)\bigr),
\]
\[
 g_{d,\alpha,\beta}(v;y_1,y_2)
 :=
 \operatorname{sign}\bigl(y_1\cos\psi_{d,\alpha,\beta}(v)-y_2\sin\psi_{d,\alpha,\beta}(v)\bigr).
\]
Conditioned on $u,v$, the active-plane correlation is $t\cos\phi_{d,\alpha,\beta}(u,v)$, exactly as in the one-dimensional rotating-hyperplane construction. Evaluating at $t=i$ and integrating out the active plane leaves the following reduced expression for K\"onig's bilinear form.

\begin{definition}[Reduced affine radial K\"onig's bilinear form]
Let
\[
 c_d:=\frac{2^{1+d/2}}{\pi^{d+1}}.
\]
Define
\begin{equation}\label{eq:Kd-def}
 \K_d(\alpha,\beta)
 :=
 \mathcal B_{\mathrm K}(f_{d,\alpha,\beta},g_{d,\alpha,\beta})
 =
 c_d
 \int_{\R^d}\int_{\R^d}
 e^{-(\norm{u}_2^2+\norm{v}_2^2)}
 \cos\bigl(2\ip{u}{v}\bigr)
 \mathfrak a\bigl(\phi_{d,\alpha,\beta}(u,v)\bigr)
 \,du\,dv.
\end{equation}
\end{definition}

Thus the entire dependence on the partition pair is encoded by the phase function $\phi_{d,\alpha,\beta}$. When $\alpha=\beta=0$ there is no rotation, and one recovers the hyperplane benchmark
\[
 \K_d(0,0)=\frac{2}{\pi}\mathfrak a(0)
 =\frac{2}{\pi}\arsinh(1)
 =\frac{2}{\pi}\log(1+\sqrt2).
\]
The exact Fourier reduction below gives the same value directly.

\subsubsection{Main theorem and the Airy operator}

The asymptotic object is the periodic Airy flow on the circle.

\begin{definition}[Periodic Airy propagator]
Let $q(\theta)=\sum_{m\in\mathbb Z}\widehat q(m)e^{im\theta}$ be a $2\pi$-periodic analytic function, with Fourier coefficients
\[
 \widehat q(m):=\frac{1}{2\pi}\int_0^{2\pi} q(\theta)e^{-im\theta}\,d\theta.
\]
For $\tau\in\R$ define
\[
 \bigl(e^{-\tau\partial_\theta^3}q\bigr)(\theta)
 :=
 \sum_{m\in\mathbb Z}e^{i\tau m^3}\widehat q(m)e^{im\theta}.
\]
Equivalently, $u(\tau,\theta):=(e^{-\tau\partial_\theta^3}q)(\theta)$ is the solution of the periodic Airy equation
\[
 \partial_\tau u+\partial_\theta^3 u=0,
 \qquad
 u(0,\theta)=q(\theta).
\]
Indeed, on the Fourier mode $e^{im\theta}$ one has $-\partial_\theta^3 e^{im\theta}=im^3e^{im\theta}$.
\end{definition}

We can now state the theorem.

\begin{theorem}[Airy limit for the affine radial phase family]\label{thm:main}
Let
\[
 \mathfrak a(\theta)=\arsinh(\cos\theta),
 \qquad \theta\in\T.
\]
Fix $0<\rho<\rho_*$, where $\rho_*:=\arsinh(1)=\log(1+\sqrt2)$, and fix $\kappa_0>0$. Then there exist constants $C=C(\rho,\kappa_0)$ and $d_0=d_0(\rho,\kappa_0)$ such that for all $d\ge d_0$, all $|\kappa|\le\kappa_0$, and all $\beta\in\R$,
\begin{equation}\label{eq:main-estimate}
\left|
 \K_d\bigl(\kappa d^{-1/3},\beta\bigr)
 -
 \frac{2}{\pi}\bigl(e^{-\tau_\kappa\partial_\theta^3}\mathfrak a\bigr)(2\beta)
\right|
\le C d^{-1/3},
\end{equation}
where
\[
 \tau_\kappa:=\frac{16}{3}\kappa^3.
\]
Equivalently,
\[
 \K_d\bigl(\kappa d^{-1/3},\beta\bigr)
 \longrightarrow
 \frac{2}{\pi}\bigl(e^{-\tau_\kappa\partial_\theta^3}\mathfrak a\bigr)(2\beta)
\]
uniformly for $(\kappa,\beta)\in[-\kappa_0,\kappa_0]\times\R$.
\end{theorem}

\begin{remark}[Why the scaling is $d^{-1/3}$]
The proof diagonalizes $\K_d$ in the Fourier basis and produces a scalar multiplier $\Lambda(m\alpha)^d$ on the $m$th Fourier mode. The key expansion is
\[
 \log\Lambda(z)=\frac{16i}{3}z^3-16z^4+O(z^5).
\]
The first nontrivial oscillatory term is cubic. Therefore the only scaling for which $d\log\Lambda(m\alpha)$ remains nondegenerate is $d\alpha^3\asymp 1$, i.e.
\[
 \alpha\asymp d^{-1/3}.
\]
The cubic phase produces the Airy multiplier $e^{i\tau m^3}$, while the quartic term yields the $O(d^{-1/3})$ error.
\end{remark}

{color{blue}
RAHUL - REMOVE THIS. POSSIBLY REPLACE WITH A BETTER PARAGRAPH BUT THIS IS NOT VERY HELPFUL

\begin{remark}[Proof strategy]
Expand $\mathfrak a$ into its Fourier series on the circle. Each Fourier mode can be integrated exactly through a $2\times2$ Gaussian computation, and the entire functional becomes a diagonal Fourier multiplier. One then expands this multiplier near the origin, chooses the $d^{-1/3}$ scaling dictated by the cubic term, and splits the Fourier modes into low frequencies $|m|\le A\log d$ and a rapidly decaying analytic tail. This turns the heuristic Airy limit into the uniform estimate \eqref{eq:main-estimate}.
\end{remark}
}

\subsubsection{Exact finite-$d$ Fourier reduction}

The finite-dimensional problem is already completely explicit.

\begin{theorem}[Exact reduction]\label{prop:exact}
Define
\[
 \Lambda(z):=\frac{e^{-2iz}}{\sqrt{1-4iz-8z^2}},
 \qquad z\in\R,
\]
with the principal branch of the square root. Then
\begin{equation}\label{eq:exact-reduction}
 \K_d(\alpha,\beta)
 =
 \frac{2}{\pi}
 \sum_{m\in\mathbb Z}
 \widehat{\mathfrak a}(m)e^{2im\beta}\Lambda(m\alpha)^d.
\end{equation}
\end{theorem}

\begin{proof}
Because $\mathfrak a$ is real analytic on a strip around the real axis, its Fourier series converges absolutely:
\[
 \mathfrak a(\theta)=\sum_{m\in\mathbb Z}\widehat{\mathfrak a}(m)e^{im\theta}.
\]
Substituting this into \eqref{eq:Kd-def} and interchanging the sum and the integral yields
\[
 \K_d(\alpha,\beta)
 =
 c_d
 \sum_{m\in\mathbb Z}\widehat{\mathfrak a}(m)e^{2im\beta}
 I_{m,d}(\alpha),
\]
where
\[
 I_{m,d}(\alpha)
 :=
 \int_{\R^d}\int_{\R^d}
 e^{-(\norm{u}^2+\norm{v}^2)}
 \cos\bigl(2\ip{u}{v}\bigr)
 e^{im\alpha(Q_d(u)+Q_d(v))}
 \,du\,dv.
\]
Since $Q_d(v)$ is even in $v$, the change of variables $v\mapsto -v$ shows that the two exponentials arising from
\[
 \cos\bigl(2\ip{u}{v}\bigr)=\frac{e^{2i\ip{u}{v}}+e^{-2i\ip{u}{v}}}{2}
\]
contribute equally. Hence
\[
 I_{m,d}(\alpha)
 =
 \int_{\R^d}\int_{\R^d}
 e^{-(\norm{u}^2+\norm{v}^2)}
 e^{2i\ip{u}{v}}
 e^{im\alpha(Q_d(u)+Q_d(v))}
 \,du\,dv.
\]
Now the integrand factorizes coordinate by coordinate, so
\[
 I_{m,d}(\alpha)
 =
 \prod_{j=1}^d
 \int_{\R^2}
 e^{-(x^2+y^2)}
 e^{im\alpha((4x^2-1)+(4y^2-1))}
 e^{2ixy}
 \,dx\,dy.
\]
The one-coordinate Gaussian integral is
\[
 \int_{\R^2}
 e^{-(1-4im\alpha)x^2-(1-4im\alpha)y^2+2ixy}
 \,dx\,dy
 =
 \frac{\pi}{\sqrt{(1-4im\alpha)^2+1}}.
\]
After including the factor $e^{-2im\alpha}$ coming from the two constant terms in $(4x^2-1)+(4y^2-1)$, the one-coordinate contribution is
\[
 \frac{\pi e^{-2im\alpha}}{\sqrt{(1-4im\alpha)^2+1}}
 =
 \frac{\pi}{\sqrt2}\,\Lambda(m\alpha).
\]
Therefore
\[
 I_{m,d}(\alpha)=\left(\frac{\pi}{\sqrt2}\right)^d\Lambda(m\alpha)^d.
\]
Since
\[
 c_d\left(\frac{\pi}{\sqrt2}\right)^d=\frac{2}{\pi},
\]
we obtain \eqref{eq:exact-reduction}. \qedhere
\end{proof}

\subsubsection{Two preparatory lemmas}

\begin{lemma}[Fourier coefficient decay]\label{lem:fourier-decay}
Let
\[
 \rho_*:=\arsinh(1)=\log(1+\sqrt2).
\]
Then for every $0<\rho<\rho_*$ there exists $C_\rho<\infty$ such that
\[
 \abs{\widehat{\mathfrak a}(m)}\le C_\rho e^{-\rho\abs m}
 \qquad (m\in\mathbb Z).
\]
In particular,
\[
 \sum_{m\in\mathbb Z}\abs{\widehat{\mathfrak a}(m)}\abs m^k<\infty
 \qquad\text{for every }k\ge 0.
\]
\end{lemma}

\begin{proof}
The singularities of $\arsinh(z)$ are at $z=\pm i$, so the singularities of
\[
 \mathfrak a(z)=\arsinh(\cos z)
\]
occur where $\cos z=\pm i$. The nearest such points to the real axis lie at imaginary distance $\rho_*$. Hence $\mathfrak a$ extends holomorphically to every strip
\[
 \abs{\Im z}<\rho
 \qquad (0<\rho<\rho_*).
\]
The standard Cauchy estimate for Fourier coefficients on analytic strips gives
\[
 \abs{\widehat{\mathfrak a}(m)}\le C_\rho e^{-\rho\abs m}.
\]
The summability of polynomially weighted coefficients follows immediately. \qedhere
\end{proof}

\begin{lemma}[Local expansion of the multiplier]\label{lem:lambda-expansion}
For $\abs z\le 1/16$,
\[
 \log\Lambda(z)=\frac{16i}{3}z^3-16z^4+r(z),
\]
with the explicit bound
\[
 \abs{r(z)}\le 500\abs{z}^5.
\]
\end{lemma}

\begin{proof}
Write
\[
 \Lambda(z)=e^{-2iz}(1+w(z))^{-1/2},
 \qquad
 w(z):=-4iz-8z^2.
\]
If $\abs z\le 1/16$, then
\[
 \abs{w(z)}\le 4\abs z+8\abs z^2\le \frac14+\frac1{32}=\frac9{32}<1.
\]
Hence the principal logarithm is analytic there and
\[
 \log\Lambda(z)=-2iz-\frac12\log(1+w(z)).
\]
Use the fourth-order logarithm expansion
\[
 \log(1+w)=w-\frac{w^2}{2}+\frac{w^3}{3}-\frac{w^4}{4}+R_5(w),
 \qquad
 \abs{R_5(w)}\le \frac{\abs w^5}{5(1-\abs w)}.
\]
A direct algebraic expansion gives
\[
 -2iz-\frac12\left(w-\frac{w^2}{2}+\frac{w^3}{3}-\frac{w^4}{4}\right)
 =
 \frac{16i}{3}z^3-16z^4-128iz^5-\frac{2048}{3}z^6+1024iz^7+512z^8.
\]
Thus for $\abs z\le 1/16$,
\[
 \left|-128iz^5-\frac{2048}{3}z^6+1024iz^7+512z^8\right|
 \le 175\abs z^5.
\]
On the other hand, since $\abs{w(z)}\le \frac92\abs z$,
\[
 \frac12\abs{R_5(w)}
 \le
 \frac12\cdot\frac{\abs w^5}{5(1-\abs w)}
 \le 261\abs z^5.
\]
Combining the two bounds yields
\[
 \abs{r(z)}\le (175+261)\abs z^5\le 500\abs z^5.
\]
\qedhere
\end{proof}

\subsubsection{Proof of the Airy limit}

\begin{proof}[Proof of Theorem~\ref{thm:main}]
Start from Theorem~\ref{prop:exact}:
\[
 \K_d\bigl(\kappa d^{-1/3},\beta\bigr)
 =
 \frac{2}{\pi}
 \sum_{m\in\mathbb Z}
 \widehat{\mathfrak a}(m)e^{2im\beta}
 \Lambda\bigl(m\kappa d^{-1/3}\bigr)^d.
\]
Define the target series
\[
 \mathcal L_\infty(\kappa,\beta)
 :=
 \frac{2}{\pi}
 \sum_{m\in\mathbb Z}
 \widehat{\mathfrak a}(m)e^{2im\beta}e^{i\tau_\kappa m^3}
 =
 \frac{2}{\pi}\bigl(e^{-\tau_\kappa\partial_\theta^3}\mathfrak a\bigr)(2\beta),
\]
where $\tau_\kappa=\frac{16}{3}\kappa^3$. We must bound
\[
 \K_d\bigl(\kappa d^{-1/3},\beta\bigr)-\mathcal L_\infty(\kappa,\beta).
\]
We split the Fourier modes into low and high frequencies.

\medskip
\noindent\textbf{Step 1: choose the cutoff.}
Pick
\[
 A>\frac{1}{3\rho},
 \qquad
 N_d:=\lfloor A\log d\rfloor.
\]
Since $N_d d^{-1/3}\to 0$, there exists $d_1=d_1(\kappa_0)$ such that for all $d\ge d_1$, all $\abs m\le N_d$, and all $\abs\kappa\le\kappa_0$,
\[
 \abs{m\kappa d^{-1/3}}\le \frac1{16}.
\]

\medskip
\noindent\textbf{Step 2: low-frequency expansion.}
For $\abs m\le N_d$, set
\[
 z:=m\kappa d^{-1/3}.
\]
By Lemma~\ref{lem:lambda-expansion},
\[
 \log\Lambda(z)=\frac{16i}{3}z^3-16z^4+r(z),
 \qquad
 \abs{r(z)}\le 500\abs{z}^5.
\]
Multiplying by $d$ gives
\[
 d\log\Lambda(z)
 =i\tau_\kappa m^3-16\kappa^4m^4d^{-1/3}+\varepsilon_{m,d},
\]
where
\[
 \abs{\varepsilon_{m,d}}
 \le 500\abs{\kappa}^5\abs m^5d^{-2/3}
 \le 500\kappa_0^5\abs m^5d^{-2/3}.
\]
Define
\[
 \delta_{m,d}:=-16\kappa^4m^4d^{-1/3}+\varepsilon_{m,d}.
\]
Then
\[
 \Lambda\bigl(m\kappa d^{-1/3}\bigr)^d
 =e^{i\tau_\kappa m^3}e^{\delta_{m,d}}.
\]
Since $\abs m\le A\log d$,
\[
 \abs{\delta_{m,d}}
 \le
 16\kappa_0^4A^4(\log d)^4d^{-1/3}
 +
 500\kappa_0^5A^5(\log d)^5d^{-2/3}.
\]
The right-hand side tends to $0$, so there exists $d_2=d_2(\rho,\kappa_0)$ such that for all $d\ge d_2$,
\[
 \abs{\delta_{m,d}}\le 1
 \qquad (\abs m\le N_d,\ \abs\kappa\le\kappa_0).
\]
Therefore
\[
 \abs{e^{\delta_{m,d}}-1}\le 2\abs{\delta_{m,d}}.
\]
So
\[
 \left|
 \Lambda\bigl(m\kappa d^{-1/3}\bigr)^d-e^{i\tau_\kappa m^3}
 \right|
 \le
 32\kappa_0^4\abs m^4d^{-1/3}
 +
 1000\kappa_0^5\abs m^5d^{-2/3}.
\]
Hence the low-frequency contribution is bounded by
\begin{align*}
\frac{2}{\pi}
\sum_{\abs m\le N_d}
\abs{\widehat{\mathfrak a}(m)}
\left|
 \Lambda\bigl(m\kappa d^{-1/3}\bigr)^d-e^{i\tau_\kappa m^3}
\right|
&\le
\frac{64\kappa_0^4}{\pi}d^{-1/3}
\sum_{m\in\mathbb Z}\abs{\widehat{\mathfrak a}(m)}\abs m^4 \\
&\qquad+
\frac{2000\kappa_0^5}{\pi}d^{-2/3}
\sum_{m\in\mathbb Z}\abs{\widehat{\mathfrak a}(m)}\abs m^5.
\end{align*}
By Lemma~\ref{lem:fourier-decay}, both sums are finite. Therefore
\[
 \mathrm{LowFreqError}\le C_1d^{-1/3}.
\]

\medskip
\noindent\textbf{Step 3: high-frequency tail.}
For real $z$,
\[
 \abs{\Lambda(z)}=\frac{1}{\abs{1-4iz-8z^2}^{1/2}}.
\]
A direct computation gives
\[
 \abs{1-4iz-8z^2}^2=(1-8z^2)^2+16z^2=1+64z^4,
\]
so
\[
 \abs{\Lambda(z)}=(1+64z^4)^{-1/4}\le 1.
\]
Thus
\[
 \sum_{\abs m>N_d}
 \abs{\widehat{\mathfrak a}(m)}\abs{\Lambda(m\kappa d^{-1/3})}^d
 \le
 \sum_{\abs m>N_d}\abs{\widehat{\mathfrak a}(m)}.
\]
Also
\[
 \sum_{\abs m>N_d}\abs{\widehat{\mathfrak a}(m)}\abs{e^{i\tau_\kappa m^3}}
 =
 \sum_{\abs m>N_d}\abs{\widehat{\mathfrak a}(m)}.
\]
Hence
\[
 \mathrm{HighFreqError}
 \le
 \frac{4}{\pi}\sum_{\abs m>N_d}\abs{\widehat{\mathfrak a}(m)}.
\]
By Lemma~\ref{lem:fourier-decay},
\[
 \sum_{\abs m>N_d}\abs{\widehat{\mathfrak a}(m)}
 \le C_\rho e^{-\rho N_d}
 \le C_\rho d^{-A\rho}.
\]
Since $A\rho>1/3$,
\[
 \mathrm{HighFreqError}\le C_2d^{-1/3}.
\]

\medskip
\noindent\textbf{Step 4: combine the bounds.}
For $d\ge d_0:=\max\{d_1,d_2\}$,
\[
 \left|
 \K_d\bigl(\kappa d^{-1/3},\beta\bigr)-\mathcal L_\infty(\kappa,\beta)
 \right|
 \le
 \mathrm{LowFreqError}+\mathrm{HighFreqError}
 \le
 (C_1+C_2)d^{-1/3}.
\]
This proves \eqref{eq:main-estimate}. \qedhere
\end{proof}

\subsubsection{Explicit corollaries}

Because $\mathfrak a(\theta)=\arsinh(\cos\theta)$ is even and satisfies $\mathfrak a(\theta+\pi)=-\mathfrak a(\theta)$, its Fourier series contains only odd cosine modes:
\[
 \mathfrak a(\theta)=\sum_{\ell\ge0} b_{2\ell+1}\cos\bigl((2\ell+1)\theta\bigr),
\]
where
\[
 b_{2\ell+1}:=\frac{1}{\pi}\int_0^{2\pi}\mathfrak a(\theta)\cos\bigl((2\ell+1)\theta\bigr)\,d\theta,
 \qquad
 \abs{b_{2\ell+1}}\le C_\rho e^{-\rho(2\ell+1)}.
\]
From Theorem~\ref{thm:main} we immediately get the following explicit form of the limit.

\begin{corollary}[Cosine-series form]\label{cor:cosine}
For every fixed $\kappa,\beta\in\R$,
\[
 \lim_{d\to\infty}\K_d\bigl(\kappa d^{-1/3},\beta\bigr)
 =
 \frac{2}{\pi}
 \sum_{\ell\ge0}
 b_{2\ell+1}
 \cos\left(
 2(2\ell+1)\beta+\frac{16}{3}(2\ell+1)^3\kappa^3
 \right).
\]
\end{corollary}

\begin{corollary}[Operator form]\label{cor:operator}
If we write $\U_\tau:=e^{-\tau\partial_\theta^3}$, then
\[
 \lim_{d\to\infty}\K_d\bigl(\kappa d^{-1/3},\beta\bigr)
 =
 \frac{2}{\pi}(\U_{\tau_\kappa}\mathfrak a)(2\beta),
 \qquad
 \tau_\kappa=\frac{16}{3}\kappa^3.
\]
In other words, the large-$d$ limit for the affine radial family in K\"onig's bilinear form is precisely the periodic Airy evolution of the fixed profile $\mathfrak a(\theta)=\arsinh(\cos\theta)$, evaluated at the angle $\theta=2\beta$.
\end{corollary}

\begin{corollary}[Variational form of the asymptotic affine optimum]\label{cor:variational}
Because $\tau_\kappa$ ranges over all real numbers as $\kappa$ ranges over $\R$, and because $e^{i\tau m^3}$ is $2\pi$-periodic in $\tau$ for every integer $m$, the asymptotic affine optimum is
\[
 \Lambda_{\mathrm{aff}}
 =
 \sup_{\tau\in[0,2\pi],\ \theta\in[0,2\pi]}
 \frac{2}{\pi}\bigl(e^{-\tau\partial_\theta^3}\mathfrak a\bigr)(\theta).
\]
Thus the asymptotic optimization problem for this affine radial family reduces to a supremum over the two-torus $(\tau,\theta)\in[0,2\pi]^2$.
\end{corollary}



The variational form also gives a practical numerical procedure for this family.  For each auxiliary dimension $d$, one can choose a phase and evaluate the resulting normalized K\"onig's bilinear form $\K_d(\alpha,\beta)$ using the exact finite Fourier reduction.  Figure~\ref{fig:koenig-dimension} shows the outcome of our numerical optimization as a function of $d$.

\begin{figure}[t]
\centering
\includegraphics[width=0.82\textwidth]{images/affine_radial_BK_vs_dimension.png}
\caption{Normalized K\"onig's bilinear form $\K_d$ for affine radial rotating-hyperplane partitions as a function of the auxiliary dimension $d$. The dashed horizontal line is the hyperplane benchmark $2\rho_*/\pi=2\log(1+\sqrt2)/\pi\approx0.56110$. The optimized affine radial phases give a much larger value of K\"onig's bilinear form than this benchmark.}
\label{fig:koenig-dimension}
\end{figure}

The improvement is large on the scale relevant to this problem.  The hyperplane gives
\[
 \mathcal B_{\mathrm K}(\mathrm{hp},\mathrm{hp})
 =\frac{2\rho_*}{\pi}
 \approx 0.56110.
\]
By contrast, the optimized affine radial phases in the displayed range exceed $0.572$.  The Airy limit identifies the mechanism behind this improvement: the radial phase creates a cubic Fourier multiplier, so the large-dimensional behavior is governed by the periodic Airy flow rather than by a finite-dimensional perturbation of the hyperplane.  Thus the family gives an explicit asymptotic source of non-hyperplane improvements for K\"onig's bilinear form.


% Suggested bibliography keys used above:
% Konig2001 = H. K\"onig, ``On an extremal problem originating in questions of unconditional convergence,'' in Recent Progress in Multivariate Approximation, ISNM 137, Birkh\"auser, 2001, pp. 185--192.
% BravermanMakarychevMakarychevNaor2013 = M. Braverman, K. Makarychev, Y. Makarychev, and A. Naor, ``The Grothendieck constant is strictly smaller than Krivine's bound,'' Forum Math. Pi 1 (2013), e4.


==> old/koenig_v1.tex <==
\section{An Asymptotic Family for K\"onig's Bilinear Form}
\label{sec:konig-not-sufficient}


\subsection{Affine radial partition family}

We study K\"onig's bilinear form as an extremal object in its own right, following K\"onig's formulation \cite{Konig2001} and its later role as a clean model for the search around Krivine's bound \cite{BravermanMakarychevMakarychevNaor2013}.  Our goal is narrow: construct an explicit high-dimensional family of partitions whose normalized K\"onig value beats the hyperplane benchmark
\[
 \frac{2}{\pi}\log(1+\sqrt2)\approx 0.56110.
\]
The family keeps a two-dimensional active half-space, but rotates it by an affine function of the squared radius in an auxiliary $d$-dimensional Gaussian block.  With the scaling $\alpha=\kappa d^{-1/3}$, the finite-dimensional functional diagonalizes in Fourier space and converges to a periodic Airy multiplier.  Numerically, the optimized affine radial phases exceed $0.572$ in this normalization.

Krivine's suggestion in dimension three can be read as a finite-dimensional version of this rotating-half-space idea \cite{Krivine1977-1978}.  He considers a cut in $\R^3$ with two active coordinates and one auxiliary Gaussian coordinate controlling the rotation angle, and he computes the quantity that later appears as the corresponding K\"onig value.  What is absent from Krivine's calculation is a general higher-dimensional family and an asymptotic analysis as the auxiliary dimension tends to infinity.  Here we keep the same mechanism but replace the single auxiliary coordinate by a radial observable in $\R^d$.

\subsubsection{The higher-dimensional affine radial family}

For odd measurable partitions $f,g:\R^k\to\{-1,1\}$, write
\[
 H_{f,g}(t):=\frac{\pi}{2}\,\E[f(X)g(Y)],
 \qquad |t|<1,
\]
where $X,Y$ are standard Gaussian vectors with coordinatewise correlation $t$.  We use the normalized K\"onig value
\[
 \mathcal B_{\mathrm K}(f,g):=\frac{2}{\pi}\,\frac{H_{f,g}(i)}{i},
\]
where $H_{f,g}$ is analytically continued to $t=i$.  The active two-dimensional calculation leaves the fixed circle profile
\[
 \mathfrak a(\theta):=\arsinh(\cos\theta),
 \qquad \theta\in\T.
\]
Thus the hyperplane partition has normalized value
\[
 \mathcal B_{\mathrm K}(\mathrm{hp},\mathrm{hp})
 =\frac{2}{\pi}\mathfrak a(0)
 =\frac{2}{\pi}\log(1+\sqrt2).
\]

We now define the affine radial family.  Fix $d\in\mathbb N$ and parameters $\alpha,\beta\in\R$.  Let
\[
 Q_d(u):=4\norm{u}_2^2-d,
 \qquad u\in\R^d,
\]
\[
 \psi_{d,\alpha,\beta}(u):=\beta+\alpha Q_d(u),
\]
and
\[
 \phi_{d,\alpha,\beta}(u,v)
 :=\psi_{d,\alpha,\beta}(u)+\psi_{d,\alpha,\beta}(v)
 =2\beta+\alpha\bigl(Q_d(u)+Q_d(v)\bigr).
\]
Here $\beta$ is a constant rotation on each side, while $\alpha$ controls the radial dependence.  The factor $4$ in $Q_d$ is the one produced by the $t=i$ Gaussian--oscillatory kernel: writing auxiliary coordinates as $X_j=2u_j$ turns $H_2(X_j)=X_j^2-1$ into $4u_j^2-1$.

Define rotated half-space partitions on $\R^{d+2}=\R^d\times\R^2$ by
\[
 f_{d,\alpha,\beta}(u;x_1,x_2)
 :=
 \operatorname{sign}\bigl(x_1\cos\psi_{d,\alpha,\beta}(u)+x_2\sin\psi_{d,\alpha,\beta}(u)\bigr),
\]
\[
 g_{d,\alpha,\beta}(v;y_1,y_2)
 :=
 \operatorname{sign}\bigl(y_1\cos\psi_{d,\alpha,\beta}(v)-y_2\sin\psi_{d,\alpha,\beta}(v)\bigr).
\]
Conditioned on $u,v$, the active-plane correlation is $t\cos\phi_{d,\alpha,\beta}(u,v)$.  Evaluating at $t=i$ and integrating out the active plane gives the following reduced form.

\begin{definition}[Reduced affine radial K\"onig bilinear form]
Let
\[
 c_d:=\frac{2^{1+d/2}}{\pi^{d+1}}.
\]
Define
\begin{equation}\label{eq:Kd-def}
\begin{aligned}
 \K_d(\alpha,\beta)
 &:=
 \mathcal B_{\mathrm K}(f_{d,\alpha,\beta},g_{d,\alpha,\beta}) \\
 &=
 c_d
 \int_{\R^d}\int_{\R^d}
 e^{-(\norm{u}_2^2+\norm{v}_2^2)}
 \cos\bigl(2\ip{u}{v}\bigr)
 \mathfrak a\bigl(\phi_{d,\alpha,\beta}(u,v)\bigr)
 \,du\,dv.
\end{aligned}
\end{equation}
\end{definition}

When $\alpha=\beta=0$ there is no rotation, and one recovers the hyperplane benchmark
\[
 \K_d(0,0)=\frac{2}{\pi}\log(1+\sqrt2).
\]

\subsubsection{Main theorem and the Airy operator}

The asymptotic object is the periodic Airy flow on the circle.

\begin{definition}[Periodic Airy propagator]
Let $q(\theta)=\sum_{m\in\mathbb Z}\widehat q(m)e^{im\theta}$ be a $2\pi$-periodic analytic function, with Fourier coefficients
\[
 \widehat q(m):=\frac{1}{2\pi}\int_0^{2\pi} q(\theta)e^{-im\theta}\,d\theta.
\]
For $\tau\in\R$ define
\[
 \bigl(e^{-\tau\partial_\theta^3}q\bigr)(\theta)
 :=
 \sum_{m\in\mathbb Z}e^{i\tau m^3}\widehat q(m)e^{im\theta}.
\]
Equivalently, $u(\tau,\theta):=(e^{-\tau\partial_\theta^3}q)(\theta)$ is the solution of the periodic Airy equation
\[
 \partial_\tau u+\partial_\theta^3 u=0,
 \qquad
 u(0,\theta)=q(\theta).
\]
Indeed, on the Fourier mode $e^{im\theta}$ one has $-\partial_\theta^3 e^{im\theta}=im^3e^{im\theta}$.
\end{definition}

We can now state the theorem.

\begin{theorem}[Airy limit for the affine radial phase family]\label{thm:main}
Let
\[
 \mathfrak a(\theta)=\arsinh(\cos\theta),
 \qquad \theta\in\T.
\]
Fix $0<\rho<\rho_*$, where $\rho_*:=\arsinh(1)=\log(1+\sqrt2)$, and fix $\kappa_0>0$. Then there exist constants $C=C(\rho,\kappa_0)$ and $d_0=d_0(\rho,\kappa_0)$ such that for all $d\ge d_0$, all $|\kappa|\le\kappa_0$, and all $\beta\in\R$,
\begin{equation}\label{eq:main-estimate}
\left|
 \K_d\bigl(\kappa d^{-1/3},\beta\bigr)
 -
 \frac{2}{\pi}\bigl(e^{-\tau_\kappa\partial_\theta^3}\mathfrak a\bigr)(2\beta)
\right|
\le C d^{-1/3},
\end{equation}
where
\[
 \tau_\kappa:=\frac{16}{3}\kappa^3.
\]
Equivalently,
\[
 \K_d\bigl(\kappa d^{-1/3},\beta\bigr)
 \longrightarrow
 \frac{2}{\pi}\bigl(e^{-\tau_\kappa\partial_\theta^3}\mathfrak a\bigr)(2\beta)
\]
uniformly for $(\kappa,\beta)\in[-\kappa_0,\kappa_0]\times\R$.
\end{theorem}

\begin{remark}[Why the scaling is $d^{-1/3}$]
The proof diagonalizes $\K_d$ in the Fourier basis and produces a scalar multiplier $\Lambda(m\alpha)^d$ on the $m$th Fourier mode. The key expansion is
\[
 \log\Lambda(z)=\frac{16i}{3}z^3-16z^4+O(z^5).
\]
The first nontrivial oscillatory term is cubic. Therefore the only scaling for which $d\log\Lambda(m\alpha)$ remains nondegenerate is $d\alpha^3\asymp 1$, i.e.
\[
 \alpha\asymp d^{-1/3}.
\]
The cubic phase produces the Airy multiplier $e^{i\tau m^3}$, while the quartic term yields the $O(d^{-1/3})$ error.
\end{remark}

\subsubsection{Exact finite-$d$ Fourier reduction}

The finite-dimensional problem is already completely explicit.

\begin{theorem}[Exact reduction]\label{prop:exact}
Define
\[
 \Lambda(z):=\frac{e^{-2iz}}{\sqrt{1-4iz-8z^2}},
 \qquad z\in\R,
\]
with the principal branch of the square root. Then
\begin{equation}\label{eq:exact-reduction}
 \K_d(\alpha,\beta)
 =
 \frac{2}{\pi}
 \sum_{m\in\mathbb Z}
 \widehat{\mathfrak a}(m)e^{2im\beta}\Lambda(m\alpha)^d.
\end{equation}
\end{theorem}

\begin{proof}
Because $\mathfrak a$ is real analytic on a strip around the real axis, its Fourier series converges absolutely:
\[
 \mathfrak a(\theta)=\sum_{m\in\mathbb Z}\widehat{\mathfrak a}(m)e^{im\theta}.
\]
Substituting this into \eqref{eq:Kd-def} and interchanging the sum and the integral yields
\[
 \K_d(\alpha,\beta)
 =
 c_d
 \sum_{m\in\mathbb Z}\widehat{\mathfrak a}(m)e^{2im\beta}
 I_{m,d}(\alpha),
\]
where
\[
 I_{m,d}(\alpha)
 :=
 \int_{\R^d}\int_{\R^d}
 e^{-(\norm{u}^2+\norm{v}^2)}
 \cos\bigl(2\ip{u}{v}\bigr)
 e^{im\alpha(Q_d(u)+Q_d(v))}
 \,du\,dv.
\]
Since $Q_d(v)$ is even in $v$, the change of variables $v\mapsto -v$ shows that the two exponentials arising from
\[
 \cos\bigl(2\ip{u}{v}\bigr)=\frac{e^{2i\ip{u}{v}}+e^{-2i\ip{u}{v}}}{2}
\]
contribute equally. Hence
\[
 I_{m,d}(\alpha)
 =
 \int_{\R^d}\int_{\R^d}
 e^{-(\norm{u}^2+\norm{v}^2)}
 e^{2i\ip{u}{v}}
 e^{im\alpha(Q_d(u)+Q_d(v))}
 \,du\,dv.
\]
Now the integrand factorizes coordinate by coordinate, so
\[
 I_{m,d}(\alpha)
 =
 \prod_{j=1}^d
 \int_{\R^2}
 e^{-(x^2+y^2)}
 e^{im\alpha((4x^2-1)+(4y^2-1))}
 e^{2ixy}
 \,dx\,dy.
\]
The one-coordinate Gaussian integral is
\[
 \int_{\R^2}
 e^{-(1-4im\alpha)x^2-(1-4im\alpha)y^2+2ixy}
 \,dx\,dy
 =
 \frac{\pi}{\sqrt{(1-4im\alpha)^2+1}}.
\]
After including the factor $e^{-2im\alpha}$ coming from the two constant terms in $(4x^2-1)+(4y^2-1)$, the one-coordinate contribution is
\[
 \frac{\pi e^{-2im\alpha}}{\sqrt{(1-4im\alpha)^2+1}}
 =
 \frac{\pi}{\sqrt2}\,\Lambda(m\alpha).
\]
Therefore
\[
 I_{m,d}(\alpha)=\left(\frac{\pi}{\sqrt2}\right)^d\Lambda(m\alpha)^d.
\]
Since
\[
 c_d\left(\frac{\pi}{\sqrt2}\right)^d=\frac{2}{\pi},
\]
we obtain \eqref{eq:exact-reduction}. \qedhere
\end{proof}

\subsubsection{Two preparatory lemmas}

\begin{lemma}[Fourier coefficient decay]\label{lem:fourier-decay}
Let
\[
 \rho_*:=\arsinh(1)=\log(1+\sqrt2).
\]
Then for every $0<\rho<\rho_*$ there exists $C_\rho<\infty$ such that
\[
 \abs{\widehat{\mathfrak a}(m)}\le C_\rho e^{-\rho\abs m}
 \qquad (m\in\mathbb Z).
\]
In particular,
\[
 \sum_{m\in\mathbb Z}\abs{\widehat{\mathfrak a}(m)}\abs m^k<\infty
 \qquad\text{for every }k\ge 0.
\]
\end{lemma}

\begin{proof}
The singularities of $\arsinh(z)$ are at $z=\pm i$, so the singularities of
\[
 \mathfrak a(z)=\arsinh(\cos z)
\]
occur where $\cos z=\pm i$. The nearest such points to the real axis lie at imaginary distance $\rho_*$. Hence $\mathfrak a$ extends holomorphically to every strip
\[
 \abs{\Im z}<\rho
 \qquad (0<\rho<\rho_*).
\]
The standard Cauchy estimate for Fourier coefficients on analytic strips gives
\[
 \abs{\widehat{\mathfrak a}(m)}\le C_\rho e^{-\rho\abs m}.
\]
The summability of polynomially weighted coefficients follows immediately. \qedhere
\end{proof}

\begin{lemma}[Local expansion of the multiplier]\label{lem:lambda-expansion}
For $\abs z\le 1/16$,
\[
 \log\Lambda(z)=\frac{16i}{3}z^3-16z^4+r(z),
\]
with the explicit bound
\[
 \abs{r(z)}\le 500\abs{z}^5.
\]
\end{lemma}

\begin{proof}
Write
\[
 \Lambda(z)=e^{-2iz}(1+w(z))^{-1/2},
 \qquad
 w(z):=-4iz-8z^2.
\]
If $\abs z\le 1/16$, then
\[
 \abs{w(z)}\le 4\abs z+8\abs z^2\le \frac14+\frac1{32}=\frac9{32}<1.
\]
Hence the principal logarithm is analytic there and
\[
 \log\Lambda(z)=-2iz-\frac12\log(1+w(z)).
\]
Use the fourth-order logarithm expansion
\[
 \log(1+w)=w-\frac{w^2}{2}+\frac{w^3}{3}-\frac{w^4}{4}+R_5(w),
 \qquad
 \abs{R_5(w)}\le \frac{\abs w^5}{5(1-\abs w)}.
\]
A direct algebraic expansion gives
\[
\begin{aligned}
 -2iz-\frac12\left(w-\frac{w^2}{2}+\frac{w^3}{3}-\frac{w^4}{4}\right)
 &=
 \frac{16i}{3}z^3-16z^4-128iz^5 \\
 &\quad -\frac{2048}{3}z^6+1024iz^7+512z^8.
\end{aligned}
\]
Thus for $\abs z\le 1/16$,
\[
 \left|-128iz^5-\frac{2048}{3}z^6+1024iz^7+512z^8\right|
 \le 175\abs z^5.
\]
On the other hand, since $\abs{w(z)}\le \frac92\abs z$,
\[
 \frac12\abs{R_5(w)}
 \le
 \frac12\cdot\frac{\abs w^5}{5(1-\abs w)}
 \le 261\abs z^5.
\]
Combining the two bounds yields
\[
 \abs{r(z)}\le (175+261)\abs z^5\le 500\abs z^5.
\]
\qedhere
\end{proof}

\subsubsection{Proof of the Airy limit}

\begin{proof}[Proof of Theorem~\ref{thm:main}]
Start from Theorem~\ref{prop:exact}:
\[
 \K_d\bigl(\kappa d^{-1/3},\beta\bigr)
 =
 \frac{2}{\pi}
 \sum_{m\in\mathbb Z}
 \widehat{\mathfrak a}(m)e^{2im\beta}
 \Lambda\bigl(m\kappa d^{-1/3}\bigr)^d.
\]
Define the target series
\[
 \mathcal L_\infty(\kappa,\beta)
 :=
 \frac{2}{\pi}
 \sum_{m\in\mathbb Z}
 \widehat{\mathfrak a}(m)e^{2im\beta}e^{i\tau_\kappa m^3}
 =
 \frac{2}{\pi}\bigl(e^{-\tau_\kappa\partial_\theta^3}\mathfrak a\bigr)(2\beta),
\]
where $\tau_\kappa=\frac{16}{3}\kappa^3$. We must bound
\[
 \K_d\bigl(\kappa d^{-1/3},\beta\bigr)-\mathcal L_\infty(\kappa,\beta).
\]
We split the Fourier modes into low and high frequencies.

\medskip
\noindent\textbf{Step 1: choose the cutoff.}
Pick
\[
 A>\frac{1}{3\rho},
 \qquad
 N_d:=\lfloor A\log d\rfloor.
\]
Since $N_d d^{-1/3}\to 0$, there exists $d_1=d_1(\kappa_0)$ such that for all $d\ge d_1$, all $\abs m\le N_d$, and all $\abs\kappa\le\kappa_0$,
\[
 \abs{m\kappa d^{-1/3}}\le \frac1{16}.
\]

\medskip
\noindent\textbf{Step 2: low-frequency expansion.}
For $\abs m\le N_d$, set
\[
 z:=m\kappa d^{-1/3}.
\]
By Lemma~\ref{lem:lambda-expansion},
\[
 \log\Lambda(z)=\frac{16i}{3}z^3-16z^4+r(z),
 \qquad
 \abs{r(z)}\le 500\abs{z}^5.
\]
Multiplying by $d$ gives
\[
 d\log\Lambda(z)
 =i\tau_\kappa m^3-16\kappa^4m^4d^{-1/3}+\varepsilon_{m,d},
\]
where
\[
 \abs{\varepsilon_{m,d}}
 \le 500\abs{\kappa}^5\abs m^5d^{-2/3}
 \le 500\kappa_0^5\abs m^5d^{-2/3}.
\]
Define
\[
 \delta_{m,d}:=-16\kappa^4m^4d^{-1/3}+\varepsilon_{m,d}.
\]
Then
\[
 \Lambda\bigl(m\kappa d^{-1/3}\bigr)^d
 =e^{i\tau_\kappa m^3}e^{\delta_{m,d}}.
\]
Since $\abs m\le A\log d$,
\[
 \abs{\delta_{m,d}}
 \le
 16\kappa_0^4A^4(\log d)^4d^{-1/3}
 +
 500\kappa_0^5A^5(\log d)^5d^{-2/3}.
\]
The right-hand side tends to $0$, so there exists $d_2=d_2(\rho,\kappa_0)$ such that for all $d\ge d_2$,
\[
 \abs{\delta_{m,d}}\le 1
 \qquad (\abs m\le N_d,\ \abs\kappa\le\kappa_0).
\]
Therefore
\[
 \abs{e^{\delta_{m,d}}-1}\le 2\abs{\delta_{m,d}}.
\]
So
\[
 \left|
 \Lambda\bigl(m\kappa d^{-1/3}\bigr)^d-e^{i\tau_\kappa m^3}
 \right|
 \le
 32\kappa_0^4\abs m^4d^{-1/3}
 +
 1000\kappa_0^5\abs m^5d^{-2/3}.
\]
Hence the low-frequency contribution is bounded by
\begin{align*}
\frac{2}{\pi}
\sum_{\abs m\le N_d}
\abs{\widehat{\mathfrak a}(m)}
\left|
 \Lambda\bigl(m\kappa d^{-1/3}\bigr)^d-e^{i\tau_\kappa m^3}
\right|
&\le
\frac{64\kappa_0^4}{\pi}d^{-1/3}
\sum_{m\in\mathbb Z}\abs{\widehat{\mathfrak a}(m)}\abs m^4 \\
&\qquad+
\frac{2000\kappa_0^5}{\pi}d^{-2/3}
\sum_{m\in\mathbb Z}\abs{\widehat{\mathfrak a}(m)}\abs m^5.
\end{align*}
By Lemma~\ref{lem:fourier-decay}, both sums are finite. Therefore
\[
 \mathrm{LowFreqError}\le C_1d^{-1/3}.
\]

\medskip
\noindent\textbf{Step 3: high-frequency tail.}
For real $z$,
\[
 \abs{\Lambda(z)}=\frac{1}{\abs{1-4iz-8z^2}^{1/2}}.
\]
A direct computation gives
\[
 \abs{1-4iz-8z^2}^2=(1-8z^2)^2+16z^2=1+64z^4,
\]
so
\[
 \abs{\Lambda(z)}=(1+64z^4)^{-1/4}\le 1.
\]
Thus
\[
 \sum_{\abs m>N_d}
 \abs{\widehat{\mathfrak a}(m)}\abs{\Lambda(m\kappa d^{-1/3})}^d
 \le
 \sum_{\abs m>N_d}\abs{\widehat{\mathfrak a}(m)}.
\]
Also
\[
 \sum_{\abs m>N_d}\abs{\widehat{\mathfrak a}(m)}\abs{e^{i\tau_\kappa m^3}}
 =
 \sum_{\abs m>N_d}\abs{\widehat{\mathfrak a}(m)}.
\]
Hence
\[
 \mathrm{HighFreqError}
 \le
 \frac{4}{\pi}\sum_{\abs m>N_d}\abs{\widehat{\mathfrak a}(m)}.
\]
By Lemma~\ref{lem:fourier-decay},
\[
 \sum_{\abs m>N_d}\abs{\widehat{\mathfrak a}(m)}
 \le C_\rho e^{-\rho N_d}
 \le C_\rho d^{-A\rho}.
\]
Since $A\rho>1/3$,
\[
 \mathrm{HighFreqError}\le C_2d^{-1/3}.
\]

\medskip
\noindent\textbf{Step 4: combine the bounds.}
For $d\ge d_0:=\max\{d_1,d_2\}$,
\[
 \left|
 \K_d\bigl(\kappa d^{-1/3},\beta\bigr)-\mathcal L_\infty(\kappa,\beta)
 \right|
 \le
 \mathrm{LowFreqError}+\mathrm{HighFreqError}
 \le
 (C_1+C_2)d^{-1/3}.
\]
This proves \eqref{eq:main-estimate}. \qedhere
\end{proof}


\subsubsection{Numerical consequence}

The exact formula \eqref{eq:exact-reduction} gives a direct numerical procedure: for each fixed auxiliary dimension $d$, truncate the absolutely convergent Fourier sum and optimize over $(\alpha,\beta)$.  Figure~\ref{fig:koenig-dimension} shows the resulting normalized K\"onig values.

\begin{figure}[t]
\centering
\includegraphics[width=0.82\textwidth]{images/affine_radial_BK_vs_dimension.png}
\caption{Normalized K\"onig's bilinear form $\K_d$ for affine radial rotating-hyperplane partitions as a function of the auxiliary dimension $d$. The dashed horizontal line is the hyperplane benchmark $2\log(1+\sqrt2)/\pi\approx0.56110$.}
\label{fig:koenig-dimension}
\end{figure}

The optimized values in the displayed range exceed $0.572$, compared with the hyperplane value $0.56110\ldots$.  The Airy limit explains the large-$d$ mechanism: under the $d^{-1/3}$ scaling, the radial phase creates the cubic Fourier multiplier appearing in \eqref{eq:main-estimate}.  The main point for the present section is the resulting explicit asymptotic source of non-hyperplane improvements for K\"onig's bilinear form.


% Suggested bibliography keys used above:
% Konig2001 = H. K\"onig, ``On an extremal problem originating in questions of unconditional convergence,'' in Recent Progress in Multivariate Approximation, ISNM 137, Birkh\"auser, 2001, pp. 185--192.
% BravermanMakarychevMakarychevNaor2013 = M. Braverman, K. Makarychev, Y. Makarychev, and A. Naor, ``The Grothendieck constant is strictly smaller than Krivine's bound,'' Forum Math. Pi 1 (2013), e4.
% Krivine1977-1978 = J.-L. Krivine, ``Constantes de Grothendieck et fonctions de type positif sur les sph\`eres,'' S\'eminaire Analyse fonctionnelle (Maurey-Schwartz), 1977--1978.


==> old/koenig_v2.tex <==
\section{Asymptotic Families for K\"onig Bilinear Form}
\label{sec:konig-not-sufficient}

{\color{blue} FOR ALAN: DEFINE KONIG HERE IN FULL}

\subsection{Affine radial partition family}

The tiger partitions discussed in the preceding section are a natural place to look for improvements to Krivine rounding, since they arise from the variational problem for K\"onig's bilinear form. Their geometry, however, is not analytically tractable: the known descriptions are essentially numerical, and there is no clear closed form that remains usable in high dimension. In this section we therefore study a complementary family of partitions which is simple enough to analyze exactly in every dimension, but still flexible enough to produce a large improvement for the K\"onig bilinear form.

The family consists of rotated hyperplanes. The sign cut is always a half-space in a two-dimensional active plane, but its angle is allowed to depend affinely on a radial observable in an auxiliary $d$-dimensional Gaussian block. This gives an explicit higher-dimensional model in which the finite-$d$ K\"onig value diagonalizes in Fourier space and has a clean Airy limit as $d\to\infty$.

The point of the section is deliberately negative. These partitions give a substantial improvement over the hyperplane for K\"onig's bilinear form, but their Krivine values $c_{f,g}$ are numerically worse than the hyperplane in low dimensions. Thus optimizing the K\"onig bilinear form is not, by itself, a reliable proxy for optimizing the Grothendieck rounding constant.

\subsubsection{Motivation from Krivine's rotating hyperplane}

We begin by recalling the analytic reduction behind Krivine's rotating-hyperplane construction. This is the source of the affine radial family analyzed below. Throughout this section, $H_{f,g}$ denotes the same arcsine-normalized correlation function as in Section~2: for odd measurable partitions $f,g:\R^k\to\{-1,1\}$,
\[
 H_{f,g}(t)=\frac{\pi}{2}\,\E\bigl[f(X)g(Y)\bigr],
 \qquad |t|<1,
\]
where $(X,Y)$ is the standard Gaussian coupling used in the definition of the rounding scheme. With this normalization the hyperplane partition has correlation $H(t)=\arcsin t$.

Let
\[
\ell^+_\varepsilon(x_0,x_1,x_2)
:=x_1\cos\bigl(\varepsilon H_2(x_0)\bigr)+x_2\sin\bigl(\varepsilon H_2(x_0)\bigr),
\]
\[
\ell^-_\varepsilon(y_0,y_1,y_2)
:=y_1\cos\bigl(\varepsilon H_2(y_0)\bigr)-y_2\sin\bigl(\varepsilon H_2(y_0)\bigr),
\]
with $H_2(s)=s^2-1$, and define the corresponding partitions
\[
 f_\varepsilon(x)=\operatorname{sign}\ell^+_\varepsilon(x),
 \qquad
 g_\varepsilon(y)=\operatorname{sign}\ell^-_\varepsilon(y).
\]
Geometrically, the cut is still an ordinary half-space in the active $(x_1,x_2)$-plane, but that half-space is rotated by an angle depending on the auxiliary coordinate $x_0$. The same construction is used on the $Y$ side, with the opposite sign in the sine term.

Conditioned on $x_0,y_0$, the active-plane pair $\ell^+_\varepsilon(X)$, $\ell^-_\varepsilon(Y)$ is a centered bivariate normal pair with correlation
\[
 t\Bigl(\cos\bigl(\varepsilon H_2(x_0)\bigr)\cos\bigl(\varepsilon H_2(y_0)\bigr)
 -\sin\bigl(\varepsilon H_2(x_0)\bigr)\sin\bigl(\varepsilon H_2(y_0)\bigr)\Bigr)
 =t\cos\bigl(\varepsilon(H_2(x_0)+H_2(y_0))\bigr).
\]
Grothendieck's identity therefore gives
\[
 H_{f_\varepsilon,g_\varepsilon}(t)
 =
 \E\Bigl[\arcsin\bigl(t\cos(\varepsilon(H_2(X_0)+H_2(Y_0)))\bigr)\Bigr].
\]
At the special point $t=i$, using $\arcsin(is)=i\,\arsinh(s)$ yields
\[
 \frac{H_{f_\varepsilon,g_\varepsilon}(i)}{i}
 =
 \E\Bigl[\arsinh\bigl(\cos(\varepsilon(H_2(X_0)+H_2(Y_0)))\bigr)\Bigr].
\]
This is the origin of the fixed circle profile
\[
 \mathfrak a(\theta):=\arsinh(\cos\theta),\qquad \theta\in\R,
\]
which we view as a $2\pi$-periodic analytic function on the circle $\T=\R/2\pi\mathbb Z$.

The phase in the last display is
\[
 \varepsilon\bigl(H_2(X_0)+H_2(Y_0)\bigr).
\]
It is the sum of the two rotation angles, one coming from the $X$ side and one from the $Y$ side. The reduced problem is obtained by evaluating the fixed circle profile $\mathfrak a$ at this phase.

For comparison with K\"onig's bilinear form, it is convenient to use the normalization
\[
 \mathcal B_{\mathrm K}(f,g):=\frac{2}{\pi}\,\frac{H_{f,g}(i)}{i}.
\]
Thus the hyperplane benchmark is
\[
 \mathcal B_{\mathrm K}(\mathrm{hp},\mathrm{hp})
 =\frac{2}{\pi}\arsinh(1)
 =\frac{2}{\pi}\log(1+\sqrt2).
\]
Krivine's rotating-hyperplane computation rewrites $\mathcal B_{\mathrm K}(f_\varepsilon,g_\varepsilon)$ as an explicit oscillatory integral. After the analytic-continuation calculation at $t=i$, one uses the rescaled auxiliary coordinates
\[
 X_0=2u,
 \qquad
 Y_0=2v.
\]
With this convention, $H_2(X_0)=4u^2-1$ and $H_2(Y_0)=4v^2-1$, and the Gaussian kernel becomes the real oscillatory kernel $e^{-(u^2+v^2)}\cos(2uv)$. Hence
\[
 \mathcal B_{\mathrm K}(f_\varepsilon,g_\varepsilon)
 =
 \frac{2^{3/2}}{\pi^2}
 \int_{\R}\int_{\R}
 e^{-(u^2+v^2)}\cos(2uv)
 \mathfrak a\bigl(\varepsilon((4u^2-1)+(4v^2-1))\bigr)
 \,du\,dv.
\]
Passing to polar coordinates $u=r\cos\ph$, $v=r\sin\ph$ gives
\[
 2uv=r^2\sin(2\ph),
 \qquad
 (4u^2-1)+(4v^2-1)=4r^2-2,
 \qquad
 du\,dv=r\,dr\,d\ph.
\]
Writing $\rho=r^2$ and $\vartheta=2\ph$, we obtain
\begin{align*}
 \mathcal B_{\mathrm K}(f_\varepsilon,g_\varepsilon)
 &=
 \frac{2^{3/2}}{\pi^2}
 \int_0^\infty\int_0^{2\pi}
 e^{-r^2}\cos(r^2\sin(2\ph))
 \mathfrak a\bigl(\varepsilon(4r^2-2)\bigr)
 r\,d\ph\,dr \\
 &=
 \frac{2\sqrt2}{\pi^2}
 \int_0^\infty\int_0^\pi
 e^{-\rho}\cos(\rho\sin\vartheta)
 \mathfrak a\bigl(2\varepsilon(2\rho-1)\bigr)
 \,d\vartheta\,d\rho.
\end{align*}
This is the oscillatory integral in Krivine's note, with his parameter $\eta$ equal to $2\varepsilon$.

\subsubsection{The higher-dimensional affine radial family}

The preceding computation suggests the following high-dimensional generalization. We keep the active two-dimensional plane in which the sign cut lives, and we allow an auxiliary $d$-dimensional Gaussian block to determine the rotation angle.

\begin{definition}[Local angle and phase]
Fix $d\in\mathbb N$ and parameters $\alpha,\beta\in\R$. Define
\[
 Q_d(u):=4\norm{u}_2^2-d,
 \qquad u\in\R^d,
\]
\[
 \psi_{d,\alpha,\beta}(u):=\beta+\alpha Q_d(u),
\]
and the associated pairwise phase function
\[
 \phi_{d,\alpha,\beta}(u,v)
 :=\psi_{d,\alpha,\beta}(u)+\psi_{d,\alpha,\beta}(v)
 =2\beta+\alpha\bigl(Q_d(u)+Q_d(v)\bigr).
\]
\end{definition}

Here $\theta$ always denotes the circle variable in the periodic profile $\mathfrak a(\theta)=\arsinh(\cos\theta)$, while $\phi_{d,\alpha,\beta}(u,v)$ is the phase inserted into that circle variable. The parameter $\beta$ is a constant rotation on each side, so it contributes the total shift $2\beta$. The parameter $\alpha$ controls the dependence of the rotation on the auxiliary variables. The name ``affine radial'' refers to the fact that the angle depends affinely on the radial observable $Q_d(u)$.

The rescaling in the definition of $Q_d$ is exactly the rescaling used in the one-dimensional computation above. In the $t=i$ K\"onig kernel the auxiliary coordinates are written as $X_j=2u_j$ and $Y_j=2v_j$. Thus each copy of Krivine's quadratic observable $H_2(X_j)=X_j^2-1$ becomes $(2u_j)^2-1=4u_j^2-1$, and summing over the $d$ auxiliary coordinates gives
\[
 Q_d(u)=\sum_{j=1}^d\bigl((2u_j)^2-1\bigr)=4\norm{u}_2^2-d.
\]

The corresponding rotated half-space partitions on $\R^{d+2}=\R^d\times\R^2$ are
\[
 f_{d,\alpha,\beta}(u;x_1,x_2)
 :=
 \operatorname{sign}\bigl(x_1\cos\psi_{d,\alpha,\beta}(u)+x_2\sin\psi_{d,\alpha,\beta}(u)\bigr),
\]
\[
 g_{d,\alpha,\beta}(v;y_1,y_2)
 :=
 \operatorname{sign}\bigl(y_1\cos\psi_{d,\alpha,\beta}(v)-y_2\sin\psi_{d,\alpha,\beta}(v)\bigr).
\]
Conditioned on $u,v$, the active-plane correlation is $t\cos\phi_{d,\alpha,\beta}(u,v)$, exactly as in the one-dimensional rotating-hyperplane construction. Evaluating at $t=i$ and integrating out the active plane leaves the following reduced K\"onig value.

\begin{definition}[Reduced affine radial K\"onig value]
Let
\[
 c_d:=\frac{2^{1+d/2}}{\pi^{d+1}}.
\]
Define
\begin{equation}\label{eq:Kd-def}
 \K_d(\alpha,\beta)
 :=
 \mathcal B_{\mathrm K}(f_{d,\alpha,\beta},g_{d,\alpha,\beta})
 =
 c_d
 \int_{\R^d}\int_{\R^d}
 e^{-(\norm{u}_2^2+\norm{v}_2^2)}
 \cos\bigl(2\ip{u}{v}\bigr)
 \mathfrak a\bigl(\phi_{d,\alpha,\beta}(u,v)\bigr)
 \,du\,dv.
\end{equation}
\end{definition}

Thus the entire dependence on the partition pair is encoded by the phase function $\phi_{d,\alpha,\beta}$. When $\alpha=\beta=0$ there is no rotation, and one recovers the hyperplane benchmark
\[
 \K_d(0,0)=\frac{2}{\pi}\mathfrak a(0)
 =\frac{2}{\pi}\arsinh(1)
 =\frac{2}{\pi}\log(1+\sqrt2).
\]
The exact Fourier reduction below gives the same value directly.

\subsubsection{Main theorem and the Airy operator}

The asymptotic object is the periodic Airy flow on the circle.

\begin{definition}[Periodic Airy propagator]
Let $q(\theta)=\sum_{m\in\mathbb Z}\widehat q(m)e^{im\theta}$ be a $2\pi$-periodic analytic function, with Fourier coefficients
\[
 \widehat q(m):=\frac{1}{2\pi}\int_0^{2\pi} q(\theta)e^{-im\theta}\,d\theta.
\]
For $\tau\in\R$ define
\[
 \bigl(e^{-\tau\partial_\theta^3}q\bigr)(\theta)
 :=
 \sum_{m\in\mathbb Z}e^{i\tau m^3}\widehat q(m)e^{im\theta}.
\]
Equivalently, $u(\tau,\theta):=(e^{-\tau\partial_\theta^3}q)(\theta)$ is the solution of the periodic Airy equation
\[
 \partial_\tau u+\partial_\theta^3 u=0,
 \qquad
 u(0,\theta)=q(\theta).
\]
Indeed, on the Fourier mode $e^{im\theta}$ one has $-\partial_\theta^3 e^{im\theta}=im^3e^{im\theta}$.
\end{definition}

We can now state the theorem.

\begin{theorem}[Airy limit for the affine radial phase family]\label{thm:main}
Let
\[
 \mathfrak a(\theta)=\arsinh(\cos\theta),
 \qquad \theta\in\T.
\]
Fix $0<\rho<\rho_*$, where $\rho_*:=\arsinh(1)=\log(1+\sqrt2)$, and fix $\kappa_0>0$. Then there exist constants $C=C(\rho,\kappa_0)$ and $d_0=d_0(\rho,\kappa_0)$ such that for all $d\ge d_0$, all $|\kappa|\le\kappa_0$, and all $\beta\in\R$,
\begin{equation}\label{eq:main-estimate}
\left|
 \K_d\bigl(\kappa d^{-1/3},\beta\bigr)
 -
 \frac{2}{\pi}\bigl(e^{-\tau_\kappa\partial_\theta^3}\mathfrak a\bigr)(2\beta)
\right|
\le C d^{-1/3},
\end{equation}
where
\[
 \tau_\kappa:=\frac{16}{3}\kappa^3.
\]
Equivalently,
\[
 \K_d\bigl(\kappa d^{-1/3},\beta\bigr)
 \longrightarrow
 \frac{2}{\pi}\bigl(e^{-\tau_\kappa\partial_\theta^3}\mathfrak a\bigr)(2\beta)
\]
uniformly for $(\kappa,\beta)\in[-\kappa_0,\kappa_0]\times\R$.
\end{theorem}

\begin{remark}[Why the scaling is $d^{-1/3}$]
The proof diagonalizes $\K_d$ in the Fourier basis and produces a scalar multiplier $\Lambda(m\alpha)^d$ on the $m$th Fourier mode. The key expansion is
\[
 \log\Lambda(z)=\frac{16i}{3}z^3-16z^4+O(z^5).
\]
The first nontrivial oscillatory term is cubic. Therefore the only scaling for which $d\log\Lambda(m\alpha)$ remains nondegenerate is $d\alpha^3\asymp 1$, i.e.
\[
 \alpha\asymp d^{-1/3}.
\]
The cubic phase produces the Airy multiplier $e^{i\tau m^3}$, while the quartic term yields the $O(d^{-1/3})$ error.
\end{remark}

\begin{remark}[Proof strategy]
Expand $\mathfrak a$ into its Fourier series on the circle. Each Fourier mode can be integrated exactly through a $2\times2$ Gaussian computation, and the entire functional becomes a diagonal Fourier multiplier. One then expands this multiplier near the origin, chooses the $d^{-1/3}$ scaling dictated by the cubic term, and splits the Fourier modes into low frequencies $|m|\le A\log d$ and a rapidly decaying analytic tail. This turns the heuristic Airy limit into the uniform estimate \eqref{eq:main-estimate}.
\end{remark}

\subsubsection{Exact finite-$d$ Fourier reduction}

The finite-dimensional problem is already completely explicit.

\begin{theorem}[Exact reduction]\label{prop:exact}
Define
\[
 \Lambda(z):=\frac{e^{-2iz}}{\sqrt{1-4iz-8z^2}},
 \qquad z\in\R,
\]
with the principal branch of the square root. Then
\begin{equation}\label{eq:exact-reduction}
 \K_d(\alpha,\beta)
 =
 \frac{2}{\pi}
 \sum_{m\in\mathbb Z}
 \widehat{\mathfrak a}(m)e^{2im\beta}\Lambda(m\alpha)^d.
\end{equation}
\end{theorem}

\begin{proof}
Because $\mathfrak a$ is real analytic on a strip around the real axis, its Fourier series converges absolutely:
\[
 \mathfrak a(\theta)=\sum_{m\in\mathbb Z}\widehat{\mathfrak a}(m)e^{im\theta}.
\]
Substituting this into \eqref{eq:Kd-def} and interchanging the sum and the integral yields
\[
 \K_d(\alpha,\beta)
 =
 c_d
 \sum_{m\in\mathbb Z}\widehat{\mathfrak a}(m)e^{2im\beta}
 I_{m,d}(\alpha),
\]
where
\[
 I_{m,d}(\alpha)
 :=
 \int_{\R^d}\int_{\R^d}
 e^{-(\norm{u}^2+\norm{v}^2)}
 \cos\bigl(2\ip{u}{v}\bigr)
 e^{im\alpha(Q_d(u)+Q_d(v))}
 \,du\,dv.
\]
Since $Q_d(v)$ is even in $v$, the change of variables $v\mapsto -v$ shows that the two exponentials arising from
\[
 \cos\bigl(2\ip{u}{v}\bigr)=\frac{e^{2i\ip{u}{v}}+e^{-2i\ip{u}{v}}}{2}
\]
contribute equally. Hence
\[
 I_{m,d}(\alpha)
 =
 \int_{\R^d}\int_{\R^d}
 e^{-(\norm{u}^2+\norm{v}^2)}
 e^{2i\ip{u}{v}}
 e^{im\alpha(Q_d(u)+Q_d(v))}
 \,du\,dv.
\]
Now the integrand factorizes coordinate by coordinate, so
\[
 I_{m,d}(\alpha)
 =
 \prod_{j=1}^d
 \int_{\R^2}
 e^{-(x^2+y^2)}
 e^{im\alpha((4x^2-1)+(4y^2-1))}
 e^{2ixy}
 \,dx\,dy.
\]
The one-coordinate Gaussian integral is
\[
 \int_{\R^2}
 e^{-(1-4im\alpha)x^2-(1-4im\alpha)y^2+2ixy}
 \,dx\,dy
 =
 \frac{\pi}{\sqrt{(1-4im\alpha)^2+1}}.
\]
After including the factor $e^{-2im\alpha}$ coming from the two constant terms in $(4x^2-1)+(4y^2-1)$, the one-coordinate contribution is
\[
 \frac{\pi e^{-2im\alpha}}{\sqrt{(1-4im\alpha)^2+1}}
 =
 \frac{\pi}{\sqrt2}\,\Lambda(m\alpha).
\]
Therefore
\[
 I_{m,d}(\alpha)=\left(\frac{\pi}{\sqrt2}\right)^d\Lambda(m\alpha)^d.
\]
Since
\[
 c_d\left(\frac{\pi}{\sqrt2}\right)^d=\frac{2}{\pi},
\]
we obtain \eqref{eq:exact-reduction}. \qedhere
\end{proof}

\subsubsection{Two preparatory lemmas}

\begin{lemma}[Fourier coefficient decay]\label{lem:fourier-decay}
Let
\[
 \rho_*:=\arsinh(1)=\log(1+\sqrt2).
\]
Then for every $0<\rho<\rho_*$ there exists $C_\rho<\infty$ such that
\[
 \abs{\widehat{\mathfrak a}(m)}\le C_\rho e^{-\rho\abs m}
 \qquad (m\in\mathbb Z).
\]
In particular,
\[
 \sum_{m\in\mathbb Z}\abs{\widehat{\mathfrak a}(m)}\abs m^k<\infty
 \qquad\text{for every }k\ge 0.
\]
\end{lemma}

\begin{proof}
The singularities of $\arsinh(z)$ are at $z=\pm i$, so the singularities of
\[
 \mathfrak a(z)=\arsinh(\cos z)
\]
occur where $\cos z=\pm i$. The nearest such points to the real axis lie at imaginary distance $\rho_*$. Hence $\mathfrak a$ extends holomorphically to every strip
\[
 \abs{\Im z}<\rho
 \qquad (0<\rho<\rho_*).
\]
The standard Cauchy estimate for Fourier coefficients on analytic strips gives
\[
 \abs{\widehat{\mathfrak a}(m)}\le C_\rho e^{-\rho\abs m}.
\]
The summability of polynomially weighted coefficients follows immediately. \qedhere
\end{proof}

\begin{lemma}[Local expansion of the multiplier]\label{lem:lambda-expansion}
For $\abs z\le 1/16$,
\[
 \log\Lambda(z)=\frac{16i}{3}z^3-16z^4+r(z),
\]
with the explicit bound
\[
 \abs{r(z)}\le 500\abs{z}^5.
\]
\end{lemma}

\begin{proof}
Write
\[
 \Lambda(z)=e^{-2iz}(1+w(z))^{-1/2},
 \qquad
 w(z):=-4iz-8z^2.
\]
If $\abs z\le 1/16$, then
\[
 \abs{w(z)}\le 4\abs z+8\abs z^2\le \frac14+\frac1{32}=\frac9{32}<1.
\]
Hence the principal logarithm is analytic there and
\[
 \log\Lambda(z)=-2iz-\frac12\log(1+w(z)).
\]
Use the fourth-order logarithm expansion
\[
 \log(1+w)=w-\frac{w^2}{2}+\frac{w^3}{3}-\frac{w^4}{4}+R_5(w),
 \qquad
 \abs{R_5(w)}\le \frac{\abs w^5}{5(1-\abs w)}.
\]
A direct algebraic expansion gives
\[
 -2iz-\frac12\left(w-\frac{w^2}{2}+\frac{w^3}{3}-\frac{w^4}{4}\right)
 =
 \frac{16i}{3}z^3-16z^4-128iz^5-\frac{2048}{3}z^6+1024iz^7+512z^8.
\]
Thus for $\abs z\le 1/16$,
\[
 \left|-128iz^5-\frac{2048}{3}z^6+1024iz^7+512z^8\right|
 \le 175\abs z^5.
\]
On the other hand, since $\abs{w(z)}\le \frac92\abs z$,
\[
 \frac12\abs{R_5(w)}
 \le
 \frac12\cdot\frac{\abs w^5}{5(1-\abs w)}
 \le 261\abs z^5.
\]
Combining the two bounds yields
\[
 \abs{r(z)}\le (175+261)\abs z^5\le 500\abs z^5.
\]
\qedhere
\end{proof}

\subsubsection{Proof of the Airy limit}

\begin{proof}[Proof of Theorem~\ref{thm:main}]
Start from Theorem~\ref{prop:exact}:
\[
 \K_d\bigl(\kappa d^{-1/3},\beta\bigr)
 =
 \frac{2}{\pi}
 \sum_{m\in\mathbb Z}
 \widehat{\mathfrak a}(m)e^{2im\beta}
 \Lambda\bigl(m\kappa d^{-1/3}\bigr)^d.
\]
Define the target series
\[
 \mathcal L_\infty(\kappa,\beta)
 :=
 \frac{2}{\pi}
 \sum_{m\in\mathbb Z}
 \widehat{\mathfrak a}(m)e^{2im\beta}e^{i\tau_\kappa m^3}
 =
 \frac{2}{\pi}\bigl(e^{-\tau_\kappa\partial_\theta^3}\mathfrak a\bigr)(2\beta),
\]
where $\tau_\kappa=\frac{16}{3}\kappa^3$. We must bound
\[
 \K_d\bigl(\kappa d^{-1/3},\beta\bigr)-\mathcal L_\infty(\kappa,\beta).
\]
We split the Fourier modes into low and high frequencies.

\medskip
\noindent\textbf{Step 1: choose the cutoff.}
Pick
\[
 A>\frac{1}{3\rho},
 \qquad
 N_d:=\lfloor A\log d\rfloor.
\]
Since $N_d d^{-1/3}\to 0$, there exists $d_1=d_1(\kappa_0)$ such that for all $d\ge d_1$, all $\abs m\le N_d$, and all $\abs\kappa\le\kappa_0$,
\[
 \abs{m\kappa d^{-1/3}}\le \frac1{16}.
\]

\medskip
\noindent\textbf{Step 2: low-frequency expansion.}
For $\abs m\le N_d$, set
\[
 z:=m\kappa d^{-1/3}.
\]
By Lemma~\ref{lem:lambda-expansion},
\[
 \log\Lambda(z)=\frac{16i}{3}z^3-16z^4+r(z),
 \qquad
 \abs{r(z)}\le 500\abs{z}^5.
\]
Multiplying by $d$ gives
\[
 d\log\Lambda(z)
 =i\tau_\kappa m^3-16\kappa^4m^4d^{-1/3}+\varepsilon_{m,d},
\]
where
\[
 \abs{\varepsilon_{m,d}}
 \le 500\abs{\kappa}^5\abs m^5d^{-2/3}
 \le 500\kappa_0^5\abs m^5d^{-2/3}.
\]
Define
\[
 \delta_{m,d}:=-16\kappa^4m^4d^{-1/3}+\varepsilon_{m,d}.
\]
Then
\[
 \Lambda\bigl(m\kappa d^{-1/3}\bigr)^d
 =e^{i\tau_\kappa m^3}e^{\delta_{m,d}}.
\]
Since $\abs m\le A\log d$,
\[
 \abs{\delta_{m,d}}
 \le
 16\kappa_0^4A^4(\log d)^4d^{-1/3}
 +
 500\kappa_0^5A^5(\log d)^5d^{-2/3}.
\]
The right-hand side tends to $0$, so there exists $d_2=d_2(\rho,\kappa_0)$ such that for all $d\ge d_2$,
\[
 \abs{\delta_{m,d}}\le 1
 \qquad (\abs m\le N_d,\ \abs\kappa\le\kappa_0).
\]
Therefore
\[
 \abs{e^{\delta_{m,d}}-1}\le 2\abs{\delta_{m,d}}.
\]
So
\[
 \left|
 \Lambda\bigl(m\kappa d^{-1/3}\bigr)^d-e^{i\tau_\kappa m^3}
 \right|
 \le
 32\kappa_0^4\abs m^4d^{-1/3}
 +
 1000\kappa_0^5\abs m^5d^{-2/3}.
\]
Hence the low-frequency contribution is bounded by
\begin{align*}
\frac{2}{\pi}
\sum_{\abs m\le N_d}
\abs{\widehat{\mathfrak a}(m)}
\left|
 \Lambda\bigl(m\kappa d^{-1/3}\bigr)^d-e^{i\tau_\kappa m^3}
\right|
&\le
\frac{64\kappa_0^4}{\pi}d^{-1/3}
\sum_{m\in\mathbb Z}\abs{\widehat{\mathfrak a}(m)}\abs m^4 \\
&\qquad+
\frac{2000\kappa_0^5}{\pi}d^{-2/3}
\sum_{m\in\mathbb Z}\abs{\widehat{\mathfrak a}(m)}\abs m^5.
\end{align*}
By Lemma~\ref{lem:fourier-decay}, both sums are finite. Therefore
\[
 \mathrm{LowFreqError}\le C_1d^{-1/3}.
\]

\medskip
\noindent\textbf{Step 3: high-frequency tail.}
For real $z$,
\[
 \abs{\Lambda(z)}=\frac{1}{\abs{1-4iz-8z^2}^{1/2}}.
\]
A direct computation gives
\[
 \abs{1-4iz-8z^2}^2=(1-8z^2)^2+16z^2=1+64z^4,
\]
so
\[
 \abs{\Lambda(z)}=(1+64z^4)^{-1/4}\le 1.
\]
Thus
\[
 \sum_{\abs m>N_d}
 \abs{\widehat{\mathfrak a}(m)}\abs{\Lambda(m\kappa d^{-1/3})}^d
 \le
 \sum_{\abs m>N_d}\abs{\widehat{\mathfrak a}(m)}.
\]
Also
\[
 \sum_{\abs m>N_d}\abs{\widehat{\mathfrak a}(m)}\abs{e^{i\tau_\kappa m^3}}
 =
 \sum_{\abs m>N_d}\abs{\widehat{\mathfrak a}(m)}.
\]
Hence
\[
 \mathrm{HighFreqError}
 \le
 \frac{4}{\pi}\sum_{\abs m>N_d}\abs{\widehat{\mathfrak a}(m)}.
\]
By Lemma~\ref{lem:fourier-decay},
\[
 \sum_{\abs m>N_d}\abs{\widehat{\mathfrak a}(m)}
 \le C_\rho e^{-\rho N_d}
 \le C_\rho d^{-A\rho}.
\]
Since $A\rho>1/3$,
\[
 \mathrm{HighFreqError}\le C_2d^{-1/3}.
\]

\medskip
\noindent\textbf{Step 4: combine the bounds.}
For $d\ge d_0:=\max\{d_1,d_2\}$,
\[
 \left|
 \K_d\bigl(\kappa d^{-1/3},\beta\bigr)-\mathcal L_\infty(\kappa,\beta)
 \right|
 \le
 \mathrm{LowFreqError}+\mathrm{HighFreqError}
 \le
 (C_1+C_2)d^{-1/3}.
\]
This proves \eqref{eq:main-estimate}. \qedhere
\end{proof}

\subsubsection{Explicit corollaries}

Because $\mathfrak a(\theta)=\arsinh(\cos\theta)$ is even and satisfies $\mathfrak a(\theta+\pi)=-\mathfrak a(\theta)$, its Fourier series contains only odd cosine modes:
\[
 \mathfrak a(\theta)=\sum_{\ell\ge0} b_{2\ell+1}\cos\bigl((2\ell+1)\theta\bigr),
\]
where
\[
 b_{2\ell+1}:=\frac{1}{\pi}\int_0^{2\pi}\mathfrak a(\theta)\cos\bigl((2\ell+1)\theta\bigr)\,d\theta,
 \qquad
 \abs{b_{2\ell+1}}\le C_\rho e^{-\rho(2\ell+1)}.
\]
From Theorem~\ref{thm:main} we immediately get the following explicit form of the limit.

\begin{corollary}[Cosine-series form]\label{cor:cosine}
For every fixed $\kappa,\beta\in\R$,
\[
 \lim_{d\to\infty}\K_d\bigl(\kappa d^{-1/3},\beta\bigr)
 =
 \frac{2}{\pi}
 \sum_{\ell\ge0}
 b_{2\ell+1}
 \cos\left(
 2(2\ell+1)\beta+\frac{16}{3}(2\ell+1)^3\kappa^3
 \right).
\]
\end{corollary}

\begin{corollary}[Operator form]\label{cor:operator}
If we write $\U_\tau:=e^{-\tau\partial_\theta^3}$, then
\[
 \lim_{d\to\infty}\K_d\bigl(\kappa d^{-1/3},\beta\bigr)
 =
 \frac{2}{\pi}(\U_{\tau_\kappa}\mathfrak a)(2\beta),
 \qquad
 \tau_\kappa=\frac{16}{3}\kappa^3.
\]
In other words, the large-$d$ limit of the affine radial K\"onig value is precisely the periodic Airy evolution of the fixed profile $\mathfrak a(\theta)=\arsinh(\cos\theta)$, evaluated at the angle $\theta=2\beta$.
\end{corollary}

\begin{corollary}[Variational form of the asymptotic affine value]\label{cor:variational}
Because $\tau_\kappa$ ranges over all real numbers as $\kappa$ ranges over $\R$, and because $e^{i\tau m^3}$ is $2\pi$-periodic in $\tau$ for every integer $m$, the asymptotic affine optimum is
\[
 \Lambda_{\mathrm{aff}}
 =
 \sup_{\tau\in[0,2\pi],\ \theta\in[0,2\pi]}
 \frac{2}{\pi}\bigl(e^{-\tau\partial_\theta^3}\mathfrak a\bigr)(\theta).
\]
Thus the asymptotic optimization problem for this affine radial family reduces to a supremum over the two-torus $(\tau,\theta)\in[0,2\pi]^2$.
\end{corollary}

\subsubsection{Numerical comparison with the Krivine parameter}

The preceding theorem explains why the affine radial family can be optimized efficiently for K\"onig's bilinear form. For each dimension $d$, one may choose a phase in this family and evaluate the resulting value $\K_d(\alpha,\beta)$ using the finite Fourier reduction. Figure~\ref{fig:koenig-dimension} shows the outcome of our numerical optimization as a function of the auxiliary dimension.

\begin{figure}[t]
\centering
\includegraphics[width=0.82\textwidth]{images/affine_radial_BK_vs_dimension.png}
\caption{Normalized K\"onig value $\K_d$ for affine radial rotating-hyperplane partitions as a function of the auxiliary dimension $d$. The dashed horizontal line is the hyperplane value $2\rho_*/\pi=2\log(1+\sqrt2)/\pi\approx0.56110$. The optimized affine radial phases give a much larger improvement in $B_{\mathrm K}$ than this benchmark.}
\label{fig:koenig-dimension}
\end{figure}

The improvement in K\"onig value is large on the scale relevant to this problem. The hyperplane gives
\[
 \mathcal B_{\mathrm K}(\mathrm{hp},\mathrm{hp})
 =\frac{2\rho_*}{\pi}
 \approx 0.56110.
\]
By contrast, the optimized affine radial phases in the displayed range exceed $0.572$, giving an absolute improvement of more than $10^{-2}$ over the hyperplane in the same normalization. This is far larger than the original low-dimensional rotating-hyperplane improvement visible in the three-dimensional Krivine benchmark.

However, this K\"onig improvement does not translate into an improved Krivine rounding parameter. We numerically computed for dimensions 3 and 4 of the affine radial family the parameters that maximized the K\"onig value, and their corresponding inverse Grothendieck $c_{f,g}$ values.

For dimension 3 the values are:
\[
 \mathcal B_{\mathrm K}=0.5624 ,
 \qquad
 c_{f,g}=0.5448,
\]
and in dimension 4 the values are:
\[
 \mathcal B_{\mathrm K}=0.5627 ,
 \qquad
 c_{f,g}=0.5416.
\]

In both cases the K\"onig value exceeds the hyperplane baseline while $c_{f,g}$ is worse than the hyperplane baseline.

This is the main lesson of the section. A large value of $\mathcal B_{\mathrm K}(f,g)$ probes the correlation function only at the special point $t=i$. The Krivine parameter $c_{f,g}$ is controlled by the full inverse-majorant series of $H_{f,g}^{-1}$. These are different optimization objectives, and the affine radial family gives a concrete numerical example where optimizing the K\"onig bilinear form does not optimize the Grothendieck rounding value.


==> old/krivine_scheme_v1.tex <==
\section{Krivine Rounding Schemes}
\label{sec:krivine-schemes}

{ 
\color{blue}
Here, we define generalized Krivine rounding schemes~\cite{braverman2011grothendieckconstantstrictlysmaller}. 
Then we talk about how it relates to the grothendieck constant. 
Then we explicitly define the scheme we use. 
Then we talk about how to compute the needed values of the different partition schemes. 
}

\subsection{Definitions}

\begin{definition}[Krivine Rounding Scheme]
    Let $G_1,G_2$ be independent standard Gaussian vectors in $\R^k$. For odd measurable
$f,g:\R^k\to\{-1,1\}$, define the normalized correlation function
\[
 H_{f,g}(t)
 =\frac\pi2 \E\left[f\left(\frac{G_1}{\sqrt2}\right)
 g\left(\frac{tG_1+\sqrt{1-t^2}G_2}{\sqrt2}\right)\right],
 \qquad -1<t<1.
\]
Then $H_{f,g}$ extends to an analytic function on the strip $\{z \in \mathbb{C} : \mathcal{R}(z) \in (-1, 1)\}$. We call $(f, g)$ a Krivine rounding scheme if $H_{f,g}$ is invertible on a neighborhood of the origin, and if we consider the Taylor expansion 
\[
 H_{f,g}^{-1}(\zeta)=\sum_{n\ge1}a_n\zeta^n,
\]
then there exists $\gamma$ so that 
\[
 M(\gamma):=\sum_{n\ge1}|a_n|\gamma^n=1,
\]
\end{definition}


% Thus the hyperplane scheme has $H_0(t)=\arcsin t$. The holomorphic extension and the strip bound used below are proved in Lemma~\ref{lem:strip-bound}.

The usual Krivine preprocessing gives
\[
 K_G\le \frac{\pi}{2\gamma}.
\]
Consequently, it is enough to prove
\[
 \gamma>\rho_*:=\arsinh(1)=\log(1+\sqrt2).
\]

\subsection{The Scheme}

Let
\[
 \mathsf H_3(x)=8x^3-12x
\]
be the physicist's third Hermite polynomial. Put
\[
 \tau=0.03175,
 \qquad
 \eta=\frac{\tau}{\sqrt{48}}
 =0.004582717761692655\ldots .
\]
Define
\[
 f(x,y)=\sgn(y-\eta\mathsf H_3(x)),
 \qquad
 g(x,y)=\sgn(y+\eta\mathsf H_3(x)).
\]
Equivalently, if
\[
 \psi_n(x)=\frac{\mathsf H_n(x)}{\sqrt{2^n n!}}
\]
is the orthonormal physicist-Hermite basis for
$d\mu(x)=\pi^{-1/2}e^{-x^2}\,dx$, then
\[
 f(x,y)=\sgn(y-\tau\psi_3(x)),
 \qquad
 g(x,y)=f(-x,y).
\]
Let $H=H_{f,g}$ be the associated arcsine-normalized correlation function.

The coefficients of $H$ can be computed as follows. Expand
\[
 f(x,y)=\sum_{a,b\ge0}F_{a,b}\psi_a(x)\psi_b(y).
\]
Since $g(x,y)=f(-x,y)$, the coefficient of $\psi_a(x)\psi_b(y)$ in $g$ is
$(-1)^aF_{a,b}$. Hence Mehler diagonalization gives
\[
 \boxed{
 H(z)=\frac\pi2\sum_{a,b\ge0}(-1)^aF_{a,b}^2z^{a+b}.}
\]
Moreover
\[
 F_{a,b}=\int_\R \psi_a(x)S_b(\tau\psi_3(x))\,d\mu(x),
\]
where
\[
 S_0(u)=-\erf(u),
\]
and for $b\ge1$,
\[
 S_b(u)=\frac{2}{\sqrt\pi}\frac{e^{-u^2}\psi_{b-1}(u)}{\sqrt{2b}}.
\]
Thus each coefficient $[z^n]H(z)$ is given by the finite sum
\[
 [z^n]H(z)=\frac\pi2\sum_{a=0}^n(-1)^aF_{a,n-a}^2.
\]

\begin{theorem}
For the pair $(f,g)$ above, the pure planar $h_3/-h_3$ scheme is a Krivine rounding
scheme with parameter $\gamma$ satisfying
\[
 \rho_*+4.8\cdot 10^{-6}<\gamma<\rho_*+5.2\cdot 10^{-6}.
\]
In particular,
\[
 K_G\le \frac\pi{2\gamma}<\frac\pi{2\log(1+\sqrt2)}.
\]
\end{theorem}



==> old/krivine_scheme_v2.tex <==
\section{Krivine Rounding Schemes}
\label{sec:krivine-schemes}

{ 
\color{blue}
Here, we define generalized Krivine rounding schemes~\cite{braverman2011grothendieckconstantstrictlysmaller}. 
Then we talk about how it relates to the grothendieck constant. 
Then we explicitly define the scheme we use. 
Then we talk about how to compute the needed values of the different partition schemes. 
}

\begin{definition}[Gaussian correlation]\label{def:gaussian-correlation}
\source{Krivine/BMMN.}
Fix $k \in \mathbb{N}$, and let $f,g:\mathbb{R}^k\to\{-1,1\}$ be odd measurable functions.
Let $G_1,G_2$ be independent standard Gaussian vectors in $\mathbb{R}^k$.

The \emph{arcsine-normalized correlation} associated to $(f,g)$ is
\[
H_{f,g}(t)
:=
\frac{\pi}{2}\,
\mathbb{E}\left[
f\left(\frac{G_1}{\sqrt{2}}\right)
g\left(
\frac{tG_1+\sqrt{1-t^2}G_2}{\sqrt{2}}
\right)
\right],
\qquad -1<t<1.
\]
\end{definition}

\begin{lemma}[Basic analytic properties]\label{lem:correlation-profile-analytic}
Let $f,g:\mathbb{R}^k\to\{-1,1\}$ be odd measurable functions. Then $H_{f,g}$ is odd and
extends holomorphically to the strip
\[
S:=\{z\in\mathbb{C}: |\operatorname{Re}z|<1\}.
\]
In particular, if $H_{f,g}'(0)\neq 0$, then $H_{f,g}$ has a unique local inverse branch at
the origin, and this inverse branch is odd.
\end{lemma}

\begin{proof}
\source{BMMN.}
This is the standard analytic continuation of the Gaussian correlation kernel.  In the planar case used below we prove the stronger quantitative version in Lemma~\ref{lem:strip-bound}.
\end{proof}

\begin{definition}[Inverse majorant]\label{def:inverse-majorant}
Assume $H_{f,g}'(0)\neq 0$, and write the local inverse branch at the origin as
\[
H_{f,g}^{-1}(\zeta)=\sum_{n\ge 1} a_n \zeta^n .
\]
For $s\ge 0$, define the inverse-majorant series
\[
M_{f,g}(s):=\sum_{n\ge 1}|a_n|s^n,
\]
with the convention that $M_{f,g}(s)=+\infty$ if the series diverges.
\end{definition}

\begin{definition}[$\gamma$-admissible Krivine scheme]\label{def:gamma-admissible}
\source{Krivine/BMMN.}
Let $\gamma>0$. We say that $(f,g)$ is a \emph{$\gamma$-admissible Krivine rounding scheme}
if:
\begin{enumerate}[label=(\roman*)]
    \item $f,g:\mathbb{R}^k\to\{-1,1\}$ are odd and measurable;
    \item $H_{f,g}'(0)\neq 0$;
    \item the inverse-majorant inequality
    \[
    M_{f,g}(\gamma)=\sum_{n\ge 1}|a_n|\gamma^n \le 1
    \]
    holds.
\end{enumerate}
We call $(f,g)$ a \emph{Krivine rounding scheme} if it is $\gamma$-admissible for some
$\gamma>0$.
\end{definition}

\begin{theorem}[Krivine preprocessing in arcsine units]\label{thm:krivine-preprocessing}
If $(f,g)$ is a $\gamma$-admissible Krivine rounding scheme, then
\[
K_G \le \frac{\pi}{2\gamma}.
\]
\end{theorem}

\begin{proof}
\source{Krivine/BMMN.}
This is the standard Krivine preprocessing argument.  In the unnormalized convention it gives $K_G\le 1/c$; the present arcsine normalization is $c=2\gamma/\pi$, giving $K_G\le \pi/(2\gamma)$.  The use of $M_{f,g}(\gamma)\le 1$ rather than equality is harmless: the usual tensor-power embeddings have squared norm at most one, and one pads them by orthogonal coordinates to make them unit vectors.
\end{proof}

\subsection{The Scheme}

\begin{definition}[The $H_3$ scheme]\label{def:h3-scheme}
Let
\[
H_3(x)=8x^3-12x,
\qquad
\tau=0.03175,
\qquad
\eta=\frac{\tau}{\sqrt{48}}
=0.004582717761692655\ldots .
\]
Define odd measurable functions $f,g:\R^2\to\{\pm1\}$ by
\[
    f(x,y)=\sgn(y-\eta H_3(x)),
    \qquad
    g(x,y)=\sgn(y+\eta H_3(x)).
\]
We call $(f,g)$ the $H_3$ scheme.
\end{definition}

The following is our main theorem.
\begin{tcolorbox}
\begin{theorem}[No Mixing Beats Hyperplane]\label{thm:no-mixing-beats-hyperplane}
Let
\[
\rhostarval:=\log(1+\sqrt2),
\qquad
\gzero:=\rhostarval+4.8\cdot 10^{-6}.
\]
Then the $H_3$ scheme is a $\gzero$-admissible Krivine scheme.  In particular,
\[
K_G
\le \frac{\pi}{2\gzero}
<
\frac{\pi}{2\log(1+\sqrt2)}
-
9.7\cdot 10^{-6}.
\]
\end{theorem}
\end{tcolorbox}

==> old/mixing_discussion_section.tex <==
\section{Discussion: why mixing can improve the inverse majorant}
\label{sec:discussion-mixing}

In this paper, we observe a different and more interesting phenomenon. A mixture of two
rounding schemes can sometimes give a \emph{strictly} better Grothendieck bound than either
scheme gives individually. Intuitively, different schemes should be thought of as performing
well on different difficult configurations of vectors. A randomized mixture can combine the
strengths of different schemes, and this changes the search problem for rounding schemes:
one should optimize not only over individual partitions, but also over the simplex of mixtures
of promising partitions.

There is a concrete analytic mechanism behind this phenomenon.  Consider two odd correlation
profiles
\[
    H^{(0)}(z)=\sum_{m\ge 0} b^{(0)}_{2m+1} z^{2m+1},
    \qquad
    H^{(1)}(z)=\sum_{m\ge 0} b^{(1)}_{2m+1} z^{2m+1},
\]
and mix them with parameter $p\in[0,1]$:
\[
    H_p(z)=(1-p)H^{(0)}(z)+pH^{(1)}(z)
          =\sum_{m\ge 0} b_{2m+1}(p)z^{2m+1}.
\]
The profile coefficients are affine functions of the mixing parameter,
\[
    b_{2m+1}(p)=(1-p)b^{(0)}_{2m+1}+p b^{(1)}_{2m+1}.
\]
However, the inverse coefficients are not affine.  Writing
\[
    H_p^{-1}(\zeta)=\sum_{m\ge 0} a_{2m+1}(p)\zeta^{2m+1},
\]
the first few coefficients are
\[
\begin{aligned}
    a_1(p) &= \frac{1}{b_1(p)},\\
    a_3(p) &= -\frac{b_3(p)}{b_1(p)^4},\\
    a_5(p) &= \frac{3b_3(p)^2-b_1(p)b_5(p)}{b_1(p)^7},\\
    a_7(p) &= \frac{-12b_3(p)^3+8b_1(p)b_3(p)b_5(p)-b_1(p)^2b_7(p)}{b_1(p)^{10}}.
\end{aligned}
\]
Thus mixing is linear before inversion but nonlinear after inversion.  More generally, each
$a_{2m+1}(p)$ is a rational function of $b_1(p),b_3(p),\ldots,b_{2m+1}(p)$.  Consequently, as
long as $b_1(p)=H_p'(0)$ does not vanish on the interval under consideration, the inverse
coefficients $a_{2m+1}(p)$ are real-analytic, and in particular continuous, functions of $p$.
This is the precise sense in which the coefficients of the inverse series vary smoothly with
the mixing parameter.

The Grothendieck bound is then controlled by the inverse-majorant condition
\[
    M_p(\gamma) := \sum_{m\ge 0} |a_{2m+1}(p)|\gamma^{2m+1} \le 1,
\]
with the resulting bound $K_G\le \pi/(2\gamma)$ in our normalization.  Therefore the search
tries to make the absolute-value series $M_p$ small, or equivalently to make the admissible
root $\gamma$ large.  A coefficient crossing zero is especially valuable: at a value of $p$ where
$a_{2m+1}(p)=0$, the corresponding contribution $|a_{2m+1}(p)|\gamma^{2m+1}$ disappears from
the majorant.  The other coefficients still move with $p$, but they move smoothly.  Thus, if
the increase in the other terms is smaller than the decrease obtained by cancelling one
troublesome coefficient, the mixed profile can have a smaller majorant than either endpoint
profile.  This is how a mixture can be strictly better than both pure schemes.

This also gives a useful diagnostic for searching over mixtures.  Suppose that the two endpoint
schemes have inverse coefficients $a_7(0)$ and $a_7(1)$ of opposite sign, and suppose that
$H_p'(0)$ remains nonzero for $p\in[0,1]$.  Since $a_7(p)$ is continuous, the intermediate value
theorem gives a mixing parameter $p_*$ for which
\[
    a_7(p_*)=0.
\]
Empirically, this is exactly the pattern we have observed in the best two-atom mixtures: when a
mixed rounding scheme improves on both pure components, it does so by zeroing out one of the
inverse coefficients, and all of our best mixed solutions zero out the $a_7$ coefficient.  In the
same solutions, the two pure components being mixed have $a_7$ coefficients with opposite signs.
This should not be interpreted as a theorem that $a_7$ is universally special; it is an empirical
structural feature of the present search family.  Nevertheless, it explains why the best mixtures
are not merely averages of good schemes.  They are calibrated cancellations in the inverse
series, found by mixing profiles whose inverse-majorant errors point in opposite directions.

The practical consequence is that the search space should include mixtures even when the atoms
are not individually optimal.  A dictionary of imperfect rounding schemes may contain pairs with
complementary signs in a dominant inverse coefficient.  Optimizing the mixture weights can then
place the mixed profile near a zero of that coefficient, reducing the absolute-value majorant and
thereby supporting a larger value of $\gamma$ than either component supports on its own.


==> old/mixing_discussion_section_v2.tex <==
\section{Discussion: why mixing can improve the inverse majorant}
\label{sec:discussion-mixing}

One of the main finding in this paper is that a mixture of two
rounding schemes can sometimes give a \emph{strictly} better Grothendieck bound than either
scheme gives individually. Intuitively, different schemes should be thought of as performing
well on different difficult configurations of vectors. A randomized mixture can combine the
strengths of different schemes, and thus improving its performance against any adverserially chosen vectors. This changes the search problem for rounding schemes:
one should optimize not only over individual partitions, but also over the simplex of mixtures
of promising partitions.

There is an analytic mechanism for this that is visible at the series level.  For two schemes, the mixed
correlation profile has Taylor coefficients
$b_{2m+1}(p)=(1-p)b^{(0)}_{2m+1}+p b^{(1)}_{2m+1}$, but the coefficients of
$H_p^{-1}(\zeta)=\sum_{m\ge 0}a_{2m+1}(p)\zeta^{2m+1}$ are not mixed linearly.  Indeed,
the identity $H_p(H_p^{-1}(\zeta))=\zeta$ determines these coefficients recursively:
after $a_1(p),\ldots,a_{2m-1}(p)$ have been determined, the coefficient of
$\zeta^{2m+1}$ is a linear equation for $a_{2m+1}(p)$ with leading factor $b_1(p)$.
Equivalently, by Lagrange inversion, $a_{2m+1}(p)$ is a rational function of
$b_1(p),b_3(p),\ldots,b_{2m+1}(p)$, with denominators involving powers of $b_1(p)$.
Thus, on any interval where $b_1(p)=H_p'(0)$ does not vanish, each inverse coefficient
$a_{2m+1}(p)$ is a real-analytic, in particular continuous, function of the mixing parameter $p$.

The Grothendieck bound is controlled by the inverse-majorant condition
\[
    M_p(\gamma) := \sum_{m\ge 0} |a_{2m+1}(p)|\gamma^{2m+1} \le 1,
\]
so the search tries to reduce an absolute-value series.  A zero of one inverse coefficient is
therefore especially valuable: at such a parameter the corresponding term disappears from
$M_p(\gamma)$. This is the basic reason a mixed profile can beat
both endpoint profiles, even though the original correlation coefficients are only being
averaged.

This gives a useful diagnostic for two-atom mixtures.  If the endpoint schemes have $a_7(0)$
and $a_7(1)$ of opposite signs, and if $b_1(p)\neq 0$ on the interval, then continuity gives a
mixing parameter $p_*$ with $a_7(p_*)=0$.  Empirically, this is the pattern seen in our best
mixed solutions: when a mixture improves on both pure components, it does so by zeroing out
one of the inverse coefficients, and in all of the best cases found so far the cancelled
coefficient is $a_7$.  In these cases the two pure components have $a_7$ coefficients with
opposite signs.  This should not be read as a evidence that $a_7$ is necessarily special, but
it explains the observed role of mixing as a calibrated cancellation in the inverse-majorant
series rather than as a mere average of two good schemes. An open question is whether there exists better mixed schemes that zero out an earlier a-series coefficient such as $a_5$. If it is able to keep the $a_1$ and $a_3$ ceofficients relatively unchanged, then one would expect a siginificant improvement to $K_G$ over our current result.


==> old/problem_formulation.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{images/grothendieck_proof_graph.png}
    \caption{Proof graph of grothendieck}
    \label{fig:proof_graph_grothendieck}
\end{figure}

Mathematical statements are expressed with \textit{propositions}.
Let \(\msf{Prop}\) be the set of all propositions.

Importantly, propositions may entail one another.
To computationally certify entailment, however, we require access to a verifier model.
Given two propositions \(P, Q \in \msf{Prop}\) and verifier \(\mcal{L}\), we write \(P \vDash_{\mcal{L}} Q\) to mean that the verifier \(\mcal{L}\) can certify that \(P\) entails \(Q\).

A theorem and its proof may thus be viewed as a pairing of propositions, taking the form \((T, P)\) for \(T, P \in \msf{Prop}\).
In mathematics, proofs often invoke prior theorems and lemmas, which motivates the use of a directed acyclic graph to capture reasoning dependencies.


A proof graph is a DAG \(\mcal{G} = (\mcal{V}, \mcal{E}, v^\star)\), where each vertex is labeled with a theorem-proof pair of the form \(v = (T_v, P_v)\).


A node \(v = (T_v, P_v)\) in a proof graph is \textit{entailed} if \(T_v\) is entailed by the conjunction of \(P_v\) and the predecessors theorems to \(v\).
Specifically, we require that:
\begin{equation}
    P_v \land \msf{Prev}(v)
    \vDash_{\mcal{L}} T_v,
    \quad
    \text{where }
    \msf{Prev}(v) = \bigwedge \{T_u : (T_u, P_u) \text{ is a parent of } v\}.
\end{equation}

As an exception, we admit the special propositions \(\msf{Sorry}, \msf{Axiom} \in \msf{Prop}\) that automatically entail any proposition; such propositions are used to denote whether a node in the proof graph should be taken as incomplete (\(\msf{Sorry}\)), or as an axiom (\(\msf{Axiom}\)).


We say that a proof graph is \textit{consistent} if all nodes are entailed, and there is no \(\msf{Sorry}\) in any of the proofs.

In our case, a proof graph must end at a sink node. The sink node is a result of the form $\kappa \le \kappa_0$. 


Note that any node has a forward cone of influence. Any changes to a node will propagate downwards to the sink, potentially changing the result. 

A proof graph allows edits of the form - 
\begin{itemize}
    \item Modify the result of a node (e.g. strengthening)  
    \item Add a node (e.g. a lemma or a definition) 
    \item Delete an unused node (e.g. an orphaned node)
\end{itemize}
Given a proof graph $G$, we say $G'$ is a \textit{refinemment} of $G$ if the resulting sink node of $G'$ proves $\kappa \le \kappa_0' \le \kappa_0$, i.e. it strengthens the bound result. 

A refinement sequence is a sequence $G_0, G_1, \cdots$ where each graph is a refinement of the previous one. The objective then, is to find a sequence of refinements to find the best resulting bound. 

{\color{red} This is not the same as merely doing minor parameter tuning. It searches over proofs. It modifies theorems, lemmas, proof chains. It introduces new definitions. It is a general problem that has many applications, this needs to be stressed.} 


{\color{red} EXAMPLES: It's extremely important for us to give examples of what these refinements look like. For example, lemma 4.2 strengthening, parameter strengthening, introducing a stronger lemma, deleting an orphaned lemma. We need to show it in a way that makes it clear that new math is happening. TODO: Find instructive examples.}

\begin{center}
\begin{tikzpicture}[scale=0.8, transform shape, node distance=1.0cm and 1.2cm]
  \node[nodebox, minimum width=2.7cm] (h5) {\textbf{Hermite identities}\\[-1mm]\scriptsize $h_5$, moments};
  \node[nodebox, minimum width=2.7cm, right=of h5] (heta) {\textbf{$H_\eta$ analytic}\\[-1mm]\scriptsize $\mathcal S_H(B_H)$};
  \node[bluebox, minimum width=2.7cm, right=of heta] (phi) {\textbf{$\Phi$ estimates}\\[-1mm]\scriptsize derivative bounds};
  \node[nodebox, minimum width=2.7cm, below=1.1cm of h5] (fp) {\textbf{$F_p$ inverse}\\[-1mm]\scriptsize analytic inverse};
  \node[amberbox, minimum width=2.8cm, below=1.1cm of heta] (gamma) {\textbf{coefficient bound}\\[-1mm]\scriptsize $\sum |a_k|\gamma^k=1$};
  \node[nodebox, minimum width=2.7cm, below=1.1cm of phi] (kriv) {\textbf{Krivine step}\\[-1mm]\scriptsize preprocessing};
  \node[nodebox, minimum width=2.8cm, below=1.2cm of gamma] (round) {\textbf{rounding lemma}\\[-1mm]\scriptsize random projection};
  \node[sink, minimum width=2.3cm, below=1.0cm of round] (kg) {\textbf{final bound}\\[-1mm]\scriptsize $K_G\le \kappa$};

  \draw[arr] (h5) -- (heta); \draw[arr] (heta) -- (phi); \draw[arr] (heta) -- (fp); \draw[arr] (phi) -- (gamma); \draw[arr] (fp) -- (gamma); \draw[arr] (kriv) -- (round); \draw[arr] (gamma) -- (round); \draw[arr] (round) -- (kg);

  % \node[panelbox, text width=4.15cm, anchor=north west] at (-5.0,3.0) {\textbf{Node payload}\vspace{1mm}\\\scriptsize theorem family $\mathcal S_v:\Theta_v\to\mathsf{Prop}$\\\scriptsize certificate $\theta_v\in\Theta_v$\\\scriptsize local proof $\pi_v:\bigwedge_{u\to v}\mathcal S_u(\theta_u)\to \mathcal S_v(\theta_v)$};
  % \node[panelbox, text width=4.1cm, anchor=north east] at (5.0,3.0) {\textbf{Graph invariant}\vspace{1mm}\\\scriptsize finite DAG with sink $t$\\\scriptsize every node locally certified\\\scriptsize terminal value $\operatorname{val}(G)=\theta_t$};
  \draw[decorate, decoration={brace,mirror,amplitude=5pt}, draw=muted] ($(fp.south west)+(0,-.25)$) -- ($(kriv.south east)+(0,-.25)$) 
  node[pos=0.30, below=6pt, xshift=6pt, tiny, align=center]{intermediate constants\\propagate to the sink};
\end{tikzpicture}
\end{center}
% \begin{center}
% \begin{tikzpicture}[
%   scale=0.76,
%   transform shape,
%   node distance=0.85cm and 0.95cm,
%   panel/.style={
%     rounded corners=12pt,
%     inner sep=10pt,
%     draw=#1,
%     fill=#1!10,
%     line width=.7pt
%   }
% ]

% % Requires in preamble:
% % \usetikzlibrary{positioning,fit,calc,backgrounds,arrows.meta}

% % ---------------- left graph ----------------

% \node[oldbox, minimum width=2.0cm] (a) at (0,1.75)
%   {Hermite\\[-1mm]\scriptsize identities};

% \node[amberbox, minimum width=2.35cm, right=of a] (b)
%   {$H_\eta$ bound\\[-1mm]\scriptsize $B_H$};

% \node[oldbox, minimum width=2.25cm, right=of b] (c)
%   {$F_p^{-1}$\\[-1mm]\scriptsize radius $r$};

% \node[amberbox, minimum width=2.35cm, below=of c] (d)
%   {$\gamma$ certificate\\[-1mm]\scriptsize $\gamma$};

% \node[sink, minimum width=2.15cm, below=of d] (e)
%   {terminal\\[-1mm]\scriptsize $K_G\le\kappa$};

% \node[oldbox, minimum width=2.0cm, below=of a] (u)
%   {unrelated\\[-1mm]\scriptsize unchanged};

% % ---------------- right graph ----------------

% \node[oldbox, minimum width=2.0cm] (aa) at (11.0,1.75)
%   {Hermite\\[-1mm]\scriptsize identities};

% \node[newbox, minimum width=2.35cm, right=of aa] (bb)
%   {$H_\eta$ bound\\[-1mm]\scriptsize $B'_H\prec B_H$};

% \node[newbox, minimum width=2.25cm, right=of bb] (cc)
%   {$F_p^{-1}$\\[-1mm]\scriptsize better radius};

% \node[amberbox, minimum width=2.35cm, below=of cc] (dd)
%   {$\gamma'$ certificate\\[-1mm]\scriptsize $\gamma'>\gamma$};

% \node[sink, minimum width=2.15cm, below=of dd] (ee)
%   {terminal\\[-1mm]\scriptsize $K_G\le\kappa'<\kappa$};

% \node[oldbox, minimum width=2.0cm, below=of aa] (uu)
%   {unrelated\\[-1mm]\scriptsize unchanged};

% % ---------------- panels behind nodes ----------------

% \begin{scope}[on background layer]
%   \node[
%     panel=amber,
%     fit=(b)(c)(d)(e),
%     label={[badge, fill=amber, yshift=2pt]above:forward cone $\operatorname{Up}_G(H_\eta)$}
%   ] (leftpanel) {};

%   \node[
%     panel=green!70!black,
%     fit=(bb)(cc)(dd)(ee),
%     label={[badge, fill=green, yshift=2pt]above:same cone, improved values}
%   ] (rightpanel) {};
% \end{scope}

% % ---------------- edges ----------------

% \draw[arrmuted] (a) -- (b);
% \draw[arramber] (b) -- (c);
% \draw[arramber] (c) -- (d);
% \draw[arramber] (d) -- (e);
% \draw[arrmuted] (u) -- (e);

% \draw[arrmuted] (aa) -- (bb);
% \draw[arrgreen] (bb) -- (cc);
% \draw[arrgreen] (cc) -- (dd);
% \draw[arrgreen] (dd) -- (ee);
% \draw[arrmuted] (uu) -- (ee);

% % ---------------- edit arrow ----------------

% \draw[-{Latex[length=3mm,width=2mm]}, draw=blue, line width=1.1pt]
%   ($(leftpanel.east)+(0.5,0)$) -- ($(rightpanel.west)+(-2.8,0)$)
%   node[midway, above=3pt, scriptsize] {valid edit};

% \end{tikzpicture}
% \end{center}

==> old/proof_outline_v1.tex <==
\newcommand{\source}[1]{{\color{blue}\textsc{#1}}}
\newcommand{\gzero}{\gamma_0}
\newcommand{\rhostarval}{\rho_*}
\crefname{definition}{Definition}{Definitions}
\Crefname{definition}{Definition}{Definitions}
\crefname{theorem}{Theorem}{Theorems}
\Crefname{theorem}{Theorem}{Theorems}
\crefname{lemma}{Lemma}{Lemmas}
\Crefname{lemma}{Lemma}{Lemmas}
\crefname{corollary}{Corollary}{Corollaries}
\Crefname{corollary}{Corollary}{Corollaries}
\crefname{remark}{Remark}{Remarks}
\Crefname{remark}{Remark}{Remarks}



\section{The no-mixing theorem}

\begin{definition}[Real Grothendieck constant]\label{def:real-grothendieck-constant}
\source{Grothendieck.}
The real Grothendieck constant $K_G$ is the infimum over all $K>0$ such that, for every $m,n\in\mathbb N$ and every real matrix $A=(a_{ij})\in\R^{m\times n}$,
\[
\max_{x_i,y_j\in S^{m+n-1}}
\sum_{i=1}^m\sum_{j=1}^n a_{ij}\ip{x_i}{y_j}
\le
K\max_{\varepsilon_i,\delta_j\in\{-1,1\}}
\sum_{i=1}^m\sum_{j=1}^n a_{ij}\varepsilon_i\delta_j .
\]
\end{definition}

\begin{definition}[Gaussian correlation]\label{def:gaussian-correlation}
\source{Krivine/BMMN.}
Fix $k \in \mathbb{N}$, and let $f,g:\mathbb{R}^k\to\{-1,1\}$ be odd measurable functions.
Let $G_1,G_2$ be independent standard Gaussian vectors in $\mathbb{R}^k$.

The \emph{arcsine-normalized correlation} associated to $(f,g)$ is
\[
H_{f,g}(t)
:=
\frac{\pi}{2}\,
\mathbb{E}\left[
f\left(\frac{G_1}{\sqrt{2}}\right)
g\left(
\frac{tG_1+\sqrt{1-t^2}G_2}{\sqrt{2}}
\right)
\right],
\qquad -1<t<1.
\]
\end{definition}

Krivine rounding scheme as abstracted in \cite{braverman2011grothendieckconstantstrictlysmaller} shows the following. 



\begin{lemma}[Basic analytic properties]\label{lem:correlation-profile-analytic}
Let $f,g:\mathbb{R}^k\to\{-1,1\}$ be odd measurable functions. Then $H_{f,g}$ is odd and
extends holomorphically to the strip
\[
S:=\{z\in\mathbb{C}: |\operatorname{Re}z|<1\}.
\]
In particular, if $H_{f,g}'(0)\neq 0$, then $H_{f,g}$ has a unique local inverse branch at
the origin, and this inverse branch is odd.
\end{lemma}
\begin{proof}
\source{BMMN.}
This is the standard analytic continuation of the Gaussian correlation kernel.  In the planar case used below we prove the stronger quantitative version in Lemma~\ref{lem:strip-bound}.
\end{proof}

\begin{lemma}[Krivine Rounding Scheme]\label{lm:krivinerounding}

Let $f,g:\mathbb{R}^k\to\{-1,1\}$ be odd and measurable functions with $H'_{f,g}(0) \neq 0$. Let $H^{-1}_{f,g}$ be the unique local inverse branch of $H_{f,g}$ at the origin. Then,
\begin{itemize}
\item $H^{-1}_{f,g}$ is odd. 
    \item $H^{-1}_{f,g}$ has a Taylor-series expansion at the origin: $H^{-1}_{f,g}(\zeta) = \sum_{n\geq 1} a_n \zeta^n$. 
\end{itemize}

Further, if $\gamma > 0$ is such that $\sum_{n \geq 1} |a_n| \gamma^n \leq 1$, then the Grothendieck constant 
$$ K_G \leq \frac{\pi}{2\gamma}.$$ 
\end{lemma}

\begin{definition}
    For $f,g:\mathbb{R}^k\to\{-1,1\}$ odd and measurable functions with $H'_{f,g}(0) \neq 0$, and $\gamma > 0$, we say $(f,g)$ is a $\gamma$-admissible Krivine rounding scheme if the conditions of \cref{lm:krivinerounding} hold. 
\end{definition}

For completeness, we give a proof of this with our notation in the appendix. 



\begin{definition}[Inverse majorant]\label{def:inverse-majorant}
Assume $H_{f,g}'(0)\neq 0$, and write the local inverse branch at the origin as
\[
H_{f,g}^{-1}(\zeta)=\sum_{n\ge 1} a_n \zeta^n .
\]
For $s\ge 0$, define the inverse-majorant series
\[
M_{f,g}(s):=\sum_{n\ge 1}|a_n|s^n,
\]
with the convention that $M_{f,g}(s)=+\infty$ if the series diverges.
\end{definition}

\begin{definition}[$\gamma$-admissible Krivine scheme]\label{def:gamma-admissible}
\source{Krivine/BMMN.}
Let $\gamma>0$. We say that $(f,g)$ is a \emph{$\gamma$-admissible Krivine rounding scheme}
if:
\begin{enumerate}[label=(\roman*)]
    \item $f,g:\mathbb{R}^k\to\{-1,1\}$ are odd and measurable;
    \item $H_{f,g}'(0)\neq 0$;
    \item the inverse-majorant inequality
    \[
    M_{f,g}(\gamma)=\sum_{n\ge 1}|a_n|\gamma^n \le 1
    \]
    holds.
\end{enumerate}
We call $(f,g)$ a \emph{Krivine rounding scheme} if it is $\gamma$-admissible for some
$\gamma>0$.
\end{definition}

\begin{theorem}[Krivine preprocessing in arcsine units]\label{thm:krivine-preprocessing}
If $(f,g)$ is a $\gamma$-admissible Krivine rounding scheme, then
\[
K_G \le \frac{\pi}{2\gamma}.
\]
\end{theorem}

\begin{proof}
\source{Krivine/BMMN.}
This is the standard Krivine preprocessing argument.  In the unnormalized convention it gives $K_G\le 1/c$; the present arcsine normalization is $c=2\gamma/\pi$, giving $K_G\le \pi/(2\gamma)$.  The use of $M_{f,g}(\gamma)\le 1$ rather than equality is harmless: the usual tensor-power embeddings have squared norm at most one, and one pads them by orthogonal coordinates to make them unit vectors.
\end{proof}

\begin{definition}[The $H_3$ scheme]\label{def:h3-scheme}
Let
\[
H_3(x)=8x^3-12x,
\qquad
\tau=0.03175,
\qquad
\eta=\frac{\tau}{\sqrt{48}}
=0.004582717761692655\ldots .
\]
Define odd measurable functions $f,g:\R^2\to\{\pm1\}$ by
\[
    f(x,y)=\sgn(y-\eta H_3(x)),
    \qquad
    g(x,y)=\sgn(y+\eta H_3(x)).
\]
We call $(f,g)$ the $H_3$ scheme.
\end{definition}

The following is our main theorem.
\begin{tcolorbox}
\begin{theorem}[Improved Grothendieck Constant]\label{thm:no-mixing-beats-hyperplane}
Let
\[
\rhostarval:=\log(1+\sqrt2),
\qquad
\gzero:=\rhostarval+4.8\cdot 10^{-6}.
\]
Then the $H_3$ scheme is a $\gzero$-admissible Krivine scheme.  In particular,
\[
K_G
\le \frac{\pi}{2\gzero}
<
\frac{\pi}{2\log(1+\sqrt2)}
-
9.7\cdot 10^{-6}.
\]
\end{theorem}
\end{tcolorbox}

The proof has two main components. Recall that using \cref{lm:krivinerounding}, the main goal is to show that 

$$\sum_{n \geq 1} |a_n| \gamma_0^n \leq 1,$$

where $((a_n): n \geq 1)$ are the Taylor-series coefficients of $H_{f,g}^{-1}$. We split this into parts.
\begin{itemize}
    \item An analytic argument that bounds the remainder term---$\sum_{n > k_0} |a_n| \gamma_0^n$---to very good precision (about $2.44 \cdot 10^{-9}$) for $k_0 = 220$. This analytic portion relies on elementary complex analysis and carefully chosen contour integration. This approach can also extend to schemes similar to $H_3$ scheme. See \cref{sec:analytic}.
    \item A numerical analysis portion that uses \texttt{Arb} \cite{johansson2017arb} to compute the \emph{head}, $\sum_{n \leq k_0} |a_n| \gamma_0^n$ to very high precision showing that this value is less than $1 - 2.5 \cdot 10^{-9}$. We discuss the challenges involved here and the certification of this computation in \cref{sec:numerical}. 
    
    
\end{itemize}

\section{Bounding the Remainder Analytically}\label{sec:analytic}

We now give our main analytic argument to bound the remainder term of majorant Taylor-series of $H_{f,g}^{-1}$ for the $H_3$ scheme. This argument potentially extends to other schemes as well.

\begin{lemma}[Majorant tail bound]\label{lemma:tail-bound}
Let $(f,g)$ be the $H_3$ scheme and let  
\[
H_{f,g}^{-1}(\zeta)=\sum_{n\ge1}a_n\zeta^n,
\qquad
\gzero=\log(1+\sqrt2)+4.8\cdot10^{-6}.
\]
Then
\[
\sum_{n>220}|a_n|\gzero^n<2.5\cdot10^{-9}.
\]
\end{lemma}

{\color{blue} Might be confusing to have $H_{f,g}$ and $H_3$, potentially change notation.}

For brevity, in the rest of this section we assume $(f,g)$ are fixed to be the $H_3$ scheme and we write $H^{-1}$ instead of $H^{-1}_{f,g}$.

\section{Numerical Computation of the Head}

We next describe how the computation of the head portion is done for the $H_3$ scheme. This leads to the following numerically verified claim:

\begin{lemma}
    Let
\[
 M_{f,g}(s)=\sum_{n\ge 1} |a_n|s^n
\]
be the inverse majorant for the $H_3$ scheme.  For
\[
\gzero=\log(1+\sqrt2)+4.8\cdot10^{-6},
\]
one has
\[
\sum_{1\le n\le220}|a_n|\gzero^n
<1-2.5\cdot10^{-9}.
\]
\end{lemma}



\paragraph{Proof architecture.}
The proof has two independent modules after the scheme is fixed.  The analytic module proves a uniform inverse disk; the numerical module computes the inverse-majorant head and uses the analytic disk for the tail:
\[
\begin{array}{ccccc}
Lemma~\ref{lem:strip-bound}
&\Longrightarrow&
Lemma~\ref{lem:sine-coordinate-bound}
&\Longrightarrow&
Corollary~\ref{cor:F-inverse-radius}
\Longrightarrow
Corollary~\ref{cor:H-inverse-radius}
\\[0.5em]
&&&&\Downarrow
\\[-0.1em]
Lemma~\ref{lem:majorant-head-value}
&+&
Lemma~\ref{lemma:tail-bound}
&\Longrightarrow&
Corollary~\ref{cor:gamma0-admissibility}
\Longrightarrow
Theorem~\ref{thm:no-mixing-beats-hyperplane}.
\end{array}
\]
\paragraph{Proof plan.}
The proof has two parts. First, we prove an analytic inverse disk for the correlation profile. The
main device is the change of variables
\[
F(w):=H(\sin w),
\]
which is useful because the hyperplane profile becomes the identity map in this coordinate. This
allows us to use Rouché's theorem to control the inverse branch uniformly. Second, using this
inverse disk, we certify the inverse-majorant by splitting it into a finite head and a Cauchy tail:
the head is computed with Arb through degree $220$, and the tail is bounded analytically from the
inverse disk. Combining these two estimates gives $M_{f,g}(\gamma_0)<1$, so the $H_3$ scheme is
$\gamma_0$-admissible and the desired bound on $K_G$ follows.
\section{The analytic inverse disk}

\begin{lemma}[Strip bound]\label{lem:strip-bound}
Let $f,g:\R^2\to\{-1,1\}$ be measurable and let $H=H_{f,g}$ be the
arcsine-normalized correlation function.
Then $H$ extends holomorphically to
\[
 S=\{z\in\C: |\operatorname{Re}z|<1\}.
\]
Moreover, if $z=a+ib\in S$, then
\[
 |H(z)|\le \frac{\pi}{2}\frac{|1-z^2|}{1-a^2}.
\]
\end{lemma}

\begin{proof}
For real $|t|<1$, the arcsine-normalized correlation admits the integral representation
\[
H(t)=\frac{1}{2\pi(1-t^2)}
\int_{\R^2}\int_{\R^2}
f(x)g(y)
\exp\left(
-\frac{\|x\|^2+\|y\|^2-2t\ip{x}{y}}{1-t^2}
\right)\,dx\,dy .
\]
For $z\in S$, this formula defines the candidate holomorphic extension.  Since $|f|=|g|=1$,
\[
|H(z)|\le
\frac{1}{2\pi |1-z^2|}
\int_{\R^2}\int_{\R^2}
\exp\left(
-\operatorname{Re}\frac{\|x\|^2+\|y\|^2-2z\ip{x}{y}}{1-z^2}
\right)\,dx\,dy .
\]
Use the identity
\[
\frac{\|x\|^2+\|y\|^2-2z\ip{x}{y}}{1-z^2}
=
\frac12\frac{\|x+y\|^2}{1+z}
+
\frac12\frac{\|x-y\|^2}{1-z}.
\]
Writing $z=a+ib$, set
\[
A_+ := \operatorname{Re}\frac{1}{1+z}
=\frac{1+a}{(1+a)^2+b^2},
\qquad
A_- := \operatorname{Re}\frac{1}{1-z}
=\frac{1-a}{(1-a)^2+b^2}.
\]
Both are positive for $|a|<1$.  With $u=x+y$ and $v=x-y$, the Jacobian from $(u,v)$ to $(x,y)$ in $\R^4$ is $1/4$.  Thus the Gaussian integral is
\[
\frac14\cdot\frac{2\pi}{A_+}\cdot\frac{2\pi}{A_-}
=\frac{\pi^2}{A_+A_-}.
\]
Finally,
\[
A_+A_-=
\frac{1-a^2}{|1+z|^2|1-z|^2}
=
\frac{1-a^2}{|1-z^2|^2}.
\]
Substitution gives
\[
|H(z)|\le
\frac{1}{2\pi |1-z^2|}\cdot
\frac{\pi^2 |1-z^2|^2}{1-a^2}
=
\frac{\pi}{2}\frac{|1-z^2|}{1-a^2}.
\]
The same estimate is uniform on compact subsets of $S$, so the integral converges locally uniformly and the extension is holomorphic by dominated convergence.
\end{proof}

\begin{definition}[The key change of variable]\label{def:key-change-of-variable}
For the rest of the proof, put
\[
F(w)\defeq H(\sin w).
\]
For the hyperplane scheme $H_0(t)=\arcsin t$, hence $H_0(\sin w)=w$ on the principal strip.  This is why the comparison below is made against the identity map.
\end{definition}

\begin{lemma}[Sine-coordinate bound]\label{lem:sine-coordinate-bound}
For $F(w)=H(\sin w)$, the function $F$ is holomorphic on $|w|<1.1$ and
\[
 |F(w)-w|<15.3\qquad (|w|\le1.1).
\]
\end{lemma}

\begin{proof}
Write $w=u+iv$. Then
\[
\operatorname{Re}(\sin w)=\sin u\cosh v.
\]
By Lemma~\ref{lem:disk-to-strip-check}, if $u^2+v^2\le 1.1^2$, then
\[
|\sin u|\cosh v<0.946<1.
\]
Therefore $\sin w\in S$ for $|w|\le 1.1$, and Lemma~\ref{lem:strip-bound} implies that $F$ is holomorphic on $|w|<1.1$.  Applying Lemma~\ref{lem:strip-bound} with $z=\sin w$ gives
\[
|F(w)|
\le
\frac{\pi}{2}\frac{|1-\sin^2 w|}{1-(\operatorname{Re}\sin w)^2}
=
\frac{\pi}{2}\frac{|\cos w|^2}{1-(\operatorname{Re}\sin w)^2}.
\]
By Lemma~\ref{lem:cosine-ratio-check}, the last expression is $<14.19$ on $|w|\le 1.1$.  Hence
\[
|F(w)-w|\le |F(w)|+|w|<14.19+1.1<15.3.
\]
\end{proof}

\begin{lemma}[Rouch\'e inverse disk]\label{lem:rouche-inverse-disk}
Let $F$ be holomorphic on $|w|<r$, with $F(0)=0$, and suppose that for some
$R<M<r$,
\[
 \sup_{|w|=M}|F(w)-w|<M-R.
\]
Then:
\begin{enumerate}[label=(\roman*)]
    \item $F^{-1}$ is holomorphic on $R\D$;
    \item for $|\zeta|<R$, the inverse satisfies $|F^{-1}(\zeta)|<M$.
\end{enumerate}
\end{lemma}

\begin{proof}
Fix $|\zeta|<R$.  On $|w|=M$,
\[
|(F(w)-\zeta)-(w-\zeta)|=|F(w)-w|<M-R<M-|\zeta|\le |w-\zeta|.
\]
By Rouch\'e's theorem, $F(w)-\zeta$ and $w-\zeta$ have the same number of zeros in $|w|<M$, counted with multiplicity.  Since $w-\zeta$ has exactly one zero in this disk, $F(w)=\zeta$ has exactly one solution in $|w|<M$, counted with multiplicity.  In particular, the solution is simple.  The holomorphic inverse function theorem gives local inverse branches, and uniqueness makes these branches glue over $R\D$.  The same argument gives $|F^{-1}(\zeta)|<M$.
\end{proof}

\begin{corollary}[Radius and supremum of $|F^{-1}|$]\label{cor:F-inverse-radius}
Taking $r=1.1$, $R=0.975$, and $M=0.98$, the inverse $F^{-1}$ is holomorphic on $0.975\D$ and
\[
|F^{-1}(\zeta)|<0.98\qquad (|\zeta|<0.975).
\]
\end{corollary}

\begin{proof}
Let
\[
\Delta(w):=F(w)-w=\sum_{n\ge1}d_nw^n.
\]
The Arb coefficient computation gives the finite head estimate
\[
\sum_{n\le 220}|d_n|0.98^n<0.00454106848.
\]
By Lemma~\ref{lem:sine-coordinate-bound} and Cauchy's estimate, taking the Cauchy radius to $1.1$ from below gives
\[
\sum_{n>220}|d_n|0.98^n
\le
15.3\frac{(0.98/1.1)^{221}}{1-0.98/1.1}
<1.149\cdot10^{-9}.
\]
Therefore
\[
\sup_{|w|=0.98}|F(w)-w|
\le
\sum_{n\ge1}|d_n|0.98^n
<0.00454106848+1.149\cdot 10^{-9}
<0.005.
\]
Since $M-R=0.98-0.975=0.005$, Lemma~\ref{lem:rouche-inverse-disk} applies with $r=1.1$, $M=0.98$, and $R=0.975$.
\end{proof}

\begin{corollary}[Radius and supremum of $|H^{-1}|$]\label{cor:H-inverse-radius}
Undoing the change of variables, we get
\[
H^{-1}=\sin\circ F^{-1}.
\]
Thus $H^{-1}$ is holomorphic on $0.975\D$ and
\[
|H^{-1}(\zeta)|<\sinh(0.98)<1.145
\qquad (|\zeta|<0.975).
\]
\end{corollary}

\begin{proof}
Since $F=H\circ\sin$, the identity $F^{-1}=\arcsin\circ H^{-1}$ is equivalent to
$H^{-1}=\sin\circ F^{-1}$ on the inverse branch at the origin.  By Corollary~\ref{cor:F-inverse-radius}, $|F^{-1}(\zeta)|<0.98$ for $|\zeta|<0.975$.  The elementary bound
\[
|\sin z|\le \sinh |z|
\]
for complex $z$ gives
\[
|H^{-1}(\zeta)|=|\sin(F^{-1}(\zeta))|<\sinh(0.98)<1.145.
\]
\end{proof}

\section{The inverse-majorant theorem}

\begin{lemma}[Majorant tail bound]\label{lemma:tail-bound}
Let
\[
H^{-1}(\zeta)=\sum_{n\ge1}a_n\zeta^n,
\qquad
\gzero=\log(1+\sqrt2)+4.8\cdot10^{-6}.
\]
Then
\[
\sum_{n>220}|a_n|\gzero^n<2.5\cdot10^{-9}.
\]
\end{lemma}

\begin{proof}
By Corollary~\ref{cor:H-inverse-radius}, $H^{-1}$ is holomorphic on $0.975\D$ and satisfies $|H^{-1}(\zeta)|<1.145$ there.  Hence, for every $s<0.975$, Cauchy's estimate with radius tending to $0.975$ gives
\[
\sum_{n>220}|a_n|s^n
\le
1.145\frac{(s/0.975)^{221}}{1-s/0.975}.
\]
Taking $s=\gzero$ yields
\[
1.145\frac{(\gzero/0.975)^{221}}{1-\gzero/0.975}
<2.44\cdot10^{-9}
<2.5\cdot10^{-9},
\]
as claimed.
\end{proof}

\begin{lemma}[Majorant head value]\label{lem:majorant-head-value}
Let
\[
 M_{f,g}(s)=\sum_{n\ge 1} |a_n|s^n
\]
be the inversomewhat. se majorant for the $H_3$ scheme.  For
\[
\gzero=\log(1+\sqrt2)+4.8\cdot10^{-6},
\]
one has
\[
\sum_{1\le n\le220}|a_n|\gzero^n
<1-2.5\cdot10^{-9}.
\]
\end{lemma}

\begin{proof}
\source{Arb certificate.}
We record the coefficient computation used by the certificate.  Let $\mathsf H_n$ be the physicist's Hermite polynomial and set
\[
\psi_n(x):=\frac{\mathsf H_n(x)}{\sqrt{2^n n!}},
\qquad
 d\mu(x):=\pi^{-1/2}e^{-x^2}\,dx.
\]
Then $\{\psi_n\}_{n\ge0}$ is an orthonormal basis for $L^2(\mu)$.  Expanding
\[
f(x,y)=\sum_{a,b\ge0}F_{a,b}\psi_a(x)\psi_b(y),
\]
and using $g(x,y)=f(-x,y)$, the coefficient of $\psi_a(x)\psi_b(y)$ in $g$ is $(-1)^aF_{a,b}$.  Mehler diagonalization gives
\[
H(z)=\frac{\pi}{2}\sum_{a,b\ge0}(-1)^aF_{a,b}^2z^{a+b},
\]
so
\[
[z^n]H(z)=\frac{\pi}{2}\sum_{a=0}^{n}(-1)^aF_{a,n-a}^2.
\]
The two-dimensional coefficients reduce to one-dimensional integrals:
\[
F_{a,b}=\int_{\R}\psi_a(x)S_b(\tau\psi_3(x))\,d\mu(x),
\]
where
\[
S_0(u)=-\erf(u),
\qquad
S_b(u)=\frac{2}{\sqrt\pi}e^{-u^2}\frac{\psi_{b-1}(u)}{\sqrt{2b}}
\quad (b\ge1).
\]
These formulas determine the Taylor coefficients of $H$ through degree $220$ using one-dimensional Arb integrations and outward-rounded interval arithmetic.

Since $H$ is odd, the inverse has only odd coefficients.  Writing
\[
H(z)=z\Phi(z^2),
\]
Lagrange inversion gives
\[
a_{2k+1}=\frac{1}{2k+1}[t^k]\Phi(t)^{-(2k+1)},
\qquad
 a_{2k}=0.
\]
Applying this formula with Arb ball arithmetic gives the certified enclosure
\[
\sum_{n\le220}|a_n|\gzero^n<0.999999729.
\]
Since $0.999999729<1-2.5\cdot10^{-9}$, the stated bound follows.  Independent floating-point and PyTorch checks are useful diagnostics, but the displayed inequality is certified only by the outward-rounded Arb computation.
\end{proof}

\begin{corollary}[$\gamma_0$-admissibility]\label{cor:gamma0-admissibility}
For the $H_3$ scheme,
\[
M_{f,g}(\gzero)<1.
\]
Consequently, the scheme is $\gzero$-admissible.
\end{corollary}

\begin{proof}
By Lemma~\ref{lem:majorant-head-value},
\[
\sum_{1\le n\le220}|a_n|\gzero^n<1-2.5\cdot10^{-9}.
\]
By Lemma~\ref{lemma:tail-bound},
\[
\sum_{n>220}|a_n|\gzero^n<2.5\cdot10^{-9}.
\]
Adding the two inequalities gives $M_{f,g}(\gzero)<1$.  The inverse branch exists on a neighborhood of $\gzero\overline{\D}$ by Corollary~\ref{cor:H-inverse-radius}, since $\gzero<0.975$.  Thus the $H_3$ scheme satisfies Definition~\ref{def:gamma-admissible}.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:no-mixing-beats-hyperplane}]
By Corollary~\ref{cor:gamma0-admissibility}, the $H_3$ scheme is $\gzero$-admissible.  Applying Theorem~\ref{thm:krivine-preprocessing} gives
\[
K_G\le \frac{\pi}{2\gzero}.
\]
Finally, with $\rhostarval=\log(1+\sqrt2)$ and $\gzero=\rhostarval+4.8\cdot10^{-6}$,
\[
\frac{\pi}{2\rhostarval}-\frac{\pi}{2\gzero}
=
\frac{\pi(4.8\cdot10^{-6})}{2\rhostarval\gzero}
>9.7\cdot10^{-6}.
\]
Therefore
\[
K_G
\le
\frac{\pi}{2\gzero}
<
\frac{\pi}{2\log(1+\sqrt2)}-9.7\cdot10^{-6}.
\]
\end{proof}

% \begin{remark}[Equality convention]\label{rem:equality-convention}
% The equality convention for Krivine schemes can also be recovered.  The same Arb computation gives
% \[
% \sum_{n\le220}|a_n|(\rhostarval+5.2\cdot10^{-6})^n>1.000000291.
% \]
% Since $M_{f,g}$ is continuous on $[0,0.975)$, there exists
% \[
% \gamma\in(\rhostarval+4.8\cdot10^{-6},\rhostarval+5.2\cdot10^{-6})
% \]
% with $M_{f,g}(\gamma)=1$.
% \end{remark}

\section{Generalization.}

\begin{theorem}[Mixed Krivine]\label{thm:mixed-krivine-certificate}
Let $L\in\mathbb N$. For each $\ell\in\{1,\dots,L\}$, let
\[
f_\ell,g_\ell:\mathbb R^{k_\ell}\to\{-1,1\}
\]
be odd measurable functions, and let $H_\ell$ be their arcsine-normalized correlation profile:
\[
H_\ell(t)
=
\frac{\pi}{2}
\mathbb E\left[
f_\ell\left(\frac{G_1}{\sqrt2}\right)
g_\ell\left(
\frac{tG_1+\sqrt{1-t^2}G_2}{\sqrt2}
\right)
\right].
\]
Let $\lambda_1,\dots,\lambda_L\ge 0$ satisfy $\sum_{\ell=1}^L\lambda_\ell=1$, and define the mixed profile
\[
H_\lambda(t):=\sum_{\ell=1}^L\lambda_\ell H_\ell(t).
\]

Assume that $H_\lambda$ has a local inverse at the origin,
\[
H_\lambda^{-1}(\zeta)=\sum_{n\ge1}a_n\zeta^n,
\]
and that this inverse is holomorphic on a neighborhood of $\gamma\overline{\mathbb D}$ for some
$\gamma>0$. If
\[
M_\lambda(\gamma):=\sum_{n\ge1}|a_n|\gamma^n\le 1,
\]
then
\[
K_G\le \frac{\pi}{2\gamma}.
\]
\end{theorem}

\begin{theorem}[Finite mixed-profile theorem]\label{thm:finite-mixed-profile-certificate}
Let $H_\lambda=\sum_{\ell=1}^L\lambda_\ell H_\ell$ be a mixed profile as in
\Cref{thm:mixed-krivine-certificate}. Define
\[
F(w):=H_\lambda(\sin w).
\]
Fix numbers
\[
0<R<M<r_0,
\qquad
N\in\mathbb N,
\qquad
\gamma<R.
\]
Assume the following four certified inequalities.

\begin{enumerate}
    \item \textbf{Sine-coordinate analytic bound.}
    The function $F$ is holomorphic on $|w|<r_0$, and
    \[
    |F(w)-w|\le B
    \qquad (|w|\le r_0).
    \]

    \item \textbf{Finite perturbation bound.}
    Writing
    \[
    F(w)-w=\sum_{n\ge1}d_nw^n,
    \]
    one has
    \[
    \sum_{n\le N}|d_n|M^n
    +
    B\frac{(M/r_0)^{N+1}}{1-M/r_0}
    <
    M-R.
    \]

    \item \textbf{Finite inverse-majorant head.}
    Writing
    \[
    H_\lambda^{-1}(\zeta)=\sum_{n\ge1}a_n\zeta^n,
    \]
    one has
    \[
    \sum_{n\le N}|a_n|\gamma^n
    \le
    1-T.
    \]

    \item \textbf{Cauchy tail domination.}
    The tail margin satisfies
    \[
    \sinh(M)\frac{(\gamma/R)^{N+1}}{1-\gamma/R}
    \le T.
    \]
\end{enumerate}

Then
\[
K_G\le \frac{\pi}{2\gamma}.
\]
\end{theorem}

\begin{proof}
By the finite perturbation bound,
\[
\sup_{|w|=M}|F(w)-w|<M-R.
\]
Rouche's theorem therefore implies that $F^{-1}$ is holomorphic on $R\mathbb D$ and satisfies
\[
|F^{-1}(\zeta)|<M
\qquad (|\zeta|<R).
\]
Since
\[
H_\lambda^{-1}(\zeta)=\sin(F^{-1}(\zeta)),
\]
we get
\[
|H_\lambda^{-1}(\zeta)|
<
\sinh(M)
\qquad (|\zeta|<R).
\]
Cauchy's estimate gives
\[
\sum_{n>N}|a_n|\gamma^n
\le
\sinh(M)\frac{(\gamma/R)^{N+1}}{1-\gamma/R}
\le T.
\]
Combining this with the finite inverse-majorant head gives
\[
M_\lambda(\gamma)
=
\sum_{n\ge1}|a_n|\gamma^n
\le
(1-T)+T
\le 1.
\]
The conclusion now follows from \Cref{thm:mixed-krivine-certificate}.
\end{proof}

\begin{remark}[What mixing changes]
Mixing changes the correlation profile before inversion:
\[
H_\lambda=\sum_{\ell}\lambda_\ell H_\ell.
\]
The inverse-majorant is then computed for $H_\lambda^{-1}$, not by mixing the inverse-majorants of the components. This is the point at which mixing can improve the final constant.
\end{remark}


% \appendix
% \section{Sine-coordinate maximization checks}

% \begin{lemma}[Disk-to-strip check]\label{lem:disk-to-strip-check}
% Let $\rho=1.1$.  For all $u,v\in\R$ with $u^2+v^2\le\rho^2$,
% \[
% |\sin u|\cosh v<0.946.
% \]
% \end{lemma}

% \begin{proof}
% Since $\rho<\pi/2$, by symmetry we may assume $0\le u\le\rho$ and $v\ge0$.  For fixed $u$, $\cosh v$ is increasing in $v\ge0$, so it suffices to maximize
% \[
% \varphi(u):=\sin u\cosh s(u),
% \qquad
% s(u):=\sqrt{\rho^2-u^2},
% \qquad
% 0\le u\le\rho.
% \]
% For $0<u<\rho$,
% \[
% \varphi'(u)=\sin u\cosh s(u)
% \left(\cot u-\frac{u}{s(u)}\tanh s(u)\right).
% \]
% Let
% \[
% h(u):=\cot u-\frac{u}{s(u)}\tanh s(u).
% \]
% The function $u\mapsto\cot u$ is strictly decreasing.  Also
% \[
% A(s):=\frac{\tanh s}{s}
% \]
% is strictly decreasing for $s>0$, since
% \[
% A'(s)=\frac{s\operatorname{sech}^2s-\tanh s}{s^2}<0,
% \]
% the final inequality being equivalent to $\sinh s\cosh s-s>0$.  Since $s(u)$ is decreasing, $A(s(u))$ is increasing, and hence $uA(s(u))$ is increasing.  Therefore $h$ is strictly decreasing.

% Outward-rounded Taylor bounds give
% \[
% h(0.898)>0.796708-0.793956>0,
% \qquad
% h(0.900)<0.793553-0.796524<0.
% \]
% Thus the unique maximizer $u_*$ of $\varphi$ lies in $(0.898,0.900)$.  Take $c=0.899$.  On $[0.898,0.900]$,
% \[
% \varphi''(u)=
% \sin u\cosh s\left(\frac{u^2}{s^2}-1\right)
% -2\frac{u}{s}\cos u\sinh s
% -\frac{\rho^2}{s^3}\sin u\sinh s,
% \]
% where $s=s(u)$.  Throughout this interval,
% \[
% s^2\ge0.4,
% \qquad
% 0.632<s<0.636,
% \qquad
% \cosh s<1.21,
% \qquad
% \sinh s<0.68.
% \]
% These bounds give $|\varphi''(u)|<7$.  Since $|u_*-c|\le10^{-3}$,
% \[
% \varphi(u_*)\le \varphi(c)+\frac72\cdot10^{-6}.
% \]
% Now
% \[
% s(c)^2=1.21-0.899^2=0.401799<0.6339^2,
% \]
% so $\cosh s(c)<\cosh(0.6339)<1.20774$.  Also,
% \[
% \sin(0.899)<0.899-\frac{0.899^3}{6}+\frac{0.899^5}{120}<0.7828.
% \]
% Thus
% \[
% \varphi(c)<0.7828\cdot1.20774<0.945419,
% \]
% and consequently
% \[
% \varphi(u_*)<0.945419+0.0000035<0.946.
% \]
% \end{proof}

% \begin{lemma}[Cosine-ratio check]\label{lem:cosine-ratio-check}
% For every $w\in\C$ with $|w|\le1.1$,
% \[
% \frac{\pi}{2}\frac{|\cos w|^2}{1-(\operatorname{Re}\sin w)^2}<14.19.
% \]
% \end{lemma}

% \begin{proof}
% Write $w=u+iv$ and put $\rho=1.1$.  We maximize over $u^2+v^2\le\rho^2$.  We have
% \[
% \operatorname{Re}(\sin w)=\sin u\cosh v,
% \qquad
% |\cos w|^2=\cos^2u+\sinh^2v.
% \]
% It is enough to bound
% \[
% Q(u,v):=\frac{\cos^2u+\sinh^2v}{1-\sin^2u\cosh^2v}.
% \]
% The denominator is positive by Lemma~\ref{lem:disk-to-strip-check}.  Set
% \[
% x:=\sin^2u,
% \qquad
% y:=\sinh^2v.
% \]
% Then
% \[
% Q(u,v)=\frac{1-x+y}{1-x-xy},
% \]
% and, for fixed $x$,
% \[
% \frac{\partial}{\partial y}\frac{1-x+y}{1-x-xy}
% =
% \frac{(1-x)^2}{(1-x-xy)^2}>0.
% \]
% Thus, for each fixed $u$, the maximum occurs at $|v|=\sqrt{\rho^2-u^2}$.  By evenness in $u$, it remains to maximize
% \[
% \Phi(u):=
% \frac{\cos^2u+\sinh^2s(u)}{1-\sin^2u\cosh^2s(u)},
% \qquad
% s(u):=\sqrt{\rho^2-u^2},
% \qquad
% 0\le u\le\rho.
% \]
% For $0<u<\rho$, differentiating gives
% \[
% \Phi'(u)=
% \frac{\sinh(2s)\cos u}{(1-\sin^2u\cosh^2s)^2}
% \left[
% \sin u\tanh s(1+\cosh^2s)
% -\frac{u}{s}\cos u(1+\sin^2u)
% \right],
% \]
% where $s=s(u)$.  The prefactor is positive.  Therefore the sign of $\Phi'(u)$ is the sign of $A(u)-1$, where
% \[
% A(u):=\frac{s(u)\tan u\tanh s(u)(1+\cosh^2s(u))}{u(1+\sin^2u)}.
% \]
% We show that $A$ is strictly decreasing.  Let
% \[
% B(s):=s\tanh s(1+\cosh^2s).
% \]
% Then
% \[
% \frac{d}{du}\log A(u)
% =
% \left(\frac{1}{\sin u\cos u}-\frac{1}{u}\right)
% -\frac{\sin(2u)}{1+\sin^2u}
% -\frac{u}{s}\frac{B'(s)}{B(s)}.
% \]
% Moreover,
% \[
% \frac{B'(s)}{B(s)}
% =
% \frac{1}{s}
% +
% \frac{1}{\sinh s\cosh s}
% +
% \frac{2\sinh s\cosh s}{1+\cosh^2s}.
% \]
% Since
% \[
% \frac{2\sinh s\cosh s}{1+\cosh^2s}\ge \tanh s
% \qquad\text{and}\qquad
% \frac{1}{\sinh s\cosh s}+\tanh s=\coth s>\frac1s,
% \]
% we have $B'(s)/B(s)>2/s$.  On the other hand, for $0<u<\rho$,
% \[
% \sin u\cos u=\frac12\sin(2u)>u-\frac23u^3.
% \]
% Therefore
% \[
% \frac{1}{\sin u\cos u}-\frac1u
% =
% \frac{u-\sin u\cos u}{u\sin u\cos u}
% <\frac{2u}{3-2u^2}
% <\frac{2u}{\rho^2-u^2}
% =\frac{2u}{s^2}.
% \]
% Combining the estimates gives
% \[
% \frac{d}{du}\log A(u)
% <
% \frac{2u}{s^2}
% -\frac{\sin(2u)}{1+\sin^2u}
% -\frac{2u}{s^2}
% <0.
% \]
% Thus $A$ is strictly decreasing.  Since $A(u)>1$ for small $u>0$ and $A(u)\to0$ as $u\uparrow\rho$, the function $\Phi$ increases up to the unique point where $A(u)=1$ and decreases afterward.

% A final outward-rounded interval computation gives
% \[
% A(0.8289364)>1.0000019,
% \qquad
% A(0.8289372)<0.9999992.
% \]
% Hence the maximizer lies in
% \[
% I=[0.8289364,0.8289372].
% \]
% Evaluating $\Phi$ on this interval, again with outward-rounded interval arithmetic, gives
% \[
% \Phi(I)\subset[9.0332175,9.03345993].
% \]
% Consequently
% \[
% \sup_{|w|\le1.1}
% \frac{\pi}{2}\frac{|\cos w|^2}{1-(\operatorname{Re}\sin w)^2}
% =
% \frac{\pi}{2}\sup_{0\le u\le\rho}\Phi(u)
% \le
% \frac{\pi}{2}\cdot9.03345993
% <14.18973<14.19.
% \]
% \end{proof}

==> old/related_work.tex <==
\paragraph{AI Assisted Mathematical Reasoning}
AI-assisted mathematics has developed along two closely related axes: natural-language mathematical reasoning and machine-checkable formal proof. On the natural-language side, benchmarks such as MATH and GSM8K, together with verifier training and process-supervision methods, established the now-standard pattern in which a model proposes many candidate derivations and a learned or explicit verifier selects, grades, or refines them  \citep{2103.03874,2110.14168,lightman2024verifystepbystep}. 
The evaluation frontier has since moved from contest and proof benchmarks such as MiniF2F, OlympiadBench, Omni-MATH, and IMO-ProofBench to research-facing suites such as FrontierMath, UQ, and FirstProof \citep{zheng2021minif2f,he2024olympiadbench,gao2024omni,luong2025robustmathematicalreasoning,glazer2024frontiermath,nie2025uqassessinglanguagemodels,abouzaid2026proof}. On the formal side, Lean and Mathlib provide a small trusted kernel and a large community-maintained mathematical library \citep{deMoura2015lean,mathlib2020}, enabling work on LLM-guided theorem proving, retrieval-augmented premise selection, and semantic search over formal libraries \citep{polu2020generative,yang2023leandojo,gao2024semanticsearchmathlib4}. Systems such as AlphaGeometry, AlphaGeometry 2, and AlphaProof demonstrate that learned search, symbolic reasoning, and formal feedback can be coupled tightly enough to reach medal-level performance on olympiad mathematics \citep{Trinh2024-alphageometry-1,chervonyi2025goldmedalistperformancesolvingolympiad-alphageometry2,Hubert2025}. Our work is adjacent to this verification-centered line, but targets a different use case: rather than solving a self-contained problem or autoformalizing a finished proof, we study how to refine an existing quantitative proof by exposing its dependency graph, optimizing local estimates, and certifying that improved numerical constants propagate through the argument.

\paragraph{AI Assisted Research Results}
Recent work has begun to move from benchmark performance toward AI-assisted mathematical and scientific research. Aletheia reports a generator--verifier--reviser agent for research-level mathematics, with contributions to eigenweights in arithmetic geometry, independence-polynomial inequalities, Erd\H{o}s problems, and FirstProof \citep{feng2026towardsautonomousmathematicsresearch,Feng2026,LeeSeo2026,erdos,feng2026aletheiatacklesfirstproofautonomously}. In a complementary direction, Rethlas and Archon combine natural-language search with Lean formalization to resolve and formally verify an open problem in commutative algebra \citep{ju2026automatedconjectureresolutionformal}. Other recent case studies include AI-assisted or AI-guided work on algebraic geometry, extremal descendant integrals, accelerated optimization, convex analysis, probability, combinatorics, and broader scientific discovery workflows \citep{bryan2026motivic,schmitt2025extremal,jang2025point,salim2025acceleratingmathematicalresearchlanguage,ivanisvili2025counterexamplemajorityoptimalitynicd,bubeck2025earlyscienceaccelerationexperiments,woodruff2026acceleratingscientificresearchgemini,georgiev2025mathematicalexplorationdiscoveryscale}. These results show that frontier models can be useful as mathematical collaborators, especially when a project benefits from breadth of knowledge, large-scale exploration, calculation, or persistent search. At the same time, the literature repeatedly emphasizes that correctness, novelty, and significance remain difficult to evaluate: research problems are often single-use, expert verification is scarce, and models can produce hallucinated references, vacuous interpretations, or plausible arguments with hidden gaps \citep{feng2026towardsautonomousmathematicsresearch,abouzaid2026proof,tao2024bestpractices,tao2026erdosai}. Our setting is deliberately more constrained. We do not aim to replace domain experts or claim broad autonomous discovery; instead, we use AI to search within a fixed proof architecture, improve explicit constants, and produce auditable artifacts whose local numerical and formal obligations can be checked independently.

\paragraph{AI Agentic Frameworks}
The strongest recent systems increasingly wrap frontier models in agentic workflows that combine generation, verification, tool use, memory, search, and revision. For natural-language mathematics, Aletheia uses interacting generator, verifier, and reviser components, while Huang and Yang show that a model-agnostic solver--verifier--refinement pipeline can substantially improve performance on IMO 2025 problems \citep{feng2026towardsautonomousmathematicsresearch,huang2025winninggoldimo2025}. For formal and hybrid mathematics, Rethlas/Archon separates informal exploration from Lean formalization; Seed-Prover 1.5, Aristotle, Ax-Prover, Numina-Lean-Agent, and ARIA represent a parallel trend toward tool-using theorem-proving agents that call proof assistants, retrieval engines, informal reasoners, and decomposition planners \citep{ju2026automatedconjectureresolutionformal,chen2025seedprover,achim2025aristotle,tredici2025axprover,liu2026numinaleagent,wang2025aria}. A related line studies open-ended scientific or mathematical search through coding agents, evolutionary program improvement, and test-time discovery procedures, including AlphaEvolve, ThetaEvolve, Learning to Discover at Test Time, and large-scale mathematical exploration systems \citep{novikov2025alphaevolvecodingagentscientific,wang2025thetaevolvetesttimelearningopen,yuksekgonul2026learningdiscovertesttime,georgiev2025mathematicalexplorationdiscoveryscale}. Our framework fits within this agentic turn, but its objective and granularity are different: partial formalization anchors the proof skeleton, numerical feedback identifies promising local refinements, proof-search agents tighten the corresponding lemmas, and quantitative dependency propagation converts these local improvements into a certified global bound. This makes proof refinement a middle ground between fully autonomous theorem discovery and conventional proof engineering: the human supplies the mathematical objective and high-level proof architecture, while the agentic system searches the space of permissible refinements under formal and numerical checks.

==> old/remove_analytic_obstruction_v1.tex <==
\section{Removing The Main Analytic Obstruction}
\label{sec:analytic-obstruction}

\paragraph{Proof architecture.}
The proof has two independent modules after the scheme is fixed.  The analytic module proves a uniform inverse disk; the numerical module computes the inverse-majorant head and uses the analytic disk for the tail:
\[
\begin{array}{ccccc}
Lemma~\ref{lem:strip-bound}
&\Longrightarrow&
Lemma~\ref{lem:sine-coordinate-bound}
&\Longrightarrow&
Corollary~\ref{cor:F-inverse-radius}
\Longrightarrow
Corollary~\ref{cor:H-inverse-radius}
\\[0.5em]
&&&&\Downarrow
\\[-0.1em]
Lemma~\ref{lem:majorant-head-value}
&+&
Lemma~\ref{lemma:tail-bound}
&\Longrightarrow&
Corollary~\ref{cor:gamma0-admissibility}
\Longrightarrow
Theorem~\ref{thm:no-mixing-beats-hyperplane}.
\end{array}
\]
\paragraph{Proof plan.}
The proof has two parts. First, we prove an analytic inverse disk for the correlation profile. The
main device is the change of variables
\[
F(w):=H(\sin w),
\]
which is useful because the hyperplane profile becomes the identity map in this coordinate. This
allows us to use Rouché's theorem to control the inverse branch uniformly. Second, using this
inverse disk, we certify the inverse-majorant by splitting it into a finite head and a Cauchy tail:
the head is computed with Arb through degree $220$, and the tail is bounded analytically from the
inverse disk. Combining these two estimates gives $M_{f,g}(\gamma_0)<1$, so the $H_3$ scheme is
$\gamma_0$-admissible and the desired bound on $K_G$ follows.

\subsection{The analytic inverse disk}.


Define
\[
 F(w):=H(\sin w).
\]
The point of this substitution is that for the hyperplane scheme
\[
 H_0(\sin w)=\arcsin(\sin w)=w
\]
on the principal strip $|\operatorname{Re}w|<\pi/2$. Hence $F$ should be compared to
the identity, not to $\arcsin$.


\begin{lemma}[uniform strip bound]\label{lem:strip-bound}
Let $f,g:\R^2\to\{-1,1\}$ be measurable and let $H=H_{f,g}$ be the
arcsine-normalized correlation function, so that for real $|t|<1$,
\[
 H(t)=\frac{1}{2\pi(1-t^2)}
 \int_{\R^2}\int_{\R^2}
 f(x)g(y)\exp\left(-\frac{\|x\|^2+\|y\|^2-2t\langle x,y\rangle}{1-t^2}\right)dxdy.
\]
Then $H$ extends holomorphically to
\[
 S=\{z\in\C: |\operatorname{Re}z|<1\}.
\]
Moreover, if $z=a+ib\in S$, then
\[
 |H(z)|\le \frac{\pi}{2}\frac{|1-z^2|}{1-a^2}.
\]
\end{lemma}

\begin{proof}
It is enough to prove the stated bound, since the same estimate, uniformly on compact
subsets of $S$, gives absolute convergence of the integral and holomorphy by dominated
convergence. Fix $z=a+ib\in S$. Since $|f|=|g|=1$,
\[
 |H(z)|\le
 \frac{1}{2\pi|1-z^2|}
 \int_{\R^2}\int_{\R^2}
 \exp\left(-\operatorname{Re}\frac{\|x\|^2+\|y\|^2-2z\langle x,y\rangle}{1-z^2}\right)dxdy.
\]
Use the identity
\[
 \frac{\|x\|^2+\|y\|^2-2z\langle x,y\rangle}{1-z^2}
 =\frac12\frac{\|x+y\|^2}{1+z}
  +\frac12\frac{\|x-y\|^2}{1-z}.
\]
Set
\[
 A_+=\operatorname{Re}\frac1{1+z}
 =\frac{1+a}{(1+a)^2+b^2},
 \qquad
 A_-=\operatorname{Re}\frac1{1-z}
 =\frac{1-a}{(1-a)^2+b^2}.
\]
Because $|a|<1$, both $A_+$ and $A_-$ are positive. With the change of variables
\[
 u=x+y,
 \qquad
 v=x-y,
\]
the Jacobian from $(u,v)$ to $(x,y)$ in $\R^4$ is $1/4$. Hence
\[
 \begin{aligned}
 &\int_{\R^2}\int_{\R^2}
 \exp\left(-\operatorname{Re}\frac{\|x\|^2+\|y\|^2-2z\langle x,y\rangle}{1-z^2}\right)dxdy  \\
 &\qquad =\frac14
 \int_{\R^2}\int_{\R^2}
 \exp\left(-\frac12A_+\|u\|^2-\frac12A_-\|v\|^2\right)dudv \\
 &\qquad =\frac14\cdot\frac{2\pi}{A_+}\cdot\frac{2\pi}{A_-}
 =\frac{\pi^2}{A_+A_-}.
 \end{aligned}
\]
Therefore
\[
 |H(z)|\le \frac{\pi}{2|1-z^2|}\frac1{A_+A_-}.
\]
Finally,
\[
 A_+A_-
 =\frac{1-a^2}{((1+a)^2+b^2)((1-a)^2+b^2)}
 =\frac{1-a^2}{|1+z|^2|1-z|^2}
 =\frac{1-a^2}{|1-z^2|^2}.
\]
Substitution gives
\[
 |H(z)|\le
 \frac{\pi}{2|1-z^2|}\cdot\frac{|1-z^2|^2}{1-a^2}
 =\frac{\pi}{2}\frac{|1-z^2|}{1-a^2}.
\]
\end{proof}

\begin{lemma}[sine-coordinate bound]\label{lem:sine-bound}
For $F(w)=H(\sin w)$, the function $F$ is holomorphic on $|w|<1.1$ and
\[
 |F(w)-w|<15.3\qquad (|w|\le1.1).
\]
\end{lemma}

\begin{proof}
Write $w=u+iv$. Then
\[
 \operatorname{Re}(\sin w)=\sin u\cosh v.
\]
A one-variable interval maximization on $u^2+v^2\le1.1^2$ gives
\[
 |\sin u|\cosh v<0.946<1.
\]
Thus $\sin w\in S$ for $|w|\le1.1$, and $F(w)=H(\sin w)$ is holomorphic on
$|w|<1.1$ by Lemma~\ref{lem:strip-bound}. Applying Lemma~\ref{lem:strip-bound} to
$z=\sin w$ gives
\[
 |F(w)|
 \le \frac{\pi}{2}\frac{|1-\sin^2w|}{1-(\operatorname{Re}\sin w)^2}
 =\frac{\pi}{2}\frac{|\cos w|^2}{1-(\operatorname{Re}\sin w)^2}.
\]
A direct interval maximization on $|w|\le1.1$ gives
\[
 \frac{\pi}{2}\frac{|\cos w|^2}{1-(\operatorname{Re}\sin w)^2}<14.19.
\]
Hence $|F(w)-w|\le |F(w)|+|w|<14.19+1.1<15.3$.
\end{proof}


% {
% % \color{red}

% \begin{lemma}[Rouche inverse disk]
% Let $F$ be holomorphic on $|w|<r$, with $F(0)=0$, and suppose that for some $R < M<r$ ,
% \[
%  \sup_{|w|=R}|F(w)-w|<M-R.
% \]
% Then, we have 
% \begin{enumerate}
%     \item $F^{-1}$ is holomorphic on $R\D$,
%     \item For $|\zeta|<R$,  the inverse satisfies $|F^{-1}(\zeta)|<M$.
% \end{enumerate}
% \end{lemma}

% \begin{proof}
% Fix $|\zeta|<R$. On $|w|=R$,
% \[
%  |(F(w)-\zeta)-(w-\zeta)|=|F(w)-w|<M-R\le M-|\zeta|\le |w-\zeta|.
% \]
% By Rouche's theorem, $F(w)-\zeta$ and $w-\zeta$ have the same number of zeros in
% $|w|<r$, counted with multiplicity. Since $w-\zeta$ has exactly one zero there,
% $F(w)=\zeta$ has exactly one solution in $|w|<M$. This solution is simple, and the
% local analytic inverse branches glue by uniqueness.
% \end{proof}
% }

% \begin{lemma}[Rouche inverse disk]
% Let $F$ be holomorphic on $|w|<R$, with $F(0)=0$, and suppose that for some $r<R$ and $s<r$,
% \[
%  \sup_{|w|=r}|F(w)-w|<r-s.
% \]
% Then $F^{-1}$ is holomorphic on $s\D$, and for $|\zeta|<s$ the inverse satisfies
% $|F^{-1}(\zeta)|<r$.
% \end{lemma}

% \begin{proof}
% Fix $|\zeta|<s$. On $|w|=r$,
% \[
%  |(F(w)-\zeta)-(w-\zeta)|=|F(w)-w|<r-s\le r-|\zeta|\le |w-\zeta|.
% \]
% By Rouche's theorem, $F(w)-\zeta$ and $w-\zeta$ have the same number of zeros in
% $|w|<r$, counted with multiplicity. Since $w-\zeta$ has exactly one zero there,
% $F(w)=\zeta$ has exactly one solution in $|w|<r$. This solution is simple, and the
% local analytic inverse branches glue by uniqueness.
% \end{proof}

% Write
% \[
%  D(w):=F(w)-w=\sum_{n\ge1}d_nw^n.
% \]
% The coefficient computation gives
% \[
%  \sum_{n\le220}|d_n|\,0.98^n<0.00454106848.
% \]
% The preceding strip bound gives the Cauchy tail
% \[
%  \sum_{n>220}|d_n|\,0.98^n
%  \le 15.3\frac{(0.98/1.1)^{221}}{1-0.98/1.1}
%  <1.15\cdot10^{-9}.
% \]
% Therefore
% \[
%  \sup_{|w|=0.98}|F(w)-w|<0.004541070<0.005=0.98-0.975.
% \]
% By the Rouche lemma, $F^{-1}$ is holomorphic on $0.975\D$ and
% \[
%  |F^{-1}(\zeta)|<0.98\qquad(|\zeta|<0.975).
% \]
% Since
% \[
%  H^{-1}(\zeta)=\sin(F^{-1}(\zeta)),
% \]
% it follows that $H^{-1}$ is holomorphic on $0.975\D$ and
% \[
%  |H^{-1}(\zeta)|<\sinh(0.98)<1.145.
% \]

\begin{lemma}[Rouche inverse disk]
Let $F$ be holomorphic on $|w|<r$, with $F(0)=0$, and suppose that for some
$R<M<r$,
\[
 \sup_{|w|=M}|F(w)-w|<M-R.
\]
Then:
\begin{enumerate}
    \item $F^{-1}$ is holomorphic on $R\D$;
    \item for $|\zeta|<R$, the inverse satisfies $|F^{-1}(\zeta)|<M$.
\end{enumerate}
\end{lemma}

\begin{proof}
Fix $|\zeta|<R$. On the circle $|w|=M$ we have
\[
 |(F(w)-\zeta)-(w-\zeta)|
 =
 |F(w)-w|
 <
 M-R
 <
 M-|\zeta|
 \le |w-\zeta|.
\]
By Rouche's theorem, the functions $F(w)-\zeta$ and $w-\zeta$ have the same
number of zeros in $|w|<M$, counted with multiplicity. Since $w-\zeta$ has
exactly one zero in $|w|<M$, the equation
\[
F(w)=\zeta
\]
has exactly one solution in $|w|<M$, counted with multiplicity. In particular,
this solution is simple.

Thus for every $\zeta\in R\D$ there is a unique $w\in M\D$ with $F(w)=\zeta$.
Since the solution is simple, the holomorphic inverse function theorem gives a
local holomorphic inverse near each $\zeta$. These local inverse branches agree
on overlaps by uniqueness, and therefore glue to a single holomorphic inverse
branch on $R\D$.

Finally, the construction gives $|F^{-1}(\zeta)|<M$ for every $|\zeta|<R$.
\end{proof}

Let
\[
  \Delta(w):=F(w)-w=\sum_{n\ge1}d_nw^n.
\]
The finite coefficient computation gives
\[
  \sum_{n\le220}|d_n|\,0.98^n<0.00454106848.
\]
By Lemma~\ref{lem:sine}, Cauchy's estimate, with the Cauchy radius tending up to $1.1$, gives
\[
 \sum_{n>220}|d_n|\,0.98^n
 \le 15.3\frac{(0.98/1.1)^{221}}{1-0.98/1.1}
 <1.149\cdot10^{-9}.
\]
Therefore
\[
  \sup_{|w|=0.98}|F(w)-w|
  <0.00454106848+1.149\cdot10^{-9}
  <0.004541070<0.005.
\]
Apply Lemma~\ref{lem:rouche} with
\[
  r=1.1,
  \qquad
  M=0.98,
  \qquad
  R=0.975.
\]
Then $F^{-1}$ is holomorphic on $0.975\D$, and
\[
  |F^{-1}(\zeta)|<0.98\qquad(|\zeta|<0.975).
\]
Since $H^{-1}(\zeta)=\sin(F^{-1}(\zeta))$, we have
\[
  |H^{-1}(\zeta)|<\sinh(0.98)<1.145
  \qquad(|\zeta|<0.975).
\]

\subsection{The inverse-majorant certificate}

Let
\[
 H^{-1}(\zeta)=\sum_{n\ge1}a_n\zeta^n.
\]
Since $H$ is odd, only odd $a_n$ occur. Write
\[
 H(z)=z\Phi(z^2).
\]
Lagrange inversion gives
\[
 a_{2k+1}=\frac{1}{2k+1}[t^k]\Phi(t)^{-(2k+1)},
 \qquad a_{2k}=0.
\]
The finite inverse-majorant sums through degree $220$ are
\[
 \sum_{n\le220}|a_n|\rho_*^n
 <0.999992967,
\]
\[
 \sum_{n\le220}|a_n|(\rho_*+4.8\cdot10^{-6})^n
 <0.999999729,
\]
and
\[
 \sum_{n\le220}|a_n|(\rho_*+5.2\cdot10^{-6})^n
 >1.000000291.
\]
For any $s<0.975$, Cauchy's estimate from the preceding section gives
\[
 \sum_{n>220}|a_n|s^n
 \le
 1.145\frac{(s/0.975)^{221}}{1-s/0.975}.
\]
At $s=\rho_*+4.8\cdot10^{-6}$ this is less than $2.5\cdot10^{-9}$. Hence
\[
 \sum_{n\ge1}|a_n|\rho_*^n<1
\]
and even
\[
 \sum_{n\ge1}|a_n|(\rho_*+4.8\cdot10^{-6})^n<1.
\]
On the other hand, the finite sum alone implies
\[
 \sum_{n\ge1}|a_n|(\rho_*+5.2\cdot10^{-6})^n>1.
\]
Thus, by continuity of
\[
 M(s)=\sum_{n\ge1}|a_n|s^n,
\]
there exists $\gamma$ with
\[
 \rho_*+4.8\cdot10^{-6}<\gamma<\rho_*+5.2\cdot10^{-6}
\]
and
\[
 M(\gamma)=1.
\]
The Krivine criterion in arcsine units now gives
\[
 K_G\le\frac\pi{2\gamma}<\frac\pi{2\rho_*}
 =\frac\pi{2\log(1+\sqrt2)}.
\]
This proves the theorem.

==> old/results.tex <==
{\bf \color{red} For each constant below, do the following: 

Problem:
\begin{itemize}
    \item What constant is being bounded?
    \item What was the previous state of knowledge?
\end{itemize}


Original proof architecture:
\begin{itemize}
\item What proof are we starting from?
\item What are the major lemmas?
\item Which parts are formalized?
\item Which parts are assumed/axiomatized?
\end{itemize}

Final bound:
\begin{itemize}
    \item Previous bound:
    \item New bound:
    \item {\color{blue} Human verification}
\end{itemize}
}

\subsection{The Grothendieck Constant}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/cr_progression.png}
    \caption{$C_r$ value run}
    \label{fig:cr_prog}
\end{figure}

The last effective bound is by Krivine from 1979. This bound is $K_G \le \frac{2}{\pi} \log(1 + \sqrt{2})$. This was conjectured optimal until it was disproven in Braverman et al, but the authors did not provide an explicit bound. We first formalized their paper and got a bound of $K_G \le \frac{2}{\pi} \log(1 + \sqrt{2}) - 10^{-\text{placeholder}}$.

We improve this $K_G \le \frac{2}{\pi} \log(1 + \sqrt{2}) - 10^{-\text{better placeholder}}$. The delta we gain is almost $\text{placeholder}$ over Braverman. 

We start from a formalization of braverman paper. We scaffold lemma 5.4 where the a bound on a value $C_r$ is proved. Proving this lemma requires a lot of sub-lemmas that are included in the graph node. These nodes are refined. 





\subsection{The Korenblum constant}

==> old/tiger_partitions.tex <==
\section{Tiger partitions}
\label{sec:tiger-partitions}

K\"onig's two-dimensional oscillatory form is $B_K(f,g)=\iint_{\mathbb R^2\times\mathbb R^2} f(x)g(y)e^{-(\|x\|^2+\|y\|^2)/2}\sin\langle x,y\rangle\,dx\,dy$ for sign partitions $f,g:\mathbb R^2\to\{-1,1\}$; we use the normalization $\widetilde B_K(f,g)=B_K(f,g)/(2\pi^2)$.  The hyperplane partition $f_0(x_1,x_2)=g_0(x_1,x_2)=\mathrm{sign}(x_2)$ has value $c_K=(2/\pi)\log(1+\sqrt2)$.  K\"onig conjectured that hyperplanes maximize this form in every dimension, a statement which would have implied Krivine's conjectured value for the Grothendieck constant, but Braverman--Makarychev--Makarychev--Naor disproved it in dimension two \cite{BMMN}.  For Grothendieck rounding, however, the relevant quantity is not just $\widetilde B_K$: if $H_{f,g}^{-1}(z)=\sum_n a_nz^n$ is the inverse Hermite correlation series, the certificate is the majorant root $c_{f,g}$ determined by $\sum_n |a_n|c_{f,g}^n=1$, and $c_{f,g}=\widetilde B_K(f,g)$ only under the alternating-sign condition on the inverse coefficients.

The best-response map for $B_K$ is $\sigma(f)(y)=\mathrm{sign}\big(\int_{\mathbb R^2} f(x)e^{-\|x\|^2/2}\sin\langle x,y\rangle\,dx\big)$, so a K\"onig maximizer should satisfy the two-cycle equations $\sigma(f)=g$ and $\sigma(g)=f$.  We call a non-hyperplane odd limit, or stable period-two limit, of the iteration $f,\sigma(f),\sigma^2(f),\ldots$ a tiger partition or tiger pair.  Numerically, we tested $1000$ random odd initial partitions, drawn from hyperplane perturbation, DSL-random, multicurve, and pixel-random families, on a symmetric $600\times600$ grid in $[-8,8]^2$ with Hermite truncation degree $18$; the sigma dynamics reliably found strong K\"onig candidates, with typical normalized value $\widetilde B_K(f,g)\approx0.5619>c_K\approx0.56110$, and most runs entered a stable oscillatory two-cycle rather than a fixed point.

The same experiments show that tiger partitions are poor Grothendieck rounding schemes.  Across all $1000$ runs, no tiger pair gave a genuine improvement in the majorant constant: generic oscillatory tiger pairs had $c_{f,g}\approx0.508$, far below $c_K$, and the two marginal values near $c_K$ were grid-error-scale returns to the hyperplane fixed point.  Even mixing each tiger Hermite $b$-series with the hyperplane $b$-series failed to extract an improving direction: every one-dimensional mixture was optimized at the pure hyperplane endpoint $p^*=0$.  Thus tiger partitions appear to be excellent optimizers for K\"onig's bilinear form but misleading for the Grothendieck constant; the obstruction is structural, since $\widetilde B_K$ is a single oscillatory value that can hide cancellations, whereas $c_{f,g}$ depends on the full inverse series through absolute values and penalizes the non-alternating coefficients produced by the tiger dynamics.


==> old/tiger_partitions_old.tex <==
% Section draft: Tiger partitions.
% Assumes the main paper loads amsmath and amssymb.  Replace the citation key
% \cite{BMMN} below with the bibliography key used in the main paper.

\section{Tiger partitions}
\label{sec:tiger-partitions}

{
\color{blue}
THIS ENTIRE SECTION SHOULD BE 2-3 paragraphs. DEFINE KONIG, TIGER PARTITIONS, SHOW EXPERIMENTS, EXPLAIN WHY THIS IS SIGNIFCANT IN A FEW SHORT SENTENCES. 
}

The experiments in this section test a natural idea suggested by the history of the
Grothendieck problem: perhaps the partitions that optimize K\"onig's oscillatory
bilinear form are also good, or even optimal, for the Grothendieck rounding constant
obtained from the inverse Hermite series.  The conclusion is the opposite.  Tiger
partitions are extremely good for K\"onig's bilinear form, and the sigma iteration
reliably finds such partitions, but the same partitions appear to be poor for the
Grothendieck-relevant majorant constant $c_{f,g}$.

\subsection{K\"onig's bilinear form}
\label{subsec:konig-bilinear-form}

For measurable sign functions $f,g:\mathbb R^k\to\{-1,1\}$, define the oscillatory
Gaussian bilinear form
\begin{equation}
  B_K^{\mathrm{raw}}(f,g)
  := \int_{\mathbb R^k}\int_{\mathbb R^k}
       f(x)g(y)\exp\left(-\frac{\|x\|^2+\|y\|^2}{2}\right)
       \sin\langle x,y\rangle\,dx\,dy .
  \label{eq:konig-raw}
\end{equation}
In this section we work in dimension $k=2$ and use the normalized form
\begin{equation}
  \widetilde B_K(f,g) := \frac{B_K^{\mathrm{raw}}(f,g)}{2\pi^2}.
  \label{eq:konig-normalized}
\end{equation}
With this convention the hyperplane partition
\begin{equation}
  f_0(x_1,x_2)=g_0(x_1,x_2)=\mathrm{sign}(x_2)
\end{equation}
satisfies
\begin{equation}
  \widetilde B_K(f_0,g_0)
  = c_K
  := \frac{2}{\pi}\log(1+\sqrt 2).
  \label{eq:krivine-cK}
\end{equation}

The form \eqref{eq:konig-raw} entered the subject through K\"onig's intermediate
extremal problem.  K\"onig conjectured that, for every dimension, the hyperplane
partition maximizes $B_K^{\mathrm{raw}}$ among all sign partitions.  A positive answer
would have implied Krivine's conjectured value
$K_G=\pi/(2\log(1+\sqrt2))$.  Braverman, Makarychev, Makarychev and Naor
(BMMN) disproved this conjecture in dimension two, thereby opening the door to
rounding schemes based on two-dimensional projections rather than random hyperplanes
\cite{BMMN}.  The key point for us is that K\"onig's form is a natural proxy for
Grothendieck rounding only under an additional sign-alternation condition on the
inverse series.

To spell this out, let $H_{f,g}$ denote the Krivine correlation function associated
with $f,g$ and write, near the origin,
\begin{equation}
  H_{f,g}^{-1}(z)=\sum_{j\ge 0} a_{2j+1}z^{2j+1}.
\end{equation}
The Krivine majorant constant is the positive solution of
\begin{equation}
  \sum_{j\ge 0}|a_{2j+1}|c^{2j+1}=1,
  \label{eq:majorant-c}
\end{equation}
when such a solution exists.  This is the quantity that certifies the upper bound
$K_G\le 1/c$.  If the inverse coefficients alternate, i.e.
\begin{equation}
  \mathrm{sign}(a_{2j+1})=(-1)^j \qquad (j\ge 0),
  \label{eq:alternating-condition}
\end{equation}
then the absolute values in \eqref{eq:majorant-c} evaluate the inverse at the imaginary
axis, and BMMN's identity gives
\begin{equation}
  c(f,g)=\frac{H_{f,g}(i)}{i}
        = \frac{B_K^{\mathrm{raw}}(f,g)}{(\sqrt 2\pi)^k}.
  \label{eq:alternating-bk-identity}
\end{equation}
Thus, in dimension two and with the normalization \eqref{eq:konig-normalized},
\begin{equation}
  c(f,g)=\widetilde B_K(f,g)
  \qquad\text{for alternating Krivine schemes.}
  \label{eq:dimension-two-alternating}
\end{equation}
Without alternation, there is no reason for $\widetilde B_K$ and $c_{f,g}$ to move in
the same direction: $\widetilde B_K$ is a single oscillatory value, while $c_{f,g}$ is
controlled by the full inverse power series with absolute values.

\subsection{The sigma operator and tiger partitions}
\label{subsec:sigma-tiger}

The K\"onig form is linear in each argument.  If $f$ is fixed, the choice of $g$ that
maximizes $B_K^{\mathrm{raw}}(f,g)$ is obtained pointwise.  This gives the sigma
operator
\begin{equation}
  \sigma(f)(y)
  := \mathrm{sign}\left(
      \int_{\mathbb R^2}
        f(x)\exp\left(-\frac{\|x\|^2}{2}\right)
        \sin\langle x,y\rangle\,dx
     \right),
  \label{eq:sigma-operator}
\end{equation}
with an arbitrary convention on the null set where the argument vanishes.  Equivalently,
\begin{equation}
  B_K^{\mathrm{raw}}(f,g)
  = \int_{\mathbb R^2}
      g(y)\exp\left(-\frac{\|y\|^2}{2}\right)
      \left[\int_{\mathbb R^2}f(x)\exp\left(-\frac{\|x\|^2}{2}\right)
        \sin\langle x,y\rangle\,dx\right]dy,
\end{equation}
so $g=\sigma(f)$ is the best response to $f$.  Similarly, $f=\sigma(g)$ is the best
response to $g$.  Hence a maximizing pair $(f_{\max},g_{\max})$ for $B_K^{\mathrm{raw}}$
should satisfy the coupled equations
\begin{equation}
  \sigma(f_{\max})=g_{\max},
  \qquad
  \sigma(g_{\max})=f_{\max}.
  \label{eq:tiger-fixed-equations}
\end{equation}
This observation motivates iterating $\sigma^2$ from an initial sign partition.  The
sine kernel also annihilates the centrally even part of $f$, so $\sigma(f)$ depends only
on $f(x)-f(-x)$ and is itself odd under $y\mapsto -y$.  Thus, once the iteration starts
from an odd partition, oddness is preserved.

We use the following terminology.  A \emph{tiger pair} is a pair $(f,g)$ of odd sign
partitions satisfying the two-cycle equations \eqref{eq:tiger-fixed-equations}, or a
numerical limit/period-two limit of the iteration
\begin{equation}
  f,\ \sigma(f),\ \sigma^2(f),\ldots.
\end{equation}
When the even iterates converge, we call the limiting sign function $f_\infty$ a
\emph{tiger partition}, and write $g_\infty=\sigma(f_\infty)$.  This matches the
terminology introduced by BMMN: their computations suggested that, for many initial
conditions different from the hyperplane fixed point, the even iterates converge to a
visually striped partition of the plane, the ``tiger partition.''  BMMN asked for an
analytic description of this limit and conjectured that the pair
$(f_\infty,\sigma(f_\infty))$ gives the maximizers of K\"onig's bilinear form in the
plane \cite{BMMN}.

There is an important distinction between this BMMN conjecture and the optimization
problem studied here.  BMMN's tiger conjecture is a conjecture about maximizing
$B_K^{\mathrm{raw}}$.  Our question is whether tiger pairs also maximize the
Grothendieck-relevant constant $c_{f,g}$.  These would be the same question for
alternating schemes, by \eqref{eq:dimension-two-alternating}.  The experiments below
show that the tiger pairs found by $\sigma$ are very far from this alternating regime.

\subsection{Experimental setup}
\label{subsec:tiger-experimental-setup}

We generated $1000$ random odd partitions of $\mathbb R^2$, $250$ from each of four
families, and applied the sigma operator until convergence or until a stable oscillation
was detected.  All computations were performed on a symmetric $600\times 600$ grid on
$[-8,8]^2$, with Hermite truncation degree $18$.  The symmetry of the grid enforces the
oddness condition
\begin{equation}
  f(-x_1,-x_2)=-f(x_1,x_2)
\end{equation}
exactly at the discrete level.  The four initial families were:
\begin{enumerate}
  \item \emph{Hyperplane perturbations:}
  \begin{equation}
    f(x,y)=\mathrm{sign}\left(y-\sum_{k\in\{1,3,5,7,9\}}c_kh_k(x)\right),
  \end{equation}
  with random odd-Hermite coefficients.

  \item \emph{DSL random partitions:} starting from $\mathrm{sign}(y)$, we applied
  $15$--$50$ random sign flips on centrally symmetric geometric regions.

  \item \emph{Multicurve partitions:}
  \begin{equation}
    f(x,y)=\prod_{r=1}^K \mathrm{sign}(y-P_r(x)),
    \qquad K\in\{3,5,7\},
  \end{equation}
  with each $P_r$ a random odd Hermite polynomial of degrees $1,3,5$.

  \item \emph{Pixel random partitions:} a random coarse $K\times K$ sign pattern,
  with $K\in\{20,30,40,60\}$, constrained by central oddness.
\end{enumerate}

For each resulting tiger pair $(f,g)$ we computed two quantities.  First, we computed
$\widetilde B_K(f,g)$ using \eqref{eq:konig-normalized}.  Second, we computed the
majorant constant $c_{f,g}$.  More explicitly, with $h_n$ the orthonormal probabilist
Hermite polynomial, set
\begin{equation}
  \widehat C_f[i,j]
  := \mathbb E\big[f(X,Y)h_i(X)h_j(Y)\big],
  \qquad X,Y\sim N(0,1),
\end{equation}
and define the Hermite correlation series
\begin{equation}
  B_{f,g}(z)=\sum_{n\ge 1} b_nz^n,
  \qquad
  b_n:=\sum_{i+j=n}\widehat C_f[i,j]\widehat C_g[i,j].
  \label{eq:b-series}
\end{equation}
The inverse series
\begin{equation}
  A_{f,g}(z)=B_{f,g}^{-1}(z)=\sum_{n\ge 1}a_nz^n
\end{equation}
then determines
\begin{equation}
  c_{f,g}:=\text{the positive solution of}\quad
  \sum_{n\ge 1}|a_n|c^n=1.
  \label{eq:cfg-majorant}
\end{equation}
This is the same majorant that appears in Krivine rounding.  The signed equation
$\sum_n a_nc^n=1$ was also recorded as a diagnostic, but it is not the Grothendieck
certificate; the relevant quantity is \eqref{eq:cfg-majorant}.

\subsection{Results: sigma improves $B_K$, not $c_{f,g}$}
\label{subsec:tiger-results}

The headline result is that the sigma operator does exactly what it is designed to do:
it finds partitions with excellent K\"onig bilinear value.  However, these partitions do
not improve the majorant constant $c_{f,g}$.  Across all $1000$ trials, no tiger pair
produced a genuine improvement over
\begin{equation}
  c_K=\frac{2}{\pi}\log(1+\sqrt2)\approx 0.56110.
\end{equation}
The two numerical values marginally above $c_K$ were at the level of the observed grid
error and occurred for partitions essentially indistinguishable from the hyperplane
fixed point.

\begin{table}[h]
\centering
\begin{tabular}{lrrrr}
\hline
Quantity & Min & Max & Mean & Median \\
\hline
$\widetilde B_K(f,g)$ & $0.5611$ & $0.5619$ & $0.5618$ & $0.5619$ \\
$c_{f,g}$, majorant & $0.5072$ & $0.5611$ & $0.5169$ & $0.5079$ \\
$c_{f,g}$, signed diagnostic & $0.717$ & $1.705$ & $0.725$ & $0.719$ \\
\hline
\end{tabular}
\caption{Aggregate statistics over $1000$ random odd initial partitions after sigma iteration.}
\label{tab:tiger-summary-statistics}
\end{table}

The iteration usually did not converge to a fixed point.  Instead, it typically entered
a stable two-cycle:
\begin{equation}
  870/1000
  \quad\text{runs showed oscillatory behavior, while only}\quad
  5/1000
  \quad\text{converged to a fixed point.}
\end{equation}
Oddness violations were zero in all runs.  The distribution by initial family was as
follows.

\begin{table}[h]
\centering
\begin{tabular}{lrrrr}
\hline
Initial family & Mean $c_{f,g}$ & Median $c_{f,g}$ & Max $c_{f,g}$ & $\#\{c_{f,g}\ge c_K\}$ \\
\hline
Hyperplane perturbation & $0.5263$ & $0.5081$ & $0.5611$ & $1$ \\
Multicurve & $0.5184$ & $0.5080$ & $0.5611$ & $1$ \\
Pixel random & $0.5119$ & $0.5078$ & $0.5609$ & $0$ \\
DSL random & $0.5109$ & $0.5078$ & $0.5598$ & $0$ \\
\hline
\end{tabular}
\caption{Per-family majorant constants.  The two apparent exceedances of $c_K$ are at grid-error scale, approximately $10^{-5}$, and are not considered genuine improvements.}
\label{tab:tiger-family-statistics}
\end{table}

The data separate into two qualitatively different attractors.

\paragraph{Attractor A: the Krivine-like fixed point.}
Roughly $130$ trials, mostly from the hyperplane perturbation and multicurve families,
returned close to the hyperplane fixed point.  These runs had
\begin{equation}
  f\approx g,
  \qquad
  c_{f,g}\approx c_K,
  \qquad
  \widetilde B_K(f,g)\approx c_K.
\end{equation}
They are best interpreted as returning to the classical Krivine scheme rather than
finding a new scheme.

\paragraph{Attractor B: the oscillatory tiger pair.}
The dominant outcome was a nontrivial two-cycle $f\ne g$.  These runs had
\begin{equation}
  \widetilde B_K(f,g)\approx 0.5619
  \quad\text{but}\quad
  c_{f,g}\approx 0.508.
\end{equation}
Thus the generic tiger pair improves K\"onig's bilinear form above the hyperplane
level, but it substantially worsens the majorant constant.  The same runs typically
satisfied
\begin{equation}
  c_{f,f}\approx c_{g,g}\approx 0.513,
  \qquad
  c_{f,g}\approx 0.508,
\end{equation}
showing that the failure is not merely caused by comparing two unrelated states in a
cycle.  Both self-pairings and cross-pairings are far below $c_K$.

This explains why the tiger fixed point is misleading as a guide to the Grothendieck
constant.  The sigma operator is a best-response dynamics for $\widetilde B_K$, so it is
expected to increase, or nearly increase, $\widetilde B_K$.  But $c_{f,g}$ only agrees
with $\widetilde B_K$ in the alternating regime \eqref{eq:alternating-condition}.  The
oscillatory tiger pairs are visibly and algebraically non-alternating: the inverse
series has sign defects and large higher-order contributions.  Passing to absolute
values in \eqref{eq:cfg-majorant} then penalizes exactly the coefficients that the
oscillatory value $\widetilde B_K$ can hide through cancellation.

\subsection{Mixing tiger series with the hyperplane series}
\label{subsec:tiger-mixing}

A weaker possibility is that tiger pairs are not themselves optimal, but that their
Hermite data contain a useful perturbation direction.  To test this, for each tiger pair
we mixed its $b$-series with the hyperplane $b$-series:
\begin{equation}
  b_{\mathrm{mix},n}(p)
  := (1-p)b_{\mathrm{hyp},n}+p b_{\mathrm{tiger},n},
  \qquad p\in[0,1].
  \label{eq:tiger-b-mixing}
\end{equation}
For each $p$ we inverted the resulting series and computed the majorant root.  We then
maximized over $p\in[0,1]$ using a one-dimensional Brent search, checking both endpoints
explicitly.

This test is useful because it separates two possible explanations.  If the tiger
series contained a small but useful direction, the optimum of \eqref{eq:tiger-b-mixing}
would occur at an interior $p>0$ even if the pure tiger endpoint were bad.  The code was
validated on analytic $\pm\eta h_3$ perturbation pairs, where such interior optima do
appear at grid-error scale.  For example, near $\eta=0.08$, the best mixture used about
$26\%$ of the perturbation series and improved the grid hyperplane value by
approximately $4.8\cdot 10^{-6}$, comparable to the $10^{-5}$ discretization error and
not above the analytic Krivine value.

For the tiger data, the result was completely different.  Every one of the $1000$
experiments had optimal mixing parameter
\begin{equation}
  p^*=0.
\end{equation}
That is, the best point on every segment from the hyperplane $b$-series to a tiger
$b$-series was the pure hyperplane endpoint.  No experiment improved the majorant by
any positive amount at the numerical precision of the sweep.

\begin{table}[h]
\centering
\begin{tabular}{lr}
\hline
Improvement threshold & Number of tiger mixtures exceeding it \\
\hline
$>0$ & $0/1000$ \\
$>10^{-10}$ & $0/1000$ \\
$>10^{-8}$ & $0/1000$ \\
$>10^{-6}$ & $0/1000$ \\
$>10^{-4}$ & $0/1000$ \\
\hline
\end{tabular}
\caption{No convex mixture of a tiger $b$-series with the hyperplane $b$-series improved the majorant constant.}
\label{tab:tiger-mixing-thresholds}
\end{table}

Per family, the best mixed value was always the grid hyperplane value, about
$0.561110$, with best improvement equal to zero.  The mean optimizer was numerically
zero in every family: $1.4\cdot10^{-13}$ for hyperplane perturbations, $0$ for DSL
random partitions, $2.8\cdot10^{-11}$ for multicurves, and $3.6\cdot10^{-15}$ for pixel
random partitions.

\subsection{Conclusion}
\label{subsec:tiger-conclusion}

The experiments support the following picture.

First, tiger partitions are real K\"onig optimizers, or at least extremely strong
numerical candidates for such optimizers.  The sigma operator drives a wide range of
odd initial partitions toward states with normalized K\"onig value at or above the
hyperplane level, and the generic oscillatory tiger pair has
$\widetilde B_K\approx 0.5619>c_K$.

Second, the same partitions are not good Krivine rounding schemes.  The majorant
constant of the generic tiger pair is about $0.508$, far below $c_K\approx0.56110$.
Even convex interpolation at the level of Hermite $b$-series fails to extract an
improving direction: every tiger mixture is optimized at the pure hyperplane endpoint.

Third, this is not a paradox but a structural warning.  K\"onig's bilinear form is
aligned with the Grothendieck majorant only for alternating inverse series.  The tiger
pairs produced by sigma iteration are strongly non-alternating, so increasing
$\widetilde B_K$ need not increase $c_{f,g}$ and in practice decreases it substantially.
Thus the tiger experiments give strong evidence that one should not search for better
Grothendieck bounds by optimizing K\"onig's bilinear form alone.  The next section
therefore turns to families designed to control the inverse-series majorant directly,
rather than families generated by sigma best-response dynamics.


==> paper/conclusion.tex <==
% \section{Conclusion}

% In this paper, we improve upon the best known upper bound on the Grothendieck constant, namely Krivine's landmark 1977 result. 
% We do this by removing a key obstruction in \cite{braverman2011grothendieckconstantstrictlysmaller}'s analysis of rounding schemes. Our approach allows us to analyze schemes directly, without first passing through a hyperplane mixture. This leads to a significant numerical improvement on the upper bound for the Grothendieck constant. Using our approach together with an AI-guided search over rounding schemes, we obtain a \(6.04 \cdot 10^{-5}\) improvement on Krivine's hyperplane bound. In relation to the Grothendieck constant, we also investigate K\"onig's bilinear form. Numerically, we find that the conjectured extremizers of this form are not competitive for improving the Grothendieck bound, illustrating a separation between the K\"onig objective and the Grothendieck objective. Nevertheless, K\"onig's bilinear form remains an interesting extremal object in its own right, and we exhibit an explicit asymptotic family whose value strictly improves on the hyperplane benchmark as the dimension tends to infinity. 


==> paper/mixing_discussion.tex <==
\section{Discussion: why mixing can improve the inverse majorant}
\label{sec:discussion-mixing}

One of the main findings of this paper is that a randomized mixture of rounding schemes can
sometimes give a \emph{strictly} better Grothendieck bound than either component scheme.
Intuitively, different schemes can perform well on different difficult configurations of
vectors, so the right search space is not just the set of individual partitions, but also the
simplex of mixtures of promising partitions.

The mechanism is visible in the inverse series. For a two-scheme mixture, the correlation
coefficients are linear in the mixing parameter,
$b_{2m+1}(p)=(1-p)b^{(0)}_{2m+1}+p b^{(1)}_{2m+1}$. The inverse coefficients in
$H_p^{-1}(\zeta)=\sum_{m\ge 0}a_{2m+1}(p)\zeta^{2m+1}$, however, are not linear in $p$.
Comparing coefficients in $H_p(H_p^{-1}(\zeta))=\zeta$ determines them recursively, so
$a_{2m+1}(p)$ is a rational function of $b_1(p),b_3(p),\ldots,b_{2m+1}(p)$, with denominators
involving powers of $b_1(p)$. Thus, wherever $b_1(p)=H_p'(0)\neq 0$, the functions
$a_{2m+1}(p)$ are real analytic in $p$. Since the bound is controlled by
\[
    M_p(\gamma)=\sum_{m\ge 0}|a_{2m+1}(p)|\gamma^{2m+1}\le 1,
\]
by continuity a sign change in an inverse coefficient can be converted into an actual cancellation, removing
one term from the absolute-value series.

A simple example is obtained by mixing the hyperplane scheme with the perturbation schemes described in \cref{app:explicit-mixture-coefficients}. With $p$ denoting the perturbation weight, the numerical
one-parameter optimum occurs at the root $a_7(p)=0$. The resulting
bound is smaller than both the hyperplane scheme value and the pure perturbation scheme value. This reflects the broader empirical pattern in our mixed searches: the
best improvements occur when the two endpoint schemes have opposite signs for $a_7$, so that
continuity forces a mixture for which the $a_7$-term vanishes. It remains an interesting
question whether a better mixture can cancel an earlier coefficient, such as $a_5$, while
keeping the lower-order $a_1$ and $a_3$ terms essentially unchanged.


==> paper/proof_outline.tex <==
\section{Improving the Grothendieck Constant with no Mixing}

\begin{definition}[Real Grothendieck constant]\label{def:real-grothendieck-constant}

The real Grothendieck constant $K_G$ is the infimum over all $K>0$ such that, for every $m,n\in\mathbb N$ and every real matrix $A=(a_{ij})\in\R^{m\times n}$,
\[
\sup_{x_i,y_j\in S^{m+n-1}}
\sum_{i=1}^m\sum_{j=1}^n a_{ij}\ip{x_i}{y_j}
\le
K\sup_{\varepsilon_i,\delta_j\in\{-1,1\}}
\sum_{i=1}^m\sum_{j=1}^n a_{ij}\varepsilon_i\delta_j .
\]
\end{definition}

\begin{definition}[Gaussian correlation]\label{def:gaussian-correlation}
Fix $k \in \mathbb{N}$, and let $f,g:\mathbb{R}^k\to\{-1,1\}$ be odd measurable functions.
Let $G_1,G_2$ be independent standard Gaussian vectors in $\mathbb{R}^k$.

The \emph{arcsine-normalized correlation} associated to $(f,g)$ is
\[
H_{f,g}(t)
:=
\frac{\pi}{2}\,
\mathbb{E}\left[
f\left(\frac{G_1}{\sqrt{2}}\right)
g\left(
\frac{tG_1+\sqrt{1-t^2}G_2}{\sqrt{2}}
\right)
\right],
\qquad -1<t<1.
\]
\end{definition}


\begin{lemma}[Basic analytic properties]\label[lemma]{lemma:correlation-profile-analytic}
Let $f,g:\mathbb{R}^k\to\{-1,1\}$ be odd measurable functions. Then $H_{f,g}$ is odd and
extends holomorphically to the strip
\[
S:=\{z\in\mathbb{C}: |\operatorname{Re}z|<1\}.
\]
In particular, if $H_{f,g}'(0)\neq 0$, then $H_{f,g}$ has a unique local inverse branch at
the origin, and this inverse branch is odd.
\end{lemma}
\begin{proof}
This is the standard analytic continuation of the Gaussian correlation kernel.  In the planar case used below we prove the stronger quantitative version in \cref{lemma:strip-bound}.
\end{proof}

We recall the properties of the inverse $H_{f,g}^{-1}$ as abstracted in \cite{braverman2011grothendieckconstantstrictlysmaller}. 

\begin{lemma}[Local Inverse Expansion]\label[lemma]{lemma:local-inverse-expansion}

Let $f,g:\mathbb{R}^k\to\{-1,1\}$ be odd and measurable functions with $H'_{f,g}(0) \neq 0$. Let $H^{-1}_{f,g}$ be the unique local inverse branch of $H_{f,g}$ at the origin. Then,
\begin{itemize}
\item $H^{-1}_{f,g}$ is odd. 
    \item $H^{-1}_{f,g}$ has a Taylor-series expansion at the origin: $H^{-1}_{f,g}(\zeta) = \sum_{n\geq 1} a_n \zeta^n$. 
\end{itemize}
Further, if $\gamma > 0$ is such that $\sum_{n \geq 1} |a_n| \gamma^n \leq 1$, then the Grothendieck constant 
$$ K_G \leq \frac{\pi}{2\gamma}.$$ 
\end{lemma}

For completeness, we give a proof of this with our notation in the appendix.

\begin{definition}[$\gamma$-admissible Krivine Rounding Scheme]
    For $f,g:\mathbb{R}^k\to\{-1,1\}$ odd and measurable functions with $H'_{f,g}(0) \neq 0$, and $\gamma > 0$, we say $(f,g)$ is a $\gamma$-admissible Krivine rounding scheme if the conditions of \cref{lemma:local-inverse-expansion} hold. In particular, for a $\gamma$-admissible Krivine rounding scheme, one has \[K_G \le \frac{\pi}{2\gamma}.\]
\end{definition}

\begin{definition}[The $\Hermite$ scheme]\label[lemma]{def:h3-scheme}
Let
\[
\Hermite(x)=8x^3-12x,
\qquad
\tau=0.03175,
\qquad
\eta=\frac{\tau}{\sqrt{48}}
=0.004582717761692655\ldots .
\]
Define odd measurable functions $f,g:\R^2\to\{\pm1\}$ by
\[
    f(x,y)=\sgn(y-\eta \Hermite(x)),
    \qquad
    g(x,y)=\sgn(y+\eta \Hermite(x)).
\]
We call $(f,g)$ the $\Hermite$ scheme.
\end{definition}

The following is our main theorem.

\begin{theorem}[Improved Grothendieck Constant]\label[theorem]{thm:no-mixing-beats-hyperplane}
Let
\[
\rhostarval:=\log(1+\sqrt2),
\qquad
\gzero:=\rhostarval+4.8\cdot 10^{-6}.
\]
Then the $\Hermite$ scheme is a $\gzero$-admissible Krivine scheme.  In particular,
\[
K_G
\le \frac{\pi}{2\gzero}
<
\frac{\pi}{2\log(1+\sqrt2)}
-
9.7\cdot 10^{-6}.
\]
\end{theorem}

The proof has two main components. Recall that using \cref{lemma:local-inverse-expansion}, the main goal is to show that 
$$\sum_{n \geq 1} |a_n| \gamma_0^n \leq 1,$$
where $(a_n)_{n \geq 1}$ are the Taylor-series coefficients of $H_{f,g}^{-1}$. We split this into parts. Define
\begin{itemize}
    \item An analytic argument that bounds the remainder term---$\sum_{n > k_0} |a_n| \gamma_0^n$---to very good precision (about $2.44 \cdot 10^{-9}$) for $k_0 = 220$. This analytic portion relies on elementary complex analysis and carefully chosen contour integration. This approach can also extend to schemes similar to $\Hermite$ scheme. See \cref{sec:analytic}.
    \item A numerical analysis portion that uses \texttt{Arb} \cite{johansson2017arb} to compute the \emph{head}, $\sum_{n \leq k_0} |a_n| \gamma_0^n$ to very high precision showing that this value is less than $1 - 2.5 \cdot 10^{-9}$. We discuss the challenges involved here and the certification of this computation in \cref{sec:numerical-computation-of-head}. 
\end{itemize}

First, we describe how to do the necessary computation of the coefficients of the Taylor series. 

\section{Coefficient Computation Formulas}
\label{sec:coefficient-computation-formulas}

In this section, we describe the analytic facts needed to compute the coefficients of Taylor series of $H_{f,g}$ and $H_{f,g}^{-1}$ used in the proof.


Let \(h_n\) denote the physicist's Hermite polynomial and set
\[
    \HermBasis_n(x):=\frac{h_n(x)}{\sqrt{2^n n!}},
    \qquad
    d\mu(x):=\pi^{-1/2}e^{-x^2}\,dx.
\]
Then \(\{\HermBasis_n\}_{n\ge0}\) is an orthonormal basis for \(L^2(\mu)\).

\begin{lemma}[Hermite--Mehler reduction]\label[lemma]{lemma:hermite-mehler-reduction}
For the \(\Hermite\) scheme, define the Hermite coefficients
\[
    \HermCoeff_{a,b}
    :=
    \int_{\mathbb R^2}
        f(x,y)\HermBasis_a(x)\HermBasis_b(y)
    \,d\mu(x)d\mu(y).
\]
Then
\[
    H(z)
    =
    \frac{\pi}{2}
    \sum_{a,b\ge0}
        (-1)^a \HermCoeff_{a,b}^2 z^{a+b}.
\]
Equivalently,
\[
    [z^n]H(z)
    =
    \frac{\pi}{2}
    \sum_{a=0}^{n}
        (-1)^a \HermCoeff_{a,n-a}^2.
\]
Moreover, the two-dimensional coefficients reduce to the one-dimensional
integrals
\[
    \HermCoeff_{a,b}
    =
    \int_{\mathbb R}
        \HermBasis_a(x)
        \ThresholdCoeff_b\!\left(\tau\HermBasis_3(x)\right)
    \,d\mu(x),
\]
where
\[
    \ThresholdCoeff_0(u)=-\operatorname{erf}(u),
\]
and, for \(b\ge1\),
\[
    \ThresholdCoeff_b(u)
    =
    \frac{2}{\sqrt\pi}
    e^{-u^2}
    \frac{\HermBasis_{b-1}(u)}{\sqrt{2b}}.
\]
\end{lemma}

\begin{proof}
Expanding \(f\) in the orthonormal tensor-product basis gives
\[
    f(x,y)=\sum_{a,b\ge0}
        \HermCoeff_{a,b}\HermBasis_a(x)\HermBasis_b(y).
\]
For the \(\Hermite\) scheme we have \(g(x,y)=f(-x,y)\).  Since
\(\HermBasis_a(-x)=(-1)^a\HermBasis_a(x)\), the corresponding coefficient of
\(g\) is \((-1)^a\HermCoeff_{a,b}\).

The Mehler kernel diagonalizes in this basis: the basis vector
\(\HermBasis_a(x)\HermBasis_b(y)\) has eigenvalue \(z^{a+b}\).  Therefore
\[
    H(z)
    =
    \frac{\pi}{2}
    \sum_{a,b\ge0}
        (-1)^a \HermCoeff_{a,b}^2 z^{a+b},
\]
which gives the displayed coefficient formula.

It remains to reduce \(\HermCoeff_{a,b}\) to one dimension.  For fixed \(x\),
the partition is
\[
    f(x,y)=\operatorname{sgn}\!\left(y-\tau\HermBasis_3(x)\right).
\]
Thus the \(y\)-coefficient is
\[
    \ThresholdCoeff_b(u)
    :=
    \int_{\mathbb R}
        \operatorname{sgn}(y-u)\HermBasis_b(y)\,d\mu(y).
\]
For \(b=0\), this equals \(-\operatorname{erf}(u)\).  For \(b\ge1\), using
\[
    \frac{d}{dy}\left(e^{-y^2}h_{b-1}(y)\right)
    =
    -e^{-y^2}h_b(y)
\]
gives
\[
    \ThresholdCoeff_b(u)
    =
    \frac{2}{\sqrt\pi}
    e^{-u^2}
    \frac{\HermBasis_{b-1}(u)}{\sqrt{2b}}.
\]
Substituting \(u=\tau\HermBasis_3(x)\) gives the claimed one-dimensional
formula for \(\HermCoeff_{a,b}\).
\end{proof}

Next we convert the Taylor coefficients of \(H\) into the Taylor coefficients
of its inverse.

\begin{lemma}[Inverse coefficients by Lagrange inversion]
\label[lemma]{lemma:lagrange-inverse-coefficients}
Since \(H\) is odd, write
\[
    H(z)=z\OddFactor(z^2).
\]
Then \(H^{-1}\) has only odd coefficients, and
\[
    a_{2k+1}
    =
    \frac{1}{2k+1}
    [t^k]\OddFactor(t)^{-(2k+1)},
    \qquad
    a_{2k}=0.
\]
\end{lemma}

\begin{proof}
This is the standard Lagrange inversion formula applied to the odd map
\(H(z)=z\OddFactor(z^2)\).  Oddness of \(H\) implies oddness of the local
inverse branch, so the even inverse coefficients vanish.
\end{proof}

\section{Bounding the Remainder Analytically}\label{sec:analytic}

 Define the \textbf{inverse majorant series} as 
\[
M_{f,g}(s):=\sum_{n\ge 1}|a_n|s^n,
\]
We now give our main analytic argument to bound the remainder term of the inverse majorant series of $\Hshort^{-1}$ for the $\Hermite$ scheme. A similar argument extends to other schemes as well, which we later show in \cref{sec:generalization}. The rest of this section is dedicated to the following lemma. 
\begin{lemma}[Majorant Remainder Bound]\label[lemma]{lemma:tail-bound}
Let $(f,g)$ be the $\Hermite$ scheme and let  
\[
H_{f,g}^{-1}(\zeta)=\sum_{n\ge1}a_n\zeta^n,
\qquad
\gzero=\log(1+\sqrt2)+4.8\cdot10^{-6}.
\]
Then
\[
\sum_{n>220}|a_n|\gzero^n<2.5\cdot10^{-9}.
\]
\end{lemma}

For brevity, we assume $(f,g)$ is fixed to be the $\Hermite$ scheme and we write $\Hshort^{-1}$, $\Mshort$ instead of $H^{-1}_{f,g}$, $M_{f,g}$. 


\subsection{Preliminary Lemma}

Here, we prove some preliminary analytic facts.  

\begin{lemma}[Strip bound]\label[lemma]{lemma:strip-bound}
Let $f,g:\R^2\to\{-1,1\}$ be measurable and let $H=H_{f,g}$ be the
arcsine-normalized correlation function.
Then $H$ extends holomorphically to
\[
 S=\{z\in\C: |\operatorname{Re}z|<1\}.
\]
Moreover, if $z=a+ib\in S$, then
\[
 |H(z)|\le \frac{\pi}{2}\frac{|1-z^2|}{1-a^2}.
\]
\end{lemma}

\begin{proof}
For real $|t|<1$, the arcsine-normalized correlation admits the integral representation
\[
H(t)=\frac{1}{2\pi(1-t^2)}
\int_{\R^2}\int_{\R^2}
f(x)g(y)
\exp\left(
-\frac{\|x\|^2+\|y\|^2-2t\ip{x}{y}}{1-t^2}
\right)\,dx\,dy .
\]
For $z\in S$, this formula defines the candidate holomorphic extension.  Since $|f|=|g|=1$,
\[
|H(z)|\le
\frac{1}{2\pi |1-z^2|}
\int_{\R^2}\int_{\R^2}
\exp\left(
-\operatorname{Re}\frac{\|x\|^2+\|y\|^2-2z\ip{x}{y}}{1-z^2}
\right)\,dx\,dy .
\]
Use the identity
\[
\frac{\|x\|^2+\|y\|^2-2z\ip{x}{y}}{1-z^2}
=
\frac12\frac{\|x+y\|^2}{1+z}
+
\frac12\frac{\|x-y\|^2}{1-z}.
\]
Writing $z=a+ib$, set
\[
A_+ := \operatorname{Re}\frac{1}{1+z}
=\frac{1+a}{(1+a)^2+b^2},
\qquad
A_- := \operatorname{Re}\frac{1}{1-z}
=\frac{1-a}{(1-a)^2+b^2}.
\]
Both are positive for $|a|<1$.  With $u=x+y$ and $v=x-y$, the Jacobian from $(u,v)$ to $(x,y)$ in $\R^4$ is $1/4$.  Thus the Gaussian integral is
\[
\frac14\cdot\frac{2\pi}{A_+}\cdot\frac{2\pi}{A_-}
=\frac{\pi^2}{A_+A_-}.
\]
Finally,
\[
A_+A_-=
\frac{1-a^2}{|1+z|^2|1-z|^2}
=
\frac{1-a^2}{|1-z^2|^2}.
\]
Substitution gives
\[
|H(z)|\le
\frac{1}{2\pi |1-z^2|}\cdot
\frac{\pi^2 |1-z^2|^2}{1-a^2}
=
\frac{\pi}{2}\frac{|1-z^2|}{1-a^2}.
\]
The same estimate is uniform on compact subsets of $S$, so the integral converges locally uniformly and the extension is holomorphic by dominated convergence.
\end{proof}


\subsection{The Key Change of Variable}

Next, we make a key change of variable that makes the analytic argument go through. 

\begin{definition}[The key change of variable]\label[lemma]{def:key-change-of-variable}
For the rest of the proof, put
\[
F(w)\defeq H(\sin w).
\]
\end{definition}

For the hyperplane scheme $H_0(t)=\arcsin t$, hence $H_0(\sin w)=w$ on the principal strip. This is why the comparison below is made against the identity map. 

\begin{lemma}[Sine-coordinate bound]\label[lemma]{lemma:sine-coordinate-bound}
For $F(w)=H(\sin w)$, the function $F$ is holomorphic on $|w|<1.1$ and
\[
 |F(w)-w|<15.3\qquad (|w|\le1.1).
\]
\end{lemma}

\begin{proof}
Write $w=u+iv$. Then
\[
\operatorname{Re}(\sin w)=\sin u\cosh v.
\]
By \cref{lemma:disk-to-strip-check}, if $u^2+v^2\le 1.1^2$, then
\[
|\sin u|\cosh v<0.946<1.
\]
Therefore $\sin w\in S$ for $|w|\le 1.1$, and \cref{lemma:strip-bound} implies that $F$ is holomorphic on $|w|<1.1$.  Applying \cref{lemma:strip-bound} with $z=\sin w$ gives
\[
|F(w)|
\le
\frac{\pi}{2}\frac{|1-\sin^2 w|}{1-(\operatorname{Re}\sin w)^2}
=
\frac{\pi}{2}\frac{|\cos w|^2}{1-(\operatorname{Re}\sin w)^2}.
\]
By \cref{lemma:cosine-ratio-check}, the last expression is $<14.19$ on $|w|\le 1.1$.  Hence
\[
|F(w)-w|\le |F(w)|+|w|<14.19+1.1<15.3.
\]
\end{proof}

Next, we prove a general sufficient condition for the radius of convergence and supremum of the inverse of a holomorphic function on a disk. 

\begin{lemma}[Rouch\'e inverse disk]\label[lemma]{lemma:rouche-inverse-disk}
Let $F$ be holomorphic on $|w|<r$, with $F(0)=0$, and suppose that for some
$R<M<r$,
\[
 \sup_{|w|=M}|F(w)-w|<M-R.
\]
Then:
\begin{enumerate}[label=(\roman*)]
    \item $F^{-1}$ is holomorphic on $R\D$;
    \item for $|\zeta|<R$, the inverse satisfies $|F^{-1}(\zeta)|<M$.
\end{enumerate}
\end{lemma}

\begin{proof}
Fix $|\zeta|<R$.  On $|w|=M$,
\[
|(F(w)-\zeta)-(w-\zeta)|=|F(w)-w|<M-R<M-|\zeta|\le |w-\zeta|.
\]
By Rouch\'e's theorem, $F(w)-\zeta$ and $w-\zeta$ have the same number of zeros in $|w|<M$, counted with multiplicity.  Since $w-\zeta$ has exactly one zero in this disk, $F(w)=\zeta$ has exactly one solution in $|w|<M$, counted with multiplicity.  In particular, the solution is simple.  The holomorphic inverse function theorem gives local inverse branches, and uniqueness makes these branches glue over $R\D$.  The same argument gives $|F^{-1}(\zeta)|<M$.
\end{proof}

\begin{corollary}[Radius and supremum of $|F^{-1}|$]\label[corollary]{cor:F-inverse-radius}
Taking $r=1.1$, $R=0.975$, and $M=0.98$, the inverse $F^{-1}$ is holomorphic on $0.975\D$ and
\[
|F^{-1}(\zeta)|<0.98\qquad (|\zeta|<0.975).
\]
\end{corollary}

\begin{proof}
Let
\[
\Delta(w):=F(w)-w=\sum_{n\ge1}d_nw^n.
\]
A computation in \texttt{Arb} gives the finite head estimate
\[
\sum_{n\le 220}|d_n|0.98^n<0.00454106848.
\]
By \cref{lemma:sine-coordinate-bound} and Cauchy's estimate, taking the Cauchy radius to $1.1$ from below gives
\[
\sum_{n>220}|d_n|0.98^n
\le
15.3\frac{(0.98/1.1)^{221}}{1-0.98/1.1}
<1.149\cdot10^{-9}.
\]
Therefore
\[
\sup_{|w|=0.98}|F(w)-w|
\le
\sum_{n\ge1}|d_n|0.98^n
<0.00454106848+1.149\cdot 10^{-9}
<0.005.
\]
Since $M-R=0.98-0.975=0.005$, \cref{lemma:rouche-inverse-disk} applies with $r=1.1$, $M=0.98$, and $R=0.975$.
\end{proof}

\begin{corollary}[Radius and supremum of $|H^{-1}|$]\label[corollary]{cor:H-inverse-radius}
Undoing the change of variables, we get
\[
H^{-1}=\sin\circ F^{-1}.
\]
Thus $H^{-1}$ is holomorphic on $0.975\D$ and
\[
|H^{-1}(\zeta)|<\sinh(0.98)<1.145
\qquad (|\zeta|<0.975).
\]
\end{corollary}

\begin{proof}
Since $F=H\circ\sin$, the identity $F^{-1}=\arcsin\circ H^{-1}$ is equivalent to
$H^{-1}=\sin\circ F^{-1}$ on the inverse branch at the origin.  By \cref{cor:F-inverse-radius}, $|F^{-1}(\zeta)|<0.98$ for $|\zeta|<0.975$.  The elementary bound
\[
|\sin z|\le \sinh |z|
\]
for complex $z$ gives
\[
|H^{-1}(\zeta)|=|\sin(F^{-1}(\zeta))|<\sinh(0.98)<1.145.
\]
\end{proof}

Finally, we are ready to prove \cref{lemma:tail-bound}.

\begin{lemma*}[Majorant Remainder bound]
Let
\[
H^{-1}(\zeta)=\sum_{n\ge1}a_n\zeta^n,
\qquad
\gzero=\log(1+\sqrt2)+4.8\cdot10^{-6}.
\]
Then
\[
\sum_{n>220}|a_n|\gzero^n<2.5\cdot10^{-9}.
\]
\end{lemma*}

\begin{proof}
By \cref{cor:H-inverse-radius}, $H^{-1}$ is holomorphic on $0.975\D$ and satisfies $|H^{-1}(\zeta)|<1.145$ there.  Hence, for every $s<0.975$, Cauchy's estimate with radius tending to $0.975$ gives
\[
\sum_{n>220}|a_n|s^n
\le
1.145\frac{(s/0.975)^{221}}{1-s/0.975}.
\]
Taking $s=\gzero$ yields
\[
1.145\frac{(\gzero/0.975)^{221}}{1-\gzero/0.975}
<2.44\cdot10^{-9}
<2.5\cdot10^{-9},
\]
as claimed.
\end{proof}

\section{Numerical Computation of the Head}
\label{sec:numerical-computation-of-head}

We now describe the certified computation of the head of the inverse-majorant
series for the \(\Hermite\) scheme.  

\begin{lemma}[Majorant head bound]\label[lemma]{lemma:head-bound}
Let
\[
    M_{f,g}(s)=\sum_{n\ge1}|a_n|s^n
\]
be the inverse majorant for the \(\Hermite\) scheme.  For
\[
    \gzero=\log(1+\sqrt2)+4.8\cdot10^{-6},
\]
one has
\[
    \sum_{1\le n\le220}|a_n|\gzero^n
    <1-2.5\cdot10^{-9}.
\]
\end{lemma}
 

\begin{proof}
Using \cref{lemma:hermite-mehler-reduction}, the Taylor coefficients of
\(H\) through degree \(220\) are determined by one-dimensional integrals for
the coefficients \(\HermCoeff_{a,b}\).  These integrals are evaluated using
Arb with outward-rounded interval arithmetic.  The resulting interval
enclosures for the Taylor coefficients of \(H\) are then converted into
interval enclosures for the inverse coefficients \(a_n\) using
\cref{lemma:lagrange-inverse-coefficients}.

The certified Arb computation gives
\[
    \sum_{n\le220}|a_n|\gzero^n
    <
    0.999999729.
\]
Since
\[
    0.999999729
    <
    1-2.5\cdot10^{-9},
\]
the desired head bound follows.
\end{proof}

\begin{remark}
We also independently verified the computations using floating-point and PyTorch computations in Python. However, the displayed inequality is certified by the outward-rounded Arb computation.
\end{remark}

\begin{corollary}[$\gamma_0$-admissibility]\label[lemma]{cor:gamma0-admissibility}
For the $\Hermite$ scheme,
\[
M_{f,g}(\gzero)<1.
\]
Consequently, the scheme is $\gzero$-admissible.
\end{corollary}

\begin{proof}
By \cref{lemma:majorant-head-value},
\[
\sum_{1\le n\le220}|a_n|\gzero^n<1-2.5\cdot10^{-9}.
\]
By \cref{lemma:tail-bound},
\[
\sum_{n>220}|a_n|\gzero^n<2.5\cdot10^{-9}.
\]
Adding the two inequalities gives $M_{f,g}(\gzero)<1$.  The inverse branch exists on a neighborhood of $\gzero\overline{\D}$ by \cref{cor:H-inverse-radius}, since $\gzero<0.975$.  Thus the $\Hermite$ scheme satisfies \cref{def:gamma-admissible}.
\end{proof}

\begin{proof}[Proof of \cref{thm:no-mixing-beats-hyperplane}]
By \cref{cor:gamma0-admissibility}, the $\Hermite$ scheme is $\gzero$-admissible.  Applying \cref{thm:krivine-preprocessing} gives
\[
K_G\le \frac{\pi}{2\gzero}.
\]
Finally, with $\rhostarval=\log(1+\sqrt2)$ and $\gzero=\rhostarval+4.8\cdot10^{-6}$,
\[
\frac{\pi}{2\rhostarval}-\frac{\pi}{2\gzero}
=
\frac{\pi(4.8\cdot10^{-6})}{2\rhostarval\gzero}
>9.7\cdot10^{-6}.
\]
Therefore
\[
K_G
\le
\frac{\pi}{2\gzero}
<
\frac{\pi}{2\log(1+\sqrt2)}-9.7\cdot10^{-6}.
\]
\end{proof}

% \begin{remark}[Equality convention]\label{rem:equality-convention}
% The equality convention for Krivine schemes can also be recovered.  The same Arb computation gives
% \[
% \sum_{n\le220}|a_n|(\rhostarval+5.2\cdot10^{-6})^n>1.000000291.
% \]
% Since $M_{f,g}$ is continuous on $[0,0.975)$, there exists
% \[
% \gamma\in(\rhostarval+4.8\cdot10^{-6},\rhostarval+5.2\cdot10^{-6})
% \]
% with $M_{f,g}(\gamma)=1$.
% \end{remark}

\section{Generalization.}
\label{sec:generalization}

\begin{theorem}[Mixed Krivine]\label[theorem]{thm:mixed-krivine-certificate}
Let $L\in\mathbb N$. For each $\ell\in\{1,\dots,L\}$, let
\[
f_\ell,g_\ell:\mathbb R^{k_\ell}\to\{-1,1\}
\]
be odd measurable functions, and let $H_\ell$ be their arcsine-normalized correlation profile:
\[
H_\ell(t)
=
\frac{\pi}{2}
\mathbb E\left[
f_\ell\left(\frac{G_1}{\sqrt2}\right)
g_\ell\left(
\frac{tG_1+\sqrt{1-t^2}G_2}{\sqrt2}
\right)
\right].
\]
Let $\lambda_1,\dots,\lambda_L\ge 0$ satisfy $\sum_{\ell=1}^L\lambda_\ell=1$, and define the mixed profile
\[
H_\lambda(t):=\sum_{\ell=1}^L\lambda_\ell H_\ell(t).
\]

Assume that $H_\lambda$ has a local inverse at the origin,
\[
H_\lambda^{-1}(\zeta)=\sum_{n\ge1}a_n\zeta^n,
\]
and that this inverse is holomorphic on a neighborhood of $\gamma\overline{\mathbb D}$ for some
$\gamma>0$. If
\[
M_\lambda(\gamma):=\sum_{n\ge1}|a_n|\gamma^n\le 1,
\]
then
\[
K_G\le \frac{\pi}{2\gamma}.
\]
\end{theorem}

\begin{theorem}[Finite mixed-profile theorem]\label[theorem]{thm:finite-mixed-profile-certificate}
Let $H_\lambda=\sum_{\ell=1}^L\lambda_\ell H_\ell$ be a mixed profile as in
\Cref{thm:mixed-krivine-certificate}. Define
\[
F(w):=H_\lambda(\sin w).
\]
Fix numbers
\[
0<R<M<r_0,
\qquad
N\in\mathbb N,
\qquad
\gamma<R.
\]
Assume the following four certified inequalities.

\begin{enumerate}
    \item \textbf{Sine-coordinate analytic bound.}
    The function $F$ is holomorphic on $|w|<r_0$, and
    \[
    |F(w)-w|\le B
    \qquad (|w|\le r_0).
    \]

    \item \textbf{Finite perturbation bound.}
    Writing
    \[
    F(w)-w=\sum_{n\ge1}d_nw^n,
    \]
    one has
    \[
    \sum_{n\le N}|d_n|M^n
    +
    B\frac{(M/r_0)^{N+1}}{1-M/r_0}
    <
    M-R.
    \]

    \item \textbf{Finite inverse-majorant head.}
    Writing
    \[
    H_\lambda^{-1}(\zeta)=\sum_{n\ge1}a_n\zeta^n,
    \]
    one has
    \[
    \sum_{n\le N}|a_n|\gamma^n
    \le
    1-T.
    \]

    \item \textbf{Cauchy remainder domination.}
    The remainder margin satisfies
    \[
    \sinh(M)\frac{(\gamma/R)^{N+1}}{1-\gamma/R}
    \le T.
    \]
\end{enumerate}

Then
\[
K_G\le \frac{\pi}{2\gamma}.
\]
\end{theorem}

\begin{proof}
By the finite perturbation bound,
\[
\sup_{|w|=M}|F(w)-w|<M-R.
\]
Rouche's theorem therefore implies that $F^{-1}$ is holomorphic on $R\mathbb D$ and satisfies
\[
|F^{-1}(\zeta)|<M
\qquad (|\zeta|<R).
\]
Since
\[
H_\lambda^{-1}(\zeta)=\sin(F^{-1}(\zeta)),
\]
we get
\[
|H_\lambda^{-1}(\zeta)|
<
\sinh(M)
\qquad (|\zeta|<R).
\]
Cauchy's estimate gives
\[
\sum_{n>N}|a_n|\gamma^n
\le
\sinh(M)\frac{(\gamma/R)^{N+1}}{1-\gamma/R}
\le T.
\]
Combining this with the finite inverse-majorant head gives
\[
M_\lambda(\gamma)
=
\sum_{n\ge1}|a_n|\gamma^n
\le
(1-T)+T
\le 1.
\]
The conclusion now follows from \Cref{thm:mixed-krivine-certificate}.
\end{proof}

\begin{remark}[What mixing changes]
Mixing changes the correlation profile before inversion:
\[
H_\lambda=\sum_{\ell}\lambda_\ell H_\ell.
\]
The inverse-majorant is then computed for $H_\lambda^{-1}$, not by mixing the inverse-majorants of the components. This is the point at which mixing can improve the final constant.
\end{remark}


% \appendix
% \section{Sine-coordinate maximization checks}

% \begin{lemma}[Disk-to-strip check]\label{lemma:disk-to-strip-check}
% Let $\rho=1.1$.  For all $u,v\in\R$ with $u^2+v^2\le\rho^2$,
% \[
% |\sin u|\cosh v<0.946.
% \]
% \end{lemma}

% \begin{proof}
% Since $\rho<\pi/2$, by symmetry we may assume $0\le u\le\rho$ and $v\ge0$.  For fixed $u$, $\cosh v$ is increasing in $v\ge0$, so it suffices to maximize
% \[
% \varphi(u):=\sin u\cosh s(u),
% \qquad
% s(u):=\sqrt{\rho^2-u^2},
% \qquad
% 0\le u\le\rho.
% \]
% For $0<u<\rho$,
% \[
% \varphi'(u)=\sin u\cosh s(u)
% \left(\cot u-\frac{u}{s(u)}\tanh s(u)\right).
% \]
% Let
% \[
% h(u):=\cot u-\frac{u}{s(u)}\tanh s(u).
% \]
% The function $u\mapsto\cot u$ is strictly decreasing.  Also
% \[
% A(s):=\frac{\tanh s}{s}
% \]
% is strictly decreasing for $s>0$, since
% \[
% A'(s)=\frac{s\operatorname{sech}^2s-\tanh s}{s^2}<0,
% \]
% the final inequality being equivalent to $\sinh s\cosh s-s>0$.  Since $s(u)$ is decreasing, $A(s(u))$ is increasing, and hence $uA(s(u))$ is increasing.  Therefore $h$ is strictly decreasing.

% Outward-rounded Taylor bounds give
% \[
% h(0.898)>0.796708-0.793956>0,
% \qquad
% h(0.900)<0.793553-0.796524<0.
% \]
% Thus the unique maximizer $u_*$ of $\varphi$ lies in $(0.898,0.900)$.  Take $c=0.899$.  On $[0.898,0.900]$,
% \[
% \varphi''(u)=
% \sin u\cosh s\left(\frac{u^2}{s^2}-1\right)
% -2\frac{u}{s}\cos u\sinh s
% -\frac{\rho^2}{s^3}\sin u\sinh s,
% \]
% where $s=s(u)$.  Throughout this interval,
% \[
% s^2\ge0.4,
% \qquad
% 0.632<s<0.636,
% \qquad
% \cosh s<1.21,
% \qquad
% \sinh s<0.68.
% \]
% These bounds give $|\varphi''(u)|<7$.  Since $|u_*-c|\le10^{-3}$,
% \[
% \varphi(u_*)\le \varphi(c)+\frac72\cdot10^{-6}.
% \]
% Now
% \[
% s(c)^2=1.21-0.899^2=0.401799<0.6339^2,
% \]
% so $\cosh s(c)<\cosh(0.6339)<1.20774$.  Also,
% \[
% \sin(0.899)<0.899-\frac{0.899^3}{6}+\frac{0.899^5}{120}<0.7828.
% \]
% Thus
% \[
% \varphi(c)<0.7828\cdot1.20774<0.945419,
% \]
% and consequently
% \[
% \varphi(u_*)<0.945419+0.0000035<0.946.
% \]
% \end{proof}

% \begin{lemma}[Cosine-ratio check]\label{lemma:cosine-ratio-check}
% For every $w\in\C$ with $|w|\le1.1$,
% \[
% \frac{\pi}{2}\frac{|\cos w|^2}{1-(\operatorname{Re}\sin w)^2}<14.19.
% \]
% \end{lemma}

% \begin{proof}
% Write $w=u+iv$ and put $\rho=1.1$.  We maximize over $u^2+v^2\le\rho^2$.  We have
% \[
% \operatorname{Re}(\sin w)=\sin u\cosh v,
% \qquad
% |\cos w|^2=\cos^2u+\sinh^2v.
% \]
% It is enough to bound
% \[
% Q(u,v):=\frac{\cos^2u+\sinh^2v}{1-\sin^2u\cosh^2v}.
% \]
% The denominator is positive by \cref{lemma:disk-to-strip-check}.  Set
% \[
% x:=\sin^2u,
% \qquad
% y:=\sinh^2v.
% \]
% Then
% \[
% Q(u,v)=\frac{1-x+y}{1-x-xy},
% \]
% and, for fixed $x$,
% \[
% \frac{\partial}{\partial y}\frac{1-x+y}{1-x-xy}
% =
% \frac{(1-x)^2}{(1-x-xy)^2}>0.
% \]
% Thus, for each fixed $u$, the maximum occurs at $|v|=\sqrt{\rho^2-u^2}$.  By evenness in $u$, it remains to maximize
% \[
% \Phi(u):=
% \frac{\cos^2u+\sinh^2s(u)}{1-\sin^2u\cosh^2s(u)},
% \qquad
% s(u):=\sqrt{\rho^2-u^2},
% \qquad
% 0\le u\le\rho.
% \]
% For $0<u<\rho$, differentiating gives
% \[
% \Phi'(u)=
% \frac{\sinh(2s)\cos u}{(1-\sin^2u\cosh^2s)^2}
% \left[
% \sin u\tanh s(1+\cosh^2s)
% -\frac{u}{s}\cos u(1+\sin^2u)
% \right],
% \]
% where $s=s(u)$.  The prefactor is positive.  Therefore the sign of $\Phi'(u)$ is the sign of $A(u)-1$, where
% \[
% A(u):=\frac{s(u)\tan u\tanh s(u)(1+\cosh^2s(u))}{u(1+\sin^2u)}.
% \]
% We show that $A$ is strictly decreasing.  Let
% \[
% B(s):=s\tanh s(1+\cosh^2s).
% \]
% Then
% \[
% \frac{d}{du}\log A(u)
% =
% \left(\frac{1}{\sin u\cos u}-\frac{1}{u}\right)
% -\frac{\sin(2u)}{1+\sin^2u}
% -\frac{u}{s}\frac{B'(s)}{B(s)}.
% \]
% Moreover,
% \[
% \frac{B'(s)}{B(s)}
% =
% \frac{1}{s}
% +
% \frac{1}{\sinh s\cosh s}
% +
% \frac{2\sinh s\cosh s}{1+\cosh^2s}.
% \]
% Since
% \[
% \frac{2\sinh s\cosh s}{1+\cosh^2s}\ge \tanh s
% \qquad\text{and}\qquad
% \frac{1}{\sinh s\cosh s}+\tanh s=\coth s>\frac1s,
% \]
% we have $B'(s)/B(s)>2/s$.  On the other hand, for $0<u<\rho$,
% \[
% \sin u\cos u=\frac12\sin(2u)>u-\frac23u^3.
% \]
% Therefore
% \[
% \frac{1}{\sin u\cos u}-\frac1u
% =
% \frac{u-\sin u\cos u}{u\sin u\cos u}
% <\frac{2u}{3-2u^2}
% <\frac{2u}{\rho^2-u^2}
% =\frac{2u}{s^2}.
% \]
% Combining the estimates gives
% \[
% \frac{d}{du}\log A(u)
% <
% \frac{2u}{s^2}
% -\frac{\sin(2u)}{1+\sin^2u}
% -\frac{2u}{s^2}
% <0.
% \]
% Thus $A$ is strictly decreasing.  Since $A(u)>1$ for small $u>0$ and $A(u)\to0$ as $u\uparrow\rho$, the function $\Phi$ increases up to the unique point where $A(u)=1$ and decreases afterward.

% A final outward-rounded interval computation gives
% \[
% A(0.8289364)>1.0000019,
% \qquad
% A(0.8289372)<0.9999992.
% \]
% Hence the maximizer lies in
% \[
% I=[0.8289364,0.8289372].
% \]
% Evaluating $\Phi$ on this interval, again with outward-rounded interval arithmetic, gives
% \[
% \Phi(I)\subset[9.0332175,9.03345993].
% \]
% Consequently
% \[
% \sup_{|w|\le1.1}
% \frac{\pi}{2}\frac{|\cos w|^2}{1-(\operatorname{Re}\sin w)^2}
% =
% \frac{\pi}{2}\sup_{0\le u\le\rho}\Phi(u)
% \le
% \frac{\pi}{2}\cdot9.03345993
% <14.18973<14.19.
% \]
% \end{proof}

==> paper/proof_outline_statements.tex <==
% Outline:
% \begin{enumerate}
%     \item Definition of Grothendieck constant: numerical improvement. 
%     \item Rounding schemes and analysis. 
%     \item Main theorem: For f = blah, g=blah, we have constant < blah.
%     \item Proof outline: (0) We do a variable change to simplify analysis. (1) Numerical computation of Taylor series upto 220. (2) Bounding the remainder term. 

%     The variable change helps, and changes how the remainder term is bounded. 
%     \item Bounding the remainder term without mixing. This is new, and deviates significantly from \cite{braverman2011grothendieckconstantstrictlysmaller}. Make this as modular as  possible. 
%     \item Section on numerical computation: Discuss computation and cross-verification with pytorch, etc. Why this is trustable (why can't this just be a floating point artifact)?
%     \item AI-guided search of rounding schemes. 
%     \item Koenig bilinear form: Related to Grothendieck. Main result. Best constant, higher dimensions give the constant. Not clear if it is realizable in two-dimensions.  
% \end{enumerate}

\begin{definition}[Real Grothendieck constant]
The real Grothendieck constant $K_G$ is the infimum over all $K>0$ such that, for every $m,n\in\mathbb N$ and every real matrix $A=(a_{ij})\in\R^{m\times n}$,
\[
\max_{x_i,y_j\in S^{m+n-1}}
\sum_{i=1}^m\sum_{j=1}^n a_{ij}\ip{x_i}{y_j}
\le
K\max_{\varepsilon_i,\delta_j\in\{-1,1\}}
\sum_{i=1}^m\sum_{j=1}^n a_{ij}\varepsilon_i\delta_j .
\]
\end{definition}

\begin{definition}[Gaussian correlation]
Fix $k \in \mathbb{N}$, and let $f,g:\mathbb{R}^k\to\{-1,1\}$ be odd measurable functions.
Let $G_1,G_2$ be independent standard Gaussian vectors in $\mathbb{R}^k$.

The \emph{arcsine-normalized correlation} associated to $(f,g)$ is
\[
H_{f,g}(t)
:=
\frac{\pi}{2}\,
\mathbb{E}\left[
f\left(\frac{G_1}{\sqrt{2}}\right)
g\left(
\frac{tG_1+\sqrt{1-t^2}G_2}{\sqrt{2}}
\right)
\right],
\qquad -1<t<1.
\]
\end{definition}

\begin{lemma}[Basic analytic properties]\label{lem:correlation-profile-analytic}
Let $f,g:\mathbb{R}^k\to\{-1,1\}$ be odd measurable functions. Then $H_{f,g}$ is odd and
extends holomorphically to the strip
\[
S:=\{z\in\mathbb{C}: |\operatorname{Re}z|<1\}.
\]
In particular, if $H_{f,g}'(0)\neq 0$, then $H_{f,g}$ has a unique local inverse branch at
the origin, and this inverse branch is odd.
\end{lemma}

\begin{definition}[Inverse majorant]
Assume $H_{f,g}'(0)\neq 0$, and write the local inverse branch at the origin as
\[
H_{f,g}^{-1}(\zeta)=\sum_{n\ge 1} a_n \zeta^n .
\]
For $s\ge 0$, define the inverse-majorant series
\[
M_{f,g}(s):=\sum_{n\ge 1}|a_n|s^n,
\]
with the convention that $M_{f,g}(s)=+\infty$ if the series diverges.
\end{definition}

\begin{definition}[$\gamma$-admissible Krivine scheme]
Let $\gamma>0$. We say that $(f,g)$ is a \emph{$\gamma$-admissible Krivine rounding scheme}
if:
\begin{enumerate}
    \item $f,g:\mathbb{R}^k\to\{-1,1\}$ are odd and measurable;
    \item $H_{f,g}'(0)\neq 0$;
    \item the inverse-majorant inequality 
    \[
    M_{f,g}(\gamma)=\sum_{n\ge 1}|a_n|\gamma^n \le 1
    \]
    holds.
\end{enumerate}
We call $(f,g)$ a \emph{Krivine rounding scheme} if it is $\gamma$-admissible for some
$\gamma>0$.
\end{definition}

\begin{theorem}[Krivine preprocessing in arcsine units]\label{thm:krivine-preprocessing}
If $(f,g)$ is a $\gamma$-admissible Krivine rounding scheme, then
\[
K_G \le \frac{\pi}{2\gamma}.
\]
\end{theorem}

% \begin{definition}[Krivine Rounding Scheme]
%     Let $G_1,G_2$ be independent standard Gaussian vectors in $\R^k$. For odd measurable
% $f,g:\R^k\to\{-1,1\}$, define the normalized correlation function
% \[
%  H_{f,g}(t)
%  =\frac\pi2 \E\left[f\left(\frac{G_1}{\sqrt2}\right)
%  g\left(\frac{tG_1+\sqrt{1-t^2}G_2}{\sqrt2}\right)\right],
%  \qquad -1<t<1.
% \]
% Then $H_{f,g}$ extends to an analytic function on the strip $\{z \in \mathbb{C} : \mathcal{R}(z) < 1\}$. We call $(f, g)$ a Krivine rounding scheme if $H_{f,g}$ is invertible on a neighborhood of the origin.

%  and if we consider the Taylor expansion 
% \[
%  H_{f,g}^{-1}(\zeta)=\sum_{n\ge1}a_n\zeta^n,
% \]
% then there exists $\gamma$ so that 
% \[
%  M(\gamma):=\sum_{n\ge1}|a_n|\gamma^n=1,
% \]
% \end{definition}


% % Thus the hyperplane scheme has $H_0(t)=\arcsin t$. The holomorphic extension and the strip bound used below are proved in Lemma~\ref{lem:strip-bound}.
% \begin{theorem}[Krivine/Braverman Preprocessing]
%     Using the usual Krivine preprocessing, we have $K_G \le \frac{\pi}{2\gamma}$. 
% \end{theorem}

\begin{definition}[The $H_3$ scheme]

Let \(H_3(x)=8x^3-12x\), and set
\[
 \tau=0.03175,
 \qquad
 \eta=\frac{\tau}{\sqrt{48}}
 =0.004582717761692655\ldots .
\]
Define odd measurable functions \(f,g:\R^2\to\{\pm1\}\) by
\[
    f(x,y)=\sgn(y-\eta H_3(x)),
    \qquad
    g(x,y)=\sgn(y+\eta H_3(x)).
\]
We define the rounding scheme $(f,g)$ as the $H_3$ scheme.
\end{definition}
The following is our main theorem. 
\begin{tcolorbox}
    \begin{theorem}[No Mixing Beats Hyperplane]
Let \[\gamma_0 = \log(1 + \sqrt{2}) + 4.8 \cdot 10^{-6}.
\] Then the $H_3$ scheme is a $\gamma_0$-admissible Krivine scheme. In particular, 
    \[
    K_G
    \le \frac{\pi}{2\gamma} \le 
   \frac{\pi}{2\log(1+\sqrt2)} - 
    9.7\cdot 10^{-6}
    \]
\end{theorem}
\end{tcolorbox}

% {\color{blue} Proof outline.}


\begin{lemma}[Strip bound]

Let $f,g:\R^2\to\{-1,1\}$ be measurable and let $H=H_{f,g}$ be the
arcsine-normalized correlation function.
Then $H$ extends holomorphically to
\(
 S=\{z\in\C: |\operatorname{Re}z|<1\}.
\)
Moreover, if $z=a+ib\in S$, then
\[
 |H(z)|\le \frac{\pi}{2}\frac{|1-z^2|}{1-a^2}.
\]
\end{lemma}

\begin{definition}[The Key Change of Variable]
Define $F \defeq H(\sin(w))$. 
\end{definition}

\begin{lemma}[Sine Coordinate Bound]

For $F(w)=H(\sin w)$, the function $F$ is holomorphic on $|w|<1.1$ and
\[
 |F(w)-w|<15.3\qquad (|w|\le1.1).
\]
    
\end{lemma}

\begin{lemma}[Rouche Inverse Disk]

Let $F$ be holomorphic on $|w|<r$, with $F(0)=0$, and suppose that for some
$R<M<r$,
\[
 \sup_{|w|=M}|F(w)-w|<M-R.
\]
Then:
\begin{enumerate}
    \item $F^{-1}$ is holomorphic on $R\D$;
    \item for $|\zeta|<R$, the inverse satisfies $|F^{-1}(\zeta)|<M$.
\end{enumerate}
\end{lemma}

\begin{corollary}[Radius and Supremum of $|F^{-1}|$]

Taking $r= 1.1, R = 0.975, M = 0.98$, $F^{-1}$  is holomorphic on $0.975\D$ and
\[
|F^{-1}(\zeta)|< 0.98.
\]
\end{corollary}

\begin{corollary}[Radius and Supremum of $|H^{-1}|$]
Undoing the change of variables, we get $H^{-1} =  \sin \circ F^{-1}$ is holomorphic on $0.975\D$ and
\[
|H^{-1}(\zeta)|<\sinh(0.98)<1.145.
\]

\end{corollary}

\begin{lemma}[Majorant Tail bound]
\label{lemma:tail-bound}
Let 
$
M_{f,g}(\zeta)=\sum_{n\ge 1} |a_n|\zeta^n. 
$
be the majorant. Then for $\zeta = \gamma_0$, we have the tail bound  \[\sum_{n\ge 220} |a_n|\zeta^n < 2.5 \cdot 10^{-9}\]
\end{lemma}


% Let's put this at the end for now. Proof of this is just plugging into Arb. I think maybe a significant portion of this should be how we compute the hermite machinery in Arb.
\begin{lemma}[Majorant Head Value]
\label{lemma:finite-majorant-value}
Let
$
 M_{f,g}(\zeta)=\sum_{n\ge 1} |a_n|\zeta^n.
$
Then for $\zeta = \gamma_0$, we have the finite majorant value \[\sum_{1\le n\le 220} |a_n|\zeta^n < 1 - 2.5 \cdot 10^{-9} \]
\end{lemma}

\begin{corollary}[$\gamma_0$-admissibility]
    Combining Lemma~\ref{lemma:finite-majorant-value} and Lemma~\ref{lemma:tail-bound}, we get \[M_{f,g} (\gamma_0) < 1\] and thus $H_3$ is $\gamma_0$-admissible.     
\end{corollary}


 


==> paper/remove_analytic_obstruction.tex <==
\section{\color{blue} Proof of The No-Mixing Theorem}
\label{sec:analytic-obstruction}
The proof has two parts. First, we prove an analytic inverse disk for the correlation profile. The
main device is the change of variables
\[
F(w):=H(\sin w),
\]
which is useful because the hyperplane profile becomes the identity map in this coordinate. This
allows us to use Rouché's theorem to control the inverse branch uniformly. Second, using this
inverse disk, we certify the inverse-majorant by splitting it into a finite head and a Cauchy tail:
the head is computed with Arb through degree $220$, and the tail is bounded analytically from the
inverse disk. Combining these two estimates gives $M_{f,g}(\gamma_0)<1$, so the $H_3$ scheme is
$\gamma_0$-admissible and the desired bound on $K_G$ follows.
\[
\begin{array}{ccccc}
Lemma~\ref{lem:strip-bound}
&\Longrightarrow&
Lemma~\ref{lem:sine-coordinate-bound}
&\Longrightarrow&
Corollary~\ref{cor:F-inverse-radius}
\Longrightarrow
Corollary~\ref{cor:H-inverse-radius}
\\[0.5em]
&&&&\Downarrow
\\[-0.1em]
Lemma~\ref{lem:majorant-head-value}
&+&
Lemma~\ref{lemma:tail-bound}
&\Longrightarrow&
Corollary~\ref{cor:gamma0-admissibility}
\Longrightarrow
Theorem~\ref{thm:no-mixing-beats-hyperplane}.
\end{array}
\]


\subsection{The analytic inverse disk}.

\begin{lemma}[Strip bound]\label{lem:strip-bound}
Let $f,g:\R^2\to\{-1,1\}$ be measurable and let $H=H_{f,g}$ be the
arcsine-normalized correlation function.
Then $H$ extends holomorphically to
\[
 S=\{z\in\C: |\operatorname{Re}z|<1\}.
\]
Moreover, if $z=a+ib\in S$, then
\[
 |H(z)|\le \frac{\pi}{2}\frac{|1-z^2|}{1-a^2}.
\]
\end{lemma}

\begin{proof}
For real $|t|<1$, the arcsine-normalized correlation admits the integral representation
\[
H(t)=\frac{1}{2\pi(1-t^2)}
\int_{\R^2}\int_{\R^2}
f(x)g(y)
\exp\left(
-\frac{\|x\|^2+\|y\|^2-2t\ip{x}{y}}{1-t^2}
\right)\,dx\,dy .
\]
For $z\in S$, this formula defines the candidate holomorphic extension.  Since $|f|=|g|=1$,
\[
|H(z)|\le
\frac{1}{2\pi |1-z^2|}
\int_{\R^2}\int_{\R^2}
\exp\left(
-\operatorname{Re}\frac{\|x\|^2+\|y\|^2-2z\ip{x}{y}}{1-z^2}
\right)\,dx\,dy .
\]
Use the identity
\[
\frac{\|x\|^2+\|y\|^2-2z\ip{x}{y}}{1-z^2}
=
\frac12\frac{\|x+y\|^2}{1+z}
+
\frac12\frac{\|x-y\|^2}{1-z}.
\]
Writing $z=a+ib$, set
\[
A_+ := \operatorname{Re}\frac{1}{1+z}
=\frac{1+a}{(1+a)^2+b^2},
\qquad
A_- := \operatorname{Re}\frac{1}{1-z}
=\frac{1-a}{(1-a)^2+b^2}.
\]
Both are positive for $|a|<1$.  With $u=x+y$ and $v=x-y$, the Jacobian from $(u,v)$ to $(x,y)$ in $\R^4$ is $1/4$.  Thus the Gaussian integral is
\[
\frac14\cdot\frac{2\pi}{A_+}\cdot\frac{2\pi}{A_-}
=\frac{\pi^2}{A_+A_-}.
\]
Finally,
\[
A_+A_-=
\frac{1-a^2}{|1+z|^2|1-z|^2}
=
\frac{1-a^2}{|1-z^2|^2}.
\]
Substitution gives
\[
|H(z)|\le
\frac{1}{2\pi |1-z^2|}\cdot
\frac{\pi^2 |1-z^2|^2}{1-a^2}
=
\frac{\pi}{2}\frac{|1-z^2|}{1-a^2}.
\]
The same estimate is uniform on compact subsets of $S$, so the integral converges locally uniformly and the extension is holomorphic by dominated convergence.
\end{proof}

\begin{definition}[The key change of variable]\label{def:key-change-of-variable}
For the rest of the proof, put
\[
F(w)\defeq H(\sin w).
\]
For the hyperplane scheme $H_0(t)=\arcsin t$, hence $H_0(\sin w)=w$ on the principal strip.  This is why the comparison below is made against the identity map.
\end{definition}

\begin{lemma}[Sine-coordinate bound]\label{lem:sine-coordinate-bound}
For $F(w)=H(\sin w)$, the function $F$ is holomorphic on $|w|<1.1$ and
\[
 |F(w)-w|<15.3\qquad (|w|\le1.1).
\]
\end{lemma}

\begin{proof}
Write $w=u+iv$. Then
\[
\operatorname{Re}(\sin w)=\sin u\cosh v.
\]
By Lemma~\ref{lem:disk-to-strip-check}, if $u^2+v^2\le 1.1^2$, then
\[
|\sin u|\cosh v<0.946<1.
\]
Therefore $\sin w\in S$ for $|w|\le 1.1$, and Lemma~\ref{lem:strip-bound} implies that $F$ is holomorphic on $|w|<1.1$.  Applying Lemma~\ref{lem:strip-bound} with $z=\sin w$ gives
\[
|F(w)|
\le
\frac{\pi}{2}\frac{|1-\sin^2 w|}{1-(\operatorname{Re}\sin w)^2}
=
\frac{\pi}{2}\frac{|\cos w|^2}{1-(\operatorname{Re}\sin w)^2}.
\]
By Lemma~\ref{lem:cosine-ratio-check}, the last expression is $<14.19$ on $|w|\le 1.1$.  Hence
\[
|F(w)-w|\le |F(w)|+|w|<14.19+1.1<15.3.
\]
\end{proof}

\begin{lemma}[Rouch\'e inverse disk]\label{lem:rouche-inverse-disk}
Let $F$ be holomorphic on $|w|<r$, with $F(0)=0$, and suppose that for some
$R<M<r$,
\[
 \sup_{|w|=M}|F(w)-w|<M-R.
\]
Then:
\begin{enumerate}[label=(\roman*)]
    \item $F^{-1}$ is holomorphic on $R\D$;
    \item for $|\zeta|<R$, the inverse satisfies $|F^{-1}(\zeta)|<M$.
\end{enumerate}
\end{lemma}

\begin{proof}
Fix $|\zeta|<R$.  On $|w|=M$,
\[
|(F(w)-\zeta)-(w-\zeta)|=|F(w)-w|<M-R<M-|\zeta|\le |w-\zeta|.
\]
By Rouch\'e's theorem, $F(w)-\zeta$ and $w-\zeta$ have the same number of zeros in $|w|<M$, counted with multiplicity.  Since $w-\zeta$ has exactly one zero in this disk, $F(w)=\zeta$ has exactly one solution in $|w|<M$, counted with multiplicity.  In particular, the solution is simple.  The holomorphic inverse function theorem gives local inverse branches, and uniqueness makes these branches glue over $R\D$.  The same argument gives $|F^{-1}(\zeta)|<M$.
\end{proof}

\begin{corollary}[Radius and supremum of $|F^{-1}|$]\label{cor:F-inverse-radius}
Taking $r=1.1$, $R=0.975$, and $M=0.98$, the inverse $F^{-1}$ is holomorphic on $0.975\D$ and
\[
|F^{-1}(\zeta)|<0.98\qquad (|\zeta|<0.975).
\]
\end{corollary}

\begin{proof}
Let
\[
\Delta(w):=F(w)-w=\sum_{n\ge1}d_nw^n.
\]
The Arb coefficient computation gives the finite head estimate
\[
\sum_{n\le 220}|d_n|0.98^n<0.00454106848.
\]
By Lemma~\ref{lem:sine-coordinate-bound} and Cauchy's estimate, taking the Cauchy radius to $1.1$ from below gives
\[
\sum_{n>220}|d_n|0.98^n
\le
15.3\frac{(0.98/1.1)^{221}}{1-0.98/1.1}
<1.149\cdot10^{-9}.
\]
Therefore
\[
\sup_{|w|=0.98}|F(w)-w|
\le
\sum_{n\ge1}|d_n|0.98^n
<0.00454106848+1.149\cdot 10^{-9}
<0.005.
\]
Since $M-R=0.98-0.975=0.005$, Lemma~\ref{lem:rouche-inverse-disk} applies with $r=1.1$, $M=0.98$, and $R=0.975$.
\end{proof}

\begin{corollary}[Radius and supremum of $|H^{-1}|$]\label{cor:H-inverse-radius}
Undoing the change of variables, we get
\[
H^{-1}=\sin\circ F^{-1}.
\]
Thus $H^{-1}$ is holomorphic on $0.975\D$ and
\[
|H^{-1}(\zeta)|<\sinh(0.98)<1.145
\qquad (|\zeta|<0.975).
\]
\end{corollary}

\begin{proof}
Since $F=H\circ\sin$, the identity $F^{-1}=\arcsin\circ H^{-1}$ is equivalent to
$H^{-1}=\sin\circ F^{-1}$ on the inverse branch at the origin.  By Corollary~\ref{cor:F-inverse-radius}, $|F^{-1}(\zeta)|<0.98$ for $|\zeta|<0.975$.  The elementary bound
\[
|\sin z|\le \sinh |z|
\]
for complex $z$ gives
\[
|H^{-1}(\zeta)|=|\sin(F^{-1}(\zeta))|<\sinh(0.98)<1.145.
\]
\end{proof}

\subsection{The inverse-majorant theorem}

\begin{lemma}[Majorant tail bound]\label{lemma:tail-bound}
Let
\[
H^{-1}(\zeta)=\sum_{n\ge1}a_n\zeta^n,
\qquad
\gzero=\log(1+\sqrt2)+4.8\cdot10^{-6}.
\]
Then
\[
\sum_{n>220}|a_n|\gzero^n<2.5\cdot10^{-9}.
\]
\end{lemma}

\begin{proof}
By Corollary~\ref{cor:H-inverse-radius}, $H^{-1}$ is holomorphic on $0.975\D$ and satisfies $|H^{-1}(\zeta)|<1.145$ there.  Hence, for every $s<0.975$, Cauchy's estimate with radius tending to $0.975$ gives
\[
\sum_{n>220}|a_n|s^n
\le
1.145\frac{(s/0.975)^{221}}{1-s/0.975}.
\]
Taking $s=\gzero$ yields
\[
1.145\frac{(\gzero/0.975)^{221}}{1-\gzero/0.975}
<2.44\cdot10^{-9}
<2.5\cdot10^{-9},
\]
as claimed.
\end{proof}

\begin{lemma}[Majorant head value]\label{lem:majorant-head-value}
Let
\[
 M_{f,g}(s)=\sum_{n\ge 1} |a_n|s^n
\]
be the inversomewhat. se majorant for the $H_3$ scheme.  For
\[
\gzero=\log(1+\sqrt2)+4.8\cdot10^{-6},
\]
one has
\[
\sum_{1\le n\le220}|a_n|\gzero^n
<1-2.5\cdot10^{-9}.
\]
\end{lemma}

\begin{proof}
\source{Arb certificate.}
We record the coefficient computation used by the certificate.  Let $\mathsf H_n$ be the physicist's Hermite polynomial and set
\[
\psi_n(x):=\frac{\mathsf H_n(x)}{\sqrt{2^n n!}},
\qquad
 d\mu(x):=\pi^{-1/2}e^{-x^2}\,dx.
\]
Then $\{\psi_n\}_{n\ge0}$ is an orthonormal basis for $L^2(\mu)$.  Expanding
\[
f(x,y)=\sum_{a,b\ge0}F_{a,b}\psi_a(x)\psi_b(y),
\]
and using $g(x,y)=f(-x,y)$, the coefficient of $\psi_a(x)\psi_b(y)$ in $g$ is $(-1)^aF_{a,b}$.  Mehler diagonalization gives
\[
H(z)=\frac{\pi}{2}\sum_{a,b\ge0}(-1)^aF_{a,b}^2z^{a+b},
\]
so
\[
[z^n]H(z)=\frac{\pi}{2}\sum_{a=0}^{n}(-1)^aF_{a,n-a}^2.
\]
The two-dimensional coefficients reduce to one-dimensional integrals:
\[
F_{a,b}=\int_{\R}\psi_a(x)S_b(\tau\psi_3(x))\,d\mu(x),
\]
where
\[
S_0(u)=-\erf(u),
\qquad
S_b(u)=\frac{2}{\sqrt\pi}e^{-u^2}\frac{\psi_{b-1}(u)}{\sqrt{2b}}
\quad (b\ge1).
\]
These formulas determine the Taylor coefficients of $H$ through degree $220$ using one-dimensional Arb integrations and outward-rounded interval arithmetic.

Since $H$ is odd, the inverse has only odd coefficients.  Writing
\[
H(z)=z\Phi(z^2),
\]
Lagrange inversion gives
\[
a_{2k+1}=\frac{1}{2k+1}[t^k]\Phi(t)^{-(2k+1)},
\qquad
 a_{2k}=0.
\]
Applying this formula with Arb ball arithmetic gives the certified enclosure
\[
\sum_{n\le220}|a_n|\gzero^n<0.999999729.
\]
Since $0.999999729<1-2.5\cdot10^{-9}$, the stated bound follows.  Independent floating-point and PyTorch checks are useful diagnostics, but the displayed inequality is certified only by the outward-rounded Arb computation.
\end{proof}

\begin{corollary}[$\gamma_0$-admissibility]\label{cor:gamma0-admissibility}
For the $H_3$ scheme,
\[
M_{f,g}(\gzero)<1.
\]
Consequently, the scheme is $\gzero$-admissible.
\end{corollary}

\begin{proof}
By Lemma~\ref{lem:majorant-head-value},
\[
\sum_{1\le n\le220}|a_n|\gzero^n<1-2.5\cdot10^{-9}.
\]
By Lemma~\ref{lemma:tail-bound},
\[
\sum_{n>220}|a_n|\gzero^n<2.5\cdot10^{-9}.
\]
Adding the two inequalities gives $M_{f,g}(\gzero)<1$.  The inverse branch exists on a neighborhood of $\gzero\overline{\D}$ by Corollary~\ref{cor:H-inverse-radius}, since $\gzero<0.975$.  Thus the $H_3$ scheme satisfies Definition~\ref{def:gamma-admissible}.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:no-mixing-beats-hyperplane}]
By Corollary~\ref{cor:gamma0-admissibility}, the $H_3$ scheme is $\gzero$-admissible.  Applying Theorem~\ref{thm:krivine-preprocessing} gives
\[
K_G\le \frac{\pi}{2\gzero}.
\]
Finally, with $\rhostarval=\log(1+\sqrt2)$ and $\gzero=\rhostarval+4.8\cdot10^{-6}$,
\[
\frac{\pi}{2\rhostarval}-\frac{\pi}{2\gzero}
=
\frac{\pi(4.8\cdot10^{-6})}{2\rhostarval\gzero}
>9.7\cdot10^{-6}.
\]
Therefore
\[
K_G
\le
\frac{\pi}{2\gzero}
<
\frac{\pi}{2\log(1+\sqrt2)}-9.7\cdot10^{-6}.
\]
\end{proof}
